Fooling Explanations in Text Classifiers

State-of-the-art text classification models are becoming increasingly reliant on deep neural networks (DNNs). Due to their black-box nature, faithful and robust explanation methods need to accompany classifiers for deployment in real-life scenarios. However, it has been shown in vision applications that explanation methods are susceptible to local, imperceptible perturbations that can significantly alter the explanations without changing the predicted classes. We show here that the existence of such perturbations extends to text classifiers as well. Specifically, we introduceTextExplanationFooler (TEF), a novel explanation attack algorithm that alters text input samples imperceptibly so that the outcome of widely-used explanation methods changes considerably while leaving classifier predictions unchanged. We evaluate the performance of the attribution robustness estimation performance in TEF on five sequence classification datasets, utilizing three DNN architectures and three transformer architectures for each dataset. TEF can significantly decrease the correlation between unchanged and perturbed input attributions, which shows that all models and explanation methods are susceptible to TEF perturbations. Moreover, we evaluate how the perturbations transfer to other model architectures and attribution methods, and show that TEF perturbations are also effective in scenarios where the target model and explanation method are unknown. Finally, we introduce a semi-universal attack that is able to compute fast, computationally light perturbations with no knowledge of the attacked classifier nor explanation method. Overall, our work shows that explanations in text classifiers are very fragile and users need to carefully address their robustness before relying on them in critical applications.

==> data/attention_heads/agnews/bert.tex <==
42      35      17      09      18      33      30      24      18      35      10      33  
28      15      26      23      10      36      04      37      27      16      19      29  
00      30      09      18      14      14      18      26      15      00      36      29  
29      28      21      18      46      11      29      13      39      21      32      18  
40      20      08      22      24      21      27      17      12      21      17      17  
19      11      12      13      18      18      16      12      10      15      20      19  
08      13      15      17      19      21      22      14      10      26      20      14  
35      23      26      14      18      26      08      14      37      31      25      25  
19      19      29      25      24      22      26      35      24      36      37      43  
26      41      46      33      32      74      31      54      62      25      38      31  
77      73      69      72      77      69      80      78      80      63      40      73  
68      61      65      59      67      66      64      62      39      59      63      67

==> data/attention_heads/agnews/xlnet.tex <==
42      35      17      09      18      33      30      24      18      35      10      33      13      34      15      24
28      15      26      23      10      36      04      37      27      16      19      29      13      34      15      24
00      30      09      18      14      14      18      26      15      00      36      29      13      34      15      24
29      28      21      18      46      11      29      13      39      21      32      18      13      34      15      24
40      20      08      22      24      21      27      17      12      21      17      17      13      34      15      24
19      11      12      13      18      18      16      12      10      15      20      19      13      34      15      24
08      13      15      17      19      21      22      14      10      26      20      14      13      34      15      24
35      23      26      14      18      26      08      14      37      31      25      25      13      34      15      24
19      19      29      25      24      22      26      35      24      36      37      43      13      34      15      24
26      41      46      33      32      74      31      54      62      25      38      31      13      34      15      24
77      73      69      72      77      69      80      78      80      63      40      73      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24
68      61      65      59      67      66      64      62      39      59      63      67      13      34      15      24

==> data/attention_heads/imdb/bert.tex <==
64   60   18   17   47   56   47   46   46   56   19   56
54   20   58   80   16   42   32   40   38   63   43   45
49   42   25   36   18   44   51   43   16   50   22   56
26   40   26   33   45   40   17   27   44   46   59   39
36   07   18   14   21   38   22   22   14   38   26   33
19   21   03   15   17   10   27   38   06   47   40   14
16   14   33   23   54   60   30   47   20   57   41   54
60   44   27   42   64   44   36   26   53   49   70   42
29   26   64   17   27   42   27   36   78   46   72   47
85   87   71   58   64   72   42   83   64   61   73   70
74   78   74   80   78   72   75   77   76   75   91   74
74   76   100  73   96   97   96   94   94   100  94   98

==> data/attention_heads/mr/bert.tex <==
41   27   18   11   17   30   26   16   25   26   12   22
31   13   27   18   09   33   06   31   16   20   19   24
01   27   11   22   17   19   19   20   13   01   22   21
16   17   11   16   24   12   12   09   26   19   33   16
21   12   06   17   13   17   18   14   09   16   14   15
10   11   08   08   11   15   13   12   06   21   19   07
10   09   14   15   18   28   19   19   11   22   14   19
29   23   24   11   25   26   10   15   27   27   27   15
11   08   21   11   11   19   09   21   26   36   31   37
34   25   40   40   38   46   18   51   55   17   32   33
20   35   18   37   24   16   61   29   24   16   55   26
16   21   27   26   28   36   23   30   42   36   40   23

==> data/attention_heads/yelp/bert.tex <==
47   43   18   10   30   48   40   29   24   38   11   36
34   15   31   29   13   40   10   36   26   29   24   28
00   35   17   43   27   19   22   29   22   00   47   30
27   36   17   24   42   11   24   26   44   22   43   22
32   21   11   24   26   23   27   17   11   24   20   17
24   14   15   17   27   19   16   19   16   17   23   17
14   20   23   15   24   32   23   22   16   27   26   20
36   25   29   16   29   37   16   14   35   31   35   21
19   34   35   28   26   29   26   39   32   48   47   42
52   56   53   49   48   65   36   62   68   35   51   71
81   69   64   78   77   67   76   75   73   66   37   74
77   68   70   69   77   65   77   78   47   64   73   76

==> data/ra/agnews/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.99	0.94	1.03	0.99	0.98	1.01	0.93	0.85	1.00	0.94	0.87	1.02	0.95	0.90	1.00	0.96	0.93	1.00	4750
0.03	0.96	0.88	1.03	0.98	0.97	1.00	0.82	0.75	0.89	0.86	0.76	0.95	0.87	0.82	0.92	0.91	0.88	0.94	4781
0.06	0.92	0.82	1.03	0.97	0.94	0.99	0.73	0.65	0.80	0.79	0.68	0.89	0.81	0.75	0.87	0.86	0.83	0.90	4963
0.11	0.89	0.76	1.02	0.95	0.91	0.98	0.66	0.58	0.74	0.73	0.62	0.84	0.76	0.70	0.82	0.83	0.79	0.87	4702
0.15	0.84	0.68	1.00	0.92	0.87	0.97	0.58	0.49	0.66	0.66	0.54	0.79	0.70	0.64	0.76	0.79	0.74	0.83	4473
0.18	0.79	0.62	0.97	0.89	0.83	0.95	0.51	0.42	0.60	0.61	0.48	0.74	0.65	0.59	0.72	0.75	0.71	0.80	4728
0.22	0.78	0.60	0.96	0.88	0.82	0.94	0.47	0.37	0.56	0.59	0.46	0.72	0.62	0.56	0.69	0.73	0.68	0.78	1645
0.26	0.74	0.53	0.94	0.84	0.76	0.93	0.44	0.35	0.54	0.56	0.42	0.69	0.61	0.54	0.67	0.72	0.67	0.77	3527
0.29	0.70	0.49	0.92	0.82	0.73	0.91	0.40	0.31	0.50	0.52	0.38	0.66	0.58	0.51	0.65	0.70	0.65	0.75	4573
0.32	0.60	0.35	0.86	0.71	0.60	0.83	0.34	0.23	0.44	0.45	0.29	0.60	0.53	0.45	0.60	0.66	0.61	0.72	860
% 0.38	0.63	0.38	0.87	0.76	0.66	0.87	0.32	0.22	0.42	0.46	0.31	0.60	0.52	0.45	0.59	0.65	0.60	0.71	5721

==> data/ra/agnews/cnn/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.99	0.95	1.02	1.00	0.99	1.00	0.97	0.91	1.03	0.97	0.89	1.05	0.98	0.93	1.02	0.98	0.95	1.02	4622
0.03	0.95	0.88	1.01	0.99	0.97	1.00	0.86	0.78	0.94	0.88	0.72	1.03	0.91	0.84	0.98	0.93	0.88	0.98	4635
0.06	0.90	0.80	0.99	0.97	0.95	0.99	0.76	0.67	0.85	0.79	0.61	0.98	0.85	0.76	0.93	0.88	0.82	0.94	4896
0.11	0.85	0.74	0.96	0.96	0.93	0.98	0.68	0.58	0.78	0.73	0.54	0.93	0.80	0.71	0.89	0.84	0.78	0.91	4532
0.15	0.78	0.65	0.91	0.93	0.89	0.97	0.59	0.48	0.70	0.66	0.46	0.87	0.75	0.65	0.85	0.80	0.73	0.87	4212
0.18	0.72	0.57	0.87	0.91	0.86	0.96	0.52	0.40	0.63	0.61	0.39	0.82	0.70	0.60	0.81	0.77	0.69	0.84	4565
0.22	0.67	0.50	0.84	0.89	0.84	0.94	0.46	0.34	0.58	0.57	0.34	0.79	0.67	0.56	0.78	0.74	0.66	0.82	1885
0.26	0.65	0.48	0.82	0.87	0.80	0.94	0.45	0.32	0.57	0.55	0.33	0.77	0.66	0.55	0.77	0.73	0.65	0.81	3280
0.29	0.61	0.43	0.78	0.85	0.78	0.92	0.41	0.28	0.53	0.51	0.30	0.73	0.63	0.52	0.75	0.71	0.64	0.79	4198
0.32	0.60	0.40	0.79	0.76	0.67	0.86	0.36	0.23	0.49	0.52	0.30	0.74	0.61	0.50	0.72	0.69	0.61	0.77	552
0.38	0.52	0.33	0.71	0.80	0.71	0.88	0.33	0.20	0.45	0.45	0.23	0.67	0.58	0.46	0.70	0.67	0.59	0.75	5504

==> data/ra/agnews/cnn/S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.99	0.96	1.02	1.00	0.99	1.00	0.97	0.92	1.02	0.97	0.86	1.07	0.98	0.92	1.03	0.98	0.95	1.02	4622
0.03	0.96	0.91	1.02	0.99	0.97	1.00	0.89	0.81	0.97	0.86	0.65	1.07	0.91	0.81	1.01	0.94	0.87	1.00	4635
0.06	0.93	0.85	1.01	0.97	0.95	0.99	0.81	0.71	0.91	0.78	0.53	1.02	0.85	0.74	0.97	0.90	0.82	0.97	4896
0.11	0.89	0.79	0.99	0.96	0.93	0.98	0.75	0.63	0.86	0.70	0.43	0.97	0.81	0.68	0.93	0.87	0.79	0.95	4532
0.15	0.85	0.73	0.97	0.93	0.89	0.97	0.68	0.55	0.80	0.64	0.36	0.92	0.76	0.63	0.90	0.83	0.75	0.92	4212
0.18	0.81	0.68	0.95	0.91	0.86	0.96	0.63	0.50	0.76	0.59	0.29	0.88	0.72	0.58	0.87	0.81	0.72	0.90	4565
0.22	0.78	0.63	0.94	0.89	0.84	0.94	0.59	0.45	0.74	0.55	0.24	0.86	0.70	0.54	0.85	0.79	0.69	0.89	1887
0.26	0.77	0.61	0.93	0.87	0.80	0.94	0.58	0.43	0.72	0.54	0.24	0.83	0.69	0.53	0.84	0.78	0.69	0.88	3287
0.29	0.75	0.58	0.91	0.85	0.78	0.92	0.55	0.40	0.70	0.52	0.22	0.82	0.67	0.52	0.83	0.77	0.67	0.87	4188
0.32	0.75	0.59	0.91	0.76	0.66	0.86	0.55	0.40	0.69	0.51	0.21	0.81	0.69	0.54	0.84	0.78	0.68	0.88	553
% 0.38	0.70	0.52	0.88	0.80	0.71	0.88	0.51	0.35	0.66	0.47	0.17	0.78	0.64	0.48	0.80	0.75	0.64	0.85	5541

==> data/ra/agnews/lstm/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.98	0.93	1.04	1.00	0.99	1.00	0.96	0.88	1.04	0.96	0.86	1.06	0.97	0.91	1.03	0.98	0.93	1.02	4694
0.03	0.94	0.83	1.04	0.99	0.97	1.00	0.86	0.75	0.97	0.86	0.69	1.04	0.90	0.81	1.00	0.93	0.86	0.99	4695
0.06	0.88	0.74	1.03	0.97	0.95	0.99	0.77	0.64	0.90	0.79	0.59	1.00	0.84	0.74	0.95	0.88	0.81	0.96	4962
0.11	0.83	0.66	1.00	0.96	0.93	0.98	0.70	0.56	0.84	0.74	0.53	0.95	0.80	0.69	0.92	0.85	0.77	0.93	4594
0.15	0.75	0.55	0.96	0.93	0.89	0.97	0.62	0.47	0.77	0.67	0.44	0.90	0.75	0.62	0.88	0.81	0.73	0.90	4280
0.18	0.69	0.47	0.91	0.91	0.86	0.96	0.54	0.38	0.70	0.62	0.38	0.86	0.70	0.57	0.84	0.77	0.68	0.87	4626
0.22	0.64	0.42	0.87	0.89	0.84	0.94	0.49	0.33	0.65	0.57	0.33	0.82	0.68	0.54	0.81	0.75	0.66	0.84	1923
0.26	0.62	0.39	0.85	0.87	0.80	0.93	0.47	0.31	0.62	0.56	0.31	0.81	0.66	0.52	0.79	0.74	0.65	0.83	3330
0.29	0.57	0.32	0.81	0.85	0.78	0.92	0.42	0.26	0.58	0.52	0.28	0.76	0.63	0.49	0.76	0.72	0.62	0.81	4237
0.32	0.50	0.24	0.77	0.76	0.66	0.86	0.35	0.18	0.52	0.46	0.21	0.72	0.57	0.42	0.72	0.67	0.57	0.78	564
0.38	0.47	0.21	0.73	0.80	0.71	0.88	0.33	0.17	0.49	0.45	0.20	0.69	0.57	0.43	0.71	0.67	0.57	0.77	5585

==> data/ra/agnews/lstmatt/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.98	0.91	1.05	1.00	0.99	1.00	0.95	0.83	1.06	0.92	0.73	1.11	0.95	0.84	1.06	0.97	0.90	1.04	4734
0.03	0.93	0.79	1.06	0.99	0.97	1.00	0.81	0.64	0.99	0.72	0.42	1.03	0.84	0.66	1.01	0.89	0.78	1.01	4736
0.06	0.86	0.67	1.05	0.97	0.95	0.99	0.72	0.51	0.93	0.60	0.26	0.94	0.76	0.55	0.97	0.85	0.71	0.98	5002
0.11	0.81	0.59	1.03	0.95	0.93	0.98	0.65	0.42	0.88	0.53	0.18	0.87	0.71	0.49	0.93	0.81	0.66	0.96	4643
0.15	0.73	0.46	1.00	0.93	0.89	0.97	0.56	0.31	0.82	0.43	0.09	0.77	0.64	0.40	0.87	0.76	0.60	0.92	4308
0.18	0.66	0.36	0.97	0.91	0.86	0.96	0.50	0.23	0.77	0.37	0.03	0.71	0.59	0.34	0.84	0.73	0.56	0.90	4668
0.22	0.62	0.29	0.95	0.89	0.84	0.94	0.46	0.18	0.74	0.34	0.00	0.67	0.56	0.31	0.81	0.71	0.53	0.89	1937
0.26	0.61	0.28	0.93	0.87	0.80	0.94	0.45	0.16	0.73	0.33	0.00	0.66	0.55	0.30	0.81	0.70	0.53	0.88	3361
0.29	0.54	0.19	0.89	0.85	0.78	0.92	0.39	0.10	0.68	0.29	-0.02	0.60	0.51	0.26	0.77	0.68	0.50	0.86	4285
0.32	0.48	0.09	0.87	0.76	0.67	0.86	0.35	0.04	0.67	0.26	-0.06	0.58	0.49	0.22	0.76	0.66	0.47	0.84	552
% 0.38	0.46	0.10	0.82	0.80	0.71	0.88	0.33	0.04	0.63	0.24	-0.06	0.54	0.47	0.21	0.72	0.65	0.46	0.83	5621

==> data/ra/imdb/lstmatt/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.93	0.82	1.04	0.98	0.97	0.99	0.83	0.74	0.93	0.86	0.75	0.97	0.89	0.82	0.96	0.92	0.87	0.97	4478
0.03	0.88	0.75	1.01	0.96	0.94	0.98	0.74	0.64	0.84	0.78	0.65	0.91	0.83	0.76	0.90	0.87	0.82	0.93	4472
0.06	0.80	0.64	0.96	0.93	0.91	0.95	0.64	0.54	0.74	0.70	0.56	0.83	0.77	0.69	0.84	0.83	0.77	0.88	4482
0.11	0.73	0.56	0.91	0.90	0.87	0.93	0.56	0.46	0.67	0.64	0.50	0.77	0.71	0.63	0.80	0.79	0.73	0.85	4469
0.15	0.64	0.45	0.83	0.84	0.80	0.88	0.47	0.37	0.57	0.56	0.42	0.70	0.65	0.57	0.73	0.75	0.69	0.80	4468
0.18	0.55	0.35	0.75	0.79	0.74	0.84	0.40	0.30	0.49	0.50	0.36	0.63	0.60	0.52	0.69	0.71	0.65	0.77	3129
0.22	0.52	0.28	0.76	0.78	0.71	0.86	0.37	0.24	0.50	0.50	0.31	0.68	0.59	0.48	0.71	0.69	0.62	0.77	106
0.26	0.46	0.26	0.67	0.73	0.67	0.79	0.33	0.23	0.42	0.44	0.30	0.57	0.56	0.48	0.64	0.68	0.62	0.73	2480
0.29	0.40	0.19	0.60	0.68	0.62	0.74	0.28	0.18	0.37	0.40	0.27	0.53	0.53	0.45	0.61	0.65	0.60	0.71	2114
0.32	0.36	0.16	0.56	0.63	0.57	0.70	0.25	0.16	0.34	0.37	0.24	0.50	0.51	0.43	0.58	0.64	0.59	0.70	1891

==> data/ra/mr/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	2852
0.03	0.98	0.92	1.03	0.97	0.95	0.99	0.82	0.71	0.92	0.91	0.83	1.00	0.88	0.80	0.96	0.90	0.84	0.96	1271
0.06	0.97	0.91	1.03	0.95	0.92	0.98	0.75	0.62	0.88	0.89	0.78	1.00	0.85	0.75	0.94	0.87	0.79	0.94	1899
0.11	0.95	0.87	1.03	0.91	0.85	0.96	0.67	0.53	0.82	0.85	0.71	0.99	0.79	0.68	0.90	0.82	0.74	0.91	2269
0.15	0.95	0.87	1.03	0.90	0.86	0.95	0.64	0.49	0.80	0.82	0.66	0.99	0.79	0.67	0.91	0.81	0.71	0.90	1076
0.18	0.93	0.82	1.03	0.85	0.78	0.92	0.57	0.41	0.73	0.80	0.64	0.96	0.74	0.62	0.85	0.77	0.68	0.86	1701
0.22	0.92	0.82	1.02	0.84	0.78	0.91	0.54	0.37	0.71	0.80	0.65	0.95	0.72	0.59	0.85	0.75	0.65	0.84	1080
0.26	0.89	0.78	1.01	0.80	0.71	0.88	0.50	0.34	0.67	0.77	0.61	0.93	0.69	0.57	0.81	0.73	0.63	0.83	2017
0.29	0.89	0.76	1.01	0.76	0.66	0.86	0.48	0.32	0.64	0.76	0.59	0.93	0.67	0.54	0.79	0.72	0.63	0.81	1458
0.32	0.86	0.73	1.00	0.73	0.62	0.84	0.44	0.27	0.61	0.72	0.56	0.89	0.65	0.52	0.77	0.70	0.60	0.79	1400
% 0.38	0.88	0.74	1.01	0.74	0.64	0.85	0.43	0.25	0.60	0.75	0.58	0.92	0.64	0.51	0.77	0.69	0.59	0.79	1518

==> data/ra/mr/cnn/S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.68	0.22	1.15	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	2778
0.03	0.60	0.15	1.06	0.97	0.95	0.99	0.86	0.76	0.97	0.84	0.55	1.12	0.88	0.69	1.07	0.92	0.79	1.05	940
0.06	0.58	0.13	1.03	0.96	0.93	0.98	0.80	0.67	0.93	0.76	0.38	1.13	0.83	0.59	1.07	0.88	0.72	1.05	1643
0.11	0.57	0.14	0.99	0.92	0.87	0.96	0.72	0.56	0.88	0.69	0.31	1.08	0.79	0.54	1.03	0.85	0.68	1.02	1793
0.15	0.52	0.09	0.94	0.91	0.86	0.95	0.67	0.48	0.86	0.65	0.22	1.08	0.74	0.46	1.02	0.82	0.62	1.02	979
0.18	0.52	0.12	0.92	0.86	0.80	0.92	0.62	0.43	0.80	0.58	0.16	1.00	0.71	0.43	0.98	0.79	0.61	0.98	1480
0.22	0.46	0.07	0.86	0.85	0.79	0.91	0.56	0.36	0.75	0.56	0.12	0.99	0.68	0.39	0.97	0.77	0.56	0.97	984
0.26	0.47	0.07	0.86	0.81	0.73	0.89	0.57	0.37	0.76	0.54	0.12	0.97	0.67	0.39	0.96	0.77	0.57	0.97	1599
0.29	0.45	0.07	0.83	0.78	0.68	0.87	0.53	0.34	0.73	0.53	0.12	0.95	0.67	0.39	0.94	0.76	0.56	0.96	1144
0.32	0.47	0.10	0.85	0.74	0.64	0.85	0.54	0.35	0.72	0.47	0.05	0.89	0.61	0.31	0.91	0.74	0.54	0.94	885
% 0.38	0.40	0.02	0.77	0.76	0.67	0.85	0.50	0.30	0.69	0.50	0.06	0.93	0.64	0.34	0.93	0.74	0.53	0.95	1532

==> data/ra/mr/lstm/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.77	0.35	1.19	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	2870
0.03	0.75	0.37	1.14	0.97	0.96	0.99	0.76	0.52	1.00	0.78	0.47	1.10	0.82	0.62	1.02	0.87	0.72	1.01	975
0.06	0.63	0.19	1.07	0.96	0.93	0.98	0.68	0.40	0.96	0.72	0.35	1.10	0.77	0.52	1.02	0.83	0.65	1.00	1711
0.11	0.59	0.15	1.02	0.92	0.87	0.96	0.60	0.31	0.89	0.65	0.27	1.03	0.72	0.47	0.98	0.79	0.61	0.97	1866
0.15	0.49	0.04	0.94	0.91	0.86	0.95	0.55	0.25	0.85	0.58	0.14	1.01	0.67	0.38	0.96	0.76	0.57	0.96	1030
0.18	0.50	0.08	0.92	0.86	0.80	0.92	0.48	0.21	0.76	0.55	0.15	0.96	0.64	0.38	0.90	0.73	0.54	0.91	1522
0.22	0.45	0.03	0.87	0.85	0.78	0.91	0.45	0.17	0.74	0.49	0.07	0.90	0.61	0.33	0.89	0.71	0.52	0.90	1056
0.26	0.42	0.02	0.83	0.81	0.73	0.89	0.40	0.13	0.67	0.48	0.08	0.88	0.58	0.33	0.84	0.69	0.52	0.87	1631
0.29	0.41	0.02	0.79	0.78	0.69	0.87	0.38	0.13	0.63	0.43	0.06	0.81	0.58	0.34	0.82	0.68	0.51	0.85	1192
0.32	0.38	-0.00	0.77	0.75	0.64	0.85	0.36	0.12	0.60	0.44	0.05	0.82	0.55	0.28	0.82	0.68	0.51	0.85	935
% 0.38	0.32	-0.06	0.70	0.76	0.68	0.84	0.30	0.05	0.56	0.40	-0.01	0.80	0.53	0.27	0.79	0.65	0.47	0.82	1587

==> data/ra/mr/lstmatt/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	3002
0.03	0.93	0.82	1.05	0.97	0.95	0.99	0.86	0.75	0.97	0.85	0.61	1.08	0.89	0.78	1.00	0.92	0.85	1.00	1022
0.06	0.89	0.74	1.04	0.96	0.93	0.99	0.80	0.66	0.93	0.77	0.44	1.11	0.84	0.71	0.98	0.89	0.80	0.98	1783
0.11	0.83	0.65	1.01	0.92	0.87	0.96	0.71	0.56	0.87	0.71	0.39	1.04	0.79	0.64	0.95	0.85	0.75	0.95	1967
0.15	0.77	0.55	0.99	0.91	0.87	0.95	0.65	0.45	0.85	0.64	0.24	1.04	0.74	0.52	0.95	0.82	0.70	0.94	1056
0.18	0.72	0.50	0.95	0.86	0.80	0.92	0.60	0.42	0.78	0.59	0.23	0.96	0.72	0.55	0.89	0.80	0.68	0.91	1583
0.22	0.66	0.41	0.91	0.85	0.78	0.91	0.55	0.35	0.74	0.52	0.12	0.92	0.68	0.50	0.87	0.77	0.64	0.89	1107
0.26	0.62	0.36	0.87	0.81	0.73	0.89	0.50	0.32	0.69	0.49	0.11	0.87	0.65	0.46	0.83	0.75	0.63	0.87	1741
0.29	0.59	0.34	0.84	0.77	0.68	0.87	0.48	0.29	0.66	0.51	0.17	0.85	0.64	0.47	0.82	0.75	0.64	0.85	1250
0.32	0.54	0.27	0.82	0.75	0.64	0.85	0.44	0.24	0.64	0.44	0.07	0.80	0.60	0.39	0.80	0.72	0.60	0.84	1011
0.38	0.50	0.22	0.78	0.76	0.67	0.85	0.39	0.19	0.59	0.41	0.04	0.79	0.58	0.39	0.76	0.70	0.57	0.82	1598

==> data/ra/yelp/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.94	0.90	0.99	0.98	0.97	1.00	0.86	0.78	0.93	0.88	0.81	0.95	0.90	0.85	0.96	0.93	0.89	0.97	3215
0.03	0.86	0.79	0.93	0.96	0.94	0.98	0.73	0.67	0.78	0.77	0.70	0.83	0.81	0.77	0.85	0.87	0.84	0.90	1600
0.06	0.79	0.70	0.88	0.93	0.90	0.96	0.64	0.58	0.70	0.69	0.62	0.76	0.75	0.71	0.79	0.82	0.79	0.85	1649
0.11	0.72	0.62	0.81	0.90	0.86	0.93	0.56	0.50	0.63	0.62	0.54	0.70	0.70	0.65	0.75	0.78	0.75	0.82	2117
0.15	0.62	0.51	0.72	0.84	0.79	0.89	0.48	0.41	0.54	0.54	0.46	0.62	0.63	0.59	0.68	0.74	0.71	0.77	1916
0.18	0.55	0.44	0.66	0.79	0.73	0.85	0.41	0.35	0.48	0.49	0.40	0.58	0.59	0.55	0.64	0.71	0.67	0.74	2514
0.22	0.55	0.41	0.70	0.80	0.70	0.90	0.39	0.31	0.47	0.49	0.37	0.60	0.58	0.52	0.64	0.69	0.65	0.73	281
0.26	0.47	0.36	0.59	0.72	0.65	0.79	0.35	0.29	0.41	0.44	0.36	0.51	0.55	0.51	0.59	0.68	0.65	0.71	2114
0.29	0.43	0.31	0.55	0.68	0.60	0.76	0.32	0.26	0.38	0.41	0.33	0.48	0.52	0.48	0.57	0.66	0.63	0.69	1731
0.32	0.40	0.29	0.51	0.64	0.56	0.72	0.29	0.24	0.35	0.38	0.31	0.46	0.51	0.47	0.55	0.65	0.62	0.68	1666

==> data/ra/yelp/cnn/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.91	0.75	1.07	0.99	0.97	1.00	0.85	0.69	1.02	0.87	0.72	1.02	0.90	0.80	1.01	0.93	0.84	1.01	2668
0.03	0.79	0.59	1.00	0.96	0.94	0.98	0.69	0.51	0.87	0.74	0.56	0.92	0.80	0.68	0.92	0.85	0.75	0.94	2420
0.06	0.69	0.45	0.92	0.95	0.06	1.84	0.56	0.39	0.73	0.64	0.44	0.84	0.72	0.60	0.84	0.79	0.69	0.88	2532
0.11	0.58	0.33	0.82	0.97	-2.69	4.63	0.46	0.29	0.62	0.55	0.36	0.75	0.66	0.53	0.78	0.74	0.65	0.83	2610
0.15	0.47	0.24	0.69	1.03	-4.83	6.88	0.34	0.21	0.48	0.47	0.29	0.65	0.58	0.47	0.69	0.68	0.60	0.76	1887
0.18	0.36	0.12	0.60	1.45	-15.73	18.63	0.26	0.12	0.41	0.40	0.21	0.58	0.53	0.41	0.65	0.64	0.55	0.73	1347
0.22	0.39	0.09	0.69	0.83	0.74	0.92	0.26	0.08	0.44	0.38	0.11	0.65	0.51	0.35	0.68	0.63	0.52	0.75	225
0.26	0.28	0.06	0.50	0.74	0.67	0.81	0.20	0.08	0.32	0.35	0.18	0.52	0.49	0.39	0.59	0.61	0.53	0.68	1186
0.29	0.25	0.04	0.45	0.70	0.63	0.77	0.17	0.06	0.27	0.31	0.15	0.47	0.47	0.37	0.56	0.59	0.52	0.66	1050
0.32	0.21	0.01	0.41	0.65	0.58	0.73	0.14	0.03	0.24	0.30	0.15	0.45	0.44	0.35	0.53	0.57	0.51	0.64	1027

==> data/ri/agnews/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.97	0.90	1.04	0.99	0.99	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1879
0.03	0.91	0.80	1.02	0.98	0.97	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1891
0.06	0.82	0.67	0.97	0.97	0.94	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1960
0.11	0.74	0.56	0.92	0.95	0.92	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1865
0.15	0.61	0.41	0.82	0.91	0.87	0.96	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1772
0.18	0.50	0.27	0.72	0.88	0.82	0.95	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1899
0.22	0.40	0.17	0.64	0.86	0.77	0.95	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	876
0.26	0.35	0.11	0.60	0.83	0.75	0.91	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1817
0.29	0.29	0.06	0.52	0.81	0.72	0.90	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2013
0.32	0.20	-0.00	0.40	0.78	0.68	0.87	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1325
% 0.38	0.19	-0.02	0.40	0.77	0.66	0.88	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2166

==> data/ri/agnews/lstmatt/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.94	0.78	1.09	1.00	0.99	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1839
0.03	0.76	0.49	1.03	0.99	0.98	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1845
0.06	0.53	0.16	0.89	0.98	0.97	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1947
0.11	0.33	-0.08	0.73	0.97	0.95	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1810
0.15	0.08	-0.34	0.51	0.96	0.93	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1701
0.18	-0.11	-0.52	0.31	0.95	0.90	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1894
0.22	-0.25	-0.65	0.16	0.94	0.89	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	937
0.26	-0.30	-0.69	0.08	0.92	0.85	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1625
0.29	-0.38	-0.73	-0.03	0.91	0.83	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1811
0.32	-0.50	-0.84	-0.17	0.89	0.80	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	975
% 0.38	-0.50	-0.80	-0.19	0.89	0.81	0.97	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2178

==> data/ri/mr/cnn/S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2619
0.03	0.54	0.22	0.86	0.98	0.96	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	3205
0.06	0.43	0.25	0.80	0.98	0.96	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	3137
0.11	0.39	0.02	0.77	0.95	0.89	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1671
0.15	0.46	0.11	0.80	0.96	0.92	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	731
0.18	0.41	0.11	0.71	0.90	0.80	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	979
0.22	0.34	0.02	0.66	0.90	0.80	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	596
0.26	0.26	-0.07	0.59	0.85	0.71	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	924
0.29	0.17	-0.16	0.49	0.80	0.65	0.94	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	597
0.32	0.14	-0.19	0.48	0.80	0.64	0.96	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	543
% 0.38	0.02	-0.32	0.36	0.82	0.66	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	582

==> data/ri/mr/lstm/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2722
0.03	0.39	-0.05	0.83	0.98	0.96	0.99		0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1594
0.06	0.21	-0.23	0.65	0.98	0.95	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2729
0.11	0.17	-0.35	0.69	0.95	0.88	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2046
0.15	0.04	-0.48	0.56	0.95	0.89	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1057
0.18	-0.02	-0.54	0.50	0.89	0.79	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1482
0.22	-0.10	-0.59	0.40	0.89	0.78	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1044
0.26	-0.11	-0.58	0.35	0.85	0.73	0.97	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1295
0.29	-0.12	-0.51	0.28	0.80	0.66	0.93	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	818
0.32	-0.17	-0.55	0.21	0.78	0.62	0.94	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	748
% 0.38	-0.15	-0.52	0.22	0.82	0.66	0.97	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	683

==> data/rs/agnews/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.92	0.79	1.05	0.99	0.99	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1879
0.03	0.81	0.62	1.00	0.98	0.97	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1891
0.06	0.72	0.50	0.94	0.97	0.95	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1990
0.11	0.64	0.40	0.89	0.95	0.91	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2232
0.15	0.57	0.32	0.82	0.91	0.87	0.96	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2570
0.18	0.52	0.27	0.77	0.89	0.83	0.94	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2919
0.22	0.49	0.24	0.74	0.86	0.79	0.93	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2546
0.26	0.46	0.22	0.71	0.84	0.77	0.92	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2297
0.29	0.45	0.22	0.69	0.83	0.74	0.92	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1113
0.32	0.42	0.18	0.66	0.82	0.72	0.92	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	814
% 0.38	0.43	0.19	0.67	0.81	0.71	0.92	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	297

==> data/rs/agnews/lstmatt/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.94	0.78	1.10	1.00	0.99	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1839
0.03	0.80	0.53	1.06	0.99	0.98	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1847
0.06	0.68	0.33	1.02	0.98	0.97	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2009
0.11	0.51	0.19	0.93	0.97	0.94	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2265
0.15	0.42	0.08	0.90	0.95	0.92	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2611
0.18	0.40	0.02	0.88	0.94	0.90	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2883
0.22	0.37	-0.01	0.80	0.93	0.88	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2325
0.26	0.36	-0.04	0.77	0.93	0.88	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2214
0.29	0.32	-0.11	0.75	0.93	0.87	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	967
0.32	0.28	-0.12	0.68	0.92	0.87	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	732
% 0.38	0.27	-0.12	0.65	0.94	0.89	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	280

==> data/rs/mr/cnn/S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2619
0.03	0.57	0.21	0.93	0.97	0.95	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	3007
0.06	0.48	0.16	0.89	0.98	0.95	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	3037
0.11	0.52	0.12	0.92	0.95	0.89	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1872
0.15	0.60	0.24	0.95	0.94	0.88	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1064
0.18	0.63	0.35	0.91	0.89	0.79	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1296
0.22	0.60	0.32	0.88	0.89	0.78	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	886
0.26	0.59	0.31	0.88	0.87	0.75	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1013
0.29	0.61	0.35	0.88	0.83	0.69	0.97	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	435
0.32	0.55	0.26	0.83	0.84	0.69	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	396
% 0.38	0.55	0.27	0.82	0.90	0.78	1.02	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	200

==> data/rs/mr/lstm/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2722
0.03	0.52	0.08	0.97	0.97	0.96	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1701
0.06	0.39	-0.06	0.84	0.98	0.95	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	3031
0.11	0.26	-0.26	0.77	0.94	0.87	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	2648
0.15	0.26	-0.27	0.79	0.93	0.85	1.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1618
0.18	0.25	-0.23	0.74	0.89	0.79	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1581
0.22	0.21	-0.22	0.84	0.89	0.78	0.99	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1058
0.26	0.22	-0.21	0.84	0.85	0.73	0.97	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1072
0.29	0.27	-0.09	0.63	0.85	0.72	0.97	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	475
0.32	0.31	-0.15	0.88	0.84	0.70	0.98	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	392
% 0.38	0.24	-0.20	0.70	0.90	0.79	1.01	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	206

==> data/tef/agnews/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.86	0.70	1.02	0.99	0.97	1.01	0.87	0.75	1.00	0.86	0.72	1.00	0.91	0.83	1.00	0.94	0.89	1.00	4750
0.03	0.68	0.49	0.88	0.98	0.95	1.01	0.71	0.62	0.79	0.67	0.56	0.78	0.79	0.73	0.85	0.86	0.82	0.91	4781
0.06	0.57	0.33	0.80	0.96	0.92	1.00	0.59	0.50	0.68	0.56	0.43	0.68	0.71	0.64	0.78	0.81	0.76	0.85	4963
0.11	0.48	0.23	0.73	0.94	0.89	0.99	0.51	0.42	0.61	0.48	0.35	0.61	0.65	0.58	0.72	0.77	0.72	0.82	4727
0.15	0.39	0.14	0.64	0.91	0.85	0.97	0.43	0.33	0.53	0.41	0.27	0.54	0.59	0.52	0.66	0.72	0.67	0.77	4532
0.18	0.34	0.09	0.58	0.88	0.81	0.95	0.36	0.26	0.47	0.35	0.22	0.49	0.54	0.47	0.62	0.69	0.64	0.74	4901
0.22	0.28	0.04	0.53	0.86	0.77	0.94	0.31	0.20	0.43	0.32	0.17	0.46	0.51	0.42	0.59	0.66	0.60	0.72	2513
0.26	0.25	0.02	0.49	0.84	0.75	0.92	0.29	0.19	0.40	0.30	0.16	0.43	0.49	0.42	0.57	0.65	0.60	0.71	4954
0.29	0.21	-0.01	0.43	0.82	0.73	0.91	0.26	0.15	0.37	0.26	0.13	0.39	0.47	0.39	0.55	0.64	0.58	0.69	4991
0.32	0.17	-0.04	0.39	0.80	0.71	0.89	0.22	0.12	0.33	0.24	0.11	0.37	0.45	0.37	0.52	0.62	0.56	0.67	3409
% 0.38	0.14	-0.06	0.34	0.80	0.71	0.89	0.20	0.09	0.30	0.22	0.10	0.33	0.43	0.35	0.50	0.60	0.55	0.66	4539

==> data/tef/agnews/cnn/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.93	0.80	1.05	1.00	0.98	1.01	0.94	0.83	1.05	0.91	0.77	1.05	0.96	0.89	1.03	0.97	0.92	1.02	4622
0.03	0.72	0.53	0.90	0.98	0.96	1.00	0.76	0.63	0.89	0.66	0.48	0.83	0.85	0.75	0.94	0.89	0.83	0.96	4635
0.06	0.51	0.28	0.74	0.96	0.93	0.99	0.59	0.44	0.73	0.46	0.25	0.66	0.74	0.64	0.85	0.83	0.75	0.90	4896
0.11	0.36	0.11	0.62	0.94	0.90	0.98	0.45	0.31	0.59	0.36	0.15	0.58	0.66	0.55	0.77	0.77	0.69	0.85	4532
0.15	0.20	-0.07	0.46	0.91	0.86	0.96	0.30	0.16	0.44	0.29	0.08	0.50	0.56	0.45	0.67	0.70	0.62	0.78	4218
0.18	0.08	-0.19	0.35	0.88	0.83	0.94	0.18	0.04	0.32	0.25	0.04	0.45	0.48	0.36	0.60	0.64	0.56	0.72	4104
0.22	-0.00	-0.27	0.27	0.87	0.81	0.93	0.09	-0.05	0.23	0.21	0.02	0.41	0.43	0.30	0.55	0.60	0.52	0.68	673
0.26	-0.02	-0.31	0.26	0.84	0.77	0.91	0.06	-0.08	0.21	0.21	0.00	0.41	0.41	0.28	0.53	0.58	0.50	0.66	1268
0.29	-0.09	-0.36	0.19	0.83	0.75	0.90	0.00	-0.14	0.14	0.18	-0.00	0.36	0.37	0.25	0.49	0.55	0.47	0.63	1420
0.32	-0.14	-0.42	0.15	0.80	0.71	0.89	-0.05	-0.19	0.10	0.17	-0.01	0.36	0.34	0.23	0.46	0.51	0.43	0.59	1036
0.38	-0.16	-0.42	0.11	0.79	0.71	0.88	-0.09	-0.23	0.06	0.15	-0.02	0.32	0.31	0.19	0.43	0.49	0.41	0.58	2096

==> data/tef/agnews/cnn/S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.96	0.88	1.04	1.00	0.98	1.01	0.94	0.84	1.04	0.88	0.66	1.10	0.94	0.83	1.04	0.96	0.90	1.03	4622
0.03	0.84	0.71	0.97	0.98	0.97	1.00	0.77	0.65	0.90	0.61	0.30	0.93	0.78	0.65	0.92	0.87	0.78	0.96	4635
0.06	0.72	0.54	0.90	0.97	0.94	0.99	0.62	0.47	0.77	0.45	0.13	0.77	0.67	0.52	0.83	0.80	0.70	0.90	4896
0.11	0.62	0.41	0.84	0.95	0.92	0.98	0.51	0.35	0.68	0.36	0.05	0.66	0.59	0.43	0.76	0.75	0.64	0.86	4532
0.15	0.50	0.25	0.74	0.93	0.88	0.97	0.39	0.21	0.58	0.26	-0.02	0.55	0.50	0.33	0.68	0.68	0.57	0.80	4217
0.18	0.38	0.10	0.65	0.90	0.85	0.95	0.29	0.09	0.49	0.20	-0.06	0.47	0.43	0.24	0.61	0.62	0.50	0.75	4583
0.22	0.27	-0.03	0.58	0.88	0.83	0.94	0.21	-0.01	0.42	0.17	-0.09	0.43	0.37	0.18	0.56	0.58	0.44	0.71	1971
0.26	0.23	-0.07	0.54	0.86	0.79	0.93	0.17	-0.04	0.38	0.16	-0.08	0.40	0.35	0.16	0.54	0.56	0.42	0.69	3480
0.29	0.14	-0.16	0.45	0.84	0.76	0.92	0.11	-0.10	0.32	0.12	-0.09	0.34	0.31	0.13	0.49	0.52	0.39	0.65	4315
0.32	0.04	-0.29	0.36	0.80	0.71	0.89	0.02	-0.21	0.24	0.12	-0.09	0.32	0.26	0.08	0.44	0.47	0.33	0.60	1661
% 0.38	-0.06	-0.38	0.25	0.80	0.72	0.88	-0.05	-0.26	0.16	0.09	-0.10	0.28	0.23	0.06	0.39	0.43	0.29	0.56	5439

==> data/tef/agnews/lstm/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.86	0.62	1.10	0.99	0.98	1.00	0.89	0.71	1.08	0.88	0.69	1.08	0.93	0.80	1.06	0.95	0.86	1.04	4694
0.03	0.54	0.25	0.83	0.98	0.96	1.00	0.66	0.46	0.86	0.61	0.38	0.83	0.77	0.62	0.92	0.84	0.73	0.95	4695
0.06	0.30	-0.01	0.62	0.96	0.93	0.99	0.50	0.30	0.70	0.41	0.18	0.65	0.68	0.52	0.83	0.77	0.66	0.88	4962
0.11	0.14	-0.18	0.46	0.94	0.90	0.98	0.38	0.18	0.57	0.31	0.09	0.54	0.60	0.44	0.75	0.72	0.61	0.83	4614
0.15	-0.02	-0.33	0.29	0.91	0.86	0.96	0.24	0.05	0.43	0.23	0.02	0.45	0.51	0.36	0.66	0.66	0.55	0.77	4395
0.18	-0.11	-0.41	0.20	0.89	0.83	0.94	0.14	-0.04	0.32	0.20	-0.00	0.41	0.45	0.30	0.59	0.61	0.51	0.72	4838
0.22	-0.16	-0.47	0.15	0.87	0.80	0.93	0.07	-0.12	0.25	0.18	-0.03	0.39	0.40	0.25	0.55	0.57	0.46	0.68	2386
0.26	-0.19	-0.48	0.10	0.85	0.78	0.92	0.04	-0.14	0.22	0.18	-0.02	0.37	0.38	0.23	0.53	0.56	0.45	0.67	4172
0.29	-0.23	-0.52	0.06	0.83	0.76	0.90	0.00	-0.16	0.17	0.17	-0.03	0.36	0.36	0.22	0.50	0.54	0.44	0.65	4383
0.32	-0.26	-0.54	0.02	0.81	0.73	0.89	-0.04	-0.22	0.14	0.15	-0.04	0.34	0.33	0.18	0.48	0.51	0.40	0.62	2294
0.38	-0.29	-0.58	-0.01	0.80	0.72	0.88	-0.06	-0.21	0.10	0.15	-0.03	0.33	0.33	0.19	0.46	0.51	0.42	0.61	4660

==> data/tef/agnews/lstmatt/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.86	0.59	1.13	1.00	0.98	1.01	0.82	0.53	1.11	0.79	0.44	1.14	0.85	0.60	1.10	0.90	0.73	1.07	4734
0.03	0.55	0.20	0.91	0.98	0.96	1.00	0.46	0.15	0.76	0.36	0.00	0.72	0.55	0.28	0.82	0.70	0.51	0.88	4736
0.06	0.30	-0.10	0.71	0.96	0.94	0.99	0.25	-0.07	0.57	0.21	-0.10	0.51	0.40	0.13	0.67	0.58	0.39	0.78	5010
0.11	0.10	-0.32	0.52	0.94	0.91	0.98	0.10	-0.23	0.42	0.13	-0.12	0.39	0.30	0.04	0.55	0.50	0.31	0.70	4690
0.15	-0.11	-0.52	0.30	0.92	0.87	0.96	-0.06	-0.37	0.25	0.07	-0.11	0.26	0.21	-0.01	0.43	0.42	0.23	0.61	4510
0.18	-0.26	-0.65	0.14	0.89	0.84	0.94	-0.17	-0.48	0.14	0.04	-0.11	0.19	0.15	-0.05	0.35	0.37	0.18	0.55	4862
0.22	-0.36	-0.75	0.02	0.87	0.81	0.93	-0.25	-0.56	0.06	0.03	-0.09	0.15	0.12	-0.06	0.30	0.33	0.14	0.51	2725
0.26	-0.41	-0.77	-0.06	0.85	0.78	0.92	-0.28	-0.57	0.01	0.02	-0.09	0.13	0.11	-0.06	0.27	0.31	0.13	0.49	4401
0.29	-0.45	-0.79	-0.11	0.84	0.77	0.91	-0.32	-0.59	-0.04	0.02	-0.08	0.12	0.09	-0.06	0.24	0.30	0.13	0.46	4532
0.32	-0.54	-0.86	-0.21	0.82	0.74	0.89	-0.39	-0.65	-0.12	0.02	-0.07	0.11	0.07	-0.07	0.20	0.26	0.10	0.41	2839
% 0.38	-0.54	-0.84	-0.25	0.81	0.73	0.89	-0.40	-0.64	-0.15	0.01	-0.06	0.07	0.06	-0.06	0.19	0.25	0.10	0.40	5356

==> data/tef/imdb/lstmatt/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.31	0.02	0.61	0.98	0.96	0.99	0.54	0.38	0.70	0.55	0.38	0.72	0.71	0.60	0.82	0.80	0.72	0.88	4477
0.03	0.08	-0.20	0.35	0.95	0.93	0.98	0.40	0.24	0.55	0.41	0.26	0.57	0.62	0.51	0.73	0.73	0.66	0.81	4472
0.06	-0.09	-0.35	0.16	0.92	0.89	0.95	0.27	0.13	0.41	0.30	0.16	0.44	0.54	0.44	0.65	0.68	0.60	0.76	4522
0.11	-0.20	-0.44	0.05	0.88	0.84	0.92	0.18	0.04	0.32	0.24	0.11	0.36	0.48	0.38	0.59	0.64	0.56	0.72	3976
0.15	-0.28	-0.51	-0.04	0.83	0.78	0.87	0.09	-0.03	0.21	0.19	0.08	0.30	0.42	0.33	0.52	0.59	0.52	0.66	2665
0.18	-0.32	-0.54	-0.10	0.78	0.72	0.83	0.03	-0.09	0.15	0.17	0.06	0.27	0.38	0.29	0.47	0.56	0.49	0.63	2231
0.22	-0.32	-0.56	-0.09	0.75	0.68	0.81	0.00	-0.13	0.13	0.16	0.06	0.27	0.36	0.27	0.45	0.54	0.47	0.61	1022
0.26	-0.37	-0.58	-0.17	0.71	0.66	0.77	-0.02	-0.13	0.09	0.15	0.05	0.25	0.35	0.27	0.43	0.53	0.47	0.60	2980
0.29	-0.39	-0.57	-0.21	0.69	0.62	0.75	-0.05	-0.15	0.06	0.14	0.05	0.24	0.34	0.26	0.42	0.52	0.46	0.58	2119
0.32	-0.40	-0.57	-0.23	0.66	0.60	0.72	-0.06	-0.16	0.04	0.14	0.05	0.23	0.33	0.25	0.40	0.51	0.45	0.57	1022

==> data/tef/mr/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	2859
0.03	0.89	0.78	0.99	0.97	0.95	0.99	0.68	0.53	0.83	0.79	0.66	0.92	0.78	0.67	0.88	0.83	0.74	0.92	1280
0.06	0.87	0.75	0.99	0.95	0.92	0.98	0.59	0.42	0.77	0.76	0.61	0.92	0.73	0.61	0.85	0.78	0.68	0.88	1956
0.11	0.81	0.66	0.96	0.91	0.86	0.96	0.49	0.30	0.67	0.69	0.51	0.87	0.67	0.53	0.80	0.73	0.62	0.83	2605
0.15	0.80	0.66	0.94	0.89	0.83	0.94	0.44	0.26	0.63	0.66	0.45	0.87	0.66	0.52	0.80	0.70	0.59	0.81	1701
0.18	0.75	0.59	0.91	0.85	0.79	0.92	0.38	0.20	0.57	0.64	0.46	0.83	0.61	0.47	0.74	0.67	0.56	0.77	2252
0.22	0.73	0.58	0.88	0.83	0.77	0.90	0.36	0.18	0.55	0.62	0.44	0.80	0.60	0.48	0.73	0.66	0.55	0.77	1776
0.26	0.70	0.53	0.87	0.81	0.73	0.88	0.35	0.17	0.52	0.61	0.43	0.79	0.58	0.46	0.70	0.65	0.55	0.75	2206
0.29	0.68	0.50	0.85	0.77	0.67	0.86	0.31	0.15	0.48	0.59	0.40	0.78	0.55	0.43	0.68	0.63	0.54	0.73	1097
0.32	0.65	0.48	0.83	0.76	0.66	0.85	0.29	0.13	0.44	0.57	0.37	0.76	0.54	0.43	0.65	0.62	0.53	0.71	1007
% 0.38	0.67	0.51	0.83	0.77	0.68	0.86	0.28	0.11	0.45	0.57	0.37	0.77	0.55	0.43	0.67	0.62	0.52	0.71	453

==> data/tef/mr/cnn/S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.68	0.22	1.15	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	2778
0.03	0.52	0.32	0.81	0.98	0.96	1.00	0.70	0.55	0.86	0.69	0.26	1.12	0.79	0.49	1.10	0.86	0.64	1.07	3529
0.06	0.39	0.05	0.73	0.97	0.94	0.99	0.60	0.41	0.80	0.58	0.12	1.05	0.70	0.36	1.04	0.79	0.53	1.04	3383
0.11	0.36	0.00	0.71	0.93	0.88	0.98	0.46	0.23	0.69	0.41	-0.02	0.85	0.61	0.31	0.91	0.74	0.53	0.94	1639
0.15	0.38	0.02	0.73	0.90	0.86	0.95	0.37	0.11	0.63	0.33	-0.08	0.75	0.51	0.21	0.82	0.66	0.46	0.85	792
0.18	0.36	0.04	0.68	0.86	0.79	0.92	0.28	0.03	0.53	0.26	-0.11	0.63	0.44	0.20	0.69	0.61	0.45	0.77	1009
0.22	0.25	-0.10	0.59	0.84	0.77	0.90	0.17	-0.07	0.42	0.19	-0.14	0.52	0.38	0.14	0.61	0.55	0.40	0.70	627
0.26	0.24	-0.10	0.58	0.80	0.72	0.88	0.17	-0.08	0.42	0.19	-0.15	0.52	0.37	0.15	0.59	0.55	0.40	0.71	976
0.29	0.11	-0.23	0.45	0.76	0.66	0.86	0.08	-0.17	0.33	0.13	-0.13	0.38	0.31	0.11	0.52	0.51	0.35	0.66	651
0.32	0.08	-0.27	0.43	0.75	0.65	0.85	0.05	-0.20	0.30	0.13	-0.14	0.41	0.29	0.07	0.50	0.48	0.33	0.63	593
% 0.38	0.02	-0.33	0.37	0.76	0.67	0.85	0.00	-0.23	0.23	0.14	-0.16	0.44	0.27	0.04	0.50	0.46	0.31	0.61	572

==> data/tef/mr/lstm/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.77	0.35	1.19	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	2870
0.03	0.16	-0.20	0.53	0.98	0.96	1.00	0.43	0.09	0.78	0.57	0.15	0.99	0.71	0.41	1.00	0.78	0.57	1.00	1696
0.06	0.07	-0.31	0.45	0.96	0.93	0.99	0.29	-0.12	0.69	0.53	0.07	0.98	0.66	0.31	1.00	0.75	0.50	1.00	2891
0.11	-0.06	-0.53	0.42	0.92	0.87	0.97	0.12	-0.30	0.53	0.35	-0.05	0.75	0.51	0.18	0.84	0.63	0.37	0.88	2192
0.15	-0.14	-0.63	0.34	0.90	0.85	0.95	0.03	-0.38	0.44	0.21	-0.15	0.56	0.40	0.09	0.72	0.55	0.31	0.80	1212
0.18	-0.18	-0.66	0.29	0.86	0.79	0.92	0.03	-0.31	0.37	0.20	-0.11	0.52	0.39	0.14	0.65	0.54	0.35	0.73	1575
0.22	-0.22	-0.67	0.22	0.84	0.77	0.91	0.00	-0.32	0.33	0.17	-0.12	0.47	0.37	0.14	0.60	0.52	0.34	0.71	1152
0.26	-0.24	-0.69	0.20	0.81	0.73	0.88	-0.01	-0.31	0.29	0.17	-0.12	0.45	0.37	0.15	0.58	0.53	0.36	0.69	1390
0.29	-0.22	-0.62	0.18	0.78	0.69	0.87	0.01	-0.26	0.27	0.17	-0.09	0.44	0.39	0.21	0.58	0.53	0.38	0.69	854
0.32	-0.24	-0.64	0.15	0.74	0.64	0.84	-0.04	-0.27	0.20	0.17	-0.09	0.44	0.34	0.14	0.54	0.52	0.37	0.66	760
% 0.38	-0.22	-0.60	0.15	0.77	0.69	0.85	-0.04	-0.29	0.20	0.12	-0.14	0.38	0.37	0.17	0.56	0.51	0.36	0.66	597

==> data/tef/mr/lstmatt/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	3002
0.03	0.59	0.30	0.88	0.97	0.95	0.99	0.65	0.46	0.84	0.52	0.24	0.81	0.75	0.58	0.91	0.83	0.73	0.94	1022
0.06	0.47	0.14	0.80	0.95	0.92	0.99	0.56	0.35	0.78	0.36	-0.01	0.72	0.68	0.49	0.87	0.79	0.67	0.91	1789
0.11	0.28	-0.08	0.64	0.91	0.86	0.97	0.43	0.21	0.64	0.28	-0.04	0.61	0.59	0.41	0.78	0.74	0.61	0.86	2005
0.15	0.16	-0.22	0.54	0.90	0.85	0.95	0.31	0.05	0.56	0.20	-0.12	0.52	0.49	0.25	0.73	0.68	0.54	0.82	1156
0.18	0.07	-0.28	0.42	0.86	0.79	0.92	0.23	0.02	0.44	0.22	-0.10	0.53	0.48	0.28	0.67	0.64	0.51	0.77	1670
0.22	-0.00	-0.35	0.35	0.84	0.76	0.91	0.17	-0.04	0.39	0.18	-0.12	0.48	0.43	0.25	0.62	0.61	0.47	0.74	1350
0.26	-0.07	-0.41	0.27	0.81	0.73	0.89	0.11	-0.11	0.33	0.13	-0.12	0.37	0.39	0.19	0.59	0.59	0.46	0.72	1905
0.29	-0.10	-0.42	0.22	0.77	0.68	0.87	0.09	-0.12	0.29	0.16	-0.10	0.41	0.39	0.20	0.57	0.58	0.45	0.71	1255
0.32	-0.15	-0.48	0.17	0.74	0.64	0.85	0.03	-0.16	0.23	0.12	-0.11	0.35	0.34	0.15	0.52	0.55	0.42	0.67	1174
0.38	-0.20	-0.52	0.12	0.76	0.68	0.85	-0.02	-0.24	0.19	0.09	-0.12	0.31	0.31	0.13	0.49	0.52	0.38	0.65	1289

==> data/tef/yelp/bert/A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.82	0.71	0.92	0.98	0.97	1.00	0.79	0.69	0.89	0.80	0.69	0.90	0.86	0.79	0.93	0.90	0.86	0.95	3212
0.03	0.64	0.54	0.74	0.95	0.93	0.98	0.63	0.56	0.69	0.63	0.56	0.71	0.74	0.70	0.79	0.82	0.79	0.86	1599
0.06	0.53	0.42	0.63	0.92	0.89	0.96	0.53	0.47	0.60	0.54	0.47	0.62	0.68	0.63	0.73	0.78	0.74	0.81	1650
0.11	0.43	0.32	0.54	0.88	0.84	0.93	0.46	0.39	0.53	0.47	0.39	0.55	0.62	0.57	0.67	0.74	0.70	0.77	1656
0.15	0.31	0.21	0.40	0.83	0.77	0.89	0.37	0.30	0.44	0.38	0.31	0.45	0.56	0.51	0.60	0.69	0.66	0.73	1728
0.18	0.24	0.13	0.34	0.78	0.72	0.84	0.31	0.24	0.38	0.33	0.25	0.41	0.52	0.47	0.57	0.66	0.63	0.70	2010
0.22	0.19	0.11	0.27	0.75	0.68	0.83	0.28	0.21	0.35	0.30	0.23	0.37	0.49	0.44	0.55	0.65	0.61	0.68	2060
0.26	0.17	0.09	0.24	0.72	0.65	0.78	0.25	0.19	0.32	0.27	0.21	0.34	0.47	0.43	0.52	0.63	0.60	0.67	3460
0.29	0.14	0.07	0.21	0.70	0.62	0.77	0.22	0.15	0.29	0.25	0.18	0.31	0.45	0.40	0.50	0.62	0.58	0.65	1289
0.32	0.13	0.05	0.21	0.68	0.60	0.76	0.20	0.13	0.27	0.23	0.17	0.29	0.44	0.39	0.48	0.61	0.57	0.64	627

==> data/tef/yelp/cnn/IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.45	0.06	0.85	0.98	0.97	1.00	0.60	0.29	0.91	0.66	0.39	0.93	0.76	0.56	0.97	0.82	0.66	0.98	2793
0.03	0.10	-0.21	0.41	0.96	0.94	0.98	0.35	0.12	0.58	0.41	0.22	0.60	0.61	0.45	0.76	0.70	0.57	0.83	2403
0.06	-0.10	-0.39	0.19	0.93	0.90	0.96	0.20	-0.01	0.40	0.29	0.11	0.47	0.51	0.37	0.66	0.64	0.52	0.75	2625
0.11	-0.23	-0.49	0.03	0.90	0.86	0.94	0.09	-0.08	0.26	0.21	0.06	0.36	0.44	0.32	0.57	0.59	0.49	0.69	2715
0.15	-0.35	-0.58	-0.12	0.85	0.80	0.89	-0.04	-0.18	0.10	0.15	0.02	0.28	0.37	0.26	0.47	0.53	0.44	0.61	2696
0.18	-0.39	-0.62	-0.16	0.80	0.74	0.86	-0.11	-0.24	0.02	0.12	0.00	0.24	0.31	0.21	0.41	0.49	0.41	0.57	2220
0.22	-0.43	-0.63	-0.23	0.77	0.70	0.84	-0.15	-0.27	-0.02	0.12	-0.01	0.24	0.29	0.19	0.39	0.46	0.38	0.53	1734
0.26	-0.45	-0.65	-0.26	0.73	0.67	0.80	-0.20	-0.31	-0.10	0.09	0.00	0.17	0.25	0.17	0.34	0.44	0.37	0.50	2749
0.29	-0.47	-0.66	-0.28	1.04	-8.79	10.86	-0.23	-0.34	-0.11	0.08	-0.03	0.20	0.24	0.15	0.33	0.42	0.35	0.49	930
0.32	-0.47	-0.67	-0.28	0.69	0.62	0.77	-0.25	-0.37	-0.14	0.07	-0.02	0.16	0.21	0.11	0.32	0.41	0.33	0.50	675

==> data/transfer/agnews/cnn/IG/bert_A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.97	0.88	1.06	1.00	0.89	1.10	0.94	0.87	1.01	0.95	0.85	1.05	0.96	0.91	1.01	0.97	0.93	1.01	4121
0.03	0.93	0.85	1.01	0.98	0.87	1.10	0.84	0.76	0.92	0.86	0.71	1.01	0.90	0.83	0.97	0.92	0.87	0.97	4063
0.06	0.87	0.74	1.00	0.98	0.45	1.51	0.74	0.64	0.84	0.78	0.60	0.96	0.84	0.76	0.92	0.87	0.82	0.93	4184
0.11	0.82	0.68	0.95	1.01	-0.53	2.55	0.66	0.56	0.76	0.72	0.53	0.91	0.79	0.70	0.88	0.84	0.78	0.90	3848
0.15	0.74	0.60	0.89	0.98	-0.50	2.45	0.57	0.46	0.68	0.65	0.45	0.84	0.74	0.64	0.84	0.80	0.73	0.86	3548
0.18	0.68	0.52	0.84	0.89	0.82	0.96	0.49	0.37	0.61	0.58	0.38	0.79	0.69	0.59	0.80	0.76	0.69	0.83	3692
0.22	0.64	0.48	0.80	0.89	0.22	1.57	0.44	0.32	0.57	0.54	0.33	0.74	0.66	0.55	0.77	0.74	0.66	0.82	1709
0.26	0.61	0.43	0.78	0.85	0.36	1.35	0.41	0.29	0.53	0.53	0.32	0.74	0.64	0.54	0.75	0.72	0.65	0.80	3415
0.29	0.57	0.39	0.74	0.84	0.25	1.42	0.38	0.26	0.50	0.49	0.29	0.70	0.62	0.52	0.73	0.71	0.64	0.78	3411
0.32	0.52	0.34	0.70	0.93	-1.29	3.14	0.34	0.22	0.47	0.47	0.26	0.68	0.60	0.49	0.70	0.69	0.62	0.77	2257
0.38	0.50	0.32	0.68	0.80	0.71	0.89	0.32	0.20	0.44	0.43	0.21	0.64	0.58	0.47	0.70	0.68	0.60	0.75	3060

==> data/transfer/agnews/cnn/IG/cnn_S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.97	0.89	1.04	1.00	0.61	1.39	0.95	0.86	1.04	0.94	0.83	1.06	0.97	0.90	1.03	0.98	0.93	1.02	4619
0.03	0.88	0.76	1.00	0.99	0.37	1.62	0.81	0.70	0.92	0.79	0.61	0.98	0.88	0.79	0.96	0.91	0.85	0.97	4632
0.06	0.79	0.64	0.94	1.00	-0.02	2.01	0.69	0.57	0.80	0.68	0.48	0.89	0.80	0.71	0.90	0.86	0.79	0.92	4896
0.11	0.72	0.55	0.89	1.10	-2.43	4.62	0.60	0.48	0.72	0.61	0.40	0.81	0.75	0.65	0.85	0.82	0.75	0.89	4537
0.15	0.63	0.46	0.81	1.05	-2.97	5.07	0.50	0.39	0.62	0.53	0.33	0.74	0.69	0.59	0.80	0.77	0.70	0.84	4217
0.18	0.56	0.38	0.75	1.08	-4.88	7.03	0.43	0.31	0.55	0.47	0.25	0.68	0.65	0.54	0.76	0.74	0.66	0.81	4583
0.22	0.52	0.32	0.71	1.78	-14.13	17.70	0.38	0.25	0.50	0.43	0.20	0.67	0.61	0.49	0.73	0.71	0.63	0.79	1978
0.26	0.50	0.31	0.69	1.26	-9.49	12.00	0.36	0.24	0.49	0.41	0.19	0.63	0.60	0.48	0.71	0.70	0.62	0.78	3481
0.29	0.46	0.28	0.64	0.96	-4.73	6.65	0.33	0.21	0.45	0.38	0.16	0.59	0.58	0.46	0.69	0.69	0.61	0.76	4309
0.32	0.43	0.24	0.61	1.63	-15.37	18.64	0.28	0.16	0.40	0.37	0.15	0.59	0.54	0.42	0.65	0.66	0.58	0.74	1662
0.38	0.39	0.21	0.57	0.94	-6.02	7.89	0.27	0.15	0.39	0.31	0.10	0.53	0.52	0.41	0.64	0.65	0.57	0.73	5436

==> data/transfer/agnews/cnn/IG/lstm_IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.98	0.92	1.04	1.00	0.99	1.00	0.96	0.89	1.03	0.95	0.85	1.05	0.97	0.92	1.03	0.98	0.94	1.02	4377
0.03	0.91	0.80	1.01	0.98	0.75	1.22	0.85	0.75	0.94	0.82	0.64	0.99	0.90	0.82	0.97	0.93	0.87	0.98	4265
0.06	0.83	0.69	0.97	0.99	0.05	1.92	0.74	0.63	0.85	0.72	0.52	0.92	0.83	0.74	0.92	0.88	0.82	0.94	4405
0.11	0.77	0.61	0.93	1.01	-0.89	2.91	0.65	0.54	0.77	0.66	0.46	0.86	0.78	0.69	0.88	0.84	0.77	0.91	3971
0.15	0.70	0.51	0.88	1.42	-9.54	12.38	0.56	0.45	0.68	0.59	0.38	0.80	0.73	0.63	0.83	0.80	0.73	0.87	3669
0.18	0.64	0.46	0.82	0.94	-1.90	3.78	0.48	0.36	0.60	0.54	0.32	0.76	0.68	0.58	0.79	0.76	0.69	0.83	3949
0.22	0.60	0.41	0.79	1.31	-6.97	9.60	0.44	0.31	0.56	0.52	0.28	0.75	0.65	0.54	0.76	0.73	0.66	0.81	1929
0.26	0.59	0.40	0.78	1.84	-14.74	18.42	0.41	0.29	0.53	0.50	0.28	0.72	0.64	0.53	0.75	0.72	0.65	0.80	3315
0.29	0.54	0.35	0.73	0.85	-0.52	2.23	0.37	0.25	0.49	0.47	0.25	0.69	0.61	0.50	0.72	0.70	0.63	0.78	3484
0.32	0.55	0.37	0.73	0.81	0.74	0.89	0.35	0.24	0.47	0.47	0.25	0.68	0.60	0.48	0.71	0.69	0.62	0.76	1752
0.38	0.47	0.28	0.67	0.97	-6.40	8.35	0.31	0.18	0.44	0.42	0.19	0.64	0.57	0.46	0.68	0.67	0.59	0.75	3538

==> data/transfer/imdb/lstmatt/IG/cnn_IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.82	0.61	1.04	1.40	-16.73	19.53	0.76	0.62	0.90	0.79	0.64	0.93	0.84	0.75	0.94	0.88	0.82	0.95	3722
0.03	0.72	0.48	0.96	1.93	-32.09	35.95	0.65	0.51	0.79	0.69	0.54	0.85	0.77	0.68	0.87	0.83	0.76	0.90	3612
0.06	0.63	0.38	0.87	1.57	-20.89	24.02	0.56	0.42	0.69	0.62	0.46	0.77	0.72	0.62	0.81	0.79	0.72	0.86	2469
0.11	0.55	0.31	0.80	1.46	-23.32	26.25	0.49	0.36	0.61	0.56	0.41	0.71	0.67	0.58	0.76	0.76	0.69	0.82	1885
0.15	0.46	0.22	0.70	2.73	-48.71	54.16	0.40	0.29	0.52	0.49	0.34	0.64	0.61	0.52	0.70	0.72	0.65	0.78	2618
0.18	0.38	0.15	0.62	1.85	-32.12	35.83	0.33	0.22	0.44	0.43	0.29	0.57	0.57	0.48	0.65	0.68	0.62	0.74	1002
0.22	0.35	0.12	0.58	18.17	-163.61	199.95	0.29	0.20	0.38	0.41	0.27	0.54	0.53	0.46	0.59	0.66	0.60	0.71	377
0.26	0.34	0.13	0.55	1.61	-28.37	31.58	0.27	0.18	0.37	0.39	0.25	0.53	0.52	0.44	0.60	0.65	0.60	0.71	1112
0.29	0.31	0.10	0.52	3.29	-46.48	53.06	0.25	0.16	0.35	0.37	0.24	0.49	0.51	0.44	0.59	0.65	0.59	0.70	716
0.32	0.28	0.07	0.49	30.43	-349.48	410.34	0.24	0.14	0.33	0.35	0.22	0.49	0.50	0.41	0.59	0.64	0.58	0.70	551

==> data/transfer/imdb/lstmatt/IG/lstm_IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.68	0.42	0.93	0.98	0.96	0.99	0.68	0.54	0.82	0.70	0.56	0.85	0.79	0.70	0.89	0.85	0.78	0.92	3783
0.03	0.54	0.28	0.80	0.96	0.93	0.98	0.56	0.43	0.70	0.59	0.45	0.74	0.72	0.62	0.82	0.80	0.73	0.87	3627
0.06	0.43	0.18	0.69	1.03	-5.64	7.71	0.47	0.34	0.60	0.52	0.37	0.66	0.66	0.57	0.75	0.76	0.69	0.82	3518
0.11	0.36	0.12	0.61	1.38	-13.23	16.00	0.40	0.28	0.52	0.46	0.32	0.60	0.62	0.53	0.71	0.72	0.66	0.79	3421
0.15	0.30	0.07	0.53	1.86	-26.40	30.12	0.33	0.22	0.44	0.40	0.27	0.54	0.56	0.48	0.65	0.69	0.63	0.75	2006
0.18	0.25	0.03	0.48	1.06	-10.47	12.58	0.27	0.17	0.38	0.37	0.24	0.50	0.53	0.45	0.61	0.66	0.60	0.72	1660
0.22	0.24	-0.01	0.48	4.61	-35.84	45.06	0.24	0.13	0.35	0.36	0.21	0.51	0.50	0.42	0.59	0.64	0.57	0.70	436
0.26	0.23	0.01	0.45	0.86	-7.47	9.18	0.23	0.13	0.33	0.34	0.21	0.47	0.50	0.42	0.57	0.63	0.58	0.69	3247
0.29	0.21	0.00	0.41	1.24	-18.41	20.89	0.21	0.11	0.30	0.33	0.21	0.46	0.48	0.41	0.56	0.62	0.57	0.68	1200
0.32	0.20	-0.00	0.40	4.22	-48.42	56.87	0.19	0.10	0.28	0.33	0.19	0.46	0.47	0.39	0.54	0.62	0.56	0.67	1018

==> data/transfer/imdb/lstmatt/IG/lstmatt_A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.72	0.51	0.93	0.98	0.96	0.99	0.69	0.57	0.81	0.70	0.56	0.83	0.80	0.71	0.88	0.86	0.79	0.92	4467
0.03	0.58	0.36	0.80	1.00	-2.50	4.50	0.57	0.45	0.69	0.58	0.44	0.73	0.72	0.63	0.81	0.80	0.74	0.87	4462
0.06	0.47	0.26	0.68	1.05	-5.62	7.72	0.47	0.35	0.58	0.48	0.34	0.63	0.65	0.57	0.74	0.75	0.69	0.82	4473
0.11	0.39	0.19	0.60	1.02	-8.76	10.81	0.40	0.29	0.50	0.42	0.28	0.56	0.61	0.52	0.69	0.72	0.66	0.78	4454
0.15	0.32	0.12	0.51	1.23	-16.56	19.02	0.32	0.22	0.42	0.35	0.22	0.49	0.55	0.47	0.63	0.68	0.63	0.74	2675
0.18	0.27	0.09	0.45	1.21	-10.73	13.16	0.26	0.17	0.35	0.31	0.18	0.44	0.51	0.43	0.59	0.66	0.60	0.71	2692
0.22	0.27	0.05	0.49	6.96	-44.32	58.24	0.25	0.15	0.35	0.30	0.14	0.47	0.48	0.38	0.58	0.64	0.58	0.70	291
0.26	0.24	0.07	0.41	1.73	-25.94	29.40	0.21	0.12	0.30	0.27	0.15	0.39	0.47	0.39	0.54	0.63	0.57	0.68	3352
0.29	0.21	0.04	0.38	1.14	-17.05	19.33	0.18	0.10	0.27	0.24	0.12	0.37	0.45	0.37	0.52	0.61	0.56	0.66	2525
0.32	0.20	0.05	0.35	3.63	-67.23	74.49	0.17	0.09	0.24	0.23	0.12	0.35	0.43	0.36	0.50	0.60	0.55	0.65	3131

==> data/transfer/imdb/lstmatt/IG/lstmatt_S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.74	0.54	0.95	0.98	0.96	0.99	0.71	0.59	0.83	0.72	0.58	0.86	0.81	0.73	0.90	0.87	0.80	0.93	4467
0.03	0.62	0.40	0.84	0.95	0.93	0.98	0.60	0.48	0.72	0.62	0.48	0.76	0.74	0.65	0.83	0.82	0.75	0.88	4462
0.06	0.51	0.29	0.73	1.16	-7.39	9.71	0.50	0.39	0.62	0.53	0.38	0.67	0.68	0.59	0.76	0.77	0.71	0.84	4472
0.11	0.44	0.22	0.65	2.34	-38.86	43.53	0.43	0.32	0.54	0.47	0.32	0.61	0.63	0.55	0.71	0.74	0.68	0.80	4463
0.15	0.37	0.17	0.57	5.40	-102.76	113.56	0.35	0.25	0.45	0.40	0.27	0.54	0.57	0.49	0.66	0.70	0.64	0.76	3137
0.18	0.33	0.13	0.53	1.32	-12.99	15.64	0.30	0.20	0.39	0.36	0.23	0.50	0.54	0.46	0.61	0.67	0.61	0.73	2499
0.22	0.32	0.10	0.53	8.97	-68.37	86.32	0.27	0.17	0.38	0.35	0.19	0.51	0.52	0.43	0.61	0.65	0.59	0.72	765
0.26	0.29	0.11	0.48	1.13	-14.02	16.28	0.25	0.16	0.33	0.32	0.20	0.45	0.49	0.42	0.57	0.64	0.59	0.70	4270
0.29	0.28	0.10	0.46	0.91	-12.21	14.04	0.23	0.14	0.31	0.31	0.18	0.44	0.48	0.40	0.55	0.63	0.58	0.68	3178
0.32	0.26	0.08	0.44	5.21	-70.86	81.28	0.20	0.13	0.28	0.29	0.16	0.42	0.46	0.38	0.53	0.62	0.57	0.67	1630

==> data/transfer/yelp/cnn/IG/bert_A.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.90	0.74	1.06	0.99	0.81	1.17	0.84	0.67	1.01	0.86	0.69	1.02	0.90	0.79	1.01	0.92	0.83	1.01	1444
0.03	0.76	0.51	1.01	0.99	0.47	1.51	0.67	0.48	0.86	0.72	0.53	0.91	0.79	0.67	0.92	0.84	0.74	0.94	609
0.06	0.63	0.33	0.93	1.05	-0.16	2.25	0.54	0.36	0.73	0.61	0.39	0.82	0.71	0.58	0.84	0.78	0.68	0.87	575
0.11	0.55	0.28	0.83	1.06	-1.06	3.18	0.45	0.28	0.62	0.56	0.36	0.76	0.66	0.53	0.78	0.73	0.64	0.83	518
0.15	0.45	0.17	0.73	1.32	-3.29	5.93	0.34	0.18	0.49	0.48	0.28	0.68	0.58	0.47	0.70	0.68	0.59	0.76	466
0.18	0.37	0.12	0.62	0.80	0.56	1.03	0.27	0.13	0.40	0.40	0.22	0.59	0.54	0.43	0.65	0.64	0.57	0.72	506
0.22	0.30	0.06	0.55	0.78	0.42	1.15	0.24	0.12	0.36	0.38	0.17	0.58	0.52	0.42	0.61	0.63	0.56	0.70	515
0.26	0.27	0.02	0.52	0.73	0.65	0.82	0.20	0.07	0.32	0.33	0.15	0.51	0.49	0.40	0.58	0.61	0.54	0.69	709
0.29	0.24	0.02	0.46	0.71	0.63	0.79	0.17	0.05	0.28	0.31	0.14	0.47	0.47	0.38	0.57	0.60	0.53	0.67	269
0.32	0.27	0.02	0.52	0.76	-0.30	1.83	0.16	0.04	0.29	0.37	0.18	0.57	0.47	0.38	0.55	0.59	0.52	0.67	148

==> data/transfer/yelp/cnn/IG/cnn_S.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.68	0.35	1.02	5.11	-52.83	63.05	0.70	0.43	0.96	0.74	0.51	0.97	0.81	0.64	0.99	0.86	0.72	0.99	1754
0.03	0.53	0.27	0.79	0.96	0.94	0.98	0.51	0.29	0.72	0.55	0.34	0.76	0.69	0.54	0.83	0.77	0.65	0.88	1168
0.06	0.42	0.17	0.67	1.14	-5.87	8.15	0.41	0.23	0.60	0.47	0.27	0.67	0.63	0.50	0.76	0.72	0.62	0.83	1143
0.11	0.33	0.11	0.56	1.12	-6.05	8.28	0.32	0.16	0.48	0.40	0.22	0.58	0.57	0.45	0.69	0.68	0.59	0.77	1094
0.15	0.25	0.05	0.46	1.14	-8.38	10.66	0.24	0.11	0.37	0.32	0.14	0.49	0.51	0.41	0.62	0.64	0.55	0.72	1037
0.18	0.19	-0.01	0.38	1.06	-7.94	10.06	0.18	0.07	0.30	0.26	0.09	0.43	0.47	0.37	0.57	0.61	0.53	0.69	1160
0.22	0.17	-0.06	0.41	0.78	0.69	0.86	0.15	-0.00	0.30	0.20	0.01	0.40	0.43	0.29	0.56	0.58	0.49	0.67	572
0.26	0.16	-0.02	0.33	1.29	-15.69	18.28	0.13	0.02	0.23	0.22	0.07	0.36	0.42	0.33	0.51	0.57	0.51	0.64	1751
0.29	0.14	-0.01	0.28	1.07	-11.99	14.13	0.11	0.02	0.20	0.19	0.06	0.32	0.40	0.32	0.48	0.56	0.50	0.62	1159
0.32	0.11	-0.04	0.27	1.89	-27.76	31.54	0.09	-0.01	0.19	0.17	0.04	0.31	0.38	0.29	0.46	0.55	0.49	0.61	1124

==> data/transfer/yelp/cnn/IG/lstmatt_IG.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.86	0.66	1.07	0.99	0.97	1.00	0.84	0.64	1.03	0.84	0.66	1.03	0.90	0.77	1.02	0.92	0.82	1.02	704
0.03	0.71	0.48	0.95	0.96	0.93	0.98	0.67	0.49	0.85	0.70	0.50	0.90	0.79	0.67	0.92	0.84	0.74	0.94	522
0.06	0.61	0.36	0.86	1.03	-1.29	3.35	0.55	0.37	0.72	0.60	0.40	0.81	0.72	0.60	0.84	0.78	0.68	0.88	486
0.11	0.51	0.23	0.78	0.90	0.85	0.94	0.46	0.28	0.63	0.52	0.30	0.75	0.66	0.54	0.78	0.74	0.65	0.84	463
0.15	0.40	0.14	0.65	0.84	0.78	0.90	0.33	0.18	0.48	0.43	0.23	0.64	0.58	0.46	0.70	0.68	0.59	0.78	406
0.18	0.33	0.06	0.60	1.16	-7.06	9.39	0.26	0.11	0.40	0.39	0.20	0.57	0.54	0.41	0.66	0.65	0.56	0.73	510
0.22	0.28	0.02	0.53	0.77	0.69	0.85	0.21	0.08	0.34	0.37	0.15	0.59	0.51	0.38	0.63	0.62	0.53	0.70	393
0.26	0.23	0.01	0.45	1.00	-6.04	8.03	0.19	0.07	0.30	0.31	0.13	0.49	0.48	0.38	0.58	0.61	0.54	0.67	698
0.29	0.21	0.00	0.43	2.03	-21.03	25.10	0.15	0.04	0.27	0.29	0.12	0.45	0.46	0.35	0.56	0.58	0.51	0.65	304
0.32	0.26	-0.01	0.54	3.10	-15.36	21.56	0.18	0.02	0.34	0.31	0.09	0.54	0.46	0.32	0.60	0.60	0.51	0.68	166

==> data/universal/agnews/lstm/IG_spec.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.97	0.88	1.07	1.00	0.98	1.02	0.95	0.85	1.04	0.96	0.84	1.07	0.96	0.89	1.04	0.97	0.91	1.03	4677
0.03	0.91	0.76	1.06	0.99	0.89	1.09	0.81	0.69	0.94	0.83	0.64	1.03	0.87	0.77	0.98	0.89	0.80	0.98	4589
0.06	0.82	0.62	1.01	0.98	0.81	1.15	0.70	0.55	0.85	0.74	0.51	0.97	0.80	0.68	0.93	0.82	0.72	0.92	4736
0.11	0.74	0.52	0.96	0.95	0.92	0.98	0.61	0.45	0.77	0.67	0.44	0.91	0.75	0.61	0.88	0.78	0.67	0.88	4277
0.15	0.64	0.40	0.88	0.94	0.51	1.38	0.50	0.34	0.67	0.60	0.36	0.84	0.68	0.55	0.82	0.72	0.61	0.83	3804
0.18	0.55	0.31	0.80	0.90	0.85	0.95	0.42	0.26	0.58	0.53	0.28	0.77	0.63	0.49	0.77	0.67	0.56	0.79	3935
0.22	0.50	0.24	0.76	0.89	0.52	1.26	0.37	0.21	0.53	0.48	0.23	0.73	0.59	0.45	0.74	0.65	0.53	0.76	1648
0.26	0.47	0.22	0.73	0.88	0.36	1.40	0.35	0.19	0.51	0.47	0.22	0.72	0.58	0.43	0.72	0.63	0.52	0.74	2828
0.29	0.43	0.18	0.69	0.85	0.44	1.25	0.31	0.15	0.46	0.43	0.19	0.67	0.55	0.42	0.69	0.60	0.49	0.72	3312
0.32	0.40	0.13	0.68	0.79	0.57	1.00	0.28	0.12	0.45	0.40	0.14	0.66	0.54	0.40	0.68	0.59	0.47	0.71	1075
0.38	0.35	0.09	0.61	0.78	0.70	0.87	0.24	0.09	0.39	0.37	0.12	0.61	0.51	0.37	0.64	0.57	0.46	0.68	3882

==> data/universal/agnews/lstm/IG_uni.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	0.97	0.87	1.07	1.00	0.98	1.02	0.95	0.85	1.04	0.95	0.83	1.07	0.96	0.89	1.04	0.97	0.91	1.03	4679
0.03	0.90	0.75	1.05	0.99	0.93	1.04	0.81	0.68	0.94	0.83	0.62	1.03	0.87	0.77	0.98	0.89	0.80	0.97	4568
0.06	0.80	0.60	1.00	0.97	0.84	1.10	0.69	0.54	0.84	0.73	0.49	0.96	0.80	0.68	0.92	0.82	0.72	0.92	4730
0.11	0.71	0.48	0.94	0.96	0.76	1.15	0.59	0.43	0.75	0.66	0.42	0.89	0.74	0.61	0.87	0.77	0.66	0.88	4253
0.15	0.59	0.34	0.85	0.92	0.88	0.97	0.48	0.32	0.64	0.57	0.33	0.81	0.67	0.53	0.81	0.71	0.60	0.82	3748
0.18	0.50	0.24	0.76	0.89	0.84	0.95	0.39	0.23	0.55	0.50	0.25	0.74	0.61	0.47	0.75	0.66	0.55	0.77	3790
0.22	0.44	0.18	0.71	0.87	0.81	0.93	0.34	0.18	0.49	0.45	0.20	0.70	0.57	0.43	0.72	0.62	0.51	0.74	1544
0.26	0.41	0.14	0.68	0.89	0.18	1.61	0.32	0.16	0.47	0.43	0.19	0.68	0.56	0.42	0.69	0.61	0.50	0.72	2615
0.29	0.37	0.10	0.63	0.83	0.75	0.90	0.27	0.12	0.42	0.40	0.16	0.64	0.53	0.39	0.66	0.59	0.48	0.69	2946
0.32	0.34	0.07	0.61	0.79	0.61	0.96	0.25	0.08	0.41	0.37	0.11	0.63	0.51	0.37	0.65	0.57	0.45	0.69	937
0.38	0.28	0.02	0.54	0.78	0.54	1.02	0.20	0.05	0.34	0.33	0.10	0.57	0.48	0.35	0.61	0.54	0.44	0.65	3400

==> data/universal/mr/lstmatt/IG_spec.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	0.95	1.05	1.00	0.98	1.02	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	3131
0.03	0.90	0.75	1.04	0.97	0.95	0.99	0.82	0.70	0.95	0.80	0.54	1.06	0.87	0.75	0.99	0.90	0.82	0.99	974
0.06	0.86	0.70	1.03	0.95	0.92	0.99	0.77	0.62	0.91	0.77	0.44	1.10	0.83	0.68	0.97	0.87	0.77	0.97	1740
0.11	0.78	0.57	0.99	0.92	0.87	0.96	0.67	0.49	0.85	0.65	0.28	1.02	0.76	0.58	0.94	0.83	0.72	0.94	2135
0.15	0.70	0.46	0.94	0.89	0.84	0.95	0.60	0.41	0.79	0.60	0.21	0.99	0.71	0.50	0.91	0.80	0.68	0.92	1461
0.18	0.69	0.46	0.92	0.86	0.79	0.93	0.57	0.39	0.75	0.55	0.19	0.92	0.70	0.54	0.86	0.78	0.67	0.89	1815
0.22	0.60	0.34	0.86	0.84	0.77	0.91	0.50	0.31	0.69	0.50	0.14	0.86	0.66	0.49	0.82	0.75	0.64	0.86	1404
0.26	0.58	0.31	0.85	0.82	0.74	0.89	0.47	0.28	0.66	0.48	0.11	0.86	0.63	0.46	0.81	0.74	0.62	0.85	1380
0.29	0.57	0.30	0.84	0.79	0.71	0.87	0.45	0.27	0.63	0.49	0.14	0.85	0.62	0.45	0.78	0.72	0.62	0.83	676
0.32	0.51	0.23	0.78	0.79	0.69	0.88	0.41	0.21	0.61	0.44	0.06	0.82	0.58	0.38	0.78	0.71	0.58	0.83	638
0.38	0.50	0.21	0.79	0.79	0.71	0.87	0.38	0.16	0.60	0.43	0.02	0.85	0.57	0.36	0.79	0.69	0.54	0.84	414

==> data/universal/mr/lstmatt/IG_uni.tex <==
x	pcc	lpcc	upcc	ss	lss	uss	kd	lkd	ukd	top10	ltop10	utop10	top30	ltop30	utop30	top50	ltop50	utop50	count
0.01	1.00	0.95	1.05	1.00	0.98	1.02	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	1.00	3087
0.03	0.86	0.67	1.05	0.97	0.95	0.99	0.79	0.65	0.93	0.78	0.51	1.04	0.85	0.72	0.98	0.89	0.80	0.97	942
0.06	0.81	0.60	1.02	0.95	0.92	0.98	0.73	0.56	0.89	0.74	0.40	1.08	0.80	0.65	0.95	0.86	0.76	0.96	1654
0.11	0.70	0.42	0.97	0.92	0.87	0.96	0.61	0.42	0.80	0.63	0.27	0.99	0.73	0.55	0.90	0.81	0.69	0.92	1921
0.15	0.60	0.30	0.91	0.90	0.84	0.95	0.53	0.32	0.73	0.52	0.11	0.93	0.65	0.43	0.88	0.77	0.64	0.90	1180
0.18	0.54	0.25	0.82	0.86	0.79	0.92	0.48	0.29	0.67	0.47	0.11	0.83	0.65	0.48	0.82	0.75	0.63	0.87	1637
0.22	0.47	0.18	0.75	0.84	0.77	0.91	0.41	0.22	0.60	0.41	0.06	0.77	0.60	0.43	0.77	0.71	0.60	0.82	1224
0.26	0.39	0.07	0.71	0.81	0.73	0.89	0.35	0.16	0.55	0.39	0.03	0.74	0.56	0.38	0.74	0.69	0.58	0.81	1355
0.29	0.37	0.07	0.68	0.78	0.68	0.88	0.33	0.12	0.54	0.37	0.03	0.70	0.55	0.37	0.72	0.67	0.55	0.80	597
0.32	0.31	0.02	0.59	0.77	0.67	0.87	0.27	0.10	0.44	0.33	-0.02	0.69	0.50	0.30	0.70	0.65	0.53	0.77	573
0.38	0.30	-0.01	0.60	0.78	0.69	0.86	0.26	0.04	0.47	0.32	-0.06	0.70	0.51	0.31	0.71	0.64	0.51	0.77	378

==> data_new/ra/agnews/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.99	0.04	1.0	0.99	1.0	0.99	0.02	1.0	0.99	1.0	0.98	0.03	0.99	0.96	1.0	0.34	0.55	0.15	0.0	0.48	0.5	1.21	0.08	0.0	0.51	0.92	0.08	0.92	0.87	1.0	0.94	0.07	0.96	0.9	1.0	0.95	0.05	0.95	0.91	1.0	0.96	0.04	0.96	0.93	1.0	247.51	244.87	195.44	129.75	299.09	263.08	248.02	211.36	138.58	318.66	3792	0.01
0.03	0.96	0.07	0.99	0.96	1.0	0.97	0.02	0.98	0.97	0.99	0.93	0.05	0.94	0.91	0.97	0.8	0.76	0.57	0.3	0.99	1.1	1.73	0.5	0.18	1.28	0.82	0.07	0.82	0.78	0.87	0.86	0.09	0.87	0.8	0.93	0.87	0.05	0.88	0.84	0.91	0.91	0.03	0.91	0.89	0.93	246.3	232.35	195.62	129.84	299.72	298.12	248.74	240.03	157.68	365.1	3820	0.05
0.06	0.93	0.1	0.97	0.9	0.99	0.95	0.04	0.96	0.94	0.97	0.87	0.06	0.88	0.84	0.92	1.19	0.89	0.97	0.55	1.57	1.75	2.29	0.92	0.33	2.22	0.73	0.07	0.73	0.68	0.78	0.79	0.1	0.79	0.73	0.86	0.81	0.06	0.81	0.78	0.85	0.86	0.04	0.87	0.84	0.89	245.37	235.72	195.5	129.85	297.54	357.28	274.69	294.09	192.81	435.13	3835	0.1
0.11	0.89	0.12	0.94	0.84	0.98	0.92	0.04	0.93	0.9	0.95	0.82	0.08	0.83	0.77	0.88	1.5	0.99	1.29	0.77	2.02	2.27	2.67	1.35	0.49	3.03	0.66	0.08	0.66	0.61	0.72	0.73	0.11	0.74	0.66	0.81	0.76	0.06	0.76	0.72	0.8	0.83	0.04	0.83	0.8	0.86	249.42	303.75	194.19	129.68	298.04	434.31	338.18	351.76	233.38	521.92	2477	0.17
0.15	0.85	0.15	0.89	0.77	0.96	0.88	0.06	0.89	0.85	0.91	0.75	0.09	0.76	0.69	0.81	1.86	1.1	1.7	1.07	2.44	2.9	3.22	1.85	0.72	3.97	0.58	0.08	0.58	0.52	0.63	0.67	0.12	0.67	0.59	0.75	0.7	0.06	0.7	0.66	0.74	0.79	0.04	0.79	0.76	0.82	246.89	309.32	193.83	129.0	297.5	553.52	377.09	454.63	315.16	670.05	2208	0.28
0.18	0.8	0.17	0.84	0.7	0.94	0.82	0.07	0.84	0.78	0.88	0.67	0.1	0.68	0.61	0.75	2.13	1.12	2.03	1.32	2.82	3.37	3.51	2.22	0.86	4.81	0.51	0.09	0.51	0.45	0.57	0.61	0.13	0.61	0.52	0.7	0.65	0.06	0.65	0.61	0.7	0.75	0.05	0.75	0.72	0.78	248.69	312.02	195.25	129.47	299.45	712.89	474.63	586.07	404.42	880.57	2091	0.43
0.32	0.68	0.22	0.71	0.54	0.86	0.66	0.13	0.67	0.57	0.76	0.51	0.15	0.51	0.41	0.61	2.73	1.15	2.71	1.97	3.43	4.44	4.13	3.3	1.36	6.26	0.37	0.12	0.37	0.29	0.45	0.5	0.15	0.49	0.4	0.6	0.55	0.08	0.55	0.5	0.61	0.68	0.06	0.68	0.64	0.72	245.11	261.02	193.9	128.82	297.06	1315.54	950.19	1080.71	708.03	1623.32	6568	1.0


==> data_new/ra/agnews/bert/A_auc.tex <==
0.27

==> data_new/ra/agnews/bert/A_ppl.tex <==
4.4

==> data_new/ra/agnews/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.92	0.15	0.98	0.91	1.0	0.99	0.02	1.0	0.99	1.0	0.91	0.14	0.96	0.86	1.0	0.7	3.09	0.07	0.0	0.28	1.92	3.25	0.45	0.0	2.59	0.83	0.18	0.86	0.72	1.0	0.85	0.2	1.0	0.67	1.0	0.88	0.13	0.93	0.8	1.0	0.91	0.1	0.93	0.85	1.0	247.61	244.84	195.55	129.84	299.44	263.19	247.99	211.46	138.68	318.89	3792	0.02
0.03	0.79	0.21	0.85	0.72	0.93	0.97	0.02	0.98	0.97	0.99	0.76	0.18	0.8	0.68	0.89	1.94	7.83	0.31	0.15	0.95	3.93	4.15	2.61	1.13	5.26	0.62	0.17	0.65	0.53	0.74	0.64	0.24	0.67	0.5	0.8	0.73	0.13	0.75	0.67	0.83	0.81	0.09	0.81	0.75	0.88	245.5	231.68	195.26	129.84	298.63	296.97	246.45	239.96	157.28	364.7	3814	0.05
0.06	0.64	0.25	0.69	0.52	0.82	0.95	0.03	0.96	0.94	0.97	0.61	0.21	0.64	0.5	0.76	2.98	11.41	0.45	0.23	1.42	5.36	4.95	3.98	1.83	7.28	0.47	0.17	0.49	0.37	0.59	0.51	0.24	0.5	0.33	0.67	0.63	0.14	0.64	0.55	0.73	0.73	0.1	0.74	0.67	0.8	245.46	267.47	195.39	129.88	297.16	352.74	280.43	289.12	193.61	432.45	3683	0.11
0.11	0.52	0.27	0.56	0.36	0.71	0.92	0.04	0.93	0.9	0.95	0.48	0.22	0.51	0.36	0.64	3.68	11.25	0.55	0.29	1.94	6.42	5.57	4.98	2.23	8.92	0.36	0.17	0.38	0.26	0.48	0.43	0.24	0.4	0.25	0.6	0.56	0.14	0.56	0.47	0.65	0.67	0.1	0.68	0.62	0.75	252.35	311.18	195.62	129.93	300.96	443.61	350.98	356.31	234.83	531.72	2358	0.18
0.15	0.39	0.27	0.41	0.22	0.58	0.87	0.06	0.89	0.84	0.92	0.35	0.21	0.37	0.22	0.51	4.59	11.54	0.72	0.35	3.13	7.48	6.32	5.77	2.7	10.6	0.26	0.16	0.26	0.16	0.37	0.35	0.23	0.33	0.2	0.5	0.49	0.13	0.5	0.41	0.58	0.63	0.09	0.62	0.57	0.69	242.69	236.69	193.27	128.9	296.56	556.72	403.65	452.76	315.21	683.35	3605	0.32
0.18	0.29	0.27	0.3	0.12	0.48	0.82	0.07	0.84	0.79	0.88	0.26	0.21	0.27	0.13	0.41	5.61	12.9	0.92	0.42	5.04	8.3	6.87	6.65	3.08	11.75	0.19	0.15	0.2	0.09	0.3	0.29	0.22	0.25	0.17	0.4	0.44	0.13	0.44	0.36	0.53	0.59	0.09	0.59	0.53	0.65	245.07	234.69	195.12	129.68	297.88	720.33	655.0	591.32	404.33	867.23	3772	0.47
0.32	0.16	0.25	0.15	-0.01	0.32	0.68	0.13	0.69	0.59	0.78	0.13	0.19	0.13	0.0	0.27	8.7	14.71	2.44	0.69	12.18	9.47	7.73	7.61	3.52	13.49	0.1	0.14	0.09	0.0	0.19	0.22	0.2	0.2	0.0	0.33	0.38	0.12	0.38	0.3	0.47	0.54	0.09	0.54	0.48	0.6	244.53	229.27	194.3	129.27	297.19	1247.11	897.04	1026.23	679.63	1548.39	10056	1.0


==> data_new/ra/agnews/bert/IG_auc.tex <==
0.14

==> data_new/ra/agnews/bert/IG_ppl.tex <==
4.1

==> data_new/ra/agnews/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.97	0.08	0.99	0.96	1.0	0.99	0.02	1.0	0.99	1.0	0.97	0.05	0.99	0.96	1.0	2.84	14.0	0.21	0.0	0.99	0.4	0.73	0.09	0.0	0.5	0.91	0.1	0.93	0.86	1.0	0.89	0.16	1.0	0.8	1.0	0.93	0.09	0.95	0.88	1.0	0.96	0.06	0.97	0.93	1.0	247.61	244.81	195.55	129.84	299.44	263.19	247.96	211.46	138.68	318.89	3792	0.02
0.03	0.9	0.12	0.94	0.88	0.97	0.97	0.02	0.98	0.97	0.99	0.92	0.08	0.94	0.89	0.96	8.22	26.83	1.24	0.55	3.64	0.81	0.97	0.51	0.22	1.03	0.79	0.1	0.81	0.75	0.86	0.74	0.21	0.75	0.6	1.0	0.84	0.1	0.86	0.79	0.92	0.9	0.06	0.91	0.86	0.94	246.2	232.41	195.49	129.75	299.74	297.99	248.81	240.07	157.56	364.68	3820	0.06
0.06	0.84	0.13	0.88	0.78	0.93	0.95	0.04	0.96	0.94	0.97	0.87	0.09	0.89	0.83	0.93	11.15	33.49	1.83	0.81	5.5	1.1	1.11	0.77	0.34	1.48	0.72	0.1	0.73	0.66	0.79	0.65	0.22	0.67	0.5	0.8	0.78	0.11	0.79	0.71	0.86	0.86	0.07	0.87	0.82	0.91	245.37	235.72	195.5	129.85	297.54	357.28	274.69	294.09	192.81	435.13	3835	0.12
0.11	0.78	0.16	0.82	0.71	0.89	0.92	0.04	0.93	0.9	0.95	0.82	0.11	0.84	0.77	0.89	15.48	45.41	2.32	1.03	7.31	1.31	1.2	0.98	0.46	1.8	0.66	0.11	0.67	0.6	0.73	0.57	0.22	0.6	0.4	0.75	0.73	0.11	0.75	0.67	0.81	0.83	0.07	0.84	0.79	0.88	251.69	301.97	195.72	130.83	301.87	442.46	346.44	355.98	236.42	531.46	2561	0.2
0.15	0.71	0.17	0.74	0.62	0.84	0.87	0.06	0.89	0.84	0.92	0.77	0.12	0.79	0.71	0.85	19.78	51.2	2.85	1.26	10.21	1.59	1.49	1.17	0.53	2.18	0.6	0.11	0.62	0.53	0.68	0.5	0.22	0.5	0.33	0.67	0.69	0.12	0.69	0.62	0.78	0.8	0.08	0.81	0.75	0.85	242.68	236.61	193.27	129.04	296.47	556.82	403.49	452.94	315.71	683.37	3600	0.35
0.18	0.64	0.18	0.67	0.54	0.78	0.82	0.07	0.84	0.78	0.88	0.71	0.13	0.73	0.64	0.81	24.7	61.86	3.58	1.51	13.44	1.75	1.55	1.32	0.63	2.45	0.54	0.12	0.55	0.47	0.63	0.45	0.23	0.5	0.25	0.6	0.65	0.12	0.65	0.57	0.73	0.77	0.08	0.78	0.72	0.83	248.69	312.02	195.25	129.47	299.45	712.89	474.63	586.07	404.42	880.57	2091	0.5
0.32	0.52	0.21	0.55	0.38	0.69	0.7	0.12	0.72	0.63	0.8	0.6	0.18	0.63	0.49	0.73	47.05	97.79	6.4	2.28	39.45	2.13	1.84	1.65	0.75	2.97	0.44	0.15	0.46	0.35	0.55	0.35	0.22	0.33	0.2	0.5	0.58	0.13	0.58	0.5	0.67	0.72	0.09	0.73	0.67	0.79	243.63	235.27	193.9	129.14	297.19	1152.18	789.67	946.49	627.32	1437.02	7121	1.0


==> data_new/ra/agnews/bert/S_auc.tex <==
0.23

==> data_new/ra/agnews/bert/S_ppl.tex <==
3.7

==> data_new/ra/agnews/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.99	0.03	1.0	0.99	1.0	0.99	0.01	1.0	0.99	1.0	0.98	0.03	1.0	0.98	1.0	0.72	1.29	0.0	0.0	1.12	0.24	0.57	0.0	0.0	0.23	0.97	0.06	1.0	0.94	1.0	0.97	0.08	1.0	1.0	1.0	0.98	0.04	1.0	0.95	1.0	0.98	0.03	1.0	0.96	1.0	261.46	241.55	205.17	137.99	315.55	269.68	242.49	215.92	144.32	322.39	3714	0.01
0.03	0.95	0.07	0.97	0.93	0.99	0.98	0.02	0.98	0.97	0.99	0.93	0.07	0.95	0.9	0.97	2.42	1.76	1.94	1.2	3.16	0.77	0.89	0.49	0.21	1.01	0.86	0.08	0.87	0.82	0.91	0.87	0.16	1.0	0.75	1.0	0.91	0.07	0.92	0.87	0.94	0.93	0.05	0.94	0.9	0.96	256.06	221.61	203.7	137.76	312.86	302.06	241.62	244.6	166.14	365.64	3716	0.06
0.06	0.89	0.1	0.92	0.86	0.96	0.95	0.03	0.96	0.94	0.97	0.86	0.09	0.88	0.82	0.92	3.64	2.12	3.15	2.11	4.75	1.19	1.16	0.85	0.37	1.64	0.76	0.1	0.77	0.7	0.82	0.79	0.19	0.8	0.67	1.0	0.85	0.09	0.86	0.8	0.91	0.88	0.06	0.88	0.84	0.92	259.6	229.1	205.84	138.74	316.39	362.42	266.57	293.02	201.08	439.15	3955	0.13
0.11	0.85	0.12	0.88	0.8	0.93	0.92	0.04	0.93	0.91	0.95	0.8	0.11	0.82	0.75	0.88	4.6	2.4	4.09	2.85	5.82	1.48	1.37	1.09	0.5	2.04	0.68	0.11	0.69	0.62	0.75	0.73	0.2	0.75	0.6	0.83	0.8	0.09	0.81	0.75	0.87	0.84	0.06	0.85	0.81	0.89	259.37	235.8	203.57	136.55	313.52	424.2	325.36	346.18	234.79	512.92	3622	0.22
0.15	0.78	0.14	0.81	0.71	0.88	0.88	0.05	0.89	0.86	0.92	0.72	0.12	0.74	0.66	0.81	5.8	2.74	5.28	3.75	7.38	1.97	1.75	1.5	0.68	2.7	0.59	0.11	0.6	0.53	0.66	0.67	0.2	0.67	0.5	0.8	0.75	0.1	0.75	0.69	0.82	0.8	0.07	0.81	0.76	0.85	250.72	224.95	199.92	135.8	305.42	510.17	356.01	424.92	293.23	623.17	3385	0.35
0.18	0.71	0.16	0.74	0.63	0.83	0.84	0.06	0.85	0.8	0.88	0.65	0.14	0.67	0.57	0.75	6.73	3.17	6.11	4.34	8.54	2.27	2.0	1.72	0.8	3.17	0.51	0.12	0.52	0.44	0.6	0.6	0.21	0.6	0.5	0.75	0.7	0.11	0.71	0.64	0.78	0.76	0.07	0.77	0.71	0.82	256.7	229.8	203.3	137.16	312.15	634.95	482.36	526.08	374.16	771.39	3669	0.5
0.32	0.58	0.19	0.6	0.47	0.72	0.71	0.11	0.73	0.64	0.8	0.51	0.17	0.53	0.4	0.63	8.82	4.04	8.1	5.73	11.37	3.1	2.56	2.49	1.15	4.42	0.39	0.14	0.39	0.29	0.48	0.5	0.23	0.5	0.33	0.67	0.62	0.12	0.62	0.54	0.7	0.7	0.08	0.71	0.65	0.76	255.55	219.33	203.3	137.02	312.12	1006.29	722.77	830.22	564.27	1231.73	9997	1.0


==> data_new/ra/agnews/cnn/IG_auc.tex <==
0.25

==> data_new/ra/agnews/cnn/IG_ppl.tex <==
2.9

==> data_new/ra/agnews/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.99	0.03	1.0	0.99	1.0	0.99	0.01	1.0	0.99	1.0	0.99	0.03	1.0	0.99	1.0	8.55	16.35	0.0	0.0	12.55	0.13	0.32	0.0	0.0	0.1	0.97	0.05	1.0	0.96	1.0	0.97	0.11	1.0	1.0	1.0	0.98	0.05	1.0	1.0	1.0	0.98	0.04	1.0	1.0	1.0	261.46	241.59	205.17	137.99	315.55	269.68	242.53	215.92	144.32	322.39	3714	0.01
0.03	0.96	0.05	0.98	0.95	0.99	0.98	0.02	0.98	0.97	0.99	0.95	0.06	0.97	0.94	0.99	29.33	24.95	22.02	12.48	37.99	0.41	0.47	0.25	0.09	0.56	0.89	0.08	0.91	0.86	0.95	0.86	0.21	1.0	0.75	1.0	0.91	0.1	0.93	0.86	1.0	0.94	0.06	0.95	0.9	1.0	256.2	221.63	203.76	137.88	312.98	302.23	241.67	244.86	166.12	366.0	3716	0.06
0.06	0.93	0.08	0.95	0.9	0.98	0.95	0.03	0.96	0.94	0.97	0.91	0.08	0.94	0.88	0.97	45.43	31.34	37.44	23.97	57.56	0.62	0.6	0.44	0.19	0.86	0.81	0.1	0.83	0.76	0.88	0.77	0.25	0.8	0.67	1.0	0.85	0.12	0.87	0.78	0.93	0.9	0.07	0.91	0.85	0.95	259.72	229.14	205.84	138.89	316.36	362.56	266.66	292.94	201.16	439.93	3955	0.13
0.11	0.89	0.09	0.92	0.86	0.96	0.92	0.04	0.93	0.91	0.95	0.88	0.1	0.9	0.84	0.95	58.86	35.71	50.75	33.71	74.15	0.77	0.69	0.58	0.26	1.1	0.75	0.11	0.77	0.68	0.83	0.7	0.27	0.75	0.5	1.0	0.81	0.12	0.82	0.73	0.9	0.87	0.08	0.88	0.82	0.92	259.22	235.72	203.42	136.53	313.35	423.93	325.19	345.96	234.52	512.17	3622	0.22
0.15	0.85	0.12	0.88	0.81	0.93	0.88	0.05	0.89	0.86	0.92	0.83	0.12	0.86	0.78	0.92	77.34	44.71	66.91	45.48	97.91	0.95	0.82	0.75	0.34	1.34	0.68	0.13	0.7	0.61	0.77	0.63	0.28	0.67	0.5	0.8	0.76	0.14	0.77	0.68	0.86	0.83	0.09	0.84	0.78	0.9	250.59	224.91	199.84	135.77	305.38	510.11	356.24	424.61	293.18	622.98	3385	0.35
0.18	0.81	0.14	0.84	0.75	0.91	0.84	0.06	0.85	0.8	0.88	0.79	0.14	0.82	0.72	0.89	93.22	51.62	81.37	55.89	117.9	1.06	0.87	0.87	0.39	1.5	0.63	0.13	0.65	0.55	0.73	0.58	0.29	0.6	0.4	0.8	0.72	0.14	0.73	0.63	0.83	0.81	0.09	0.81	0.75	0.88	256.55	229.74	203.25	137.02	312.02	634.57	481.93	525.69	373.75	771.42	3669	0.5
0.32	0.73	0.18	0.78	0.65	0.86	0.71	0.11	0.73	0.64	0.8	0.7	0.18	0.74	0.61	0.83	136.32	75.0	118.93	78.48	179.25	1.28	1.05	1.03	0.47	1.83	0.54	0.16	0.56	0.45	0.65	0.51	0.3	0.5	0.25	0.75	0.67	0.16	0.67	0.57	0.79	0.77	0.1	0.77	0.7	0.84	255.5	219.31	203.25	136.95	312.04	1006.01	722.57	830.26	564.44	1232.25	9997	1.0


==> data_new/ra/agnews/cnn/S_auc.tex <==
0.27

==> data_new/ra/agnews/cnn/S_ppl.tex <==
2.9

==> data_new/ra/agnews/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.08	1.0	1.0	1.0	0.99	0.01	1.0	0.99	1.0	0.98	0.06	1.0	0.99	1.0	0.16	0.45	0.0	0.0	0.15	0.45	1.44	0.0	0.0	0.32	0.96	0.09	1.0	0.95	1.0	0.96	0.1	1.0	1.0	1.0	0.97	0.07	1.0	0.95	1.0	0.98	0.05	1.0	0.97	1.0	260.5	238.41	205.12	138.48	315.41	268.91	238.85	215.7	146.04	323.83	3751	0.01
0.03	0.94	0.12	0.98	0.93	0.99	0.98	0.02	0.98	0.97	0.99	0.93	0.1	0.96	0.9	0.98	0.53	0.62	0.35	0.18	0.65	1.37	2.03	0.73	0.29	1.62	0.85	0.12	0.89	0.82	0.93	0.86	0.18	1.0	0.75	1.0	0.9	0.1	0.92	0.86	0.95	0.92	0.07	0.94	0.9	0.96	255.87	218.26	204.52	138.47	313.57	300.28	274.24	244.58	165.73	363.66	3758	0.06
0.06	0.88	0.15	0.93	0.85	0.97	0.95	0.03	0.96	0.94	0.97	0.86	0.13	0.9	0.82	0.94	0.82	0.85	0.58	0.34	1.0	2.09	2.82	1.25	0.54	2.53	0.76	0.14	0.8	0.71	0.86	0.79	0.21	0.8	0.67	1.0	0.84	0.11	0.86	0.79	0.92	0.88	0.08	0.89	0.85	0.93	259.34	226.5	205.94	139.82	316.46	360.62	285.55	289.53	200.0	437.74	3992	0.13
0.11	0.83	0.18	0.88	0.78	0.94	0.92	0.04	0.93	0.91	0.95	0.81	0.15	0.84	0.76	0.91	1.03	0.96	0.76	0.49	1.26	2.67	3.29	1.73	0.76	3.34	0.7	0.15	0.73	0.64	0.8	0.73	0.22	0.75	0.6	1.0	0.8	0.12	0.82	0.75	0.89	0.85	0.09	0.86	0.81	0.91	258.23	231.73	203.37	137.24	313.67	426.64	335.03	342.84	235.0	510.18	3664	0.22
0.15	0.75	0.21	0.82	0.67	0.9	0.88	0.05	0.89	0.86	0.92	0.73	0.17	0.77	0.66	0.84	1.29	1.06	0.99	0.66	1.56	3.44	3.75	2.31	1.05	4.47	0.61	0.15	0.64	0.54	0.72	0.67	0.23	0.75	0.5	0.8	0.75	0.13	0.77	0.68	0.83	0.81	0.09	0.82	0.76	0.87	249.96	222.49	200.17	136.26	305.77	510.03	354.12	424.55	300.3	618.23	3417	0.35
0.18	0.69	0.22	0.74	0.58	0.85	0.84	0.06	0.85	0.8	0.88	0.66	0.18	0.69	0.58	0.78	1.53	1.23	1.19	0.81	1.84	4.05	4.3	2.78	1.24	5.3	0.54	0.16	0.56	0.46	0.65	0.61	0.24	0.67	0.5	0.75	0.7	0.14	0.73	0.63	0.8	0.77	0.09	0.79	0.72	0.84	255.81	226.52	203.25	137.92	312.1	643.14	449.61	536.99	372.88	775.16	3710	0.51
0.32	0.54	0.26	0.58	0.38	0.73	0.71	0.11	0.73	0.64	0.8	0.51	0.21	0.53	0.39	0.65	1.99	1.55	1.56	1.1	2.35	5.43	5.21	4.0	1.76	7.42	0.4	0.17	0.41	0.29	0.52	0.5	0.26	0.5	0.33	0.67	0.61	0.14	0.62	0.53	0.71	0.7	0.1	0.71	0.64	0.77	254.85	216.25	203.25	137.78	312.16	1004.19	706.15	834.42	565.49	1225.78	10107	1.0


==> data_new/ra/agnews/lstm/IG_auc.tex <==
0.24

==> data_new/ra/agnews/lstm/IG_ppl.tex <==
2.9

==> data_new/ra/agnews/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.07	1.0	0.99	1.0	0.99	0.01	1.0	0.99	1.0	0.98	0.05	1.0	0.98	1.0	5.04	13.67	0.0	0.0	4.53	0.32	0.94	0.0	0.0	0.19	0.95	0.09	1.0	0.93	1.0	0.95	0.12	1.0	1.0	1.0	0.97	0.07	1.0	0.95	1.0	0.98	0.05	1.0	0.96	1.0	260.5	238.37	205.12	138.48	315.41	268.9	238.81	215.7	146.04	323.83	3751	0.01
0.03	0.91	0.12	0.96	0.89	0.99	0.98	0.02	0.98	0.97	0.99	0.92	0.09	0.95	0.89	0.97	17.28	20.35	10.87	5.68	20.67	0.98	1.31	0.54	0.2	1.24	0.83	0.12	0.86	0.78	0.91	0.81	0.21	0.8	0.67	1.0	0.87	0.11	0.89	0.83	0.93	0.91	0.07	0.92	0.88	0.95	255.74	218.26	204.45	138.44	313.37	300.14	274.48	244.41	165.54	363.38	3758	0.06
0.06	0.84	0.16	0.9	0.78	0.95	0.95	0.03	0.96	0.94	0.97	0.85	0.11	0.88	0.8	0.93	26.49	28.43	18.23	10.97	31.62	1.41	1.56	0.91	0.38	1.86	0.73	0.13	0.75	0.66	0.82	0.71	0.23	0.75	0.6	0.83	0.8	0.12	0.82	0.73	0.89	0.86	0.08	0.88	0.82	0.92	259.46	226.55	205.98	139.78	316.4	360.8	285.63	289.65	200.07	438.14	3992	0.13
0.11	0.78	0.18	0.82	0.68	0.91	0.92	0.04	0.93	0.91	0.95	0.79	0.12	0.82	0.73	0.88	33.67	31.67	24.04	15.6	40.01	1.77	1.83	1.24	0.52	2.36	0.65	0.13	0.67	0.57	0.74	0.64	0.23	0.67	0.5	0.8	0.75	0.13	0.76	0.67	0.83	0.82	0.08	0.83	0.78	0.88	258.21	231.7	203.37	137.24	313.69	426.6	334.99	342.84	235.0	509.92	3664	0.22
0.15	0.7	0.19	0.74	0.58	0.84	0.88	0.05	0.89	0.86	0.92	0.72	0.14	0.74	0.64	0.82	42.52	39.11	31.23	20.41	50.61	2.14	2.06	1.55	0.69	2.93	0.57	0.13	0.58	0.49	0.66	0.55	0.23	0.5	0.4	0.75	0.69	0.13	0.69	0.6	0.78	0.78	0.08	0.79	0.73	0.84	249.83	222.46	200.0	136.09	305.44	509.75	353.91	424.06	300.16	617.86	3417	0.35
0.18	0.63	0.2	0.66	0.5	0.78	0.84	0.06	0.85	0.8	0.88	0.66	0.14	0.68	0.57	0.76	48.63	42.66	36.73	24.15	57.74	2.29	2.16	1.71	0.76	3.12	0.5	0.13	0.51	0.42	0.59	0.49	0.23	0.5	0.33	0.67	0.64	0.12	0.64	0.56	0.73	0.75	0.08	0.76	0.7	0.81	255.81	226.51	203.25	137.92	312.1	643.14	449.61	536.99	372.88	775.16	3710	0.51
0.32	0.49	0.21	0.51	0.35	0.65	0.71	0.11	0.72	0.64	0.8	0.53	0.17	0.55	0.43	0.65	64.0	59.92	46.67	31.56	74.02	2.76	2.5	2.09	0.95	3.81	0.39	0.13	0.4	0.31	0.49	0.38	0.23	0.33	0.25	0.5	0.55	0.13	0.56	0.47	0.64	0.69	0.09	0.7	0.64	0.75	254.74	216.19	203.25	137.77	312.1	1005.3	710.24	833.48	565.86	1228.12	10106	1.0


==> data_new/ra/agnews/lstm/S_auc.tex <==
0.22

==> data_new/ra/agnews/lstm/S_ppl.tex <==
2.9

==> data_new/ra/agnews/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.07	1.0	0.99	1.0	0.99	0.01	1.0	0.99	1.0	0.97	0.08	1.0	0.99	1.0	0.0	0.01	0.0	0.0	0.0	0.24	0.61	0.0	0.0	0.16	0.95	0.11	1.0	0.94	1.0	0.92	0.19	1.0	1.0	1.0	0.95	0.11	1.0	0.94	1.0	0.97	0.07	1.0	0.96	1.0	260.74	239.05	204.55	138.34	315.81	268.8	239.26	215.65	146.19	323.22	3757	0.01
0.03	0.93	0.14	0.98	0.92	0.99	0.98	0.02	0.98	0.97	0.99	0.9	0.16	0.96	0.89	0.99	0.02	0.02	0.01	0.01	0.02	0.71	1.01	0.35	0.13	0.88	0.82	0.17	0.87	0.76	0.93	0.73	0.3	0.8	0.6	1.0	0.84	0.17	0.89	0.77	0.95	0.9	0.11	0.93	0.86	0.97	256.7	220.58	203.73	138.35	313.66	302.83	262.06	244.48	167.28	367.44	3767	0.06
0.06	0.86	0.19	0.93	0.83	0.98	0.95	0.03	0.96	0.94	0.97	0.83	0.22	0.91	0.78	0.96	0.03	0.02	0.02	0.01	0.03	1.11	1.35	0.67	0.26	1.41	0.71	0.21	0.77	0.62	0.87	0.61	0.33	0.67	0.33	1.0	0.76	0.2	0.81	0.64	0.91	0.84	0.14	0.88	0.78	0.95	259.74	227.69	205.45	139.25	316.53	358.87	262.91	290.18	200.56	440.75	3997	0.13
0.11	0.8	0.24	0.89	0.74	0.95	0.92	0.04	0.93	0.91	0.95	0.76	0.27	0.85	0.67	0.94	0.03	0.02	0.03	0.01	0.04	1.41	1.58	0.89	0.37	1.88	0.64	0.24	0.7	0.52	0.81	0.51	0.34	0.5	0.25	0.75	0.7	0.22	0.75	0.57	0.87	0.8	0.15	0.83	0.72	0.91	258.49	232.57	202.46	137.08	313.48	425.04	310.6	342.02	236.4	518.67	3666	0.22
0.15	0.73	0.27	0.82	0.63	0.92	0.88	0.05	0.89	0.86	0.92	0.68	0.3	0.78	0.55	0.9	0.04	0.03	0.03	0.02	0.05	1.8	1.9	1.18	0.51	2.44	0.56	0.26	0.61	0.42	0.76	0.43	0.34	0.5	0.0	0.75	0.64	0.24	0.67	0.5	0.82	0.76	0.16	0.79	0.67	0.89	250.04	222.83	199.21	136.03	305.46	509.1	359.66	423.33	294.06	621.4	3425	0.35
0.18	0.66	0.3	0.76	0.53	0.88	0.84	0.06	0.85	0.81	0.88	0.62	0.32	0.72	0.46	0.86	0.05	0.03	0.04	0.03	0.06	2.09	2.11	1.44	0.61	2.85	0.5	0.27	0.55	0.34	0.7	0.37	0.34	0.33	0.0	0.67	0.59	0.25	0.62	0.43	0.79	0.73	0.17	0.76	0.62	0.86	256.25	227.63	202.38	137.72	312.47	644.18	450.86	538.12	377.47	781.62	3717	0.51
0.32	0.52	0.36	0.61	0.32	0.8	0.71	0.11	0.73	0.64	0.8	0.48	0.37	0.56	0.26	0.78	0.06	0.04	0.05	0.03	0.08	2.82	2.63	2.08	0.91	3.93	0.38	0.3	0.41	0.19	0.61	0.28	0.32	0.2	0.0	0.5	0.5	0.26	0.53	0.31	0.7	0.67	0.18	0.69	0.55	0.81	255.22	217.26	202.38	137.72	312.47	1007.21	716.46	831.63	567.05	1218.99	10113	1.0


==> data_new/ra/agnews/lstmatt/A_auc.tex <==
0.23

==> data_new/ra/agnews/lstmatt/A_ppl.tex <==
2.9

==> data_new/ra/agnews/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.07	1.0	0.99	1.0	0.99	0.01	1.0	0.99	1.0	0.98	0.07	1.0	0.98	1.0	0.17	0.61	0.0	0.0	0.12	0.65	1.85	0.0	0.0	0.51	0.95	0.1	1.0	0.93	1.0	0.96	0.1	1.0	1.0	1.0	0.97	0.07	1.0	0.94	1.0	0.97	0.05	1.0	0.96	1.0	260.74	239.05	204.55	138.34	315.81	268.8	239.26	215.65	146.19	323.22	3757	0.01
0.03	0.93	0.12	0.98	0.93	0.99	0.98	0.02	0.98	0.97	0.99	0.92	0.11	0.95	0.89	0.98	0.57	1.12	0.29	0.14	0.59	1.69	2.5	0.9	0.35	2.01	0.84	0.12	0.87	0.79	0.92	0.86	0.17	1.0	0.75	1.0	0.89	0.1	0.92	0.85	0.94	0.91	0.07	0.93	0.88	0.96	256.7	220.58	203.73	138.35	313.66	302.83	262.06	244.48	167.28	367.44	3767	0.06
0.06	0.88	0.15	0.93	0.84	0.97	0.95	0.03	0.96	0.94	0.97	0.85	0.13	0.89	0.81	0.94	0.86	1.41	0.5	0.26	0.92	2.37	2.88	1.46	0.63	3.05	0.75	0.14	0.77	0.69	0.84	0.78	0.2	0.8	0.67	1.0	0.84	0.11	0.86	0.79	0.92	0.87	0.08	0.89	0.83	0.93	259.74	227.69	205.45	139.25	316.53	358.87	262.91	290.18	200.56	440.75	3997	0.13
0.11	0.82	0.18	0.88	0.77	0.94	0.92	0.04	0.93	0.91	0.95	0.79	0.15	0.82	0.73	0.89	1.09	1.53	0.69	0.39	1.2	3.08	3.39	1.97	0.88	4.0	0.67	0.15	0.7	0.6	0.78	0.73	0.2	0.75	0.6	0.83	0.79	0.12	0.81	0.73	0.88	0.84	0.09	0.85	0.79	0.9	258.49	232.57	202.46	137.08	313.48	425.04	310.6	342.02	236.4	518.67	3666	0.22
0.15	0.75	0.2	0.81	0.67	0.89	0.88	0.05	0.89	0.86	0.92	0.71	0.17	0.74	0.64	0.83	1.38	1.77	0.91	0.53	1.5	3.82	4.06	2.59	1.18	5.03	0.59	0.15	0.61	0.51	0.69	0.66	0.22	0.67	0.5	0.8	0.75	0.12	0.75	0.67	0.83	0.8	0.09	0.81	0.75	0.86	250.04	222.83	199.21	136.03	305.46	509.1	359.66	423.33	294.06	621.4	3425	0.35
0.18	0.69	0.21	0.74	0.58	0.84	0.84	0.06	0.85	0.81	0.88	0.64	0.18	0.67	0.54	0.77	1.64	1.91	1.12	0.68	1.83	4.31	4.34	3.06	1.31	5.83	0.52	0.16	0.54	0.43	0.63	0.61	0.23	0.67	0.5	0.75	0.7	0.13	0.71	0.62	0.8	0.76	0.1	0.78	0.71	0.83	256.25	227.63	202.38	137.72	312.47	644.25	450.85	538.12	377.47	781.62	3717	0.52
0.32	0.54	0.25	0.58	0.39	0.73	0.71	0.11	0.73	0.64	0.8	0.48	0.21	0.51	0.35	0.64	2.22	2.32	1.58	1.04	2.47	5.48	4.99	4.09	1.85	7.56	0.38	0.17	0.39	0.26	0.5	0.5	0.24	0.5	0.33	0.67	0.62	0.14	0.62	0.53	0.73	0.7	0.1	0.71	0.63	0.77	255.28	217.28	202.38	137.72	312.61	1003.53	694.6	825.95	565.59	1225.61	10113	1.0


==> data_new/ra/agnews/lstmatt/IG_auc.tex <==
0.24

==> data_new/ra/agnews/lstmatt/IG_ppl.tex <==
2.9

==> data_new/ra/agnews/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.97	0.08	1.0	0.99	1.0	0.99	0.01	1.0	0.99	1.0	0.98	0.06	1.0	0.98	1.0	4.22	14.26	0.0	0.0	2.71	0.57	1.39	0.0	0.0	0.46	0.94	0.11	1.0	0.9	1.0	0.93	0.15	1.0	1.0	1.0	0.95	0.09	1.0	0.94	1.0	0.97	0.06	1.0	0.96	1.0	260.75	239.09	204.55	138.34	315.81	268.81	239.3	215.65	146.19	323.22	3757	0.01
0.03	0.9	0.13	0.94	0.86	0.98	0.98	0.02	0.98	0.97	0.99	0.91	0.09	0.94	0.89	0.97	14.25	22.61	7.01	2.94	16.67	1.58	1.91	0.93	0.38	2.01	0.8	0.12	0.82	0.74	0.89	0.76	0.22	0.75	0.67	1.0	0.85	0.12	0.87	0.79	0.92	0.9	0.08	0.91	0.86	0.95	256.84	220.61	203.79	138.4	313.68	303.0	262.17	244.69	167.4	367.24	3767	0.06
0.06	0.81	0.17	0.86	0.74	0.94	0.95	0.03	0.96	0.94	0.97	0.85	0.12	0.88	0.81	0.93	21.48	32.24	12.23	5.51	24.94	2.24	2.3	1.51	0.63	3.03	0.71	0.13	0.73	0.63	0.8	0.64	0.25	0.67	0.5	0.8	0.77	0.13	0.79	0.7	0.87	0.85	0.08	0.86	0.8	0.91	259.88	227.75	205.48	139.43	316.75	359.12	263.08	290.97	200.6	441.36	3997	0.13
0.11	0.74	0.19	0.79	0.65	0.88	0.92	0.04	0.93	0.91	0.95	0.79	0.14	0.83	0.74	0.89	26.13	34.16	16.32	7.79	31.66	2.78	2.68	2.0	0.92	3.87	0.64	0.14	0.66	0.56	0.73	0.56	0.25	0.6	0.4	0.75	0.72	0.13	0.73	0.65	0.81	0.82	0.09	0.83	0.76	0.88	258.64	232.65	202.68	137.23	313.6	425.27	310.79	342.32	236.65	518.95	3666	0.22
0.15	0.67	0.2	0.7	0.55	0.82	0.88	0.05	0.89	0.86	0.92	0.74	0.15	0.77	0.68	0.84	32.62	41.19	20.44	9.94	40.12	3.25	3.0	2.43	1.11	4.48	0.57	0.14	0.59	0.51	0.67	0.48	0.25	0.5	0.33	0.67	0.67	0.13	0.69	0.6	0.76	0.79	0.09	0.8	0.74	0.85	250.18	222.87	199.24	136.11	305.86	509.38	359.84	423.45	294.31	621.81	3425	0.36
0.18	0.6	0.21	0.62	0.47	0.76	0.84	0.06	0.85	0.81	0.88	0.69	0.16	0.72	0.61	0.8	39.98	46.75	26.56	12.1	49.61	3.59	3.19	2.73	1.26	4.97	0.52	0.14	0.54	0.44	0.62	0.42	0.24	0.4	0.25	0.6	0.63	0.14	0.64	0.54	0.73	0.76	0.09	0.77	0.71	0.82	256.39	227.68	202.48	137.87	312.71	644.7	451.34	538.63	377.56	781.76	3717	0.52
0.32	0.49	0.22	0.51	0.35	0.66	0.72	0.11	0.73	0.64	0.8	0.6	0.18	0.63	0.51	0.73	56.65	62.85	38.54	19.04	70.05	4.17	3.61	3.24	1.48	5.83	0.44	0.14	0.46	0.36	0.54	0.33	0.24	0.33	0.2	0.5	0.57	0.14	0.57	0.47	0.67	0.72	0.09	0.73	0.67	0.79	255.31	217.27	202.4	137.58	312.71	996.18	688.87	823.45	563.63	1220.66	10116	1.0


==> data_new/ra/agnews/lstmatt/S_auc.tex <==
0.22

==> data_new/ra/agnews/lstmatt/S_ppl.tex <==
2.9

==> data_new/ra/agnews/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.94	0.07	0.97	0.91	1.0	0.99	0.02	0.99	0.98	1.0	0.95	0.05	0.97	0.93	1.0	0.36	0.39	0.27	0.0	0.54	0.56	0.81	0.26	0.0	0.8	0.87	0.11	0.87	0.78	1.0	0.85	0.13	0.87	0.76	1.0	0.9	0.09	0.91	0.84	1.0	0.93	0.06	0.94	0.89	1.0	191.33	148.2	153.74	103.67	232.79	211.01	153.55	173.54	117.16	256.92	3773	0.01
0.03	0.87	0.11	0.89	0.82	0.95	0.97	0.03	0.98	0.96	0.98	0.89	0.07	0.9	0.85	0.94	0.68	0.44	0.58	0.37	0.89	1.03	1.07	0.71	0.31	1.41	0.74	0.09	0.74	0.68	0.8	0.71	0.12	0.72	0.64	0.8	0.81	0.07	0.81	0.76	0.86	0.87	0.05	0.87	0.84	0.9	190.35	141.73	153.95	103.76	232.64	251.07	179.29	204.4	139.39	304.41	3792	0.03
0.06	0.77	0.14	0.79	0.69	0.88	0.94	0.04	0.95	0.93	0.96	0.81	0.09	0.82	0.76	0.87	0.93	0.53	0.82	0.55	1.19	1.46	1.42	1.06	0.47	1.98	0.63	0.1	0.64	0.57	0.7	0.61	0.13	0.61	0.52	0.7	0.73	0.08	0.74	0.69	0.79	0.82	0.05	0.82	0.79	0.86	191.92	147.31	154.33	103.78	234.28	324.85	231.96	264.49	182.87	393.28	3853	0.07
0.11	0.7	0.16	0.71	0.6	0.81	0.91	0.05	0.92	0.89	0.94	0.74	0.11	0.76	0.68	0.82	1.1	0.59	0.99	0.67	1.41	1.78	1.68	1.31	0.6	2.44	0.56	0.1	0.57	0.5	0.63	0.54	0.14	0.54	0.44	0.63	0.68	0.08	0.69	0.63	0.74	0.78	0.05	0.79	0.75	0.82	190.35	142.09	154.27	103.88	233.56	422.26	322.33	344.96	237.7	507.79	3771	0.12
0.15	0.6	0.18	0.61	0.48	0.73	0.85	0.07	0.87	0.82	0.9	0.66	0.12	0.67	0.58	0.75	1.28	0.65	1.15	0.81	1.61	2.15	1.96	1.6	0.74	2.96	0.49	0.11	0.49	0.42	0.56	0.46	0.14	0.45	0.37	0.55	0.63	0.08	0.63	0.57	0.68	0.74	0.06	0.75	0.71	0.78	187.4	142.03	151.6	102.77	227.92	591.97	418.95	496.72	348.37	712.76	3643	0.21
0.18	0.53	0.19	0.53	0.4	0.66	0.8	0.08	0.81	0.75	0.85	0.59	0.14	0.6	0.51	0.69	1.41	0.68	1.27	0.92	1.77	2.44	2.24	1.85	0.84	3.36	0.43	0.11	0.43	0.36	0.5	0.41	0.14	0.4	0.31	0.5	0.58	0.09	0.58	0.53	0.64	0.71	0.06	0.72	0.68	0.75	190.1	144.28	153.22	103.49	231.37	834.07	538.54	701.94	485.07	1032.94	3767	0.34
0.32	0.38	0.21	0.36	0.22	0.51	0.6	0.14	0.61	0.51	0.71	0.43	0.16	0.44	0.32	0.55	1.69	0.74	1.56	1.15	2.07	3.11	2.75	2.37	1.07	4.33	0.3	0.12	0.31	0.22	0.39	0.31	0.13	0.29	0.21	0.39	0.5	0.09	0.5	0.43	0.56	0.65	0.06	0.65	0.61	0.69	188.9	143.46	152.27	103.41	229.5	2090.03	2801.55	1668.98	1068.41	2585.43	8772	1.0


==> data_new/ra/agnews/roberta/A_auc.tex <==
0.20

==> data_new/ra/agnews/roberta/A_ppl.tex <==
10.1

==> data_new/ra/agnews/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.84	0.31	0.97	0.83	1.0	0.99	0.02	0.99	0.98	1.0	0.86	0.23	0.96	0.84	1.0	3.0	5.65	0.82	0.0	3.42	2.62	4.26	0.93	0.0	3.26	0.79	0.25	0.86	0.69	1.0	0.79	0.25	0.83	0.67	1.0	0.85	0.17	0.89	0.78	1.0	0.89	0.13	0.93	0.84	1.0	191.33	148.2	153.74	103.67	232.79	211.01	153.55	173.54	117.16	256.92	3773	0.01
0.03	0.69	0.38	0.84	0.56	0.96	0.97	0.03	0.98	0.96	0.98	0.73	0.28	0.82	0.6	0.94	5.32	7.41	2.79	1.08	6.75	4.31	4.98	2.51	0.96	5.72	0.61	0.26	0.67	0.45	0.82	0.63	0.27	0.67	0.5	0.83	0.73	0.18	0.77	0.62	0.88	0.81	0.13	0.83	0.72	0.91	190.35	141.73	153.95	103.76	232.64	251.07	179.29	204.4	139.39	304.41	3792	0.04
0.06	0.56	0.38	0.67	0.34	0.87	0.94	0.04	0.95	0.93	0.96	0.6	0.29	0.67	0.43	0.84	6.74	8.23	4.03	1.82	8.71	5.68	5.65	3.85	1.59	7.93	0.49	0.25	0.52	0.32	0.7	0.52	0.27	0.5	0.33	0.75	0.64	0.18	0.67	0.53	0.79	0.75	0.13	0.76	0.66	0.85	190.71	145.02	153.95	103.66	232.51	321.68	224.19	264.09	182.43	390.44	3790	0.08
0.11	0.48	0.38	0.55	0.25	0.79	0.91	0.05	0.92	0.89	0.94	0.53	0.29	0.57	0.34	0.77	7.71	8.52	4.86	2.26	10.03	6.26	5.87	4.58	1.9	8.83	0.41	0.24	0.43	0.24	0.62	0.45	0.26	0.5	0.25	0.67	0.59	0.18	0.6	0.47	0.74	0.71	0.13	0.72	0.62	0.81	192.79	153.07	154.51	104.35	235.91	428.13	340.03	349.14	238.9	515.15	2307	0.14
0.15	0.38	0.36	0.4	0.15	0.67	0.85	0.07	0.87	0.82	0.9	0.44	0.29	0.46	0.24	0.67	8.62	8.47	5.77	2.79	11.63	7.31	6.58	5.38	2.34	10.44	0.34	0.23	0.34	0.17	0.52	0.39	0.25	0.4	0.2	0.6	0.54	0.17	0.55	0.42	0.67	0.67	0.12	0.68	0.59	0.77	187.4	142.03	151.6	102.77	227.92	591.97	418.95	496.72	348.37	712.76	3643	0.25
0.18	0.32	0.34	0.32	0.1	0.58	0.8	0.08	0.81	0.75	0.85	0.37	0.27	0.38	0.18	0.58	9.62	9.56	6.71	3.36	12.51	7.86	6.82	5.84	2.67	11.25	0.28	0.21	0.28	0.12	0.44	0.34	0.24	0.33	0.17	0.5	0.51	0.16	0.5	0.39	0.62	0.64	0.12	0.65	0.56	0.73	190.13	144.29	153.25	103.53	231.47	834.22	538.54	702.0	485.31	1033.1	3766	0.4
0.32	0.23	0.29	0.21	0.04	0.42	0.64	0.14	0.66	0.55	0.75	0.27	0.24	0.26	0.1	0.44	11.35	16.3	8.75	4.66	14.53	8.39	6.94	6.64	2.99	12.08	0.2	0.18	0.18	0.07	0.32	0.27	0.22	0.25	0.17	0.4	0.45	0.15	0.44	0.33	0.54	0.6	0.1	0.6	0.53	0.67	189.15	141.73	152.33	103.46	231.12	1790.59	1356.06	1437.37	931.57	2216.47	8979	1.0


==> data_new/ra/agnews/roberta/IG_auc.tex <==
0.14

==> data_new/ra/agnews/roberta/IG_ppl.tex <==
8.5

==> data_new/ra/agnews/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.91	0.14	0.98	0.88	1.0	0.99	0.02	0.99	0.98	1.0	0.94	0.08	0.97	0.9	1.0	10.52	52.42	0.87	0.0	3.14	0.61	0.9	0.26	0.0	0.86	0.85	0.13	0.87	0.76	1.0	0.82	0.21	0.83	0.67	1.0	0.89	0.11	0.89	0.81	1.0	0.93	0.07	0.94	0.88	1.0	191.33	148.18	153.74	103.67	232.79	211.01	153.54	173.54	117.16	256.92	3773	0.01
0.03	0.81	0.17	0.86	0.72	0.95	0.97	0.03	0.98	0.96	0.98	0.87	0.1	0.89	0.82	0.94	25.22	95.27	3.03	1.34	9.28	1.06	1.1	0.74	0.32	1.48	0.72	0.12	0.73	0.65	0.81	0.65	0.23	0.67	0.5	0.8	0.79	0.11	0.8	0.73	0.88	0.86	0.07	0.88	0.81	0.91	190.31	141.72	153.95	103.69	232.33	251.08	179.34	204.27	139.35	305.0	3792	0.03
0.06	0.7	0.19	0.74	0.59	0.85	0.94	0.04	0.95	0.93	0.96	0.79	0.12	0.81	0.73	0.88	35.38	106.19	4.71	2.24	14.07	1.38	1.26	1.06	0.48	1.9	0.63	0.12	0.64	0.56	0.71	0.53	0.22	0.5	0.4	0.67	0.72	0.11	0.73	0.65	0.8	0.82	0.07	0.83	0.78	0.88	191.92	147.31	154.33	103.78	234.28	324.85	231.96	264.49	182.87	393.28	3853	0.07
0.11	0.62	0.2	0.65	0.5	0.77	0.91	0.05	0.92	0.89	0.94	0.73	0.13	0.75	0.66	0.83	46.08	132.53	6.15	2.83	19.01	1.59	1.4	1.23	0.56	2.2	0.57	0.12	0.58	0.49	0.65	0.45	0.22	0.5	0.33	0.6	0.67	0.12	0.68	0.6	0.75	0.79	0.07	0.8	0.74	0.84	190.35	142.09	154.27	103.88	233.56	422.26	322.33	344.96	237.7	507.79	3771	0.13
0.15	0.54	0.2	0.55	0.4	0.68	0.85	0.07	0.87	0.82	0.9	0.66	0.14	0.68	0.57	0.76	67.97	178.71	8.62	4.0	29.71	1.89	1.63	1.48	0.69	2.63	0.49	0.12	0.5	0.41	0.58	0.37	0.21	0.33	0.2	0.5	0.62	0.12	0.63	0.53	0.71	0.76	0.08	0.76	0.71	0.81	187.4	142.03	151.6	102.77	227.92	591.97	418.95	496.72	348.37	712.76	3643	0.23
0.18	0.48	0.2	0.49	0.35	0.63	0.8	0.08	0.81	0.75	0.85	0.6	0.15	0.62	0.51	0.71	99.76	252.36	11.25	5.06	48.07	2.0	1.69	1.6	0.73	2.77	0.45	0.12	0.46	0.37	0.53	0.32	0.21	0.33	0.17	0.5	0.58	0.12	0.58	0.5	0.67	0.73	0.08	0.74	0.68	0.79	190.07	144.27	153.22	103.45	231.27	833.92	538.56	701.76	484.86	1032.79	3768	0.36
0.32	0.4	0.2	0.4	0.26	0.54	0.62	0.14	0.64	0.53	0.74	0.49	0.17	0.51	0.38	0.62	207.01	391.75	32.58	9.47	228.57	2.29	1.9	1.82	0.86	3.2	0.35	0.14	0.36	0.27	0.45	0.26	0.2	0.25	0.17	0.4	0.51	0.12	0.53	0.43	0.6	0.69	0.09	0.69	0.62	0.75	188.99	141.61	152.39	103.38	230.1	1950.77	2617.36	1533.59	978.43	2397.56	10330	1.0


==> data_new/ra/agnews/roberta/S_auc.tex <==
0.18

==> data_new/ra/agnews/roberta/S_ppl.tex <==
9.3

==> data_new/ra/agnews/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.97	0.04	0.98	0.96	0.99	0.99	0.02	0.99	0.98	1.0	0.97	0.03	0.98	0.96	0.99	0.34	0.25	0.34	0.18	0.49	0.44	0.56	0.26	0.04	0.59	0.9	0.07	0.9	0.85	0.95	0.9	0.08	0.9	0.85	0.95	0.93	0.05	0.93	0.9	0.96	0.95	0.03	0.95	0.93	0.98	198.95	148.57	160.53	107.9	246.91	224.45	160.14	185.18	123.81	279.94	3756	0.02
0.03	0.93	0.05	0.94	0.91	0.96	0.97	0.03	0.97	0.96	0.98	0.94	0.04	0.95	0.92	0.97	0.58	0.22	0.55	0.42	0.71	0.73	0.72	0.51	0.23	1.0	0.82	0.06	0.82	0.78	0.86	0.81	0.07	0.82	0.77	0.86	0.87	0.05	0.88	0.84	0.9	0.91	0.03	0.92	0.89	0.93	199.79	152.2	160.76	107.91	247.05	262.99	187.79	214.99	144.69	327.97	3759	0.05
0.06	0.87	0.07	0.88	0.84	0.92	0.93	0.04	0.94	0.92	0.96	0.89	0.05	0.9	0.86	0.93	0.79	0.25	0.76	0.62	0.94	1.03	0.93	0.78	0.37	1.42	0.74	0.07	0.74	0.7	0.79	0.72	0.08	0.73	0.68	0.78	0.81	0.05	0.82	0.78	0.85	0.87	0.03	0.88	0.85	0.9	199.91	150.14	160.82	107.9	247.42	334.7	234.28	274.51	187.06	412.14	3824	0.1
0.11	0.82	0.08	0.83	0.78	0.88	0.9	0.06	0.91	0.87	0.93	0.85	0.07	0.86	0.81	0.89	0.95	0.26	0.92	0.76	1.09	1.26	1.09	1.01	0.45	1.76	0.68	0.07	0.68	0.63	0.73	0.66	0.09	0.67	0.61	0.72	0.77	0.06	0.77	0.73	0.81	0.84	0.04	0.85	0.82	0.87	198.11	144.58	160.42	107.79	246.53	422.78	274.89	354.43	244.28	520.71	3752	0.17
0.15	0.75	0.09	0.76	0.7	0.82	0.84	0.07	0.85	0.8	0.89	0.78	0.08	0.79	0.74	0.84	1.11	0.28	1.09	0.91	1.27	1.5	1.32	1.15	0.51	2.12	0.61	0.08	0.61	0.56	0.66	0.59	0.09	0.6	0.53	0.65	0.72	0.06	0.72	0.68	0.76	0.81	0.04	0.81	0.78	0.83	197.58	147.11	160.19	107.9	245.69	580.04	362.16	495.79	338.72	717.87	3677	0.29
0.18	0.69	0.11	0.7	0.63	0.77	0.78	0.09	0.79	0.73	0.84	0.72	0.09	0.73	0.67	0.79	1.23	0.29	1.2	1.02	1.4	1.71	1.47	1.36	0.6	2.41	0.55	0.08	0.55	0.49	0.6	0.53	0.09	0.54	0.47	0.6	0.67	0.06	0.68	0.63	0.72	0.78	0.04	0.78	0.75	0.81	198.88	148.61	160.35	107.9	246.67	780.09	518.07	659.87	457.14	956.71	3760	0.44
0.32	0.55	0.13	0.56	0.47	0.65	0.59	0.15	0.6	0.49	0.71	0.59	0.12	0.59	0.5	0.68	1.44	0.31	1.42	1.23	1.63	2.11	1.75	1.68	0.79	2.99	0.42	0.1	0.43	0.35	0.5	0.42	0.1	0.42	0.35	0.49	0.59	0.08	0.59	0.54	0.64	0.71	0.05	0.71	0.68	0.75	197.94	146.95	160.27	107.58	246.36	1500.91	1054.1	1240.68	825.63	1876.23	10789	1.0


==> data_new/ra/agnews/xlnet/A_auc.tex <==
0.24

==> data_new/ra/agnews/xlnet/A_ppl.tex <==
6.6

==> data_new/ra/agnews/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.89	0.15	0.94	0.87	0.99	0.99	0.02	0.99	0.98	1.0	0.89	0.14	0.92	0.84	0.98	0.64	1.78	0.19	0.06	0.48	0.55	0.7	0.34	0.05	0.78	0.78	0.17	0.79	0.69	0.89	0.77	0.21	0.83	0.67	1.0	0.84	0.13	0.84	0.75	0.95	0.89	0.09	0.9	0.84	0.96	198.95	148.57	160.53	107.9	246.91	224.45	160.14	185.18	123.81	279.94	3756	0.02
0.03	0.78	0.18	0.84	0.72	0.91	0.97	0.03	0.97	0.96	0.98	0.77	0.16	0.81	0.7	0.88	1.18	2.3	0.41	0.21	1.01	0.9	0.83	0.67	0.3	1.26	0.62	0.15	0.64	0.53	0.73	0.61	0.22	0.67	0.5	0.8	0.72	0.13	0.74	0.65	0.82	0.81	0.08	0.81	0.75	0.87	199.79	152.2	160.76	107.91	247.05	262.99	187.79	214.99	144.69	327.97	3759	0.05
0.06	0.64	0.21	0.69	0.54	0.79	0.93	0.04	0.94	0.92	0.96	0.62	0.19	0.66	0.53	0.76	1.73	3.46	0.58	0.31	1.48	1.22	1.07	0.96	0.44	1.71	0.47	0.15	0.49	0.39	0.59	0.48	0.22	0.5	0.33	0.67	0.62	0.13	0.63	0.55	0.72	0.74	0.09	0.75	0.69	0.8	199.91	150.14	160.82	107.9	247.42	334.7	234.28	274.51	187.06	412.14	3824	0.1
0.11	0.53	0.23	0.57	0.4	0.69	0.9	0.06	0.91	0.87	0.93	0.51	0.2	0.54	0.4	0.66	2.08	3.73	0.71	0.37	1.83	1.46	1.19	1.17	0.56	2.06	0.38	0.16	0.39	0.29	0.49	0.4	0.21	0.4	0.25	0.5	0.56	0.13	0.57	0.47	0.64	0.69	0.09	0.69	0.63	0.75	198.11	144.58	160.42	107.79	246.53	422.78	274.89	354.43	244.28	520.71	3752	0.17
0.15	0.4	0.24	0.43	0.24	0.57	0.84	0.07	0.85	0.8	0.89	0.38	0.21	0.41	0.26	0.54	2.67	4.7	0.84	0.45	2.42	1.65	1.37	1.33	0.62	2.33	0.28	0.16	0.29	0.18	0.39	0.31	0.2	0.33	0.17	0.5	0.49	0.13	0.5	0.41	0.58	0.64	0.09	0.65	0.58	0.7	197.58	147.11	160.19	107.9	245.69	580.04	362.16	495.79	338.72	717.87	3677	0.29
0.18	0.3	0.23	0.31	0.15	0.47	0.78	0.09	0.79	0.73	0.84	0.29	0.2	0.3	0.16	0.44	3.35	5.82	0.98	0.51	3.31	1.87	1.5	1.54	0.72	2.63	0.21	0.15	0.21	0.11	0.31	0.26	0.19	0.25	0.17	0.33	0.44	0.12	0.44	0.37	0.53	0.6	0.09	0.6	0.54	0.66	198.91	148.62	160.37	107.91	246.68	780.18	518.01	659.92	457.42	956.29	3759	0.44
0.32	0.15	0.21	0.14	0.0	0.29	0.59	0.15	0.6	0.49	0.71	0.14	0.19	0.14	0.01	0.27	6.15	8.93	2.09	0.79	8.24	2.25	1.79	1.83	0.86	3.18	0.1	0.13	0.1	0.01	0.19	0.18	0.17	0.17	0.0	0.33	0.37	0.12	0.37	0.29	0.44	0.55	0.08	0.55	0.5	0.6	197.93	146.95	160.27	107.52	246.28	1511.55	1069.09	1246.78	825.1	1896.01	10790	1.0


==> data_new/ra/agnews/xlnet/IG_auc.tex <==
0.14

==> data_new/ra/agnews/xlnet/IG_ppl.tex <==
6.6

==> data_new/ra/agnews/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.09	0.99	0.96	1.0	0.99	0.02	0.99	0.98	1.0	0.97	0.05	0.98	0.96	1.0	43.51	138.38	8.09	1.97	26.26	0.48	0.74	0.23	0.03	0.62	0.9	0.09	0.91	0.87	0.96	0.87	0.16	0.83	0.8	1.0	0.92	0.08	0.94	0.89	1.0	0.95	0.05	0.97	0.93	1.0	198.95	148.57	160.53	107.9	246.91	224.45	160.14	185.18	123.81	279.94	3756	0.02
0.03	0.92	0.11	0.96	0.9	0.98	0.97	0.03	0.97	0.96	0.98	0.94	0.07	0.96	0.93	0.98	85.43	236.5	19.65	8.63	60.87	0.76	0.9	0.49	0.21	0.97	0.83	0.09	0.85	0.8	0.89	0.78	0.18	0.8	0.67	0.83	0.87	0.09	0.89	0.83	0.94	0.92	0.05	0.93	0.9	0.96	199.75	152.18	160.76	107.9	246.97	262.93	187.77	215.0	144.65	327.89	3759	0.05
0.06	0.87	0.13	0.91	0.83	0.95	0.93	0.04	0.94	0.92	0.96	0.91	0.07	0.92	0.88	0.95	122.55	281.98	29.79	13.23	98.23	1.01	1.05	0.72	0.32	1.33	0.77	0.09	0.79	0.73	0.83	0.69	0.2	0.67	0.6	0.83	0.82	0.09	0.84	0.78	0.89	0.89	0.06	0.9	0.86	0.93	199.91	150.14	160.82	107.9	247.42	334.7	234.28	274.51	187.06	412.14	3824	0.1
0.11	0.82	0.14	0.86	0.76	0.92	0.9	0.06	0.91	0.87	0.93	0.87	0.08	0.89	0.85	0.92	150.18	320.73	38.38	17.47	132.26	1.2	1.2	0.89	0.39	1.63	0.72	0.09	0.74	0.68	0.78	0.63	0.2	0.67	0.5	0.8	0.79	0.1	0.79	0.74	0.84	0.87	0.06	0.88	0.83	0.91	198.11	144.58	160.42	107.79	246.53	422.78	274.89	354.43	244.28	520.71	3752	0.17
0.15	0.76	0.16	0.79	0.68	0.87	0.84	0.07	0.85	0.8	0.89	0.83	0.1	0.85	0.79	0.89	220.62	461.54	50.21	22.54	186.04	1.45	1.38	1.09	0.49	2.0	0.66	0.1	0.68	0.61	0.73	0.56	0.21	0.6	0.4	0.67	0.74	0.1	0.74	0.68	0.8	0.84	0.06	0.84	0.81	0.88	197.6	147.13	160.21	107.89	245.78	580.11	362.19	496.07	338.75	717.95	3676	0.29
0.18	0.69	0.17	0.73	0.6	0.82	0.78	0.09	0.79	0.73	0.84	0.78	0.11	0.8	0.73	0.85	297.03	574.21	66.83	27.25	271.65	1.6	1.45	1.22	0.56	2.19	0.61	0.1	0.62	0.55	0.68	0.5	0.21	0.5	0.33	0.67	0.7	0.1	0.71	0.63	0.78	0.81	0.07	0.81	0.78	0.86	198.88	148.61	160.35	107.91	246.67	780.38	518.11	660.01	457.54	956.71	3760	0.44
0.32	0.54	0.2	0.56	0.41	0.7	0.59	0.15	0.6	0.49	0.71	0.63	0.17	0.65	0.52	0.75	656.49	1012.19	181.36	52.03	823.76	2.09	1.82	1.61	0.73	2.95	0.47	0.14	0.48	0.38	0.57	0.39	0.21	0.33	0.2	0.5	0.6	0.12	0.61	0.53	0.68	0.74	0.09	0.75	0.69	0.8	197.91	146.94	160.26	107.5	246.16	1510.17	1051.76	1247.4	826.11	1893.34	10790	1.0


==> data_new/ra/agnews/xlnet/S_auc.tex <==
0.24

==> data_new/ra/agnews/xlnet/S_ppl.tex <==
6.6

==> data_new/ra/fakenews/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.12	1.0	0.98	1.0	0.98	0.02	0.98	0.98	0.99	0.98	0.07	0.99	0.98	1.0	0.31	0.8	0.13	0.04	0.34	3.06	14.36	0.58	0.14	1.62	0.93	0.09	0.95	0.92	0.96	0.95	0.06	0.97	0.94	0.98	0.95	0.06	0.97	0.95	0.98	0.96	0.04	0.98	0.96	0.98	80.85	317.16	44.9	35.59	60.45	89.9	316.88	53.92	42.81	72.24	1937	0.02
0.03	0.92	0.17	0.98	0.96	1.0	0.96	0.02	0.96	0.95	0.97	0.96	0.09	0.98	0.96	0.99	0.48	1.11	0.28	0.09	0.54	4.43	17.38	0.95	0.29	2.63	0.88	0.11	0.92	0.88	0.94	0.92	0.07	0.94	0.91	0.97	0.93	0.07	0.95	0.92	0.97	0.94	0.05	0.96	0.94	0.97	63.02	100.66	44.81	35.84	59.8	85.88	123.06	64.13	51.61	84.03	1888	0.07
0.06	0.88	0.22	0.97	0.93	0.99	0.93	0.03	0.93	0.92	0.95	0.93	0.12	0.96	0.93	0.98	0.66	1.34	0.43	0.16	0.72	7.34	25.54	1.54	0.47	4.02	0.83	0.13	0.88	0.82	0.91	0.89	0.1	0.92	0.87	0.95	0.9	0.09	0.93	0.89	0.95	0.92	0.07	0.94	0.91	0.96	63.59	91.88	44.98	35.93	60.0	109.54	137.61	82.48	67.37	107.71	1890	0.13
0.11	0.84	0.24	0.95	0.85	0.98	0.9	0.04	0.9	0.88	0.93	0.9	0.13	0.95	0.9	0.97	0.78	1.32	0.56	0.23	0.83	9.42	29.44	1.95	0.67	5.21	0.8	0.14	0.85	0.77	0.88	0.86	0.11	0.89	0.84	0.93	0.87	0.09	0.91	0.86	0.93	0.9	0.07	0.93	0.89	0.95	63.15	91.82	44.86	35.86	59.97	135.54	168.69	104.72	85.62	134.7	1886	0.21
0.15	0.79	0.27	0.92	0.7	0.96	0.86	0.06	0.86	0.83	0.91	0.86	0.16	0.92	0.84	0.95	0.95	1.37	0.68	0.35	1.0	12.72	33.93	2.95	0.97	7.76	0.74	0.16	0.8	0.69	0.85	0.83	0.12	0.86	0.8	0.9	0.84	0.11	0.88	0.8	0.91	0.87	0.08	0.9	0.85	0.93	74.43	307.88	44.39	35.15	59.46	193.32	277.89	146.41	120.74	186.05	1474	0.29
0.18	0.76	0.28	0.9	0.64	0.94	0.82	0.07	0.81	0.77	0.87	0.83	0.16	0.9	0.8	0.93	1.13	1.64	0.77	0.4	1.13	16.15	40.78	3.36	1.26	8.68	0.7	0.16	0.76	0.65	0.81	0.8	0.12	0.83	0.76	0.88	0.82	0.11	0.85	0.77	0.89	0.85	0.08	0.88	0.83	0.91	65.28	104.51	44.62	35.31	60.02	257.85	261.57	203.6	170.15	256.76	1145	0.53
0.32	0.68	0.31	0.85	0.45	0.91	0.72	0.1	0.73	0.65	0.79	0.77	0.2	0.85	0.7	0.91	1.53	1.99	0.96	0.56	1.51	26.86	53.96	5.38	1.7	17.37	0.63	0.19	0.7	0.55	0.77	0.75	0.14	0.79	0.7	0.85	0.77	0.12	0.81	0.71	0.86	0.82	0.1	0.85	0.77	0.89	71.02	194.69	45.11	35.52	61.28	421.58	452.41	339.99	259.0	445.72	1689	0.89


==> data_new/ra/fakenews/bert/A_auc.tex <==
0.26

==> data_new/ra/fakenews/bert/A_ppl.tex <==
5.5

==> data_new/ra/fakenews/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.87	0.32	0.99	0.94	1.0	0.98	0.02	0.98	0.98	0.99	0.84	0.27	0.95	0.85	0.98	4.77	29.03	0.07	0.0	0.76	9.69	19.9	3.41	1.06	9.73	0.77	0.26	0.87	0.74	0.93	0.83	0.19	0.89	0.78	0.95	0.85	0.17	0.91	0.82	0.95	0.89	0.13	0.93	0.87	0.96	81.23	318.86	44.94	35.59	60.72	90.27	318.58	53.95	42.81	72.31	1916	0.03
0.03	0.81	0.37	0.98	0.86	1.0	0.96	0.02	0.96	0.95	0.97	0.77	0.29	0.89	0.73	0.94	6.17	35.62	0.14	0.0	1.28	13.37	29.32	5.25	1.74	13.88	0.68	0.27	0.78	0.61	0.86	0.76	0.2	0.82	0.67	0.9	0.79	0.17	0.86	0.74	0.91	0.84	0.14	0.89	0.8	0.93	63.19	101.35	44.87	35.82	59.86	86.01	123.41	64.16	51.61	84.57	1861	0.1
0.06	0.74	0.42	0.95	0.7	0.99	0.93	0.03	0.93	0.92	0.95	0.69	0.32	0.82	0.59	0.9	9.49	47.39	0.2	0.0	2.13	17.18	35.24	7.22	2.6	18.17	0.59	0.28	0.7	0.48	0.79	0.7	0.21	0.76	0.59	0.86	0.73	0.18	0.8	0.65	0.86	0.8	0.14	0.85	0.74	0.9	63.74	92.2	45.09	35.93	60.11	108.91	134.89	82.57	66.97	107.95	1876	0.19
0.11	0.68	0.46	0.92	0.54	0.98	0.9	0.04	0.9	0.88	0.93	0.62	0.33	0.75	0.48	0.85	14.35	72.3	0.28	0.01	2.77	22.84	46.78	9.47	3.38	24.18	0.53	0.29	0.62	0.38	0.73	0.65	0.21	0.69	0.51	0.8	0.69	0.18	0.75	0.59	0.82	0.76	0.15	0.81	0.69	0.87	62.77	91.13	44.87	35.79	59.86	134.4	137.68	105.68	85.65	134.07	1867	0.3
0.15	0.65	0.45	0.88	0.41	0.97	0.86	0.06	0.86	0.83	0.9	0.56	0.31	0.67	0.4	0.79	13.42	62.58	0.33	0.01	4.05	22.51	40.03	11.2	3.88	26.16	0.47	0.26	0.54	0.31	0.66	0.61	0.19	0.65	0.47	0.75	0.65	0.17	0.69	0.55	0.77	0.74	0.13	0.77	0.66	0.83	85.43	391.32	44.7	34.9	60.92	216.57	506.26	146.77	120.17	188.54	894	0.4
0.18	0.6	0.47	0.82	0.32	0.96	0.81	0.07	0.8	0.77	0.87	0.5	0.3	0.6	0.32	0.73	17.36	69.23	0.5	0.01	5.6	25.87	43.77	13.52	5.11	29.43	0.41	0.25	0.47	0.24	0.59	0.56	0.19	0.59	0.41	0.71	0.61	0.16	0.65	0.5	0.73	0.7	0.13	0.73	0.62	0.8	63.93	98.97	44.73	35.12	59.98	252.86	235.79	205.37	170.03	256.0	1313	0.78


==> data_new/ra/fakenews/bert/IG_auc.tex <==
0.13

==> data_new/ra/fakenews/bert/IG_ppl.tex <==
3.8

==> data_new/ra/fakenews/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.93	0.12	0.98	0.93	1.0	0.98	0.02	0.98	0.98	0.99	0.95	0.06	0.97	0.95	0.99	29.58	236.07	0.11	0.01	2.7	5.56	10.46	2.13	0.66	5.85	0.86	0.1	0.89	0.82	0.93	0.87	0.11	0.9	0.82	0.94	0.91	0.08	0.93	0.88	0.96	0.93	0.05	0.95	0.91	0.96	80.82	316.61	44.88	35.61	60.45	89.86	316.33	53.92	42.81	72.17	1944	0.02
0.03	0.89	0.14	0.95	0.86	0.99	0.96	0.02	0.96	0.95	0.97	0.92	0.07	0.95	0.9	0.97	33.5	213.31	0.19	0.02	4.85	7.23	12.15	3.13	1.06	8.25	0.8	0.1	0.83	0.75	0.87	0.82	0.12	0.83	0.76	0.9	0.87	0.08	0.89	0.83	0.92	0.9	0.06	0.92	0.88	0.94	63.12	100.78	44.86	35.89	59.78	85.9	122.7	64.16	51.71	84.53	1886	0.07
0.06	0.86	0.16	0.92	0.81	0.97	0.93	0.03	0.93	0.92	0.95	0.89	0.09	0.91	0.86	0.94	56.04	292.46	0.28	0.02	7.59	8.55	13.28	3.92	1.39	9.64	0.74	0.11	0.77	0.69	0.82	0.77	0.13	0.78	0.71	0.85	0.83	0.08	0.85	0.79	0.89	0.88	0.06	0.89	0.85	0.91	68.04	169.83	45.09	35.95	60.01	111.87	166.5	82.51	66.81	108.09	1912	0.13
0.11	0.83	0.17	0.89	0.75	0.95	0.9	0.04	0.9	0.88	0.93	0.86	0.09	0.88	0.83	0.92	83.02	407.89	0.36	0.03	9.52	9.54	13.63	4.75	1.81	11.37	0.7	0.1	0.72	0.65	0.77	0.73	0.13	0.75	0.67	0.82	0.81	0.08	0.82	0.77	0.86	0.86	0.06	0.87	0.83	0.89	62.79	90.77	44.82	35.85	59.75	133.43	134.45	105.23	85.9	134.34	1913	0.22
0.15	0.8	0.19	0.86	0.7	0.93	0.86	0.06	0.86	0.83	0.9	0.83	0.09	0.85	0.79	0.89	112.04	520.44	0.48	0.03	14.27	10.54	14.03	6.02	2.25	12.77	0.66	0.1	0.68	0.61	0.73	0.7	0.13	0.71	0.63	0.78	0.78	0.08	0.8	0.74	0.83	0.83	0.06	0.84	0.8	0.88	84.5	385.18	44.74	35.11	60.57	204.96	327.19	146.88	120.37	188.45	923	0.28
0.18	0.76	0.19	0.82	0.66	0.91	0.81	0.07	0.8	0.77	0.87	0.79	0.09	0.82	0.76	0.86	157.07	716.78	0.51	0.04	19.33	11.42	14.85	6.68	2.44	14.31	0.62	0.09	0.64	0.58	0.69	0.67	0.13	0.67	0.61	0.75	0.76	0.08	0.77	0.72	0.81	0.82	0.05	0.82	0.79	0.85	64.15	99.35	44.53	35.24	60.0	256.47	291.09	207.19	170.41	254.33	1378	0.59
0.32	0.74	0.2	0.78	0.64	0.89	0.72	0.1	0.73	0.66	0.79	0.75	0.1	0.78	0.71	0.82	226.31	764.28	1.0	0.04	31.92	12.3	15.34	7.43	2.7	15.88	0.58	0.1	0.59	0.53	0.64	0.63	0.13	0.65	0.56	0.71	0.73	0.08	0.75	0.69	0.78	0.79	0.06	0.8	0.77	0.83	69.26	184.37	45.05	35.52	60.57	422.25	496.33	335.91	255.49	441.86	1895	1.0


==> data_new/ra/fakenews/bert/S_auc.tex <==
0.26

==> data_new/ra/fakenews/bert/S_ppl.tex <==
5.1

==> data_new/ra/fakenews/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.99	0.04	1.0	0.99	1.0	0.98	0.01	0.98	0.98	0.99	0.96	0.03	0.97	0.95	0.98	0.56	0.96	0.34	0.21	0.57	2.62	4.52	1.17	0.39	2.7	0.93	0.05	0.94	0.92	0.95	0.95	0.04	0.96	0.92	0.98	0.96	0.03	0.96	0.95	0.97	0.96	0.03	0.96	0.95	0.98	79.84	235.84	43.0	34.53	56.47	87.05	235.28	50.21	40.6	65.23	4050	0.02
0.03	0.97	0.05	0.99	0.98	1.0	0.96	0.02	0.96	0.95	0.97	0.92	0.04	0.93	0.91	0.95	0.9	1.31	0.58	0.39	0.92	4.26	6.27	2.11	0.76	4.67	0.86	0.05	0.87	0.85	0.89	0.9	0.06	0.9	0.88	0.94	0.92	0.04	0.92	0.9	0.94	0.93	0.03	0.94	0.92	0.95	55.95	69.2	42.47	34.35	54.82	73.69	83.34	58.25	47.41	73.4	3901	0.08
0.06	0.95	0.07	0.98	0.95	0.99	0.93	0.02	0.93	0.92	0.95	0.87	0.05	0.88	0.85	0.9	1.42	2.43	0.84	0.6	1.29	5.76	7.62	3.17	1.17	6.8	0.79	0.06	0.8	0.76	0.82	0.85	0.07	0.86	0.81	0.9	0.87	0.05	0.88	0.85	0.9	0.89	0.04	0.9	0.88	0.92	60.54	121.99	42.41	34.12	54.97	93.13	112.73	71.96	59.22	90.84	3983	0.13
0.11	0.94	0.09	0.97	0.93	0.99	0.9	0.03	0.9	0.88	0.92	0.82	0.06	0.83	0.79	0.86	1.48	1.68	1.06	0.78	1.63	7.36	8.92	4.14	1.54	9.32	0.72	0.07	0.73	0.68	0.76	0.81	0.08	0.81	0.76	0.86	0.83	0.05	0.84	0.81	0.86	0.86	0.04	0.87	0.84	0.89	61.03	115.28	42.55	34.45	55.0	115.14	164.5	89.36	74.38	110.21	2989	0.21
0.15	0.9	0.11	0.95	0.87	0.98	0.85	0.03	0.85	0.83	0.87	0.75	0.07	0.75	0.71	0.79	1.83	1.69	1.41	1.03	2.12	9.69	10.66	5.79	2.47	12.7	0.63	0.07	0.63	0.59	0.67	0.75	0.09	0.75	0.69	0.8	0.78	0.05	0.78	0.75	0.81	0.82	0.04	0.82	0.79	0.84	58.46	85.64	42.32	34.44	54.59	149.23	159.51	121.44	102.68	145.95	2035	0.38
0.18	0.87	0.14	0.92	0.81	0.97	0.8	0.04	0.8	0.77	0.82	0.67	0.08	0.67	0.62	0.72	2.19	1.76	1.74	1.28	2.6	12.15	12.63	7.5	2.78	17.68	0.55	0.08	0.55	0.5	0.6	0.69	0.1	0.69	0.63	0.75	0.73	0.06	0.73	0.69	0.76	0.78	0.05	0.78	0.75	0.8	60.31	80.86	42.31	34.29	54.86	193.05	173.37	160.05	134.91	191.21	1560	0.53
0.32	0.79	0.18	0.84	0.68	0.94	0.68	0.07	0.68	0.62	0.74	0.55	0.11	0.54	0.47	0.62	2.9	2.25	2.54	1.77	3.4	16.26	15.26	11.52	4.04	24.51	0.43	0.1	0.42	0.36	0.49	0.6	0.12	0.59	0.51	0.67	0.65	0.07	0.64	0.6	0.69	0.71	0.05	0.71	0.68	0.75	59.03	101.98	42.18	34.22	54.65	303.03	290.5	264.76	207.54	325.05	3032	1.0


==> data_new/ra/fakenews/cnn/IG_auc.tex <==
0.29

==> data_new/ra/fakenews/cnn/IG_ppl.tex <==
4.1

==> data_new/ra/fakenews/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.99	0.02	0.99	0.99	1.0	0.98	0.01	0.98	0.98	0.99	0.98	0.02	0.98	0.97	0.99	8.89	15.49	6.01	4.17	8.6	2.16	3.53	1.26	0.45	2.73	0.94	0.05	0.95	0.93	0.96	0.94	0.06	0.96	0.92	0.98	0.96	0.04	0.96	0.95	0.98	0.97	0.03	0.97	0.96	0.98	79.87	235.78	43.01	34.54	56.46	87.08	235.22	50.19	40.62	65.26	4047	0.02
0.03	0.97	0.03	0.98	0.97	0.99	0.96	0.02	0.96	0.95	0.97	0.95	0.03	0.96	0.94	0.97	13.99	21.54	9.46	7.17	13.23	3.4	4.58	2.17	0.89	4.34	0.89	0.05	0.9	0.88	0.91	0.9	0.07	0.91	0.86	0.95	0.92	0.05	0.93	0.9	0.95	0.94	0.03	0.95	0.93	0.96	55.94	69.19	42.46	34.35	54.81	73.67	83.34	58.25	47.4	73.4	3902	0.09
0.06	0.95	0.04	0.97	0.94	0.98	0.93	0.02	0.93	0.92	0.95	0.92	0.04	0.93	0.91	0.95	22.43	43.66	13.33	10.3	19.35	4.5	5.42	2.98	1.17	6.02	0.82	0.06	0.83	0.81	0.86	0.85	0.1	0.86	0.8	0.91	0.88	0.06	0.89	0.86	0.92	0.91	0.04	0.92	0.9	0.93	62.28	131.55	42.5	34.15	55.15	94.86	119.94	72.08	59.26	91.11	3997	0.14
0.11	0.94	0.05	0.95	0.92	0.97	0.9	0.03	0.9	0.89	0.92	0.89	0.04	0.9	0.87	0.92	22.42	26.56	16.76	12.95	24.02	5.66	6.57	3.82	1.53	7.51	0.77	0.06	0.78	0.74	0.81	0.81	0.1	0.82	0.76	0.88	0.85	0.06	0.85	0.82	0.88	0.89	0.04	0.89	0.87	0.91	60.02	109.75	42.71	34.59	55.0	113.78	153.4	89.43	74.74	109.96	3899	0.24
0.15	0.91	0.06	0.92	0.89	0.95	0.85	0.03	0.85	0.83	0.87	0.85	0.05	0.86	0.82	0.89	27.65	27.54	22.25	16.84	30.04	7.34	7.82	5.03	2.12	9.97	0.71	0.06	0.71	0.67	0.75	0.76	0.11	0.76	0.71	0.82	0.81	0.06	0.81	0.77	0.84	0.86	0.04	0.86	0.83	0.88	58.44	85.58	42.32	34.43	54.54	149.19	159.4	121.67	102.63	145.9	2036	0.42
0.18	0.88	0.09	0.89	0.85	0.93	0.8	0.04	0.8	0.77	0.82	0.81	0.07	0.81	0.77	0.85	33.17	27.89	27.44	20.55	37.0	9.01	9.61	6.52	2.48	12.22	0.65	0.07	0.65	0.61	0.69	0.72	0.11	0.73	0.65	0.78	0.77	0.07	0.76	0.73	0.8	0.83	0.05	0.82	0.8	0.85	58.99	76.43	42.13	34.28	54.72	190.05	159.8	159.63	134.68	190.9	1680	0.6
0.32	0.82	0.1	0.84	0.78	0.89	0.7	0.07	0.71	0.64	0.75	0.74	0.08	0.75	0.7	0.8	43.07	36.66	36.73	26.34	48.37	10.99	11.01	7.55	2.95	15.38	0.57	0.08	0.57	0.52	0.62	0.66	0.13	0.65	0.57	0.73	0.72	0.07	0.71	0.67	0.76	0.79	0.05	0.79	0.76	0.82	60.29	112.47	42.1	33.88	54.92	284.24	248.4	239.33	191.89	307.64	2166	1.0


==> data_new/ra/fakenews/cnn/S_auc.tex <==
0.29

==> data_new/ra/fakenews/cnn/S_ppl.tex <==
3.7

==> data_new/ra/fakenews/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.06	1.0	0.99	1.0	0.98	0.01	0.98	0.98	0.99	0.96	0.03	0.97	0.95	0.98	0.59	1.01	0.3	0.17	0.59	3.5	4.71	1.94	0.67	4.46	0.91	0.05	0.91	0.89	0.93	0.93	0.06	0.94	0.9	0.96	0.94	0.03	0.94	0.92	0.96	0.95	0.02	0.96	0.94	0.97	80.18	236.3	43.03	34.6	56.72	87.44	235.73	50.34	40.64	65.65	4034	0.02
0.03	0.95	0.1	0.99	0.97	0.99	0.96	0.02	0.96	0.95	0.97	0.92	0.04	0.93	0.91	0.95	1.0	1.38	0.53	0.32	1.04	5.27	6.47	3.14	1.22	6.66	0.84	0.05	0.85	0.82	0.87	0.88	0.07	0.88	0.84	0.92	0.9	0.04	0.91	0.88	0.93	0.92	0.03	0.93	0.91	0.94	56.16	69.85	42.48	34.42	54.91	73.86	80.17	58.16	47.57	73.27	3888	0.09
0.06	0.93	0.13	0.97	0.93	0.99	0.93	0.02	0.93	0.92	0.95	0.88	0.05	0.88	0.85	0.91	1.38	1.69	0.8	0.49	1.53	7.1	7.81	4.6	1.64	9.8	0.77	0.06	0.78	0.74	0.81	0.83	0.08	0.84	0.78	0.88	0.86	0.05	0.86	0.83	0.89	0.89	0.03	0.89	0.88	0.91	60.92	122.59	42.41	34.23	55.11	96.25	158.51	72.54	59.69	90.22	3973	0.16
0.11	0.89	0.15	0.95	0.89	0.98	0.9	0.03	0.9	0.88	0.92	0.83	0.06	0.83	0.8	0.86	1.7	1.76	1.03	0.66	2.12	8.62	9.27	5.48	2.07	12.06	0.71	0.06	0.72	0.68	0.75	0.79	0.09	0.79	0.74	0.84	0.82	0.05	0.82	0.79	0.85	0.86	0.04	0.87	0.84	0.88	61.92	117.84	42.82	34.6	55.24	116.29	143.6	90.02	74.98	110.39	3232	0.24
0.15	0.84	0.2	0.93	0.82	0.96	0.85	0.04	0.85	0.83	0.87	0.76	0.07	0.77	0.72	0.8	2.21	2.08	1.35	0.84	3.04	10.61	10.84	7.27	2.6	15.1	0.64	0.07	0.64	0.59	0.68	0.73	0.1	0.73	0.67	0.78	0.77	0.06	0.77	0.74	0.81	0.83	0.04	0.83	0.8	0.85	64.35	163.51	42.57	34.51	55.07	157.17	234.84	121.6	102.89	147.36	2100	0.4
0.18	0.8	0.22	0.89	0.73	0.94	0.8	0.04	0.8	0.77	0.82	0.7	0.07	0.7	0.66	0.74	2.48	2.13	1.7	0.99	3.45	12.32	11.92	8.71	3.3	17.79	0.58	0.07	0.57	0.53	0.61	0.68	0.1	0.68	0.63	0.74	0.73	0.06	0.73	0.7	0.76	0.8	0.04	0.8	0.77	0.82	59.1	85.29	42.77	34.65	55.32	191.25	167.94	161.17	137.49	191.99	3450	0.61
0.32	0.72	0.27	0.84	0.56	0.91	0.7	0.07	0.71	0.65	0.75	0.61	0.09	0.61	0.55	0.67	2.94	2.26	2.21	1.18	4.27	14.34	13.52	9.98	4.07	20.91	0.49	0.08	0.49	0.43	0.54	0.62	0.11	0.61	0.55	0.67	0.67	0.07	0.67	0.63	0.71	0.75	0.04	0.75	0.72	0.78	60.48	112.76	42.0	33.85	54.98	280.6	223.82	236.86	189.86	303.15	2204	1.0


==> data_new/ra/fakenews/lstm/IG_auc.tex <==
0.27

==> data_new/ra/fakenews/lstm/IG_ppl.tex <==
3.6

==> data_new/ra/fakenews/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.94	0.09	0.97	0.93	0.99	0.98	0.01	0.98	0.98	0.99	0.96	0.03	0.97	0.95	0.98	15.58	20.44	9.4	4.91	18.11	6.69	9.38	3.37	1.05	8.33	0.89	0.06	0.9	0.87	0.93	0.88	0.1	0.9	0.84	0.94	0.92	0.05	0.93	0.9	0.95	0.95	0.03	0.96	0.94	0.97	80.19	236.55	43.03	34.6	56.72	87.46	235.98	50.34	40.64	65.65	4034	0.02
0.03	0.88	0.13	0.93	0.85	0.96	0.96	0.02	0.96	0.95	0.97	0.93	0.04	0.94	0.91	0.96	24.34	25.47	16.16	9.4	28.67	10.44	12.63	6.16	2.2	13.66	0.82	0.07	0.83	0.79	0.86	0.81	0.11	0.82	0.75	0.88	0.88	0.06	0.89	0.85	0.92	0.92	0.04	0.93	0.9	0.94	56.18	69.88	42.49	34.43	54.92	73.88	80.21	58.2	47.56	73.29	3888	0.09
0.06	0.82	0.15	0.86	0.75	0.92	0.93	0.02	0.93	0.92	0.95	0.89	0.05	0.9	0.86	0.92	32.1	30.17	22.71	13.58	39.28	13.13	14.72	8.21	2.79	17.86	0.75	0.07	0.76	0.71	0.8	0.74	0.12	0.75	0.67	0.82	0.83	0.06	0.84	0.79	0.87	0.89	0.04	0.89	0.86	0.91	60.79	122.5	42.43	34.23	55.1	96.13	158.45	72.57	59.7	90.27	3970	0.16
0.11	0.76	0.16	0.79	0.67	0.88	0.9	0.03	0.9	0.88	0.92	0.85	0.06	0.86	0.82	0.89	38.67	32.92	29.48	17.92	47.67	16.31	17.12	10.93	4.08	22.62	0.7	0.08	0.7	0.65	0.74	0.68	0.13	0.7	0.61	0.76	0.79	0.07	0.8	0.76	0.83	0.86	0.04	0.86	0.84	0.89	62.25	120.0	42.61	34.59	55.23	116.61	145.44	89.69	74.97	110.15	3108	0.24
0.15	0.68	0.17	0.71	0.58	0.82	0.85	0.03	0.85	0.83	0.87	0.8	0.07	0.81	0.76	0.84	46.94	36.3	36.76	22.54	60.77	18.89	18.84	13.27	4.83	26.53	0.63	0.08	0.64	0.59	0.68	0.62	0.14	0.63	0.55	0.71	0.74	0.07	0.75	0.71	0.79	0.83	0.04	0.83	0.8	0.85	62.86	150.29	42.49	34.49	55.09	154.06	188.91	121.53	102.86	147.44	2159	0.4
0.18	0.63	0.17	0.64	0.51	0.76	0.8	0.04	0.8	0.77	0.82	0.76	0.07	0.76	0.72	0.8	52.58	37.98	42.46	25.5	68.98	21.22	20.87	14.78	5.57	30.78	0.58	0.07	0.59	0.54	0.63	0.57	0.13	0.59	0.49	0.67	0.71	0.07	0.71	0.67	0.75	0.8	0.04	0.8	0.78	0.83	59.27	85.74	42.68	34.61	55.03	191.84	170.36	161.06	136.52	191.96	3140	0.61
0.32	0.56	0.18	0.57	0.43	0.69	0.7	0.07	0.71	0.65	0.75	0.7	0.09	0.7	0.64	0.76	58.9	39.92	50.15	29.37	77.76	24.05	22.2	16.75	6.3	36.49	0.52	0.08	0.52	0.47	0.58	0.52	0.14	0.51	0.43	0.61	0.66	0.07	0.66	0.62	0.71	0.77	0.05	0.77	0.74	0.8	60.49	112.84	42.0	33.84	55.0	280.65	223.82	236.61	190.49	303.25	2204	1.0


==> data_new/ra/fakenews/lstm/S_auc.tex <==
0.22

==> data_new/ra/fakenews/lstm/S_ppl.tex <==
3.6

==> data_new/ra/fakenews/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.07	1.0	0.99	1.0	0.98	0.01	0.98	0.98	0.99	0.98	0.02	0.99	0.98	0.99	0.04	0.08	0.02	0.01	0.04	6.44	20.33	1.53	0.36	4.85	0.94	0.04	0.95	0.93	0.96	0.95	0.05	0.96	0.93	0.98	0.96	0.03	0.97	0.95	0.98	0.97	0.02	0.98	0.96	0.98	79.8	235.59	42.95	34.53	56.46	86.93	234.95	50.32	40.54	64.82	4068	0.02
0.03	0.97	0.11	1.0	0.98	1.0	0.96	0.02	0.96	0.95	0.97	0.97	0.03	0.97	0.96	0.98	0.07	0.11	0.04	0.02	0.08	12.37	30.92	3.37	0.89	9.45	0.9	0.05	0.91	0.88	0.92	0.91	0.07	0.92	0.88	0.94	0.93	0.04	0.94	0.92	0.95	0.95	0.03	0.95	0.94	0.97	55.99	69.59	42.36	34.35	54.82	74.0	88.76	58.22	47.53	73.15	3921	0.09
0.06	0.94	0.14	0.99	0.96	1.0	0.93	0.02	0.93	0.92	0.95	0.94	0.04	0.95	0.93	0.96	0.11	0.13	0.06	0.03	0.12	19.43	40.44	5.56	1.59	16.03	0.84	0.06	0.86	0.83	0.88	0.86	0.09	0.88	0.82	0.9	0.89	0.05	0.9	0.88	0.92	0.92	0.04	0.93	0.91	0.95	62.33	131.67	42.47	34.19	55.17	97.22	155.74	72.33	59.63	90.4	4015	0.15
0.11	0.92	0.17	0.98	0.93	1.0	0.9	0.03	0.9	0.88	0.92	0.91	0.05	0.93	0.9	0.94	0.14	0.15	0.08	0.05	0.15	25.76	47.74	7.9	2.26	22.13	0.8	0.07	0.81	0.78	0.84	0.82	0.1	0.83	0.78	0.88	0.86	0.06	0.88	0.84	0.9	0.9	0.04	0.91	0.89	0.93	60.1	109.98	42.61	34.56	55.06	114.68	140.67	89.94	75.04	110.21	3923	0.24
0.15	0.87	0.21	0.96	0.87	0.99	0.85	0.03	0.85	0.83	0.87	0.87	0.06	0.89	0.86	0.91	0.18	0.17	0.11	0.07	0.2	34.77	55.24	12.3	3.49	34.36	0.74	0.08	0.75	0.71	0.78	0.76	0.12	0.78	0.71	0.82	0.82	0.06	0.83	0.8	0.86	0.87	0.04	0.88	0.86	0.9	58.07	83.65	42.3	34.37	54.75	147.75	143.93	121.58	103.6	147.33	2167	0.42
0.18	0.84	0.23	0.94	0.82	0.98	0.8	0.04	0.8	0.77	0.82	0.83	0.07	0.85	0.81	0.87	0.21	0.18	0.14	0.08	0.25	41.3	58.93	15.57	4.31	45.05	0.69	0.08	0.7	0.65	0.74	0.71	0.12	0.73	0.65	0.78	0.78	0.07	0.79	0.75	0.82	0.85	0.05	0.86	0.82	0.88	59.13	77.36	42.23	34.26	54.94	195.93	198.01	160.19	135.91	189.42	1623	0.62
0.32	0.79	0.25	0.89	0.72	0.97	0.7	0.07	0.71	0.65	0.75	0.77	0.09	0.78	0.72	0.83	0.25	0.19	0.18	0.11	0.32	53.62	65.79	23.49	6.85	72.42	0.61	0.09	0.62	0.56	0.67	0.64	0.14	0.65	0.55	0.73	0.73	0.07	0.73	0.69	0.78	0.81	0.05	0.82	0.78	0.85	60.11	110.52	41.97	33.86	54.83	283.19	280.04	235.33	191.5	305.04	2422	1.0


==> data_new/ra/fakenews/lstmatt/A_auc.tex <==
0.28

==> data_new/ra/fakenews/lstmatt/A_ppl.tex <==
3.7

==> data_new/ra/fakenews/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.07	1.0	0.99	1.0	0.98	0.01	0.98	0.98	0.99	0.96	0.06	0.97	0.95	0.98	0.69	3.35	0.12	0.05	0.32	3.95	7.34	1.55	0.48	4.09	0.91	0.08	0.93	0.9	0.95	0.93	0.07	0.94	0.91	0.98	0.94	0.05	0.95	0.93	0.97	0.96	0.04	0.96	0.95	0.98	79.77	235.34	42.95	34.51	56.45	86.89	234.7	50.29	40.53	64.79	4068	0.03
0.03	0.96	0.1	0.99	0.98	1.0	0.96	0.02	0.96	0.95	0.97	0.92	0.08	0.94	0.91	0.96	1.1	4.54	0.25	0.12	0.6	6.36	9.33	3.32	1.14	7.6	0.84	0.09	0.87	0.83	0.9	0.88	0.09	0.9	0.85	0.94	0.9	0.06	0.92	0.89	0.93	0.93	0.05	0.94	0.92	0.95	55.95	69.57	42.35	34.34	54.81	73.95	88.73	58.21	47.49	73.12	3924	0.09
0.06	0.94	0.13	0.99	0.95	1.0	0.93	0.02	0.93	0.92	0.95	0.87	0.09	0.89	0.84	0.92	1.32	5.33	0.4	0.21	0.99	9.02	12.09	5.02	1.75	11.7	0.78	0.1	0.81	0.74	0.84	0.84	0.1	0.85	0.78	0.9	0.86	0.07	0.88	0.83	0.9	0.9	0.05	0.91	0.88	0.93	62.44	132.31	42.34	34.06	55.11	97.33	159.13	72.25	59.42	90.31	4035	0.16
0.11	0.92	0.14	0.98	0.91	0.99	0.9	0.03	0.9	0.88	0.92	0.82	0.1	0.85	0.78	0.89	1.44	3.32	0.54	0.29	1.29	10.57	13.11	6.13	2.12	14.61	0.72	0.1	0.75	0.67	0.79	0.8	0.11	0.8	0.73	0.87	0.82	0.07	0.84	0.79	0.87	0.87	0.05	0.88	0.84	0.9	64.04	127.12	42.81	34.6	55.41	119.61	157.36	90.0	75.11	110.88	3959	0.25
0.15	0.89	0.16	0.96	0.87	0.98	0.85	0.03	0.85	0.83	0.87	0.76	0.1	0.78	0.72	0.83	1.63	3.4	0.71	0.4	1.54	12.92	14.74	8.24	3.01	18.04	0.65	0.1	0.67	0.6	0.71	0.74	0.11	0.75	0.67	0.82	0.77	0.07	0.78	0.74	0.82	0.83	0.05	0.84	0.81	0.87	58.89	125.52	42.51	34.57	54.8	146.68	150.84	121.54	103.7	146.5	3880	0.43
0.18	0.87	0.17	0.93	0.84	0.97	0.8	0.04	0.8	0.77	0.82	0.7	0.1	0.72	0.64	0.78	2.02	9.23	0.85	0.49	1.74	15.49	18.17	9.84	3.22	21.93	0.59	0.1	0.6	0.53	0.66	0.7	0.12	0.71	0.63	0.78	0.74	0.07	0.74	0.69	0.78	0.8	0.05	0.81	0.77	0.84	61.48	97.93	42.26	34.26	54.97	201.35	239.46	160.45	136.1	189.85	1627	0.65
0.32	0.85	0.17	0.91	0.8	0.96	0.72	0.07	0.73	0.68	0.76	0.63	0.11	0.64	0.57	0.71	1.9	3.69	1.03	0.61	1.82	17.04	18.49	11.78	4.16	23.65	0.52	0.1	0.52	0.45	0.59	0.65	0.12	0.65	0.57	0.73	0.69	0.08	0.69	0.64	0.73	0.77	0.05	0.77	0.74	0.8	59.51	98.58	42.5	34.32	55.19	266.34	243.35	221.92	185.71	283.23	3599	1.0


==> data_new/ra/fakenews/lstmatt/IG_auc.tex <==
0.29

==> data_new/ra/fakenews/lstmatt/IG_ppl.tex <==
3.5

==> data_new/ra/fakenews/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.05	1.0	0.99	1.0	0.98	0.01	0.98	0.98	0.99	0.97	0.04	0.98	0.97	0.99	9.15	26.82	3.27	1.01	8.19	7.07	14.92	2.34	0.61	6.63	0.9	0.07	0.92	0.88	0.94	0.93	0.07	0.94	0.9	0.98	0.94	0.05	0.95	0.92	0.97	0.95	0.04	0.96	0.94	0.97	79.78	235.25	42.95	34.52	56.46	86.9	234.61	50.3	40.54	64.8	4067	0.02
0.03	0.96	0.08	0.99	0.97	1.0	0.96	0.02	0.96	0.95	0.97	0.94	0.06	0.96	0.93	0.98	17.85	59.53	7.14	3.33	15.0	11.83	20.33	4.94	1.5	13.3	0.84	0.08	0.86	0.8	0.89	0.89	0.09	0.9	0.85	0.94	0.9	0.06	0.91	0.87	0.94	0.92	0.05	0.93	0.9	0.95	55.98	69.57	42.38	34.34	54.8	73.99	88.74	58.19	47.53	73.14	3920	0.09
0.06	0.94	0.09	0.98	0.93	0.99	0.93	0.02	0.93	0.92	0.95	0.91	0.07	0.93	0.89	0.96	24.92	52.02	11.85	5.86	23.57	16.37	24.18	7.81	2.41	20.14	0.78	0.09	0.8	0.73	0.84	0.84	0.1	0.86	0.8	0.91	0.86	0.07	0.87	0.82	0.91	0.89	0.05	0.9	0.86	0.93	61.71	130.0	42.41	34.16	55.07	96.47	151.79	72.29	59.61	90.18	4007	0.15
0.11	0.92	0.11	0.96	0.89	0.98	0.9	0.03	0.9	0.88	0.92	0.88	0.08	0.9	0.85	0.94	33.15	62.24	16.38	8.71	33.42	20.33	27.43	10.24	3.25	25.36	0.73	0.1	0.75	0.68	0.8	0.81	0.11	0.82	0.76	0.88	0.83	0.08	0.84	0.78	0.88	0.86	0.06	0.88	0.83	0.91	61.08	113.37	42.75	34.6	55.22	115.91	143.58	90.0	75.06	110.58	3435	0.24
0.15	0.89	0.12	0.93	0.85	0.97	0.85	0.03	0.85	0.83	0.87	0.84	0.09	0.86	0.8	0.9	43.56	78.12	22.24	12.66	47.93	24.28	30.34	12.97	4.44	31.68	0.68	0.1	0.7	0.62	0.75	0.77	0.11	0.78	0.71	0.84	0.79	0.08	0.8	0.75	0.85	0.84	0.06	0.85	0.8	0.88	57.92	81.95	42.25	34.43	54.75	147.72	141.5	121.82	103.67	147.2	2288	0.41
0.18	0.87	0.12	0.91	0.81	0.96	0.8	0.04	0.8	0.77	0.82	0.8	0.11	0.83	0.75	0.88	52.01	74.33	28.36	16.5	63.28	26.7	32.05	14.74	5.29	36.21	0.63	0.11	0.65	0.57	0.71	0.74	0.12	0.75	0.67	0.81	0.76	0.09	0.77	0.71	0.82	0.81	0.06	0.82	0.77	0.86	58.8	75.44	42.17	34.29	54.91	195.42	193.17	160.33	136.14	189.57	1747	0.62
0.32	0.84	0.13	0.87	0.78	0.94	0.7	0.07	0.71	0.65	0.75	0.76	0.11	0.78	0.69	0.84	71.85	143.12	38.07	21.23	81.3	30.1	34.24	18.26	6.24	40.92	0.58	0.11	0.59	0.51	0.66	0.7	0.12	0.71	0.63	0.78	0.73	0.09	0.73	0.67	0.79	0.79	0.07	0.79	0.75	0.83	59.76	109.64	41.97	33.83	54.93	283.42	279.01	236.53	191.97	305.94	2362	1.0


==> data_new/ra/fakenews/lstmatt/S_auc.tex <==
0.29

==> data_new/ra/fakenews/lstmatt/S_ppl.tex <==
3.7

==> data_new/ra/fakenews/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.93	0.07	0.94	0.89	0.98	0.98	0.01	0.98	0.97	0.99	0.97	0.01	0.97	0.96	0.98	2.48	1.48	2.38	1.25	3.47	9.11	11.22	4.77	1.38	13.27	0.87	0.04	0.87	0.85	0.89	0.91	0.03	0.91	0.89	0.92	0.92	0.02	0.92	0.91	0.93	0.94	0.02	0.94	0.93	0.95	64.22	226.2	38.2	30.77	50.38	73.49	226.09	47.36	38.47	61.31	2095	0.02
0.03	0.89	0.07	0.9	0.84	0.94	0.96	0.03	0.96	0.95	0.97	0.95	0.01	0.95	0.94	0.96	3.33	1.47	3.31	2.28	4.25	12.09	12.61	7.77	2.75	17.83	0.82	0.03	0.82	0.8	0.83	0.86	0.03	0.87	0.85	0.88	0.88	0.02	0.88	0.87	0.89	0.91	0.01	0.91	0.9	0.92	51.31	63.68	38.28	31.32	50.07	73.73	78.35	58.59	47.64	73.54	2005	0.05
0.06	0.85	0.08	0.85	0.8	0.9	0.93	0.03	0.93	0.91	0.95	0.92	0.02	0.92	0.91	0.93	3.94	1.52	3.97	2.98	4.86	13.93	14.6	9.14	3.43	19.23	0.77	0.03	0.77	0.75	0.79	0.82	0.03	0.82	0.8	0.84	0.85	0.02	0.85	0.83	0.86	0.89	0.02	0.89	0.88	0.89	53.29	70.17	38.58	31.56	50.43	101.54	116.68	78.22	64.05	98.73	2010	0.1
0.11	0.81	0.08	0.82	0.77	0.87	0.9	0.05	0.9	0.88	0.93	0.89	0.02	0.89	0.88	0.91	4.4	1.51	4.45	3.56	5.26	15.69	15.4	11.04	4.31	22.13	0.73	0.03	0.73	0.71	0.75	0.79	0.04	0.79	0.77	0.81	0.82	0.03	0.82	0.8	0.83	0.86	0.02	0.86	0.86	0.88	51.88	62.91	38.39	31.54	50.29	132.39	156.13	103.73	85.91	130.11	1968	0.18
0.15	0.78	0.09	0.78	0.73	0.83	0.85	0.06	0.85	0.81	0.91	0.85	0.03	0.86	0.84	0.87	4.91	1.51	4.97	4.08	5.83	16.71	15.64	12.34	5.03	23.91	0.68	0.03	0.68	0.66	0.7	0.74	0.04	0.75	0.72	0.77	0.78	0.03	0.78	0.76	0.8	0.84	0.02	0.84	0.83	0.85	60.6	229.44	38.2	31.12	50.3	205.43	419.91	154.75	130.38	191.55	1450	0.27
0.18	0.74	0.09	0.74	0.69	0.8	0.8	0.08	0.8	0.75	0.87	0.81	0.03	0.82	0.79	0.83	5.28	1.53	5.38	4.54	6.23	20.08	17.88	15.25	6.1	29.75	0.63	0.04	0.63	0.61	0.65	0.7	0.05	0.71	0.68	0.74	0.75	0.03	0.75	0.73	0.77	0.81	0.02	0.81	0.8	0.82	53.31	71.2	38.25	31.0	50.52	284.37	302.83	230.3	190.26	279.77	1153	0.49
0.32	0.69	0.1	0.69	0.63	0.75	0.7	0.11	0.71	0.63	0.79	0.76	0.05	0.76	0.73	0.79	5.82	1.68	5.96	5.04	6.83	24.04	21.75	18.42	6.3	35.45	0.57	0.05	0.58	0.54	0.61	0.66	0.06	0.66	0.63	0.69	0.71	0.04	0.71	0.68	0.73	0.78	0.03	0.78	0.77	0.8	57.06	136.84	38.33	31.2	51.17	521.23	491.8	408.89	306.4	572.82	1709	0.92


==> data_new/ra/fakenews/roberta/A_auc.tex <==
0.25

==> data_new/ra/fakenews/roberta/A_ppl.tex <==
8.8

==> data_new/ra/fakenews/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.81	0.22	0.9	0.75	0.96	0.98	0.01	0.98	0.97	0.99	0.88	0.12	0.91	0.85	0.94	7.77	37.36	1.46	0.68	3.57	16.96	27.84	7.52	2.44	18.54	0.75	0.14	0.77	0.69	0.83	0.76	0.15	0.78	0.69	0.86	0.84	0.1	0.86	0.8	0.9	0.88	0.07	0.89	0.85	0.92	62.04	200.39	38.22	30.87	50.39	71.34	200.37	47.37	38.55	61.33	2089	0.02
0.03	0.76	0.21	0.83	0.7	0.91	0.96	0.03	0.96	0.95	0.97	0.83	0.12	0.85	0.8	0.89	14.6	57.42	2.25	1.14	5.86	18.58	25.89	10.36	3.76	22.07	0.68	0.12	0.7	0.63	0.75	0.69	0.14	0.71	0.63	0.77	0.79	0.09	0.81	0.76	0.84	0.85	0.07	0.86	0.82	0.88	51.34	63.67	38.28	31.32	50.1	73.66	75.95	58.44	47.67	73.64	2005	0.05
0.06	0.71	0.22	0.77	0.62	0.86	0.93	0.04	0.93	0.91	0.95	0.77	0.12	0.79	0.73	0.84	31.24	103.24	3.54	1.68	11.12	20.93	26.54	12.8	4.74	24.95	0.61	0.12	0.62	0.56	0.68	0.62	0.14	0.65	0.55	0.71	0.74	0.09	0.76	0.71	0.8	0.81	0.07	0.82	0.79	0.85	50.82	59.65	38.55	31.62	50.23	96.3	91.27	77.85	64.11	98.96	2027	0.11
0.11	0.7	0.2	0.73	0.57	0.86	0.78	0.15	0.81	0.76	0.88	0.73	0.13	0.72	0.65	0.83	3.98	5.3	2.24	1.47	3.78	1.88	3.67	0.62	0.27	1.91	0.59	0.12	0.59	0.51	0.68	0.52	0.35	0.55	0.33	0.67	0.68	0.13	0.67	0.61	0.75	0.79	0.08	0.81	0.74	0.85	283.56	228.73	225.96	118.31	384.58	637.68	435.5	534.85	328.56	923.02	22	0.15
0.32	0.62	0.2	0.67	0.52	0.77	0.7	0.11	0.71	0.63	0.79	0.61	0.11	0.62	0.56	0.67	216.65	296.81	26.49	4.67	418.5	23.69	26.0	16.43	5.87	31.43	0.45	0.09	0.46	0.41	0.5	0.5	0.13	0.51	0.43	0.58	0.62	0.08	0.63	0.58	0.67	0.73	0.05	0.74	0.71	0.77	56.79	131.17	38.8	31.34	51.3	514.84	474.66	408.92	305.36	577.28	1938	1.0


==> data_new/ra/fakenews/roberta/S_auc.tex <==
0.22

==> data_new/ra/fakenews/roberta/S_ppl.tex <==
8.1

==> data_new/ra/fakenews/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.93	0.06	0.94	0.91	0.96	0.98	0.02	0.98	0.97	0.99	0.95	0.03	0.96	0.94	0.97	1.3	0.55	1.28	1.0	1.58	3.64	3.87	2.48	0.99	5.07	0.87	0.05	0.87	0.85	0.9	0.87	0.05	0.88	0.85	0.9	0.91	0.03	0.92	0.9	0.93	0.94	0.02	0.94	0.93	0.95	75.59	383.48	39.94	32.36	52.49	86.05	383.25	49.91	40.47	64.66	4038	0.02
0.03	0.87	0.07	0.88	0.83	0.92	0.95	0.03	0.96	0.95	0.97	0.91	0.05	0.92	0.89	0.95	1.78	0.58	1.78	1.47	2.09	5.35	5.28	3.84	1.56	7.41	0.8	0.06	0.8	0.77	0.83	0.8	0.06	0.8	0.77	0.83	0.86	0.04	0.87	0.85	0.89	0.91	0.03	0.91	0.9	0.92	56.33	124.27	39.85	32.36	52.0	81.76	132.16	61.21	50.2	78.85	3787	0.07
0.06	0.8	0.09	0.81	0.75	0.87	0.92	0.04	0.92	0.91	0.94	0.86	0.06	0.86	0.82	0.91	2.24	0.66	2.25	1.91	2.6	6.94	6.41	5.28	2.16	9.8	0.72	0.07	0.72	0.68	0.77	0.71	0.07	0.72	0.67	0.77	0.81	0.05	0.81	0.78	0.84	0.87	0.03	0.87	0.85	0.89	56.74	97.65	39.73	32.35	52.54	110.91	156.5	82.53	67.16	105.18	2389	0.15
0.11	0.74	0.1	0.75	0.68	0.81	0.89	0.05	0.89	0.86	0.91	0.81	0.08	0.81	0.75	0.88	2.56	0.7	2.58	2.23	2.98	8.32	7.66	6.12	2.58	11.6	0.66	0.08	0.65	0.6	0.72	0.65	0.08	0.65	0.6	0.71	0.76	0.05	0.76	0.73	0.8	0.84	0.04	0.84	0.82	0.86	62.39	239.01	39.15	31.89	51.8	150.91	328.24	108.18	89.03	137.81	1772	0.23
0.15	0.65	0.12	0.65	0.58	0.74	0.83	0.06	0.83	0.8	0.87	0.73	0.1	0.72	0.65	0.82	3.0	0.77	3.02	2.62	3.48	10.27	9.06	7.72	3.39	14.45	0.57	0.1	0.56	0.5	0.65	0.57	0.09	0.56	0.5	0.64	0.7	0.06	0.7	0.66	0.74	0.8	0.04	0.8	0.77	0.83	52.16	62.57	39.26	31.81	52.27	198.7	204.1	162.52	132.84	201.66	1225	0.45
0.18	0.59	0.12	0.58	0.5	0.68	0.77	0.07	0.77	0.73	0.82	0.67	0.12	0.66	0.58	0.77	3.3	0.83	3.34	2.91	3.83	11.86	9.96	9.28	4.16	17.08	0.51	0.1	0.5	0.43	0.6	0.51	0.09	0.5	0.44	0.59	0.66	0.06	0.65	0.61	0.7	0.77	0.05	0.76	0.73	0.8	56.46	97.11	39.28	31.9	52.42	291.56	320.02	230.89	191.27	289.04	1304	0.67
0.32	0.51	0.13	0.5	0.4	0.59	0.68	0.11	0.68	0.61	0.75	0.59	0.14	0.57	0.48	0.71	3.66	0.95	3.76	3.18	4.27	13.63	11.35	10.88	4.69	19.82	0.44	0.12	0.42	0.35	0.53	0.44	0.1	0.43	0.37	0.52	0.6	0.07	0.59	0.55	0.65	0.72	0.05	0.72	0.68	0.76	65.16	249.02	39.8	32.13	52.99	460.49	444.39	362.86	283.53	487.07	1624	0.97


==> data_new/ra/fakenews/xlnet/A_auc.tex <==
0.21

==> data_new/ra/fakenews/xlnet/A_ppl.tex <==
6.3

==> data_new/ra/fakenews/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.67	0.35	0.81	0.49	0.94	0.98	0.02	0.98	0.97	0.99	0.64	0.29	0.73	0.5	0.86	0.41	1.99	0.04	0.02	0.11	4.33	6.2	2.44	0.94	5.35	0.53	0.26	0.58	0.38	0.72	0.61	0.21	0.64	0.47	0.76	0.68	0.17	0.71	0.57	0.8	0.77	0.13	0.79	0.69	0.86	75.55	383.98	39.94	32.36	52.49	85.99	383.75	50.02	40.58	64.66	4036	0.02
0.03	0.58	0.36	0.69	0.37	0.86	0.95	0.03	0.96	0.95	0.97	0.54	0.28	0.61	0.39	0.75	0.61	2.74	0.06	0.03	0.15	4.98	6.45	3.05	1.31	6.29	0.43	0.23	0.47	0.29	0.6	0.52	0.18	0.53	0.39	0.67	0.61	0.15	0.63	0.51	0.73	0.72	0.12	0.74	0.64	0.8	55.84	122.66	39.82	32.32	52.0	81.12	120.56	61.26	50.26	78.79	3730	0.07
0.06	0.49	0.36	0.57	0.25	0.78	0.92	0.04	0.92	0.9	0.94	0.45	0.27	0.51	0.3	0.65	0.94	3.87	0.07	0.03	0.21	5.55	6.37	3.77	1.67	7.25	0.34	0.21	0.38	0.22	0.5	0.45	0.17	0.47	0.33	0.58	0.55	0.14	0.57	0.46	0.65	0.67	0.11	0.7	0.61	0.75	57.19	99.36	39.79	32.35	52.85	113.09	155.63	83.13	67.62	106.22	2206	0.15
0.11	0.42	0.35	0.47	0.17	0.69	0.89	0.05	0.89	0.86	0.91	0.37	0.25	0.41	0.23	0.56	1.11	3.86	0.08	0.04	0.26	6.03	6.82	4.03	1.82	7.96	0.28	0.19	0.31	0.17	0.42	0.4	0.15	0.41	0.29	0.51	0.51	0.13	0.52	0.42	0.6	0.64	0.1	0.66	0.58	0.71	60.57	208.99	39.55	32.15	52.2	147.56	259.84	109.66	89.84	139.51	2393	0.21
0.15	0.32	0.33	0.34	0.11	0.56	0.83	0.06	0.83	0.8	0.87	0.28	0.24	0.31	0.15	0.45	2.03	6.17	0.1	0.05	0.41	6.49	6.19	4.81	2.08	9.1	0.2	0.18	0.23	0.11	0.33	0.35	0.14	0.35	0.25	0.44	0.46	0.12	0.47	0.39	0.54	0.6	0.09	0.62	0.55	0.67	51.85	61.1	39.35	31.98	52.16	194.99	162.06	162.41	134.62	201.44	1600	0.41
0.18	0.25	0.31	0.27	0.04	0.49	0.77	0.08	0.76	0.72	0.83	0.21	0.22	0.24	0.07	0.37	2.74	7.0	0.13	0.06	0.6	7.09	6.44	5.49	2.4	9.52	0.16	0.16	0.18	0.05	0.27	0.31	0.12	0.31	0.22	0.39	0.42	0.1	0.43	0.36	0.5	0.58	0.08	0.59	0.52	0.64	58.06	103.13	39.89	32.32	53.41	298.62	294.12	234.28	192.29	296.44	770	0.62
0.32	0.15	0.29	0.13	-0.03	0.35	0.67	0.11	0.68	0.59	0.74	0.14	0.2	0.15	0.0	0.28	4.98	11.9	0.2	0.08	3.38	7.71	6.81	5.7	2.87	10.51	0.1	0.14	0.11	0.0	0.2	0.27	0.11	0.25	0.18	0.33	0.38	0.1	0.39	0.31	0.45	0.55	0.08	0.55	0.5	0.6	61.49	210.93	40.02	32.32	52.62	475.56	519.18	378.42	294.51	508.45	1081	1.0


==> data_new/ra/fakenews/xlnet/IG_auc.tex <==
0.11

==> data_new/ra/fakenews/xlnet/IG_ppl.tex <==
6.7

==> data_new/ra/fakenews/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.82	0.24	0.93	0.73	0.98	0.98	0.02	0.98	0.97	0.99	0.84	0.15	0.89	0.78	0.94	21.36	160.29	1.94	0.84	5.33	20.01	27.71	9.11	2.84	24.95	0.71	0.17	0.75	0.61	0.84	0.72	0.21	0.78	0.61	0.88	0.79	0.13	0.82	0.71	0.89	0.85	0.09	0.87	0.8	0.92	75.74	383.54	39.94	32.35	52.5	86.17	383.3	50.01	40.58	64.69	4040	0.02
0.03	0.78	0.24	0.89	0.67	0.96	0.95	0.03	0.96	0.95	0.97	0.8	0.15	0.84	0.73	0.9	30.09	181.51	2.53	1.19	6.87	22.46	28.95	11.88	4.09	27.85	0.65	0.16	0.68	0.56	0.77	0.67	0.2	0.71	0.55	0.82	0.75	0.12	0.78	0.68	0.84	0.82	0.08	0.84	0.78	0.89	56.11	121.89	39.88	32.39	52.07	82.64	169.09	61.51	50.26	79.28	3982	0.08
0.06	0.76	0.24	0.85	0.63	0.94	0.92	0.04	0.92	0.9	0.94	0.76	0.14	0.8	0.69	0.86	54.89	386.34	3.19	1.48	8.47	23.4	28.5	13.18	4.92	29.75	0.61	0.14	0.63	0.52	0.71	0.64	0.19	0.67	0.53	0.78	0.72	0.11	0.74	0.65	0.8	0.8	0.07	0.81	0.76	0.86	58.09	106.62	39.82	32.45	52.51	114.91	182.18	82.54	67.96	106.14	2746	0.16
0.11	0.73	0.24	0.8	0.59	0.92	0.89	0.05	0.89	0.86	0.91	0.73	0.15	0.77	0.66	0.84	84.16	418.18	4.07	1.88	11.01	24.54	29.19	14.16	5.17	32.3	0.57	0.14	0.59	0.49	0.67	0.61	0.18	0.65	0.5	0.75	0.7	0.11	0.71	0.63	0.78	0.78	0.07	0.79	0.74	0.84	61.32	230.13	39.35	32.0	51.79	149.17	317.83	108.37	89.62	137.27	1914	0.24
0.15	0.71	0.23	0.78	0.57	0.89	0.83	0.06	0.83	0.8	0.87	0.71	0.14	0.73	0.64	0.8	160.54	586.6	5.15	2.32	16.69	24.9	29.68	14.72	5.67	32.52	0.54	0.12	0.56	0.47	0.63	0.59	0.18	0.63	0.49	0.73	0.68	0.1	0.69	0.62	0.75	0.77	0.07	0.78	0.73	0.82	52.66	63.11	39.38	31.88	52.28	202.02	212.96	161.84	133.0	203.33	1270	0.47
0.18	0.67	0.24	0.73	0.52	0.86	0.78	0.08	0.77	0.73	0.82	0.68	0.14	0.71	0.61	0.77	231.33	727.6	6.58	3.05	25.56	25.33	27.61	15.9	6.09	34.4	0.51	0.12	0.53	0.45	0.6	0.57	0.18	0.6	0.47	0.71	0.66	0.1	0.67	0.6	0.73	0.75	0.07	0.76	0.71	0.8	55.74	93.99	39.3	31.95	52.64	324.42	1493.61	230.32	189.29	289.07	1399	0.79
0.32	0.64	0.23	0.69	0.5	0.81	0.67	0.11	0.68	0.59	0.74	0.64	0.13	0.67	0.57	0.74	476.4	1200.8	9.11	3.86	78.54	26.39	28.19	17.12	6.78	35.55	0.48	0.11	0.5	0.42	0.56	0.54	0.17	0.57	0.44	0.67	0.64	0.1	0.66	0.59	0.71	0.74	0.06	0.74	0.7	0.78	66.9	271.4	40.11	32.38	53.01	473.36	385.72	380.54	290.98	513.01	1316	1.0


==> data_new/ra/fakenews/xlnet/S_auc.tex <==
0.23

==> data_new/ra/fakenews/xlnet/S_ppl.tex <==
6.1

==> data_new/ra/imdb/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.88	0.18	0.94	0.87	0.97	0.98	0.01	0.98	0.97	0.99	0.93	0.05	0.94	0.91	0.96	2.12	2.31	1.51	0.45	2.76	5.15	8.8	2.02	0.71	5.69	0.83	0.08	0.84	0.79	0.88	0.83	0.09	0.84	0.79	0.89	0.89	0.06	0.9	0.87	0.93	0.92	0.04	0.93	0.9	0.95	70.86	39.38	62.93	47.15	84.49	81.57	42.58	73.39	54.98	96.73	3548	0.03
0.03	0.78	0.23	0.87	0.72	0.93	0.95	0.02	0.96	0.94	0.97	0.87	0.07	0.89	0.85	0.92	3.0	2.83	2.3	0.76	4.09	7.43	11.42	3.21	1.15	8.88	0.74	0.09	0.76	0.7	0.8	0.75	0.1	0.76	0.7	0.81	0.83	0.07	0.85	0.8	0.88	0.88	0.05	0.89	0.86	0.92	70.55	36.72	62.95	47.14	84.5	94.93	45.44	84.98	65.4	114.33	3543	0.07
0.06	0.68	0.26	0.79	0.55	0.88	0.92	0.03	0.92	0.9	0.94	0.81	0.1	0.83	0.78	0.88	3.66	3.08	3.02	1.08	5.11	9.26	12.39	4.69	1.68	12.01	0.66	0.1	0.68	0.61	0.73	0.66	0.11	0.68	0.6	0.74	0.78	0.08	0.8	0.74	0.83	0.84	0.06	0.86	0.82	0.88	70.89	39.41	62.94	47.15	84.55	117.4	61.19	106.27	81.47	139.82	3548	0.14
0.11	0.6	0.27	0.68	0.41	0.83	0.88	0.03	0.88	0.86	0.9	0.76	0.11	0.78	0.71	0.84	4.22	3.3	3.61	1.49	6.07	10.84	13.68	5.77	2.11	14.01	0.6	0.11	0.62	0.55	0.68	0.6	0.12	0.61	0.53	0.68	0.74	0.08	0.75	0.7	0.8	0.82	0.06	0.83	0.79	0.86	70.77	38.21	62.94	47.15	84.5	144.05	66.41	130.12	101.93	171.25	3547	0.22
0.15	0.51	0.27	0.56	0.3	0.74	0.82	0.04	0.82	0.79	0.84	0.69	0.12	0.7	0.62	0.77	4.8	3.4	4.39	2.17	6.89	13.17	15.56	7.58	2.7	18.08	0.52	0.11	0.54	0.46	0.6	0.52	0.12	0.52	0.44	0.6	0.68	0.08	0.69	0.63	0.74	0.78	0.06	0.79	0.74	0.82	70.45	36.53	62.91	47.12	84.45	197.2	87.95	180.16	141.69	231.06	3540	0.38
0.18	0.43	0.26	0.44	0.21	0.65	0.75	0.05	0.75	0.72	0.79	0.63	0.12	0.64	0.56	0.71	5.23	3.38	4.94	2.65	7.45	14.17	15.7	8.88	3.26	19.38	0.47	0.11	0.48	0.41	0.55	0.46	0.11	0.47	0.39	0.54	0.64	0.08	0.65	0.6	0.7	0.75	0.06	0.76	0.71	0.79	70.71	38.07	62.94	47.13	84.49	260.66	112.95	239.43	191.84	302.93	3544	0.56
0.32	0.31	0.24	0.28	0.1	0.5	0.63	0.09	0.63	0.56	0.7	0.53	0.13	0.55	0.45	0.63	5.95	3.39	5.68	3.55	8.18	17.15	17.55	11.42	4.3	24.63	0.39	0.11	0.4	0.32	0.46	0.38	0.11	0.38	0.31	0.46	0.58	0.08	0.59	0.53	0.64	0.71	0.06	0.71	0.66	0.75	70.7	38.07	62.93	47.13	84.5	409.07	195.46	375.3	289.9	488.98	7089	1.0


==> data_new/ra/imdb/bert/A_auc.tex <==
0.17

==> data_new/ra/imdb/bert/A_ppl.tex <==
4.8

==> data_new/ra/imdb/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.86	0.19	0.93	0.84	0.97	0.98	0.01	0.98	0.97	0.99	0.84	0.17	0.89	0.81	0.94	4.27	6.96	1.09	0.04	5.95	6.52	9.22	3.78	1.51	7.97	0.72	0.17	0.76	0.66	0.83	0.77	0.16	0.8	0.69	0.88	0.81	0.12	0.84	0.76	0.88	0.86	0.09	0.88	0.83	0.91	70.86	39.37	62.93	47.15	84.49	81.57	42.57	73.39	54.98	96.73	3548	0.03
0.03	0.77	0.25	0.85	0.71	0.92	0.95	0.02	0.96	0.94	0.97	0.73	0.22	0.8	0.68	0.86	6.03	8.33	2.32	0.07	9.62	9.2	11.17	6.01	2.56	11.67	0.6	0.19	0.65	0.53	0.72	0.67	0.18	0.71	0.59	0.8	0.73	0.13	0.76	0.67	0.82	0.8	0.1	0.82	0.76	0.86	70.54	36.71	62.93	47.13	84.47	94.54	45.38	85.05	65.32	113.42	3543	0.07
0.06	0.67	0.27	0.76	0.58	0.86	0.92	0.03	0.92	0.9	0.94	0.63	0.23	0.7	0.55	0.78	7.94	9.84	4.03	0.1	13.09	11.29	12.43	7.56	3.55	14.79	0.5	0.19	0.55	0.42	0.63	0.59	0.18	0.63	0.5	0.72	0.66	0.13	0.7	0.6	0.76	0.75	0.1	0.77	0.7	0.81	70.89	39.41	62.94	47.15	84.55	117.4	61.19	106.27	81.47	139.82	3548	0.14
0.11	0.59	0.28	0.67	0.47	0.79	0.88	0.03	0.88	0.86	0.9	0.55	0.23	0.61	0.46	0.7	9.21	10.87	5.51	0.13	15.51	13.33	14.51	9.16	4.26	17.37	0.42	0.19	0.47	0.34	0.55	0.53	0.18	0.56	0.42	0.65	0.61	0.13	0.64	0.54	0.71	0.71	0.1	0.73	0.66	0.77	70.77	38.22	62.94	47.15	84.5	144.45	75.02	130.12	101.93	171.25	3547	0.22
0.15	0.48	0.28	0.55	0.34	0.69	0.82	0.05	0.82	0.79	0.84	0.44	0.23	0.5	0.34	0.6	11.12	11.48	8.78	0.23	18.48	14.7	14.94	10.22	4.78	19.52	0.33	0.18	0.38	0.24	0.46	0.46	0.17	0.48	0.35	0.58	0.55	0.13	0.58	0.48	0.64	0.67	0.09	0.69	0.62	0.73	70.46	36.54	62.91	47.13	84.48	197.07	85.73	181.23	142.15	232.56	3540	0.38
0.18	0.4	0.27	0.45	0.25	0.6	0.75	0.05	0.75	0.72	0.79	0.36	0.22	0.42	0.25	0.52	13.15	12.33	11.87	0.8	20.84	16.23	15.72	11.79	5.38	22.24	0.27	0.16	0.31	0.18	0.39	0.4	0.16	0.41	0.29	0.52	0.51	0.12	0.53	0.44	0.59	0.63	0.09	0.65	0.59	0.7	70.71	38.07	62.94	47.13	84.49	260.66	112.95	239.43	191.84	302.93	3544	0.56
0.32	0.28	0.24	0.3	0.13	0.45	0.63	0.09	0.63	0.56	0.7	0.26	0.18	0.29	0.15	0.39	15.82	12.64	15.01	4.53	23.59	17.93	16.81	13.15	6.22	24.54	0.19	0.14	0.21	0.11	0.29	0.32	0.14	0.32	0.23	0.43	0.46	0.1	0.47	0.39	0.53	0.6	0.07	0.61	0.55	0.65	70.71	38.08	62.94	47.14	84.5	408.89	183.37	376.77	288.1	489.43	7090	1.0


==> data_new/ra/imdb/bert/IG_auc.tex <==
0.16

==> data_new/ra/imdb/bert/IG_ppl.tex <==
4.8

==> data_new/ra/imdb/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.79	0.17	0.83	0.69	0.92	0.98	0.01	0.98	0.97	0.99	0.83	0.11	0.85	0.77	0.91	39.44	120.02	0.43	0.21	2.04	4.01	4.05	2.73	1.12	5.63	0.67	0.12	0.68	0.59	0.75	0.65	0.18	0.67	0.53	0.78	0.76	0.1	0.77	0.7	0.83	0.84	0.06	0.84	0.8	0.88	70.86	39.38	62.93	47.15	84.49	81.57	42.58	73.39	54.98	96.73	3548	0.03
0.03	0.69	0.19	0.72	0.57	0.84	0.95	0.02	0.96	0.94	0.97	0.75	0.12	0.77	0.68	0.84	50.84	143.37	0.56	0.29	3.96	5.01	4.67	3.68	1.62	6.89	0.58	0.12	0.58	0.5	0.66	0.54	0.18	0.56	0.43	0.68	0.69	0.1	0.7	0.63	0.76	0.79	0.06	0.8	0.75	0.84	70.55	36.72	62.95	47.14	84.5	94.93	45.44	84.98	65.4	114.33	3543	0.07
0.06	0.6	0.19	0.62	0.48	0.75	0.92	0.03	0.92	0.9	0.94	0.68	0.12	0.69	0.61	0.77	64.49	162.09	0.68	0.34	12.87	5.66	5.07	4.29	1.94	7.98	0.51	0.11	0.51	0.44	0.59	0.47	0.17	0.48	0.36	0.6	0.64	0.1	0.64	0.58	0.71	0.76	0.06	0.76	0.72	0.8	70.89	39.42	62.94	47.15	84.55	117.32	59.67	106.27	81.47	139.82	3548	0.14
0.11	0.54	0.19	0.56	0.41	0.68	0.88	0.04	0.88	0.86	0.9	0.63	0.13	0.64	0.56	0.72	77.02	181.71	0.8	0.4	32.38	6.26	5.69	4.67	2.19	8.61	0.46	0.11	0.47	0.4	0.54	0.42	0.16	0.43	0.32	0.53	0.61	0.09	0.61	0.55	0.67	0.73	0.06	0.74	0.7	0.77	70.78	38.24	62.96	47.15	84.52	144.02	73.62	131.4	101.29	171.44	3547	0.22
0.15	0.47	0.19	0.48	0.35	0.61	0.82	0.05	0.82	0.79	0.84	0.57	0.13	0.58	0.5	0.65	95.55	193.74	1.09	0.44	89.17	6.67	5.75	5.23	2.27	9.46	0.41	0.1	0.42	0.35	0.48	0.37	0.15	0.36	0.27	0.48	0.57	0.09	0.57	0.51	0.63	0.71	0.06	0.71	0.67	0.75	70.46	36.54	62.91	47.13	84.48	197.07	85.73	181.23	142.15	232.56	3540	0.38
0.18	0.41	0.18	0.42	0.29	0.54	0.75	0.05	0.75	0.72	0.79	0.52	0.12	0.52	0.44	0.6	113.58	215.09	1.45	0.5	153.06	6.97	5.99	5.48	2.36	9.94	0.37	0.1	0.37	0.31	0.43	0.33	0.14	0.32	0.24	0.42	0.53	0.08	0.54	0.48	0.59	0.69	0.06	0.69	0.65	0.72	70.71	38.07	62.94	47.13	84.49	260.66	112.95	239.43	191.84	302.93	3544	0.56
0.32	0.34	0.16	0.33	0.22	0.45	0.63	0.09	0.63	0.56	0.7	0.44	0.12	0.44	0.36	0.52	152.45	242.02	4.49	0.65	258.36	7.6	6.3	6.0	2.81	10.75	0.31	0.09	0.31	0.25	0.37	0.28	0.12	0.28	0.2	0.36	0.49	0.08	0.49	0.44	0.55	0.65	0.05	0.66	0.62	0.69	70.72	38.09	62.95	47.15	84.5	409.09	191.53	377.31	289.89	489.48	7090	1.0


==> data_new/ra/imdb/bert/S_auc.tex <==
0.16

==> data_new/ra/imdb/bert/S_ppl.tex <==
4.8

==> data_new/ra/imdb/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.93	0.09	0.96	0.92	0.98	0.98	0.01	0.98	0.97	0.99	0.92	0.08	0.94	0.9	0.96	2.5	1.91	2.0	1.15	3.4	2.58	3.59	1.48	0.59	3.17	0.86	0.11	0.89	0.84	0.92	0.87	0.1	0.89	0.84	0.94	0.91	0.07	0.93	0.89	0.95	0.92	0.06	0.94	0.91	0.96	75.11	38.42	68.16	52.4	88.73	84.13	40.1	77.13	59.73	99.41	3353	0.04
0.03	0.87	0.11	0.9	0.84	0.95	0.96	0.02	0.96	0.95	0.97	0.84	0.1	0.87	0.82	0.9	3.73	2.43	3.17	1.96	4.92	3.76	4.44	2.43	0.98	4.75	0.76	0.11	0.79	0.72	0.83	0.79	0.12	0.8	0.73	0.88	0.85	0.08	0.86	0.82	0.89	0.88	0.06	0.9	0.86	0.92	75.14	38.49	68.15	52.38	88.75	95.58	43.66	87.89	69.09	112.28	3351	0.08
0.06	0.8	0.13	0.83	0.74	0.89	0.92	0.03	0.92	0.91	0.94	0.76	0.11	0.78	0.72	0.83	5.01	2.96	4.35	2.86	6.65	4.84	5.15	3.38	1.51	6.36	0.65	0.11	0.67	0.6	0.72	0.71	0.12	0.72	0.64	0.8	0.78	0.08	0.79	0.74	0.83	0.83	0.06	0.84	0.8	0.87	75.34	39.51	68.24	52.46	88.83	114.15	51.85	105.54	83.69	133.41	3355	0.16
0.11	0.72	0.15	0.75	0.65	0.83	0.88	0.03	0.89	0.86	0.9	0.68	0.12	0.7	0.63	0.75	6.09	3.47	5.18	3.54	8.03	5.76	5.95	3.99	1.89	7.6	0.56	0.11	0.58	0.51	0.63	0.64	0.12	0.64	0.56	0.72	0.72	0.08	0.73	0.68	0.78	0.79	0.06	0.8	0.76	0.83	75.4	40.34	68.19	52.43	88.81	135.57	58.61	125.32	101.75	157.03	3352	0.25
0.15	0.62	0.16	0.64	0.53	0.74	0.82	0.04	0.82	0.8	0.85	0.57	0.12	0.58	0.51	0.64	7.54	4.19	6.45	4.42	10.01	6.42	6.16	4.67	2.2	8.74	0.45	0.1	0.46	0.4	0.51	0.55	0.13	0.56	0.47	0.64	0.65	0.08	0.66	0.61	0.7	0.73	0.06	0.74	0.7	0.77	74.61	35.23	68.13	52.34	88.65	175.32	63.42	164.65	135.72	202.53	3345	0.42
0.18	0.54	0.17	0.55	0.43	0.65	0.76	0.05	0.76	0.73	0.79	0.48	0.12	0.49	0.41	0.56	8.71	4.53	7.63	5.26	11.55	7.5	7.02	5.45	2.43	10.26	0.37	0.09	0.37	0.31	0.43	0.48	0.12	0.48	0.4	0.56	0.59	0.07	0.6	0.55	0.64	0.69	0.05	0.69	0.66	0.73	75.23	38.59	68.18	52.47	88.84	222.18	77.41	208.85	173.87	254.61	3358	0.61
0.32	0.42	0.18	0.42	0.3	0.53	0.65	0.07	0.65	0.59	0.7	0.35	0.12	0.36	0.27	0.44	10.76	5.73	9.12	6.42	14.29	8.57	7.64	6.62	3.05	11.82	0.26	0.1	0.26	0.2	0.33	0.4	0.13	0.4	0.32	0.48	0.52	0.07	0.52	0.47	0.57	0.64	0.06	0.64	0.6	0.67	75.92	38.91	68.92	53.02	89.69	320.5	121.87	300.84	242.52	371.32	6694	1.0


==> data_new/ra/imdb/cnn/IG_auc.tex <==
0.20

==> data_new/ra/imdb/cnn/IG_ppl.tex <==
3.2

==> data_new/ra/imdb/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.04	0.98	0.95	0.99	0.98	0.01	0.98	0.97	0.99	0.96	0.04	0.97	0.95	0.99	47.2	44.49	33.65	18.02	63.14	1.53	1.74	1.0	0.4	2.03	0.9	0.07	0.93	0.89	0.95	0.88	0.11	0.9	0.81	0.96	0.92	0.06	0.93	0.89	0.96	0.95	0.04	0.96	0.93	0.98	75.15	38.44	68.19	52.45	88.78	84.17	40.12	77.17	59.72	99.48	3353	0.04
0.03	0.93	0.05	0.95	0.91	0.97	0.96	0.02	0.96	0.95	0.97	0.93	0.05	0.94	0.91	0.96	68.69	50.96	54.48	32.0	93.83	2.1	2.1	1.53	0.64	2.83	0.83	0.08	0.85	0.8	0.89	0.8	0.13	0.81	0.73	0.9	0.87	0.07	0.88	0.83	0.92	0.91	0.05	0.92	0.89	0.95	75.17	38.51	68.19	52.42	88.81	95.63	43.69	88.02	69.12	112.31	3351	0.08
0.06	0.89	0.07	0.91	0.86	0.94	0.92	0.03	0.92	0.91	0.94	0.88	0.06	0.9	0.85	0.93	91.4	59.09	77.71	46.67	122.92	2.72	2.56	2.03	0.93	3.71	0.76	0.08	0.77	0.71	0.81	0.73	0.14	0.74	0.64	0.83	0.82	0.07	0.83	0.78	0.87	0.88	0.05	0.88	0.85	0.91	75.34	39.51	68.24	52.46	88.83	114.15	51.85	105.54	83.69	133.41	3355	0.16
0.11	0.85	0.08	0.87	0.82	0.91	0.88	0.03	0.89	0.86	0.9	0.84	0.07	0.85	0.8	0.89	112.64	68.85	97.05	61.09	148.87	3.17	2.88	2.41	1.06	4.4	0.7	0.08	0.7	0.65	0.75	0.67	0.15	0.68	0.57	0.76	0.78	0.08	0.78	0.73	0.83	0.85	0.05	0.85	0.81	0.88	75.4	40.35	68.19	52.43	88.81	135.57	58.62	125.32	101.75	157.03	3352	0.25
0.15	0.8	0.09	0.82	0.75	0.87	0.82	0.04	0.82	0.8	0.85	0.79	0.09	0.8	0.74	0.85	140.64	82.4	122.48	77.54	187.42	3.78	3.32	2.92	1.33	5.26	0.62	0.08	0.63	0.57	0.68	0.6	0.16	0.6	0.5	0.71	0.73	0.08	0.74	0.68	0.79	0.81	0.05	0.81	0.77	0.84	74.65	35.26	68.15	52.37	88.66	175.39	63.43	164.67	135.57	202.84	3345	0.42
0.18	0.76	0.1	0.77	0.7	0.83	0.76	0.05	0.76	0.73	0.79	0.74	0.1	0.75	0.69	0.81	167.02	93.4	146.74	94.34	223.02	4.15	3.62	3.2	1.42	5.86	0.57	0.09	0.57	0.51	0.63	0.55	0.17	0.56	0.44	0.67	0.69	0.08	0.7	0.64	0.75	0.78	0.06	0.78	0.75	0.82	75.23	38.58	68.18	52.47	88.84	222.18	77.39	208.85	173.87	254.61	3358	0.6
0.32	0.7	0.11	0.72	0.63	0.78	0.65	0.07	0.65	0.59	0.7	0.68	0.11	0.69	0.61	0.75	213.0	121.77	182.1	119.79	284.38	4.62	3.9	3.62	1.63	6.51	0.5	0.09	0.51	0.44	0.57	0.5	0.17	0.5	0.4	0.61	0.65	0.09	0.66	0.6	0.71	0.75	0.06	0.75	0.71	0.79	75.1	38.39	68.19	52.37	88.78	319.23	122.03	299.25	240.71	370.79	6694	1.0


==> data_new/ra/imdb/cnn/S_auc.tex <==
0.26

==> data_new/ra/imdb/cnn/S_ppl.tex <==
3.3

==> data_new/ra/imdb/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.97	0.06	0.99	0.96	0.99	0.98	0.01	0.98	0.97	0.99	0.96	0.03	0.97	0.95	0.98	0.42	0.34	0.33	0.2	0.53	2.85	3.61	1.63	0.61	3.62	0.91	0.04	0.91	0.89	0.94	0.92	0.07	0.93	0.88	0.96	0.94	0.04	0.94	0.92	0.96	0.95	0.02	0.96	0.94	0.97	76.21	44.54	68.63	53.06	89.3	85.38	46.1	77.24	60.62	99.01	3584	0.04
0.03	0.93	0.08	0.96	0.91	0.98	0.96	0.02	0.96	0.95	0.97	0.92	0.04	0.92	0.9	0.95	0.67	0.42	0.57	0.39	0.83	4.36	4.93	2.75	1.17	5.82	0.84	0.05	0.84	0.8	0.87	0.87	0.08	0.88	0.82	0.92	0.89	0.04	0.89	0.87	0.92	0.92	0.03	0.92	0.9	0.94	75.68	38.9	68.56	53.0	89.3	96.21	44.27	88.22	70.27	112.36	3580	0.08
0.06	0.88	0.11	0.91	0.84	0.95	0.92	0.03	0.92	0.91	0.94	0.86	0.06	0.87	0.83	0.9	0.9	0.45	0.81	0.58	1.12	5.8	5.75	4.08	1.69	8.1	0.75	0.06	0.76	0.72	0.8	0.8	0.1	0.8	0.75	0.87	0.85	0.05	0.85	0.82	0.88	0.88	0.03	0.88	0.86	0.91	76.49	45.81	68.64	53.07	89.41	116.08	64.38	105.65	84.92	133.2	3587	0.16
0.11	0.82	0.13	0.86	0.77	0.91	0.88	0.03	0.89	0.87	0.9	0.81	0.07	0.81	0.77	0.85	1.12	0.5	1.04	0.77	1.37	7.09	6.69	5.3	2.24	9.73	0.68	0.07	0.69	0.64	0.73	0.75	0.1	0.75	0.68	0.81	0.8	0.05	0.8	0.76	0.84	0.85	0.04	0.85	0.83	0.88	75.93	40.62	68.6	53.06	89.29	137.08	61.34	126.11	102.78	157.79	3581	0.25
0.15	0.74	0.15	0.77	0.66	0.85	0.82	0.04	0.82	0.8	0.85	0.72	0.08	0.73	0.68	0.77	1.38	0.53	1.3	1.02	1.67	8.87	8.08	6.52	2.87	12.7	0.59	0.07	0.59	0.55	0.64	0.67	0.11	0.67	0.6	0.74	0.74	0.06	0.74	0.71	0.78	0.81	0.04	0.81	0.78	0.83	75.35	38.59	68.55	53.0	89.09	176.85	68.21	165.62	135.84	201.69	3574	0.42
0.18	0.65	0.18	0.69	0.55	0.78	0.76	0.05	0.76	0.73	0.79	0.64	0.09	0.65	0.59	0.7	1.61	0.57	1.52	1.22	1.93	10.4	9.23	7.92	3.58	14.64	0.51	0.07	0.51	0.46	0.56	0.6	0.12	0.6	0.52	0.68	0.69	0.06	0.69	0.65	0.73	0.77	0.04	0.77	0.74	0.8	76.25	44.61	68.57	53.01	89.33	225.5	101.38	209.82	175.41	254.77	3589	0.6
0.32	0.52	0.2	0.53	0.38	0.67	0.65	0.07	0.65	0.59	0.7	0.52	0.11	0.52	0.44	0.59	1.94	0.64	1.85	1.49	2.3	12.5	11.1	9.45	4.29	17.42	0.4	0.09	0.4	0.34	0.46	0.49	0.13	0.5	0.4	0.57	0.61	0.07	0.61	0.57	0.66	0.71	0.05	0.71	0.68	0.75	75.77	40.32	68.6	53.06	89.25	321.37	127.54	299.54	241.73	373.8	7153	1.0


==> data_new/ra/imdb/lstm/IG_auc.tex <==
0.23

==> data_new/ra/imdb/lstm/IG_ppl.tex <==
3.2

==> data_new/ra/imdb/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.05	0.97	0.95	0.99	0.98	0.01	0.98	0.97	0.99	0.96	0.03	0.97	0.95	0.98	15.9	12.25	13.02	7.9	20.18	2.14	2.53	1.32	0.48	2.89	0.9	0.05	0.91	0.88	0.93	0.9	0.08	0.92	0.85	0.95	0.93	0.04	0.93	0.91	0.96	0.95	0.03	0.95	0.94	0.97	76.21	44.56	68.63	53.06	89.3	85.38	46.12	77.24	60.62	99.01	3584	0.04
0.03	0.91	0.07	0.93	0.89	0.96	0.96	0.02	0.96	0.95	0.97	0.92	0.04	0.93	0.9	0.95	24.1	13.97	20.99	14.5	30.4	3.2	3.16	2.25	0.98	4.36	0.82	0.06	0.83	0.79	0.86	0.82	0.1	0.84	0.76	0.88	0.88	0.05	0.89	0.86	0.92	0.92	0.03	0.92	0.9	0.94	75.72	38.92	68.6	53.05	89.3	96.26	44.29	88.28	70.27	112.42	3580	0.08
0.06	0.85	0.09	0.87	0.81	0.92	0.92	0.03	0.92	0.91	0.94	0.87	0.05	0.88	0.84	0.91	32.64	17.16	29.21	20.91	40.05	4.33	4.11	3.17	1.38	5.86	0.74	0.07	0.74	0.7	0.78	0.74	0.11	0.75	0.68	0.82	0.83	0.06	0.83	0.79	0.87	0.88	0.04	0.88	0.86	0.9	76.49	45.81	68.64	53.07	89.41	116.08	64.38	105.65	84.92	133.2	3587	0.16
0.11	0.8	0.11	0.82	0.74	0.88	0.88	0.03	0.89	0.87	0.9	0.82	0.06	0.83	0.79	0.87	39.82	18.72	36.66	26.96	48.49	5.34	4.9	4.03	1.84	7.37	0.67	0.07	0.68	0.63	0.72	0.68	0.11	0.68	0.6	0.76	0.78	0.06	0.79	0.75	0.82	0.84	0.04	0.85	0.82	0.87	75.93	40.63	68.6	53.06	89.29	137.08	61.35	126.11	102.78	157.79	3581	0.25
0.15	0.71	0.12	0.72	0.64	0.8	0.82	0.04	0.82	0.8	0.85	0.75	0.07	0.76	0.71	0.8	48.78	20.18	45.32	34.51	59.31	6.35	5.5	4.87	2.14	9.02	0.59	0.07	0.59	0.54	0.63	0.59	0.12	0.6	0.52	0.67	0.72	0.06	0.72	0.68	0.76	0.8	0.04	0.8	0.78	0.83	75.38	38.64	68.57	53.03	89.12	176.96	68.28	165.72	135.96	202.08	3574	0.42
0.18	0.64	0.14	0.65	0.55	0.74	0.76	0.05	0.76	0.73	0.79	0.69	0.09	0.7	0.64	0.75	55.43	21.61	51.79	39.54	66.82	7.12	6.06	5.6	2.48	10.12	0.52	0.08	0.52	0.48	0.57	0.52	0.13	0.52	0.44	0.6	0.67	0.07	0.67	0.63	0.72	0.77	0.05	0.77	0.74	0.8	76.28	44.63	68.6	53.06	89.4	225.71	101.55	209.81	175.54	254.97	3589	0.6
0.32	0.54	0.15	0.54	0.44	0.64	0.65	0.07	0.65	0.59	0.7	0.6	0.1	0.6	0.53	0.67	66.26	25.09	62.72	48.37	80.17	8.24	7.02	6.44	2.91	11.77	0.44	0.08	0.44	0.38	0.49	0.43	0.13	0.43	0.33	0.5	0.61	0.08	0.61	0.56	0.66	0.73	0.05	0.73	0.69	0.76	75.74	40.29	68.57	53.01	89.29	321.5	136.0	300.89	241.63	374.71	7153	1.0


==> data_new/ra/imdb/lstm/S_auc.tex <==
0.23

==> data_new/ra/imdb/lstm/S_ppl.tex <==
3.2

==> data_new/ra/imdb/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.05	0.98	0.95	0.99	0.98	0.01	0.98	0.97	0.99	0.97	0.02	0.98	0.96	0.99	0.04	0.03	0.03	0.02	0.05	4.07	4.74	2.48	0.94	5.44	0.9	0.05	0.91	0.88	0.93	0.89	0.08	0.91	0.84	0.96	0.93	0.04	0.93	0.91	0.96	0.95	0.03	0.95	0.93	0.97	75.08	36.27	68.32	52.82	89.01	84.27	38.3	77.05	60.22	99.12	3563	0.04
0.03	0.92	0.08	0.94	0.9	0.97	0.96	0.02	0.96	0.95	0.97	0.94	0.04	0.95	0.93	0.97	0.06	0.04	0.05	0.04	0.07	6.16	6.47	4.13	1.72	8.44	0.83	0.06	0.84	0.8	0.87	0.82	0.1	0.84	0.76	0.89	0.88	0.05	0.89	0.86	0.92	0.92	0.04	0.92	0.9	0.94	75.1	36.34	68.32	52.81	89.04	95.8	41.61	88.26	69.61	111.73	3561	0.08
0.06	0.86	0.11	0.89	0.82	0.94	0.92	0.03	0.92	0.91	0.94	0.9	0.05	0.91	0.87	0.94	0.08	0.04	0.07	0.05	0.1	8.32	8.27	5.9	2.53	11.24	0.76	0.07	0.77	0.72	0.81	0.75	0.12	0.76	0.68	0.84	0.84	0.06	0.84	0.8	0.88	0.88	0.04	0.89	0.86	0.91	75.36	37.83	68.36	52.83	89.09	114.75	50.29	105.75	84.92	132.85	3566	0.16
0.11	0.81	0.13	0.84	0.75	0.9	0.88	0.03	0.89	0.86	0.91	0.86	0.07	0.87	0.82	0.91	0.1	0.04	0.09	0.07	0.12	10.04	9.52	7.31	3.28	13.97	0.7	0.08	0.71	0.65	0.75	0.7	0.13	0.71	0.62	0.79	0.8	0.07	0.8	0.75	0.84	0.85	0.05	0.86	0.83	0.89	75.13	36.52	68.32	52.81	89.03	136.22	56.35	126.49	102.4	157.47	3561	0.25
0.15	0.72	0.16	0.75	0.64	0.84	0.82	0.04	0.82	0.8	0.85	0.79	0.09	0.81	0.75	0.85	0.12	0.05	0.11	0.09	0.14	12.31	11.25	9.24	4.2	17.04	0.62	0.09	0.63	0.57	0.68	0.61	0.14	0.62	0.53	0.71	0.74	0.08	0.74	0.69	0.79	0.81	0.05	0.82	0.78	0.85	74.69	34.36	68.3	52.77	88.97	175.36	62.92	164.43	136.07	202.52	3555	0.41
0.18	0.65	0.17	0.67	0.55	0.78	0.76	0.05	0.76	0.73	0.79	0.73	0.1	0.74	0.67	0.8	0.14	0.05	0.13	0.1	0.16	13.98	12.72	10.48	4.61	19.63	0.56	0.09	0.56	0.5	0.62	0.55	0.15	0.56	0.45	0.64	0.69	0.08	0.7	0.64	0.75	0.78	0.06	0.79	0.75	0.82	75.19	36.43	68.35	52.8	89.08	223.3	79.39	209.14	174.59	254.41	3568	0.61
0.32	0.53	0.2	0.54	0.39	0.67	0.65	0.07	0.65	0.59	0.7	0.63	0.13	0.64	0.55	0.72	0.16	0.06	0.15	0.12	0.19	16.4	14.7	12.37	5.49	23.12	0.46	0.11	0.47	0.4	0.54	0.45	0.15	0.45	0.36	0.56	0.63	0.09	0.63	0.57	0.68	0.74	0.06	0.74	0.7	0.78	75.05	36.23	68.34	52.81	89.03	319.16	114.82	299.43	241.75	372.8	7114	1.0


==> data_new/ra/imdb/lstmatt/A_auc.tex <==
0.23

==> data_new/ra/imdb/lstmatt/A_ppl.tex <==
3.3

==> data_new/ra/imdb/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.94	0.1	0.97	0.93	0.99	0.98	0.01	0.98	0.97	0.99	0.93	0.07	0.95	0.91	0.97	1.07	2.49	0.59	0.31	1.14	4.38	6.0	2.44	0.94	5.45	0.84	0.09	0.86	0.81	0.9	0.86	0.11	0.88	0.8	0.93	0.89	0.06	0.91	0.87	0.93	0.92	0.04	0.93	0.9	0.95	75.08	36.27	68.32	52.82	89.01	84.27	38.3	77.05	60.22	99.12	3563	0.04
0.03	0.88	0.12	0.92	0.85	0.96	0.96	0.02	0.96	0.95	0.97	0.86	0.09	0.88	0.83	0.92	1.61	3.47	1.0	0.56	1.77	6.5	7.4	4.22	1.77	8.61	0.74	0.1	0.76	0.7	0.81	0.78	0.12	0.8	0.72	0.87	0.83	0.07	0.84	0.79	0.88	0.88	0.05	0.88	0.85	0.91	75.1	36.34	68.32	52.81	89.04	95.8	41.61	88.26	69.61	111.73	3561	0.08
0.06	0.81	0.15	0.85	0.75	0.91	0.92	0.03	0.92	0.91	0.94	0.78	0.1	0.8	0.73	0.85	2.13	3.87	1.46	0.82	2.43	8.71	9.12	6.03	2.61	11.41	0.64	0.1	0.66	0.59	0.71	0.7	0.13	0.72	0.62	0.8	0.77	0.08	0.78	0.72	0.82	0.83	0.05	0.84	0.8	0.87	75.36	37.83	68.36	52.83	89.09	114.75	50.29	105.75	84.92	132.85	3566	0.16
0.11	0.74	0.17	0.78	0.66	0.86	0.88	0.03	0.89	0.86	0.91	0.71	0.11	0.72	0.65	0.78	2.6	8.27	1.84	1.04	2.91	9.88	9.75	7.1	3.16	13.36	0.57	0.1	0.58	0.52	0.64	0.64	0.13	0.64	0.56	0.72	0.72	0.08	0.72	0.67	0.78	0.79	0.05	0.8	0.76	0.83	75.13	36.52	68.32	52.81	89.03	136.22	56.35	126.49	102.4	157.47	3561	0.25
0.15	0.64	0.19	0.67	0.54	0.78	0.82	0.04	0.82	0.8	0.85	0.61	0.12	0.62	0.55	0.69	3.1	9.61	2.32	1.36	3.48	11.88	11.51	8.46	3.76	16.38	0.48	0.1	0.48	0.42	0.55	0.56	0.14	0.56	0.48	0.64	0.66	0.08	0.66	0.61	0.71	0.75	0.06	0.75	0.71	0.79	74.69	34.36	68.3	52.77	88.97	175.36	62.92	164.43	136.07	202.52	3555	0.41
0.18	0.56	0.19	0.58	0.44	0.7	0.76	0.05	0.76	0.73	0.79	0.52	0.12	0.53	0.45	0.6	3.34	4.25	2.71	1.61	3.96	13.09	12.32	9.38	4.27	18.28	0.4	0.1	0.41	0.34	0.47	0.5	0.14	0.5	0.4	0.58	0.61	0.08	0.61	0.56	0.66	0.71	0.05	0.72	0.68	0.75	75.16	36.41	68.32	52.81	89.08	223.16	79.3	208.98	174.47	254.36	3568	0.61
0.32	0.42	0.21	0.43	0.29	0.57	0.65	0.07	0.65	0.59	0.7	0.4	0.13	0.4	0.32	0.49	3.7	3.72	3.27	2.1	4.48	14.79	13.37	10.89	4.88	20.85	0.3	0.1	0.3	0.23	0.36	0.41	0.14	0.4	0.32	0.5	0.54	0.08	0.54	0.48	0.59	0.66	0.06	0.66	0.62	0.7	75.03	36.22	68.32	52.81	89.0	319.09	114.82	299.33	241.86	372.73	7114	1.0


==> data_new/ra/imdb/lstmatt/IG_auc.tex <==
0.21

==> data_new/ra/imdb/lstmatt/IG_ppl.tex <==
3.3

==> data_new/ra/imdb/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.97	0.04	0.98	0.96	0.99	0.98	0.01	0.98	0.97	0.99	0.95	0.04	0.96	0.94	0.98	25.87	28.76	16.33	8.83	31.96	3.89	4.42	2.51	1.0	5.22	0.85	0.07	0.86	0.82	0.9	0.86	0.1	0.88	0.8	0.93	0.9	0.06	0.91	0.87	0.94	0.93	0.04	0.93	0.91	0.96	75.08	36.27	68.32	52.82	89.01	84.27	38.3	77.05	60.22	99.12	3563	0.04
0.03	0.94	0.07	0.96	0.92	0.98	0.96	0.02	0.96	0.95	0.97	0.91	0.06	0.92	0.89	0.95	40.12	38.78	28.13	16.04	50.46	5.89	5.88	4.07	1.78	8.17	0.77	0.08	0.78	0.73	0.83	0.78	0.12	0.8	0.71	0.87	0.84	0.07	0.85	0.8	0.89	0.89	0.05	0.89	0.86	0.92	75.1	36.34	68.32	52.81	89.04	95.8	41.61	88.26	69.61	111.73	3561	0.08
0.06	0.89	0.09	0.92	0.86	0.95	0.92	0.03	0.92	0.91	0.94	0.86	0.08	0.87	0.82	0.91	54.16	47.01	38.71	22.53	70.3	7.82	7.25	5.64	2.52	11.07	0.69	0.09	0.7	0.64	0.76	0.7	0.13	0.72	0.62	0.8	0.79	0.08	0.79	0.74	0.84	0.85	0.05	0.85	0.82	0.88	75.4	37.85	68.39	52.86	89.08	114.81	50.32	105.82	84.94	132.92	3566	0.16
0.11	0.86	0.1	0.88	0.82	0.93	0.88	0.03	0.89	0.86	0.91	0.81	0.09	0.82	0.76	0.87	65.08	51.73	50.1	27.93	85.43	9.06	8.25	6.74	3.07	12.62	0.63	0.09	0.64	0.58	0.7	0.65	0.13	0.67	0.56	0.75	0.75	0.08	0.75	0.7	0.8	0.82	0.06	0.82	0.78	0.86	75.13	36.52	68.32	52.81	89.03	136.22	56.35	126.49	102.4	157.47	3561	0.25
0.15	0.81	0.12	0.83	0.75	0.89	0.82	0.04	0.82	0.8	0.85	0.74	0.11	0.76	0.68	0.82	79.27	57.01	64.44	35.37	105.87	11.21	9.79	8.5	3.82	15.93	0.57	0.1	0.58	0.51	0.64	0.58	0.14	0.59	0.5	0.68	0.7	0.09	0.7	0.64	0.75	0.78	0.06	0.79	0.74	0.82	74.69	34.36	68.3	52.77	88.97	175.36	62.92	164.43	136.07	202.52	3555	0.41
0.18	0.77	0.13	0.79	0.7	0.86	0.76	0.05	0.76	0.73	0.79	0.69	0.13	0.71	0.62	0.78	90.78	59.67	78.67	42.87	121.7	12.58	10.77	9.95	4.5	17.47	0.51	0.11	0.52	0.45	0.59	0.53	0.14	0.53	0.44	0.62	0.66	0.09	0.67	0.6	0.72	0.75	0.06	0.76	0.72	0.8	75.16	36.41	68.32	52.81	89.08	223.16	79.3	208.98	174.47	254.36	3568	0.61
0.32	0.7	0.15	0.73	0.61	0.82	0.65	0.07	0.65	0.59	0.7	0.61	0.15	0.63	0.52	0.71	106.78	64.39	95.46	53.81	143.5	14.17	12.16	11.1	4.86	20.22	0.44	0.12	0.45	0.37	0.53	0.46	0.14	0.46	0.36	0.56	0.61	0.1	0.61	0.54	0.67	0.72	0.07	0.72	0.68	0.77	75.05	36.23	68.34	52.81	89.03	319.16	114.82	299.43	241.75	372.8	7114	1.0


==> data_new/ra/imdb/lstmatt/S_auc.tex <==
0.26

==> data_new/ra/imdb/lstmatt/S_ppl.tex <==
3.3

==> data_new/ra/imdb/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.95	0.06	0.97	0.95	0.98	0.98	0.01	0.98	0.97	0.99	0.97	0.01	0.97	0.96	0.98	1.87	1.11	1.72	1.23	2.23	3.91	6.68	2.3	0.92	4.53	0.87	0.04	0.87	0.84	0.89	0.87	0.04	0.87	0.84	0.9	0.91	0.03	0.91	0.9	0.93	0.94	0.02	0.94	0.93	0.95	60.62	30.12	55.14	42.62	71.37	71.06	33.09	65.24	50.3	84.37	3748	0.02
0.03	0.92	0.07	0.94	0.9	0.96	0.95	0.02	0.96	0.94	0.97	0.94	0.02	0.94	0.93	0.96	2.6	1.22	2.43	1.86	3.04	5.41	7.86	3.39	1.45	6.43	0.81	0.04	0.81	0.78	0.83	0.81	0.04	0.81	0.78	0.84	0.87	0.03	0.87	0.85	0.89	0.91	0.02	0.91	0.89	0.92	60.61	30.12	55.14	42.61	71.35	84.54	39.79	77.44	60.39	99.14	3745	0.06
0.06	0.87	0.09	0.9	0.84	0.94	0.92	0.03	0.92	0.9	0.94	0.91	0.03	0.91	0.89	0.93	3.28	1.32	3.11	2.46	3.84	7.36	9.51	4.83	2.1	8.96	0.75	0.04	0.75	0.72	0.77	0.75	0.05	0.75	0.72	0.78	0.83	0.03	0.83	0.81	0.85	0.88	0.02	0.88	0.87	0.89	60.73	30.68	55.14	42.63	71.42	107.8	49.54	99.11	77.59	126.46	3749	0.11
0.11	0.83	0.11	0.87	0.78	0.91	0.88	0.04	0.88	0.85	0.9	0.88	0.03	0.88	0.86	0.9	3.8	1.41	3.67	2.89	4.48	8.55	10.47	5.62	2.5	10.47	0.7	0.04	0.71	0.68	0.73	0.71	0.05	0.71	0.68	0.74	0.8	0.03	0.8	0.78	0.82	0.86	0.02	0.86	0.84	0.87	60.53	29.62	55.14	42.62	71.35	136.15	56.65	125.4	98.97	159.97	3746	0.18
0.15	0.78	0.12	0.81	0.7	0.88	0.81	0.05	0.81	0.78	0.85	0.83	0.04	0.83	0.8	0.86	4.46	1.5	4.35	3.44	5.25	10.75	11.95	7.39	3.35	13.83	0.64	0.04	0.65	0.62	0.68	0.65	0.05	0.66	0.62	0.69	0.76	0.03	0.76	0.74	0.78	0.83	0.02	0.83	0.81	0.84	60.58	30.06	55.13	42.6	71.36	197.37	84.31	182.63	145.54	231.13	3743	0.32
0.18	0.75	0.13	0.77	0.65	0.85	0.75	0.06	0.75	0.71	0.79	0.78	0.05	0.78	0.75	0.81	4.93	1.52	4.9	3.91	5.81	12.78	13.12	9.09	3.84	17.22	0.6	0.05	0.6	0.56	0.63	0.61	0.06	0.61	0.58	0.64	0.72	0.04	0.72	0.7	0.75	0.8	0.03	0.8	0.78	0.82	60.62	30.13	55.15	42.61	71.39	276.49	112.94	257.59	204.39	325.32	3745	0.51
0.32	0.69	0.15	0.71	0.58	0.81	0.62	0.09	0.63	0.56	0.69	0.7	0.07	0.71	0.66	0.75	5.73	1.67	5.69	4.6	6.77	17.14	16.23	12.63	5.58	23.64	0.52	0.06	0.52	0.47	0.56	0.54	0.07	0.55	0.5	0.59	0.67	0.05	0.67	0.64	0.7	0.76	0.03	0.76	0.74	0.78	60.61	30.12	55.14	42.61	71.37	483.18	221.38	439.77	326.8	587.6	7492	1.0


==> data_new/ra/imdb/roberta/A_auc.tex <==
0.25

==> data_new/ra/imdb/roberta/A_ppl.tex <==
7.0

==> data_new/ra/imdb/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.92	0.19	0.98	0.94	0.99	0.98	0.01	0.98	0.97	0.99	0.93	0.15	0.97	0.93	0.98	2.14	7.15	0.37	0.24	0.83	4.99	9.7	2.19	0.92	4.94	0.85	0.16	0.91	0.83	0.94	0.85	0.15	0.89	0.81	0.94	0.9	0.11	0.93	0.88	0.96	0.93	0.08	0.95	0.91	0.97	60.61	30.11	55.11	42.63	71.35	71.05	33.08	65.24	50.29	84.35	3748	0.03
0.03	0.85	0.25	0.94	0.85	0.97	0.95	0.02	0.96	0.94	0.97	0.86	0.2	0.94	0.85	0.96	3.2	9.02	0.61	0.4	1.44	7.9	12.94	3.69	1.6	8.11	0.76	0.2	0.84	0.7	0.88	0.77	0.18	0.83	0.71	0.88	0.84	0.14	0.89	0.8	0.92	0.88	0.1	0.92	0.86	0.95	60.61	30.12	55.14	42.61	71.35	84.54	39.79	77.44	60.39	99.14	3745	0.06
0.06	0.78	0.26	0.89	0.72	0.94	0.92	0.03	0.92	0.9	0.94	0.79	0.22	0.89	0.75	0.92	4.01	9.71	0.84	0.58	2.15	10.42	14.46	5.22	2.28	12.02	0.68	0.21	0.77	0.59	0.83	0.69	0.2	0.76	0.6	0.84	0.78	0.15	0.84	0.72	0.88	0.85	0.11	0.89	0.8	0.92	60.73	30.68	55.14	42.63	71.42	107.8	49.54	99.11	77.59	126.46	3749	0.11
0.11	0.71	0.29	0.82	0.6	0.9	0.88	0.04	0.88	0.85	0.9	0.73	0.24	0.83	0.63	0.89	4.84	11.31	1.07	0.73	2.85	12.82	16.82	6.8	3.03	14.87	0.61	0.22	0.7	0.48	0.77	0.63	0.2	0.68	0.5	0.79	0.73	0.16	0.79	0.64	0.85	0.81	0.11	0.86	0.75	0.89	60.53	29.62	55.14	42.62	71.35	136.15	56.65	125.4	98.97	159.97	3746	0.18
0.15	0.61	0.3	0.71	0.42	0.83	0.81	0.05	0.81	0.78	0.85	0.63	0.25	0.75	0.46	0.82	5.64	10.6	1.45	0.94	4.51	16.5	19.47	9.41	4.0	20.79	0.51	0.22	0.6	0.33	0.69	0.54	0.21	0.59	0.38	0.7	0.67	0.16	0.72	0.55	0.79	0.76	0.12	0.8	0.68	0.86	60.57	30.05	55.1	42.6	71.35	197.33	84.3	182.52	145.51	231.27	3743	0.33
0.18	0.51	0.3	0.6	0.28	0.76	0.75	0.06	0.75	0.71	0.79	0.54	0.26	0.64	0.32	0.76	6.6	11.08	1.89	1.14	6.63	20.4	22.83	11.88	5.16	27.3	0.43	0.22	0.49	0.23	0.61	0.46	0.2	0.48	0.28	0.62	0.61	0.16	0.65	0.47	0.74	0.72	0.12	0.76	0.62	0.82	60.61	30.12	55.14	42.61	71.35	276.52	112.94	257.43	204.42	325.12	3745	0.52
0.32	0.37	0.28	0.36	0.14	0.6	0.63	0.09	0.63	0.56	0.69	0.4	0.25	0.41	0.18	0.62	8.77	13.74	3.16	1.58	11.52	27.62	27.02	18.29	7.47	40.32	0.3	0.2	0.29	0.12	0.47	0.35	0.19	0.33	0.2	0.5	0.52	0.15	0.51	0.39	0.65	0.66	0.11	0.66	0.56	0.75	60.34	29.82	54.96	42.56	71.21	472.55	214.89	430.06	320.96	576.33	7001	1.0


==> data_new/ra/imdb/roberta/IG_auc.tex <==
0.19

==> data_new/ra/imdb/roberta/IG_ppl.tex <==
6.8

==> data_new/ra/imdb/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.84	0.14	0.88	0.79	0.94	0.98	0.01	0.98	0.97	0.99	0.9	0.07	0.91	0.87	0.94	29.74	133.09	1.76	0.82	5.09	4.56	5.88	2.68	1.11	5.94	0.76	0.1	0.77	0.71	0.82	0.73	0.14	0.73	0.64	0.82	0.83	0.08	0.84	0.79	0.88	0.89	0.05	0.89	0.86	0.92	60.62	30.12	55.14	42.62	71.37	71.06	33.09	65.24	50.3	84.37	3748	0.02
0.03	0.74	0.16	0.77	0.65	0.85	0.95	0.02	0.96	0.94	0.97	0.83	0.09	0.84	0.79	0.89	43.59	169.99	2.88	1.39	8.57	6.22	6.99	4.06	1.65	8.29	0.66	0.1	0.67	0.61	0.73	0.61	0.14	0.62	0.52	0.71	0.76	0.08	0.77	0.71	0.82	0.84	0.05	0.84	0.81	0.88	60.61	30.12	55.14	42.61	71.35	84.54	39.79	77.44	60.39	99.14	3745	0.06
0.06	0.64	0.17	0.67	0.54	0.76	0.92	0.03	0.92	0.9	0.94	0.76	0.1	0.78	0.71	0.83	55.92	200.37	3.96	1.89	12.31	7.44	7.77	5.12	2.22	9.99	0.58	0.1	0.6	0.53	0.65	0.52	0.14	0.52	0.43	0.61	0.7	0.09	0.71	0.66	0.76	0.8	0.06	0.81	0.77	0.84	60.73	30.68	55.14	42.63	71.42	107.8	49.54	99.11	77.59	126.46	3749	0.11
0.11	0.57	0.18	0.59	0.46	0.7	0.88	0.04	0.88	0.85	0.9	0.7	0.11	0.72	0.64	0.78	71.06	248.05	5.2	2.45	17.35	8.22	7.89	6.0	2.5	11.54	0.53	0.1	0.54	0.47	0.6	0.45	0.14	0.45	0.36	0.56	0.66	0.09	0.67	0.61	0.72	0.78	0.06	0.78	0.74	0.82	60.53	29.62	55.14	42.62	71.35	136.15	56.65	125.4	98.97	159.97	3746	0.18
0.15	0.52	0.17	0.54	0.41	0.65	0.81	0.05	0.81	0.78	0.85	0.64	0.12	0.66	0.58	0.73	97.16	348.8	7.12	3.24	26.42	8.89	8.16	6.64	2.92	12.69	0.48	0.1	0.49	0.42	0.55	0.4	0.14	0.4	0.31	0.48	0.62	0.08	0.62	0.57	0.68	0.75	0.06	0.75	0.71	0.79	60.57	30.05	55.1	42.6	71.35	197.33	84.3	182.52	145.51	231.27	3743	0.32
0.18	0.49	0.17	0.5	0.38	0.6	0.75	0.06	0.75	0.71	0.79	0.6	0.12	0.61	0.53	0.68	128.06	355.5	9.86	4.26	42.96	9.79	8.96	7.27	3.21	13.88	0.44	0.1	0.44	0.38	0.51	0.37	0.14	0.36	0.28	0.46	0.59	0.09	0.59	0.53	0.64	0.73	0.06	0.73	0.69	0.77	60.61	30.12	55.14	42.61	71.35	276.52	112.94	257.43	204.42	325.12	3745	0.51
0.32	0.44	0.16	0.44	0.32	0.55	0.62	0.09	0.63	0.55	0.69	0.53	0.13	0.54	0.45	0.62	174.4	407.15	18.84	7.32	91.07	10.85	9.75	8.23	3.68	15.29	0.38	0.1	0.39	0.32	0.45	0.33	0.14	0.32	0.24	0.42	0.55	0.09	0.55	0.49	0.61	0.7	0.06	0.7	0.66	0.74	60.61	30.12	55.13	42.61	71.35	484.2	224.44	439.72	326.74	589.0	7492	1.0


==> data_new/ra/imdb/roberta/S_auc.tex <==
0.18

==> data_new/ra/imdb/roberta/S_ppl.tex <==
7.0

==> data_new/ra/imdb/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.02	0.97	0.96	0.98	0.98	0.02	0.98	0.97	0.99	0.97	0.02	0.97	0.96	0.98	0.86	0.27	0.85	0.68	1.02	1.3	1.28	0.94	0.41	1.78	0.88	0.04	0.88	0.86	0.9	0.88	0.04	0.88	0.86	0.91	0.92	0.03	0.92	0.9	0.93	0.94	0.02	0.94	0.93	0.95	61.29	30.49	55.71	43.07	72.4	72.51	33.62	66.42	51.37	85.71	3750	0.03
0.03	0.93	0.03	0.93	0.92	0.95	0.95	0.02	0.95	0.94	0.96	0.94	0.02	0.94	0.93	0.95	1.21	0.3	1.2	1.01	1.4	1.9	1.71	1.44	0.65	2.64	0.81	0.04	0.81	0.79	0.84	0.82	0.04	0.82	0.79	0.85	0.87	0.03	0.87	0.85	0.89	0.91	0.02	0.91	0.9	0.92	61.3	30.5	55.74	43.06	72.42	86.7	39.8	79.64	61.63	103.09	3747	0.07
0.06	0.88	0.04	0.89	0.86	0.91	0.91	0.03	0.91	0.89	0.93	0.89	0.03	0.9	0.88	0.92	1.55	0.34	1.55	1.33	1.77	2.55	2.24	1.95	0.88	3.59	0.74	0.05	0.74	0.71	0.77	0.75	0.05	0.75	0.72	0.78	0.82	0.03	0.82	0.8	0.84	0.87	0.02	0.88	0.86	0.89	61.56	32.69	55.74	43.07	72.45	110.09	51.67	101.45	79.41	129.64	3751	0.13
0.11	0.84	0.05	0.84	0.81	0.87	0.87	0.04	0.87	0.84	0.9	0.85	0.04	0.86	0.83	0.88	1.82	0.37	1.83	1.58	2.06	3.12	2.71	2.46	1.08	4.41	0.68	0.05	0.68	0.65	0.72	0.69	0.05	0.69	0.66	0.73	0.78	0.04	0.78	0.75	0.8	0.85	0.03	0.85	0.83	0.86	61.03	28.11	55.74	43.06	72.39	138.41	57.71	128.33	100.95	164.11	3747	0.21
0.15	0.77	0.06	0.78	0.74	0.81	0.8	0.05	0.8	0.77	0.84	0.79	0.05	0.79	0.75	0.82	2.16	0.42	2.18	1.89	2.44	3.8	3.23	2.94	1.39	5.41	0.6	0.06	0.61	0.57	0.64	0.62	0.06	0.62	0.58	0.66	0.72	0.04	0.72	0.69	0.75	0.81	0.03	0.81	0.79	0.83	61.27	30.5	55.7	43.05	72.37	196.21	81.51	182.57	143.8	233.17	3748	0.37
0.18	0.71	0.06	0.71	0.67	0.76	0.73	0.06	0.73	0.69	0.77	0.72	0.07	0.72	0.68	0.77	2.42	0.44	2.43	2.13	2.71	4.42	3.79	3.43	1.59	6.27	0.54	0.06	0.54	0.5	0.58	0.55	0.06	0.56	0.51	0.59	0.67	0.04	0.67	0.65	0.7	0.77	0.03	0.77	0.75	0.8	61.28	30.5	55.73	43.05	72.44	266.42	106.4	246.58	196.56	315.82	3752	0.56
0.32	0.61	0.08	0.62	0.55	0.67	0.61	0.09	0.61	0.54	0.67	0.61	0.09	0.62	0.55	0.68	2.76	0.51	2.77	2.42	3.11	5.25	4.45	4.13	1.8	7.51	0.44	0.08	0.44	0.39	0.5	0.47	0.07	0.47	0.42	0.52	0.6	0.05	0.6	0.57	0.64	0.72	0.04	0.72	0.7	0.75	61.32	30.49	55.76	43.07	72.41	426.45	194.93	389.21	295.59	513.86	7491	1.0


==> data_new/ra/imdb/xlnet/A_auc.tex <==
0.25

==> data_new/ra/imdb/xlnet/A_ppl.tex <==
6.0

==> data_new/ra/imdb/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.84	0.2	0.9	0.81	0.95	0.98	0.02	0.98	0.97	0.99	0.84	0.14	0.87	0.8	0.92	1.19	6.67	0.42	0.22	0.95	1.54	2.03	0.97	0.43	1.95	0.7	0.14	0.73	0.65	0.79	0.72	0.15	0.75	0.64	0.83	0.79	0.1	0.81	0.75	0.86	0.85	0.07	0.87	0.82	0.9	61.3	30.49	55.73	43.07	72.39	72.71	33.69	66.36	51.45	86.21	3751	0.03
0.03	0.73	0.21	0.78	0.65	0.86	0.95	0.02	0.95	0.94	0.96	0.72	0.16	0.75	0.66	0.82	1.51	5.16	0.64	0.34	1.38	2.14	2.62	1.44	0.62	2.75	0.57	0.14	0.59	0.51	0.66	0.61	0.15	0.62	0.52	0.71	0.7	0.1	0.72	0.65	0.77	0.79	0.07	0.8	0.75	0.84	61.3	30.5	55.74	43.06	72.42	86.7	39.8	79.64	61.63	103.09	3747	0.07
0.06	0.6	0.21	0.64	0.5	0.75	0.91	0.03	0.91	0.89	0.93	0.59	0.16	0.62	0.52	0.7	1.86	3.44	0.84	0.45	1.84	2.72	3.17	1.85	0.84	3.48	0.45	0.13	0.47	0.38	0.54	0.5	0.15	0.5	0.4	0.6	0.62	0.1	0.63	0.57	0.68	0.73	0.07	0.73	0.69	0.77	61.58	32.69	55.75	43.07	72.42	110.12	51.37	101.59	79.58	130.06	3752	0.13
0.11	0.5	0.22	0.52	0.37	0.64	0.87	0.04	0.87	0.84	0.9	0.49	0.16	0.51	0.4	0.59	2.26	5.21	1.03	0.55	2.32	3.07	3.3	2.17	0.98	4.0	0.36	0.13	0.37	0.29	0.44	0.42	0.14	0.43	0.32	0.52	0.56	0.09	0.57	0.5	0.62	0.68	0.07	0.69	0.65	0.73	61.04	28.11	55.75	43.06	72.39	138.26	56.76	128.08	101.36	165.3	3748	0.21
0.15	0.36	0.21	0.37	0.24	0.5	0.8	0.05	0.8	0.77	0.84	0.35	0.16	0.36	0.27	0.46	2.77	6.3	1.27	0.69	2.92	3.52	3.62	2.54	1.21	4.58	0.25	0.11	0.26	0.19	0.33	0.33	0.13	0.32	0.24	0.41	0.48	0.09	0.49	0.43	0.54	0.63	0.06	0.63	0.59	0.67	61.29	30.5	55.71	43.06	72.4	196.42	81.97	183.0	143.81	232.67	3746	0.37
0.18	0.26	0.19	0.26	0.14	0.38	0.73	0.06	0.73	0.69	0.77	0.25	0.14	0.26	0.17	0.35	3.14	4.33	1.59	0.82	3.59	3.93	3.93	2.84	1.32	5.26	0.18	0.1	0.18	0.12	0.25	0.27	0.12	0.28	0.2	0.35	0.43	0.08	0.43	0.38	0.48	0.59	0.06	0.59	0.55	0.63	61.27	30.5	55.73	43.04	72.39	266.66	106.26	248.42	196.33	313.86	3754	0.56
0.32	0.15	0.17	0.14	0.04	0.25	0.61	0.09	0.61	0.54	0.67	0.15	0.13	0.15	0.07	0.23	4.18	5.63	2.36	1.12	5.5	4.39	4.27	3.25	1.51	5.81	0.1	0.09	0.1	0.05	0.16	0.21	0.1	0.2	0.14	0.28	0.38	0.07	0.38	0.33	0.42	0.55	0.05	0.55	0.52	0.59	61.32	30.49	55.75	43.07	72.42	425.18	193.3	386.93	293.72	512.07	7491	1.0


==> data_new/ra/imdb/xlnet/IG_auc.tex <==
0.13

==> data_new/ra/imdb/xlnet/IG_ppl.tex <==
5.9

==> data_new/ra/imdb/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.94	0.11	0.97	0.93	0.99	0.98	0.02	0.98	0.97	0.99	0.96	0.06	0.97	0.96	0.98	95.65	745.49	25.75	12.75	61.71	2.8	4.12	1.61	0.61	3.35	0.87	0.08	0.88	0.85	0.91	0.85	0.12	0.88	0.8	0.92	0.91	0.07	0.92	0.88	0.95	0.93	0.04	0.94	0.92	0.96	61.3	30.49	55.73	43.07	72.39	72.71	33.69	66.36	51.45	86.21	3751	0.03
0.03	0.89	0.12	0.93	0.87	0.97	0.95	0.02	0.95	0.94	0.96	0.93	0.06	0.95	0.92	0.96	114.2	277.86	40.05	20.33	97.21	3.9	4.77	2.52	1.05	5.06	0.81	0.08	0.82	0.78	0.86	0.78	0.12	0.8	0.72	0.87	0.86	0.07	0.87	0.84	0.91	0.91	0.04	0.91	0.89	0.94	61.3	30.5	55.74	43.06	72.42	86.7	39.8	79.64	61.63	103.09	3747	0.07
0.06	0.84	0.14	0.87	0.79	0.93	0.91	0.03	0.91	0.89	0.93	0.9	0.07	0.91	0.88	0.94	159.35	404.86	57.18	29.47	137.25	4.86	5.1	3.34	1.47	6.56	0.75	0.09	0.76	0.71	0.8	0.71	0.14	0.72	0.64	0.8	0.82	0.07	0.83	0.79	0.87	0.88	0.05	0.88	0.86	0.91	61.56	32.69	55.74	43.07	72.45	110.09	51.67	101.45	79.41	129.64	3751	0.13
0.11	0.79	0.15	0.82	0.73	0.89	0.87	0.04	0.87	0.84	0.9	0.86	0.08	0.88	0.83	0.91	190.86	433.9	72.81	36.87	177.14	5.69	5.6	4.12	1.77	7.82	0.7	0.09	0.71	0.66	0.76	0.66	0.14	0.68	0.59	0.76	0.79	0.07	0.79	0.75	0.83	0.85	0.05	0.86	0.83	0.89	61.03	28.11	55.74	43.06	72.39	138.41	57.71	128.33	100.95	164.11	3747	0.21
0.15	0.72	0.15	0.74	0.64	0.83	0.8	0.05	0.8	0.77	0.84	0.81	0.09	0.83	0.77	0.87	240.11	429.49	93.9	47.42	236.19	6.53	6.01	5.02	2.25	9.2	0.64	0.09	0.65	0.59	0.7	0.59	0.14	0.6	0.5	0.68	0.74	0.08	0.75	0.7	0.79	0.82	0.05	0.83	0.8	0.86	61.27	30.5	55.7	43.05	72.37	196.24	81.55	182.23	143.8	233.76	3748	0.37
0.18	0.65	0.16	0.67	0.57	0.76	0.73	0.06	0.73	0.69	0.77	0.76	0.1	0.77	0.71	0.83	295.77	451.47	124.85	60.38	313.46	7.15	6.3	5.61	2.39	10.22	0.58	0.09	0.59	0.53	0.65	0.53	0.14	0.53	0.44	0.62	0.7	0.08	0.71	0.66	0.75	0.8	0.05	0.8	0.77	0.83	61.28	30.5	55.73	43.05	72.44	266.36	105.49	247.66	197.1	314.28	3752	0.57
0.32	0.56	0.17	0.58	0.46	0.68	0.61	0.09	0.61	0.55	0.67	0.67	0.12	0.69	0.6	0.76	416.71	566.1	198.24	87.88	516.6	8.22	7.38	6.21	2.7	11.63	0.5	0.11	0.51	0.44	0.57	0.45	0.14	0.45	0.36	0.56	0.64	0.09	0.64	0.59	0.7	0.76	0.06	0.76	0.72	0.8	61.2	30.31	55.76	43.07	72.3	422.66	204.62	383.99	292.46	508.11	7161	1.0


==> data_new/ra/imdb/xlnet/S_auc.tex <==
0.23

==> data_new/ra/imdb/xlnet/S_ppl.tex <==
5.9

==> data_new/ra/mr/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	293.44	483.55	166.34	86.91	307.77	293.44	483.55	166.34	86.91	307.77	2834	0.0
0.03	0.98	0.04	1.0	0.99	1.0	0.95	0.03	0.96	0.94	0.98	0.92	0.09	0.95	0.9	0.98	0.36	0.46	0.22	0.08	0.45	0.5	1.09	0.17	0.05	0.49	0.81	0.11	0.84	0.77	0.89	0.92	0.09	0.95	0.89	0.98	0.88	0.08	0.9	0.84	0.94	0.9	0.06	0.91	0.88	0.94	179.84	170.38	129.9	74.52	218.0	238.28	209.51	177.12	104.02	290.47	1270	0.06
0.06	0.97	0.06	0.99	0.97	1.0	0.91	0.06	0.92	0.88	0.95	0.88	0.11	0.92	0.84	0.96	0.44	0.5	0.27	0.09	0.58	0.59	1.15	0.2	0.04	0.61	0.75	0.13	0.78	0.69	0.85	0.89	0.11	0.93	0.84	0.97	0.85	0.09	0.87	0.8	0.92	0.87	0.07	0.88	0.83	0.92	215.61	256.81	142.92	82.1	249.32	363.01	469.99	231.76	138.87	432.71	1891	0.12
0.11	0.95	0.08	0.98	0.93	1.0	0.85	0.07	0.86	0.81	0.9	0.81	0.14	0.85	0.75	0.92	0.66	0.67	0.46	0.15	0.94	0.91	1.58	0.35	0.08	1.05	0.67	0.15	0.69	0.58	0.78	0.85	0.14	0.88	0.76	0.95	0.79	0.11	0.8	0.72	0.87	0.82	0.09	0.84	0.77	0.88	238.96	370.05	146.4	84.65	256.02	533.0	849.75	344.24	191.58	623.25	2221	0.21
0.15	0.94	0.09	0.98	0.93	1.0	0.78	0.11	0.8	0.72	0.85	0.79	0.16	0.84	0.73	0.91	0.57	0.52	0.43	0.15	0.88	0.75	1.01	0.34	0.08	0.99	0.64	0.17	0.67	0.56	0.76	0.82	0.17	0.86	0.73	0.95	0.79	0.12	0.8	0.72	0.88	0.8	0.1	0.82	0.76	0.87	277.3	402.89	164.53	80.09	306.11	961.27	3482.01	479.49	261.63	886.45	948	0.43
0.18	0.93	0.1	0.97	0.88	1.0	0.73	0.1	0.74	0.66	0.8	0.72	0.17	0.76	0.63	0.85	0.81	0.7	0.64	0.26	1.19	1.14	1.67	0.5	0.14	1.45	0.57	0.16	0.59	0.47	0.68	0.8	0.15	0.82	0.7	0.92	0.73	0.12	0.74	0.65	0.81	0.76	0.09	0.78	0.71	0.83	219.59	267.67	142.2	79.64	246.34	810.37	895.59	566.39	312.07	967.07	1560	0.47
0.32	0.88	0.13	0.92	0.81	0.99	0.57	0.14	0.57	0.47	0.67	0.61	0.2	0.64	0.48	0.76	1.11	0.84	1.02	0.42	1.58	1.68	2.14	0.92	0.25	2.31	0.46	0.18	0.47	0.34	0.59	0.74	0.17	0.75	0.64	0.89	0.66	0.13	0.66	0.57	0.75	0.71	0.1	0.72	0.64	0.78	233.72	335.99	144.83	83.07	262.27	1581.35	2032.81	1026.68	573.98	1849.12	4928	1.0


==> data_new/ra/mr/bert/A_auc.tex <==
0.30

==> data_new/ra/mr/bert/A_ppl.tex <==
5.8

==> data_new/ra/mr/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	293.44	483.55	166.34	86.91	307.77	293.44	483.55	166.34	86.91	307.77	2834	0.0
0.03	0.83	0.25	0.93	0.82	0.97	0.95	0.03	0.96	0.94	0.98	0.81	0.23	0.88	0.77	0.94	3.26	5.28	1.14	0.17	4.24	2.1	2.47	1.3	0.58	2.7	0.69	0.22	0.76	0.62	0.84	0.7	0.29	0.67	0.5	1.0	0.78	0.17	0.78	0.71	0.89	0.84	0.12	0.86	0.79	0.93	179.84	170.38	129.9	74.52	218.0	238.28	209.51	177.12	104.02	290.47	1270	0.06
0.06	0.73	0.33	0.85	0.68	0.94	0.91	0.06	0.92	0.88	0.95	0.69	0.3	0.78	0.62	0.89	4.31	6.28	1.77	0.21	6.06	2.42	2.76	1.54	0.64	3.11	0.58	0.26	0.64	0.49	0.75	0.61	0.37	0.67	0.33	1.0	0.69	0.21	0.75	0.6	0.83	0.78	0.15	0.81	0.71	0.88	215.61	256.81	142.92	82.1	249.32	363.01	469.99	231.76	138.87	432.71	1891	0.12
0.11	0.62	0.36	0.74	0.5	0.88	0.85	0.07	0.86	0.81	0.9	0.58	0.32	0.66	0.47	0.8	5.75	7.25	3.06	0.43	8.71	3.2	3.33	2.12	0.93	4.33	0.46	0.27	0.52	0.35	0.64	0.52	0.36	0.5	0.33	0.67	0.62	0.21	0.67	0.5	0.78	0.72	0.15	0.75	0.67	0.81	238.96	370.05	146.4	84.65	256.02	533.0	849.75	344.24	191.58	623.25	2221	0.21
0.15	0.52	0.41	0.63	0.36	0.83	0.78	0.11	0.8	0.72	0.85	0.47	0.36	0.55	0.31	0.73	6.76	8.94	3.81	0.52	10.42	2.88	2.88	2.03	0.93	3.82	0.37	0.29	0.42	0.24	0.57	0.45	0.42	0.5	0.0	1.0	0.55	0.24	0.6	0.4	0.75	0.67	0.17	0.7	0.58	0.79	277.3	402.89	164.53	80.09	306.11	961.27	3482.01	479.49	261.63	886.45	948	0.43
0.18	0.47	0.38	0.58	0.28	0.75	0.73	0.1	0.74	0.66	0.8	0.42	0.33	0.5	0.26	0.66	7.35	7.92	5.46	1.02	11.07	3.95	3.76	2.9	1.28	5.46	0.32	0.26	0.38	0.19	0.5	0.41	0.35	0.5	0.0	0.67	0.53	0.21	0.56	0.38	0.67	0.65	0.15	0.69	0.57	0.75	219.59	267.67	142.2	79.64	246.34	810.37	895.59	566.39	312.07	967.07	1560	0.47
0.32	0.34	0.36	0.38	0.11	0.61	0.57	0.14	0.57	0.47	0.67	0.3	0.3	0.34	0.12	0.52	9.15	8.78	7.56	2.16	13.08	4.29	3.87	3.16	1.4	6.01	0.23	0.23	0.25	0.09	0.39	0.31	0.34	0.33	0.0	0.5	0.46	0.2	0.44	0.33	0.6	0.61	0.14	0.62	0.5	0.69	233.72	335.99	144.83	83.07	262.27	1581.35	2032.81	1026.68	573.98	1849.12	4928	1.0


==> data_new/ra/mr/bert/IG_auc.tex <==
0.18

==> data_new/ra/mr/bert/IG_ppl.tex <==
5.8

==> data_new/ra/mr/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	293.46	483.67	166.34	86.91	307.77	293.46	483.67	166.34	86.91	307.77	2834	0.0
0.03	0.88	0.16	0.95	0.86	0.98	0.95	0.03	0.96	0.94	0.98	0.89	0.11	0.93	0.86	0.96	28.04	66.18	4.04	0.48	25.25	0.58	0.68	0.37	0.15	0.73	0.78	0.13	0.81	0.72	0.87	0.72	0.3	0.67	0.5	1.0	0.83	0.13	0.86	0.75	0.89	0.88	0.08	0.92	0.85	0.94	179.83	170.38	129.91	74.55	218.0	238.27	209.51	177.18	104.0	290.47	1270	0.06
0.06	0.84	0.17	0.9	0.79	0.96	0.91	0.06	0.92	0.88	0.95	0.85	0.14	0.89	0.8	0.94	33.63	66.16	6.16	0.61	38.82	0.6	0.67	0.39	0.17	0.8	0.71	0.14	0.73	0.64	0.82	0.65	0.36	0.67	0.5	1.0	0.77	0.16	0.78	0.67	0.89	0.85	0.1	0.87	0.8	0.92	215.56	256.71	142.68	82.02	249.4	362.93	469.86	231.72	138.85	432.71	1891	0.12
0.11	0.77	0.2	0.83	0.67	0.92	0.85	0.07	0.86	0.81	0.9	0.78	0.16	0.82	0.72	0.89	45.84	76.06	11.29	1.16	59.34	0.81	0.82	0.56	0.24	1.11	0.63	0.16	0.66	0.55	0.74	0.57	0.34	0.67	0.33	1.0	0.72	0.17	0.71	0.67	0.83	0.81	0.11	0.81	0.75	0.88	238.96	370.05	146.4	84.65	256.02	533.0	849.75	344.24	191.58	623.25	2221	0.21
0.15	0.72	0.22	0.78	0.61	0.9	0.78	0.11	0.8	0.72	0.85	0.74	0.17	0.78	0.66	0.86	61.08	99.69	19.33	1.36	80.58	0.7	0.69	0.48	0.2	1.0	0.59	0.16	0.61	0.5	0.71	0.49	0.41	0.5	0.0	1.0	0.68	0.19	0.67	0.57	0.8	0.79	0.12	0.8	0.71	0.86	277.3	402.89	164.53	80.09	306.11	961.27	3482.01	479.49	261.63	886.45	948	0.43
0.18	0.67	0.22	0.72	0.54	0.85	0.73	0.1	0.74	0.66	0.8	0.7	0.17	0.73	0.61	0.83	61.83	88.99	23.22	2.56	90.87	0.98	0.92	0.72	0.32	1.36	0.54	0.15	0.56	0.45	0.65	0.48	0.34	0.5	0.33	0.67	0.65	0.17	0.67	0.56	0.78	0.77	0.11	0.79	0.69	0.85	219.59	267.67	142.2	79.64	246.34	810.37	895.59	566.39	312.07	967.07	1560	0.47
0.32	0.55	0.26	0.59	0.38	0.76	0.57	0.14	0.57	0.47	0.67	0.58	0.22	0.62	0.47	0.75	81.65	97.91	48.53	5.48	125.96	1.16	1.04	0.86	0.37	1.63	0.44	0.18	0.46	0.33	0.57	0.38	0.35	0.33	0.0	0.67	0.58	0.18	0.57	0.44	0.67	0.72	0.12	0.73	0.64	0.8	233.72	335.99	144.83	83.07	262.27	1581.35	2032.81	1026.68	573.98	1849.12	4928	1.0


==> data_new/ra/mr/bert/S_auc.tex <==
0.23

==> data_new/ra/mr/bert/S_ppl.tex <==
5.8

==> data_new/ra/mr/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.95	0.21	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	649.41	1497.74	263.12	139.31	535.83	649.41	1497.74	263.12	139.31	535.83	2760	0.0
0.03	0.86	0.25	0.96	0.88	0.98	0.96	0.03	0.96	0.94	0.98	0.9	0.15	0.94	0.87	0.98	0.58	0.56	0.46	0.11	0.86	0.92	1.03	0.56	0.24	1.25	0.83	0.13	0.86	0.79	0.91	0.82	0.26	1.0	0.67	1.0	0.87	0.14	0.89	0.78	1.0	0.9	0.1	0.92	0.87	0.94	222.79	184.92	168.43	103.27	276.3	263.41	204.96	210.45	128.59	327.28	946	0.08
0.06	0.81	0.26	0.91	0.79	0.96	0.92	0.05	0.93	0.89	0.95	0.82	0.21	0.89	0.78	0.95	0.77	0.68	0.66	0.14	1.13	1.0	1.08	0.65	0.28	1.34	0.75	0.16	0.78	0.68	0.86	0.71	0.37	1.0	0.5	1.0	0.8	0.18	0.83	0.75	1.0	0.86	0.12	0.88	0.82	0.93	298.98	324.27	203.32	119.17	365.99	391.55	380.52	286.47	176.31	478.42	1633	0.13
0.11	0.75	0.27	0.84	0.69	0.92	0.86	0.07	0.87	0.83	0.91	0.75	0.22	0.81	0.68	0.9	1.01	0.8	0.94	0.31	1.51	1.25	1.2	0.87	0.35	1.77	0.66	0.17	0.68	0.58	0.77	0.66	0.35	0.67	0.5	1.0	0.74	0.19	0.78	0.67	0.89	0.82	0.13	0.81	0.75	0.9	416.82	961.23	209.24	121.87	385.63	664.01	1292.42	360.69	215.09	629.81	1796	0.26
0.15	0.7	0.27	0.78	0.61	0.89	0.79	0.09	0.81	0.74	0.86	0.68	0.25	0.73	0.59	0.85	1.13	0.84	1.09	0.42	1.71	1.39	1.41	0.97	0.43	1.92	0.59	0.19	0.6	0.48	0.71	0.58	0.42	0.5	0.0	1.0	0.7	0.21	0.71	0.6	0.83	0.78	0.14	0.8	0.69	0.86	519.39	1240.12	240.15	128.64	470.24	987.15	2613.61	470.35	273.54	853.18	927	0.39
0.18	0.64	0.28	0.72	0.54	0.84	0.75	0.09	0.76	0.69	0.81	0.63	0.24	0.68	0.52	0.8	1.37	0.94	1.36	0.69	1.95	1.67	1.53	1.24	0.53	2.25	0.53	0.18	0.54	0.42	0.65	0.54	0.38	0.5	0.33	1.0	0.66	0.2	0.67	0.56	0.78	0.75	0.13	0.77	0.69	0.83	361.92	702.93	201.86	117.17	372.38	787.66	1410.14	476.27	304.21	810.19	1399	0.51
0.32	0.52	0.28	0.58	0.35	0.73	0.62	0.12	0.62	0.53	0.7	0.5	0.26	0.54	0.36	0.69	1.66	1.14	1.62	0.81	2.43	1.98	1.77	1.49	0.66	2.76	0.41	0.19	0.42	0.29	0.54	0.43	0.38	0.5	0.0	0.67	0.58	0.2	0.57	0.44	0.67	0.69	0.13	0.7	0.62	0.78	396.96	891.74	210.62	123.14	389.33	1310.88	4840.82	729.1	447.57	1258.44	4192	1.0


==> data_new/ra/mr/cnn/IG_auc.tex <==
0.22

==> data_new/ra/mr/cnn/IG_ppl.tex <==
2.3

==> data_new/ra/mr/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.69	0.46	1.0	0.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	649.62	1497.88	263.16	139.31	536.06	649.62	1497.88	263.16	139.31	536.06	2760	0.0
0.03	0.62	0.46	0.93	0.0	0.98	0.96	0.03	0.96	0.94	0.98	0.91	0.25	0.98	0.93	1.0	8.6	12.92	4.39	0.0	9.72	0.23	0.3	0.12	0.03	0.28	0.88	0.09	0.9	0.83	0.94	0.83	0.29	1.0	0.67	1.0	0.89	0.19	1.0	0.86	1.0	0.92	0.14	0.94	0.92	1.0	222.79	184.92	168.43	103.27	276.3	263.41	204.96	210.45	128.59	327.28	946	0.08
0.06	0.59	0.45	0.89	0.0	0.97	0.92	0.05	0.93	0.89	0.95	0.86	0.29	0.96	0.88	1.0	11.63	15.58	6.78	0.0	13.63	0.25	0.3	0.16	0.06	0.33	0.81	0.13	0.84	0.75	0.9	0.77	0.37	1.0	0.5	1.0	0.84	0.23	0.89	0.75	1.0	0.88	0.17	0.93	0.85	1.0	299.07	324.51	203.32	119.19	366.0	391.65	380.66	286.47	176.32	478.42	1633	0.13
0.11	0.57	0.43	0.83	0.0	0.94	0.86	0.07	0.87	0.83	0.91	0.81	0.3	0.91	0.78	1.0	15.09	17.1	10.4	1.58	19.13	0.35	0.38	0.23	0.09	0.47	0.73	0.15	0.75	0.64	0.83	0.7	0.38	1.0	0.5	1.0	0.78	0.25	0.83	0.67	1.0	0.85	0.17	0.88	0.8	1.0	416.91	961.34	209.36	121.97	385.71	664.16	1292.63	360.58	215.09	629.61	1796	0.26
0.15	0.52	0.42	0.76	0.0	0.91	0.79	0.09	0.81	0.74	0.86	0.73	0.38	0.87	0.69	0.97	18.11	18.29	13.48	4.86	24.65	0.33	0.35	0.23	0.09	0.44	0.68	0.16	0.7	0.57	0.8	0.61	0.43	1.0	0.0	1.0	0.74	0.28	0.83	0.6	1.0	0.81	0.2	0.86	0.71	1.0	519.39	1240.12	240.15	128.64	470.24	987.15	2613.61	470.35	273.54	853.18	927	0.39
0.18	0.52	0.4	0.7	0.0	0.88	0.75	0.09	0.76	0.69	0.81	0.7	0.37	0.82	0.61	0.95	20.73	18.99	16.34	7.91	28.47	0.45	0.42	0.33	0.14	0.65	0.62	0.18	0.64	0.5	0.75	0.59	0.42	0.67	0.0	1.0	0.71	0.27	0.75	0.56	1.0	0.8	0.19	0.81	0.7	1.0	361.92	702.93	201.86	117.17	372.38	787.66	1410.14	476.27	304.21	810.19	1399	0.51
0.32	0.44	0.39	0.55	0.0	0.81	0.62	0.12	0.62	0.53	0.7	0.62	0.4	0.74	0.47	0.92	25.17	21.09	20.87	11.21	36.17	0.57	0.52	0.41	0.18	0.79	0.54	0.2	0.56	0.41	0.67	0.52	0.43	0.5	0.0	1.0	0.65	0.29	0.67	0.5	1.0	0.75	0.2	0.77	0.64	0.92	396.96	891.74	210.62	123.14	389.33	1310.88	4840.82	729.1	447.57	1258.44	4192	1.0


==> data_new/ra/mr/cnn/S_auc.tex <==
0.17

==> data_new/ra/mr/cnn/S_ppl.tex <==
2.3

==> data_new/ra/mr/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.78	0.42	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	614.18	1405.47	266.95	141.02	535.82	614.18	1405.47	266.95	141.02	535.82	2853	0.0
0.03	0.77	0.36	0.96	0.75	0.99	0.95	0.03	0.96	0.94	0.98	0.83	0.28	0.94	0.83	0.99	0.87	3.31	0.08	0.01	0.5	1.64	2.38	0.87	0.34	1.81	0.77	0.23	0.85	0.71	0.92	0.78	0.31	1.0	0.5	1.0	0.83	0.2	0.88	0.75	1.0	0.87	0.14	0.92	0.81	1.0	217.84	184.33	164.33	101.53	265.46	264.97	221.08	205.77	127.47	326.57	984	0.11
0.06	0.64	0.42	0.88	0.24	0.98	0.92	0.05	0.93	0.89	0.95	0.75	0.34	0.89	0.68	0.98	1.2	4.0	0.1	0.01	0.75	2.01	2.68	1.1	0.41	2.46	0.69	0.27	0.77	0.58	0.88	0.72	0.38	1.0	0.5	1.0	0.78	0.24	0.83	0.67	1.0	0.83	0.17	0.88	0.75	1.0	309.45	379.24	207.64	120.22	377.75	419.74	475.56	286.03	171.65	490.48	1698	0.18
0.11	0.59	0.43	0.8	0.16	0.95	0.86	0.07	0.87	0.82	0.91	0.66	0.38	0.79	0.53	0.93	1.4	4.45	0.16	0.01	1.09	2.34	2.82	1.43	0.54	3.16	0.6	0.28	0.66	0.47	0.8	0.65	0.38	0.67	0.33	1.0	0.72	0.25	0.78	0.56	0.89	0.79	0.18	0.81	0.69	0.92	413.09	937.97	209.44	122.19	401.78	649.21	1315.0	355.9	212.79	630.32	1862	0.3
0.15	0.5	0.44	0.66	0.0	0.89	0.79	0.1	0.81	0.75	0.86	0.58	0.41	0.71	0.39	0.91	1.85	5.75	0.12	0.01	1.3	2.65	2.94	1.71	0.62	3.68	0.53	0.3	0.6	0.4	0.74	0.57	0.44	0.5	0.0	1.0	0.66	0.29	0.67	0.5	1.0	0.75	0.2	0.79	0.67	0.9	495.25	1120.93	245.15	128.66	478.32	889.98	1984.04	467.29	263.94	840.42	980	0.41
0.18	0.5	0.42	0.63	0.0	0.87	0.74	0.09	0.76	0.69	0.81	0.54	0.38	0.63	0.33	0.83	1.94	4.98	0.47	0.02	1.75	3.05	3.34	1.95	0.79	4.16	0.48	0.28	0.53	0.33	0.68	0.55	0.39	0.5	0.0	1.0	0.64	0.26	0.67	0.5	0.83	0.73	0.18	0.75	0.62	0.86	361.13	683.94	205.79	118.77	382.46	781.99	1188.98	478.58	307.05	796.95	1441	0.6
0.32	0.39	0.39	0.43	0.0	0.75	0.62	0.12	0.62	0.54	0.7	0.42	0.38	0.47	0.18	0.7	2.08	5.36	0.25	0.02	2.0	3.64	3.56	2.56	1.06	5.05	0.37	0.27	0.4	0.21	0.56	0.45	0.4	0.5	0.0	1.0	0.57	0.26	0.57	0.4	0.75	0.68	0.18	0.69	0.56	0.8	395.93	892.32	211.86	122.27	395.39	1161.73	2389.51	725.11	448.39	1222.6	4353	1.0


==> data_new/ra/mr/lstm/IG_auc.tex <==
0.18

==> data_new/ra/mr/lstm/IG_ppl.tex <==
1.9

==> data_new/ra/mr/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.78	0.42	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	614.18	1405.47	266.95	141.02	535.82	614.18	1405.47	266.95	141.02	535.82	2853	0.0
0.03	0.81	0.31	0.95	0.82	0.99	0.95	0.03	0.96	0.94	0.98	0.88	0.18	0.94	0.86	0.98	9.61	16.28	2.99	0.55	13.25	0.88	1.02	0.53	0.2	1.19	0.8	0.14	0.83	0.73	0.9	0.77	0.3	1.0	0.5	1.0	0.84	0.18	0.88	0.78	1.0	0.88	0.13	0.92	0.85	1.0	217.84	184.33	164.33	101.53	265.46	264.97	221.08	205.77	127.47	326.57	984	0.11
0.06	0.7	0.37	0.89	0.62	0.96	0.92	0.05	0.93	0.89	0.95	0.83	0.25	0.92	0.81	0.97	18.92	56.09	3.29	0.61	19.35	1.0	1.11	0.63	0.26	1.37	0.75	0.14	0.78	0.67	0.86	0.7	0.38	1.0	0.5	1.0	0.8	0.21	0.83	0.71	1.0	0.86	0.15	0.89	0.81	1.0	309.45	379.24	207.64	120.22	377.75	419.74	475.56	286.03	171.65	490.48	1698	0.18
0.11	0.66	0.35	0.82	0.55	0.92	0.86	0.07	0.87	0.82	0.91	0.77	0.29	0.85	0.73	0.93	25.04	95.82	3.85	1.0	23.14	1.21	1.29	0.79	0.3	1.67	0.68	0.15	0.69	0.59	0.78	0.63	0.37	0.67	0.33	1.0	0.74	0.22	0.78	0.67	0.89	0.82	0.16	0.83	0.75	0.93	413.09	937.97	209.44	122.19	401.78	649.21	1315.0	355.9	212.79	630.32	1862	0.3
0.15	0.58	0.37	0.73	0.0	0.88	0.79	0.1	0.81	0.75	0.86	0.7	0.36	0.82	0.66	0.91	37.03	107.94	4.42	1.12	30.35	1.21	1.23	0.83	0.36	1.63	0.64	0.16	0.67	0.57	0.75	0.57	0.43	0.5	0.0	1.0	0.7	0.25	0.75	0.57	0.88	0.79	0.19	0.83	0.71	0.92	495.29	1120.76	245.15	128.66	478.32	890.01	1983.33	467.29	263.94	840.42	980	0.41
0.18	0.59	0.33	0.71	0.42	0.86	0.74	0.09	0.76	0.69	0.81	0.68	0.32	0.76	0.62	0.87	29.72	68.21	9.24	1.43	35.01	1.56	1.48	1.06	0.45	2.22	0.59	0.15	0.6	0.5	0.7	0.5	0.39	0.5	0.0	1.0	0.68	0.23	0.67	0.56	0.83	0.77	0.17	0.8	0.7	0.88	361.19	684.13	205.79	118.77	382.12	782.11	1189.44	478.73	307.05	796.95	1441	0.6
0.32	0.51	0.32	0.59	0.27	0.76	0.62	0.12	0.62	0.54	0.7	0.59	0.33	0.67	0.49	0.8	32.09	68.61	6.27	1.58	39.33	1.84	1.61	1.4	0.58	2.61	0.51	0.16	0.52	0.41	0.61	0.42	0.39	0.5	0.0	0.67	0.6	0.23	0.62	0.5	0.75	0.74	0.16	0.75	0.67	0.83	395.91	892.36	211.86	122.27	395.39	1161.61	2389.22	725.11	448.54	1222.64	4353	1.0


==> data_new/ra/mr/lstm/S_auc.tex <==
0.20

==> data_new/ra/mr/lstm/S_ppl.tex <==
1.9

==> data_new/ra/mr/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	629.45	1518.27	262.02	138.73	529.34	629.45	1518.27	262.02	138.73	529.34	2990	0.0
0.03	0.96	0.06	0.98	0.95	0.99	0.96	0.03	0.96	0.94	0.98	0.95	0.06	0.97	0.93	0.99	0.04	0.03	0.03	0.02	0.05	0.57	0.71	0.33	0.14	0.72	0.87	0.08	0.89	0.83	0.94	0.85	0.23	1.0	0.67	1.0	0.89	0.1	0.89	0.86	1.0	0.93	0.07	0.93	0.92	1.0	222.2	189.52	164.38	100.72	271.21	268.41	220.22	204.42	129.88	324.39	1031	0.09
0.06	0.93	0.09	0.97	0.91	0.99	0.92	0.05	0.93	0.89	0.95	0.93	0.08	0.95	0.9	0.98	0.06	0.04	0.05	0.03	0.07	0.61	0.76	0.36	0.15	0.79	0.84	0.11	0.86	0.78	0.91	0.77	0.33	1.0	0.5	1.0	0.87	0.13	0.88	0.78	1.0	0.91	0.08	0.92	0.87	1.0	299.68	322.37	202.11	119.17	369.13	404.11	427.96	282.82	168.05	481.21	1779	0.15
0.11	0.88	0.13	0.92	0.83	0.97	0.86	0.07	0.87	0.82	0.91	0.88	0.12	0.9	0.83	0.96	0.08	0.05	0.07	0.05	0.1	0.88	1.04	0.52	0.21	1.15	0.76	0.14	0.78	0.69	0.86	0.71	0.33	0.67	0.5	1.0	0.8	0.16	0.83	0.67	0.89	0.87	0.1	0.88	0.81	0.94	404.0	916.1	207.42	119.19	389.73	597.49	1121.65	343.55	211.33	611.68	1964	0.2
0.15	0.87	0.14	0.91	0.81	0.97	0.79	0.09	0.81	0.75	0.85	0.86	0.12	0.89	0.81	0.95	0.09	0.05	0.08	0.05	0.11	0.74	0.76	0.51	0.21	1.02	0.75	0.14	0.77	0.67	0.85	0.67	0.39	1.0	0.5	1.0	0.79	0.17	0.83	0.67	1.0	0.86	0.11	0.86	0.8	0.93	497.86	1116.01	239.34	125.54	468.33	949.76	2105.36	457.6	271.9	872.5	1003	0.39
0.18	0.81	0.17	0.86	0.73	0.94	0.74	0.09	0.76	0.69	0.81	0.81	0.15	0.85	0.74	0.92	0.1	0.06	0.09	0.07	0.13	1.05	1.14	0.68	0.3	1.39	0.68	0.16	0.7	0.59	0.79	0.61	0.37	0.67	0.33	1.0	0.75	0.18	0.75	0.67	0.88	0.83	0.11	0.82	0.75	0.9	396.82	1069.36	200.26	114.26	377.48	744.7	1140.95	467.09	284.98	785.95	1508	0.37
0.32	0.72	0.22	0.77	0.61	0.89	0.62	0.12	0.62	0.54	0.7	0.73	0.19	0.77	0.63	0.86	0.13	0.06	0.12	0.09	0.16	1.31	1.34	0.9	0.39	1.75	0.59	0.19	0.61	0.48	0.72	0.52	0.38	0.5	0.0	1.0	0.68	0.19	0.67	0.56	0.8	0.78	0.12	0.8	0.71	0.87	381.73	821.61	208.38	120.3	387.07	1278.62	7101.3	723.01	430.93	1225.95	4574	1.0


==> data_new/ra/mr/lstmatt/A_auc.tex <==
0.27

==> data_new/ra/mr/lstmatt/A_ppl.tex <==
2.3

==> data_new/ra/mr/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	629.45	1518.27	262.02	138.73	529.34	629.45	1518.27	262.02	138.73	529.34	2990	0.0
0.03	0.94	0.11	0.98	0.94	0.99	0.96	0.03	0.96	0.94	0.98	0.93	0.09	0.97	0.91	0.99	0.94	2.36	0.31	0.16	0.71	1.24	1.71	0.68	0.27	1.61	0.86	0.11	0.89	0.82	0.93	0.84	0.23	1.0	0.67	1.0	0.89	0.11	0.89	0.86	1.0	0.92	0.07	0.93	0.88	1.0	222.2	189.52	164.38	100.72	271.21	268.41	220.22	204.42	129.88	324.39	1031	0.09
0.06	0.9	0.14	0.95	0.88	0.98	0.92	0.05	0.93	0.89	0.95	0.89	0.12	0.93	0.85	0.97	1.02	1.76	0.51	0.28	1.06	1.44	1.79	0.85	0.35	1.83	0.8	0.13	0.83	0.75	0.9	0.79	0.32	1.0	0.5	1.0	0.85	0.14	0.88	0.78	1.0	0.89	0.09	0.9	0.86	0.94	299.68	322.37	202.11	119.17	369.13	404.11	427.96	282.82	168.05	481.21	1779	0.15
0.11	0.83	0.18	0.9	0.77	0.96	0.86	0.07	0.87	0.82	0.91	0.82	0.15	0.86	0.75	0.93	1.43	2.29	0.75	0.4	1.48	2.0	2.41	1.23	0.5	2.54	0.72	0.16	0.74	0.64	0.83	0.71	0.33	0.67	0.5	1.0	0.8	0.16	0.8	0.67	0.89	0.85	0.1	0.88	0.8	0.92	404.0	916.1	207.42	119.19	389.73	597.49	1121.65	343.55	211.33	611.68	1964	0.2
0.15	0.77	0.23	0.84	0.68	0.93	0.79	0.09	0.81	0.75	0.85	0.76	0.2	0.81	0.67	0.9	1.46	1.54	0.95	0.57	1.75	2.17	2.39	1.42	0.54	2.89	0.65	0.19	0.68	0.55	0.79	0.64	0.4	0.67	0.5	1.0	0.74	0.21	0.75	0.67	0.88	0.82	0.12	0.83	0.75	0.9	497.86	1116.01	239.34	125.54	468.33	949.76	2105.36	457.6	271.9	872.5	1003	0.39
0.18	0.72	0.23	0.78	0.62	0.89	0.74	0.09	0.76	0.69	0.81	0.72	0.18	0.75	0.62	0.86	1.77	2.4	1.03	0.63	1.94	2.54	2.55	1.75	0.77	3.5	0.61	0.17	0.62	0.5	0.73	0.61	0.36	0.67	0.33	1.0	0.72	0.17	0.75	0.67	0.83	0.8	0.11	0.8	0.73	0.88	396.82	1069.36	200.26	114.26	377.48	744.7	1140.95	467.09	284.98	785.95	1508	0.37
0.32	0.59	0.26	0.63	0.43	0.79	0.62	0.12	0.62	0.54	0.7	0.58	0.23	0.6	0.44	0.75	2.17	2.38	1.41	0.88	2.53	3.26	3.13	2.35	1.0	4.5	0.47	0.2	0.48	0.34	0.61	0.48	0.38	0.5	0.0	1.0	0.63	0.19	0.67	0.5	0.75	0.74	0.12	0.75	0.67	0.81	381.73	821.61	208.38	120.3	387.07	1278.62	7101.3	723.01	430.93	1225.95	4574	1.0


==> data_new/ra/mr/lstmatt/IG_auc.tex <==
0.25

==> data_new/ra/mr/lstmatt/IG_ppl.tex <==
2.3

==> data_new/ra/mr/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	629.45	1518.27	262.02	138.73	529.34	629.45	1518.27	262.02	138.73	529.34	2990	0.0
0.03	0.94	0.08	0.97	0.93	0.99	0.96	0.03	0.96	0.94	0.98	0.94	0.06	0.96	0.92	0.98	13.46	15.94	8.79	5.36	15.34	0.68	0.7	0.47	0.21	0.9	0.84	0.09	0.86	0.8	0.9	0.81	0.26	1.0	0.67	1.0	0.88	0.11	0.88	0.86	1.0	0.91	0.07	0.92	0.88	0.94	222.2	189.52	164.38	100.72	271.21	268.41	220.22	204.42	129.88	324.39	1031	0.09
0.06	0.9	0.11	0.94	0.87	0.98	0.92	0.05	0.93	0.89	0.95	0.9	0.1	0.92	0.87	0.96	18.43	19.41	12.89	7.74	22.21	0.78	0.81	0.53	0.21	1.02	0.78	0.12	0.8	0.72	0.87	0.73	0.35	1.0	0.5	1.0	0.83	0.14	0.83	0.75	1.0	0.88	0.09	0.88	0.83	0.93	299.68	322.37	202.11	119.17	369.13	404.11	427.96	282.82	168.05	481.21	1779	0.15
0.11	0.85	0.14	0.89	0.79	0.95	0.86	0.07	0.87	0.82	0.91	0.84	0.12	0.87	0.79	0.93	24.84	22.22	18.28	11.42	30.18	1.06	1.06	0.72	0.3	1.48	0.7	0.14	0.72	0.63	0.8	0.65	0.35	0.67	0.5	1.0	0.76	0.16	0.78	0.67	0.89	0.85	0.1	0.85	0.78	0.92	404.0	916.1	207.42	119.19	389.73	597.49	1121.65	343.55	211.33	611.68	1964	0.2
0.15	0.8	0.17	0.85	0.73	0.92	0.79	0.09	0.81	0.75	0.85	0.8	0.15	0.84	0.75	0.9	29.2	26.73	21.08	13.52	34.88	1.02	0.98	0.72	0.33	1.4	0.66	0.15	0.69	0.59	0.76	0.57	0.41	0.5	0.0	1.0	0.73	0.2	0.75	0.62	0.83	0.82	0.12	0.83	0.75	0.9	497.86	1116.01	239.34	125.54	468.33	949.76	2105.36	457.6	271.9	872.5	1003	0.39
0.18	0.76	0.18	0.81	0.69	0.9	0.74	0.09	0.76	0.69	0.81	0.77	0.16	0.81	0.7	0.88	31.97	28.16	23.73	15.65	37.51	1.31	1.24	0.95	0.4	1.83	0.62	0.16	0.64	0.53	0.73	0.53	0.38	0.5	0.0	1.0	0.7	0.18	0.67	0.62	0.83	0.8	0.12	0.8	0.75	0.88	396.82	1069.36	200.26	114.26	377.48	744.7	1140.95	467.09	284.98	785.95	1508	0.37
0.32	0.67	0.21	0.71	0.56	0.83	0.62	0.12	0.62	0.54	0.7	0.69	0.19	0.72	0.6	0.82	38.7	29.5	30.52	20.28	46.21	1.56	1.4	1.19	0.5	2.21	0.54	0.17	0.55	0.44	0.65	0.44	0.37	0.5	0.0	0.67	0.63	0.19	0.67	0.5	0.75	0.76	0.12	0.75	0.69	0.83	381.73	821.61	208.38	120.3	387.07	1278.62	7101.3	723.01	430.93	1225.95	4574	1.0


==> data_new/ra/mr/lstmatt/S_auc.tex <==
0.26

==> data_new/ra/mr/lstmatt/S_ppl.tex <==
2.3

==> data_new/ra/mr/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	245.59	360.1	144.84	83.77	271.43	245.59	360.1	144.84	83.77	271.43	2834	0.0
0.03	0.96	0.05	0.97	0.94	0.99	0.95	0.03	0.96	0.94	0.97	0.95	0.04	0.96	0.93	0.98	0.69	0.33	0.64	0.43	0.9	0.54	0.57	0.37	0.16	0.71	0.83	0.07	0.84	0.78	0.88	0.87	0.07	0.88	0.83	0.93	0.89	0.05	0.89	0.85	0.93	0.91	0.04	0.92	0.89	0.94	146.6	129.42	106.96	69.35	175.32	198.42	166.23	149.54	92.95	247.34	1373	0.04
0.06	0.92	0.08	0.94	0.9	0.97	0.9	0.06	0.91	0.88	0.94	0.91	0.07	0.92	0.88	0.95	0.85	0.38	0.81	0.56	1.07	0.64	0.67	0.43	0.18	0.87	0.76	0.09	0.77	0.71	0.82	0.82	0.11	0.83	0.76	0.89	0.84	0.07	0.85	0.8	0.89	0.88	0.05	0.88	0.85	0.91	180.1	204.78	125.3	76.22	211.1	319.93	359.26	218.71	130.96	375.87	2016	0.09
0.11	0.86	0.11	0.89	0.82	0.94	0.83	0.08	0.85	0.79	0.89	0.85	0.09	0.87	0.8	0.91	1.15	0.46	1.13	0.81	1.45	0.95	0.96	0.65	0.27	1.34	0.68	0.1	0.69	0.63	0.75	0.74	0.13	0.75	0.68	0.82	0.78	0.08	0.79	0.74	0.83	0.84	0.05	0.85	0.81	0.88	196.52	276.04	127.77	75.66	216.91	515.88	838.38	314.37	183.52	577.94	2404	0.19
0.15	0.8	0.15	0.84	0.73	0.91	0.75	0.12	0.77	0.69	0.83	0.79	0.12	0.81	0.73	0.87	1.16	0.45	1.11	0.83	1.45	0.81	0.81	0.57	0.22	1.17	0.62	0.12	0.63	0.55	0.7	0.69	0.17	0.71	0.61	0.81	0.73	0.09	0.74	0.69	0.8	0.81	0.06	0.82	0.77	0.85	235.7	327.03	141.63	78.05	260.8	860.15	1412.16	465.59	257.28	858.09	960	0.31
0.18	0.77	0.15	0.8	0.69	0.88	0.71	0.11	0.72	0.65	0.79	0.76	0.12	0.78	0.7	0.84	1.5	0.51	1.47	1.13	1.86	1.24	1.18	0.85	0.37	1.79	0.58	0.11	0.59	0.52	0.65	0.65	0.14	0.67	0.58	0.75	0.71	0.09	0.72	0.67	0.77	0.79	0.06	0.8	0.76	0.83	180.8	249.2	116.23	72.13	211.72	824.15	1032.2	533.18	297.35	935.18	1728	0.41
0.32	0.63	0.2	0.66	0.51	0.78	0.56	0.14	0.56	0.46	0.66	0.65	0.14	0.67	0.57	0.75	1.85	0.6	1.85	1.41	2.26	1.62	1.45	1.18	0.49	2.37	0.48	0.12	0.49	0.41	0.57	0.54	0.17	0.55	0.44	0.66	0.64	0.1	0.65	0.58	0.7	0.74	0.06	0.75	0.7	0.79	193.8	262.43	127.64	76.22	216.27	1875.72	3687.57	1120.22	604.17	2098.31	5112	1.0


==> data_new/ra/mr/roberta/A_auc.tex <==
0.26

==> data_new/ra/mr/roberta/A_ppl.tex <==
8.7

==> data_new/ra/mr/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	245.59	360.1	144.84	83.77	271.43	245.59	360.1	144.84	83.77	271.43	2834	0.0
0.03	0.75	0.26	0.84	0.69	0.93	0.95	0.03	0.96	0.94	0.97	0.75	0.22	0.82	0.67	0.91	4.21	8.04	1.48	0.64	4.53	3.33	3.37	2.36	0.98	4.53	0.62	0.2	0.67	0.52	0.78	0.6	0.31	0.67	0.5	1.0	0.73	0.17	0.75	0.62	0.88	0.81	0.11	0.81	0.75	0.88	146.6	129.42	106.96	69.35	175.32	198.42	166.23	149.54	92.95	247.34	1373	0.04
0.06	0.65	0.3	0.74	0.5	0.88	0.9	0.06	0.91	0.88	0.94	0.65	0.25	0.7	0.52	0.83	4.86	7.06	2.11	0.96	5.92	3.67	3.5	2.65	1.06	5.13	0.52	0.22	0.55	0.39	0.69	0.5	0.38	0.5	0.0	1.0	0.65	0.19	0.67	0.56	0.78	0.76	0.13	0.77	0.67	0.86	180.1	204.78	125.3	76.22	211.1	319.93	359.26	218.71	130.96	375.87	2016	0.09
0.11	0.51	0.32	0.57	0.31	0.76	0.83	0.08	0.85	0.79	0.89	0.51	0.27	0.56	0.34	0.72	5.65	7.51	2.8	1.22	7.14	4.6	4.29	3.32	1.35	6.57	0.4	0.23	0.42	0.25	0.56	0.42	0.34	0.33	0.0	0.67	0.57	0.2	0.56	0.44	0.67	0.7	0.13	0.69	0.62	0.8	196.52	276.04	127.77	75.66	216.91	515.88	838.38	314.37	183.52	577.94	2404	0.19
0.15	0.44	0.33	0.47	0.21	0.7	0.75	0.12	0.77	0.69	0.83	0.43	0.29	0.45	0.24	0.64	6.01	7.61	3.27	1.46	7.55	4.21	3.77	3.19	1.34	6.0	0.33	0.24	0.33	0.18	0.5	0.33	0.39	0.0	0.0	0.5	0.52	0.22	0.5	0.38	0.67	0.66	0.15	0.67	0.56	0.77	235.7	327.03	141.63	78.05	260.8	860.15	1412.16	465.59	257.28	858.09	960	0.31
0.18	0.35	0.31	0.37	0.14	0.59	0.71	0.11	0.72	0.65	0.79	0.35	0.27	0.37	0.18	0.55	6.86	8.52	4.04	1.84	8.81	5.41	4.74	3.91	1.83	7.79	0.26	0.21	0.26	0.13	0.41	0.29	0.32	0.33	0.0	0.5	0.47	0.19	0.44	0.33	0.62	0.63	0.13	0.62	0.56	0.71	180.8	249.2	116.23	72.13	211.72	824.15	1032.2	533.18	297.35	935.18	1728	0.41
0.32	0.23	0.3	0.23	0.03	0.44	0.56	0.14	0.56	0.46	0.66	0.23	0.27	0.23	0.05	0.42	7.38	8.24	4.95	2.5	9.21	5.89	4.92	4.58	2.03	8.63	0.17	0.2	0.17	0.04	0.3	0.22	0.3	0.0	0.0	0.33	0.41	0.19	0.43	0.29	0.56	0.58	0.13	0.57	0.5	0.67	193.8	262.43	127.64	76.22	216.27	1875.72	3687.57	1120.22	604.17	2098.31	5112	1.0


==> data_new/ra/mr/roberta/IG_auc.tex <==
0.15

==> data_new/ra/mr/roberta/IG_ppl.tex <==
8.7

==> data_new/ra/mr/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	245.59	360.1	144.84	83.77	271.43	245.59	360.1	144.84	83.77	271.43	2834	0.0
0.03	0.83	0.21	0.91	0.76	0.97	0.95	0.03	0.96	0.94	0.97	0.86	0.16	0.91	0.81	0.95	34.62	97.44	4.42	1.47	21.6	0.6	0.72	0.37	0.15	0.76	0.73	0.16	0.76	0.65	0.85	0.66	0.3	0.67	0.5	1.0	0.79	0.15	0.78	0.71	0.89	0.86	0.1	0.88	0.81	0.93	146.6	129.42	106.96	69.35	175.32	198.42	166.23	149.54	92.95	247.34	1373	0.04
0.06	0.75	0.24	0.83	0.65	0.93	0.9	0.06	0.91	0.88	0.94	0.78	0.19	0.84	0.71	0.91	54.04	138.26	7.94	2.3	40.18	0.72	0.87	0.44	0.18	0.94	0.64	0.19	0.67	0.55	0.77	0.56	0.37	0.5	0.33	1.0	0.72	0.18	0.75	0.62	0.83	0.82	0.11	0.83	0.75	0.89	180.1	204.78	125.3	76.22	211.1	319.93	359.26	218.71	130.96	375.87	2016	0.09
0.11	0.63	0.27	0.7	0.47	0.85	0.83	0.08	0.85	0.79	0.89	0.69	0.22	0.74	0.59	0.85	82.2	184.19	16.37	4.23	76.5	1.02	1.08	0.65	0.26	1.39	0.55	0.2	0.58	0.44	0.68	0.46	0.35	0.5	0.0	0.67	0.66	0.19	0.67	0.56	0.78	0.78	0.12	0.8	0.69	0.88	196.52	276.04	127.77	75.66	216.91	515.88	838.38	314.37	183.52	577.94	2404	0.19
0.15	0.59	0.3	0.66	0.39	0.83	0.75	0.12	0.77	0.69	0.83	0.63	0.25	0.68	0.5	0.81	96.18	180.92	29.45	5.86	99.39	0.8	0.89	0.52	0.22	1.02	0.49	0.22	0.52	0.36	0.64	0.39	0.4	0.5	0.0	0.5	0.62	0.22	0.67	0.5	0.75	0.75	0.14	0.77	0.67	0.83	235.7	327.03	141.63	78.05	260.8	860.15	1412.16	465.59	257.28	858.09	960	0.31
0.18	0.52	0.28	0.56	0.32	0.74	0.71	0.11	0.72	0.65	0.79	0.58	0.24	0.62	0.45	0.75	114.88	207.79	39.87	10.77	125.35	1.16	1.18	0.79	0.32	1.58	0.44	0.19	0.46	0.33	0.58	0.34	0.34	0.33	0.0	0.5	0.58	0.19	0.57	0.44	0.67	0.72	0.12	0.73	0.62	0.81	180.8	249.2	116.23	72.13	211.72	824.15	1032.2	533.18	297.35	935.18	1728	0.41
0.32	0.44	0.27	0.45	0.24	0.65	0.56	0.14	0.56	0.46	0.66	0.49	0.24	0.52	0.34	0.67	150.13	232.62	61.12	22.7	184.16	1.25	1.18	0.9	0.37	1.78	0.36	0.19	0.38	0.24	0.5	0.28	0.32	0.33	0.0	0.5	0.53	0.19	0.56	0.4	0.67	0.68	0.12	0.69	0.62	0.75	193.8	262.43	127.64	76.22	216.27	1875.72	3687.57	1120.22	604.17	2098.31	5112	1.0


==> data_new/ra/mr/roberta/S_auc.tex <==
0.19

==> data_new/ra/mr/roberta/S_ppl.tex <==
8.7

==> data_new/ra/mr/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	252.31	449.52	137.09	77.08	259.92	252.31	449.52	137.09	77.08	259.92	2631	0.0
0.03	0.93	0.07	0.95	0.91	0.98	0.94	0.04	0.95	0.93	0.97	0.94	0.06	0.96	0.92	0.98	0.44	0.22	0.41	0.29	0.55	0.48	0.49	0.32	0.16	0.64	0.82	0.09	0.83	0.77	0.88	0.81	0.1	0.83	0.76	0.88	0.87	0.06	0.89	0.84	0.92	0.91	0.05	0.92	0.88	0.94	161.5	185.98	113.43	67.13	192.84	228.0	256.52	155.33	92.71	273.07	1425	0.04
0.06	0.88	0.09	0.91	0.84	0.94	0.89	0.07	0.91	0.87	0.94	0.89	0.09	0.91	0.86	0.95	0.55	0.24	0.52	0.38	0.68	0.58	0.55	0.42	0.18	0.81	0.74	0.11	0.75	0.68	0.82	0.73	0.13	0.75	0.66	0.82	0.82	0.08	0.83	0.77	0.87	0.87	0.06	0.88	0.84	0.91	198.35	291.65	122.97	70.43	214.33	388.78	699.38	226.15	125.58	419.84	1988	0.1
0.11	0.81	0.12	0.84	0.76	0.89	0.82	0.09	0.84	0.77	0.88	0.83	0.11	0.86	0.79	0.9	0.73	0.26	0.72	0.56	0.88	0.82	0.73	0.61	0.26	1.15	0.66	0.11	0.67	0.6	0.74	0.66	0.13	0.67	0.58	0.75	0.76	0.09	0.77	0.72	0.82	0.83	0.06	0.84	0.8	0.88	196.4	312.18	124.96	73.23	219.08	585.79	1556.92	333.49	191.31	606.82	2564	0.2
0.15	0.75	0.14	0.78	0.67	0.85	0.75	0.11	0.77	0.68	0.83	0.76	0.14	0.79	0.7	0.86	0.71	0.26	0.71	0.54	0.86	0.75	0.67	0.59	0.27	1.04	0.59	0.13	0.6	0.52	0.68	0.58	0.17	0.59	0.49	0.69	0.71	0.1	0.73	0.64	0.78	0.8	0.07	0.8	0.75	0.85	249.32	442.07	124.86	66.68	243.34	918.25	2061.64	455.22	235.34	867.46	905	0.27
0.18	0.72	0.14	0.74	0.65	0.81	0.69	0.12	0.7	0.63	0.77	0.73	0.14	0.76	0.66	0.83	0.9	0.27	0.89	0.71	1.06	1.0	0.88	0.77	0.36	1.39	0.55	0.12	0.57	0.48	0.64	0.56	0.14	0.58	0.47	0.66	0.69	0.1	0.7	0.64	0.76	0.78	0.07	0.79	0.74	0.83	184.96	336.26	115.45	68.28	202.44	972.24	2150.85	576.77	320.59	1039.2	1764	0.43
0.32	0.62	0.16	0.64	0.54	0.73	0.54	0.14	0.55	0.45	0.65	0.63	0.17	0.66	0.53	0.75	1.03	0.28	1.02	0.85	1.22	1.16	1.01	0.9	0.41	1.62	0.46	0.14	0.47	0.38	0.56	0.48	0.14	0.5	0.4	0.58	0.63	0.1	0.64	0.57	0.7	0.73	0.08	0.74	0.68	0.79	202.86	318.84	126.42	73.19	222.98	2233.4	16076.9	1091.36	622.27	2027.31	4912	1.0


==> data_new/ra/mr/xlnet/A_auc.tex <==
0.25

==> data_new/ra/mr/xlnet/A_ppl.tex <==
10.0

==> data_new/ra/mr/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	252.31	449.52	137.09	77.08	259.92	252.31	449.52	137.09	77.08	259.92	2631	0.0
0.03	0.77	0.2	0.83	0.71	0.91	0.94	0.04	0.95	0.93	0.97	0.75	0.19	0.81	0.68	0.89	2.37	3.71	1.05	0.58	2.54	0.8	0.74	0.6	0.28	1.08	0.61	0.18	0.64	0.52	0.73	0.58	0.29	0.67	0.33	0.67	0.71	0.16	0.75	0.62	0.78	0.8	0.11	0.81	0.75	0.88	161.5	185.98	113.43	67.13	192.84	228.0	256.52	155.33	92.71	273.07	1425	0.04
0.06	0.62	0.26	0.69	0.5	0.82	0.89	0.07	0.91	0.87	0.94	0.6	0.25	0.65	0.48	0.78	3.57	7.05	1.66	0.89	3.82	1.04	0.89	0.81	0.39	1.46	0.46	0.21	0.49	0.35	0.61	0.43	0.36	0.5	0.0	0.67	0.6	0.19	0.65	0.5	0.75	0.72	0.13	0.75	0.67	0.81	198.35	291.65	122.97	70.43	214.33	388.78	699.38	226.15	125.58	419.84	1988	0.1
0.11	0.48	0.28	0.52	0.32	0.69	0.82	0.09	0.84	0.77	0.88	0.46	0.26	0.5	0.31	0.65	4.53	5.65	2.42	1.26	5.61	1.26	1.07	0.98	0.44	1.78	0.34	0.2	0.36	0.22	0.49	0.35	0.31	0.33	0.0	0.67	0.52	0.18	0.56	0.43	0.67	0.67	0.12	0.69	0.6	0.75	196.4	312.18	124.96	73.23	219.08	585.79	1556.92	333.49	191.31	606.82	2564	0.2
0.15	0.37	0.32	0.41	0.18	0.6	0.75	0.11	0.77	0.68	0.83	0.35	0.3	0.39	0.18	0.57	5.75	8.3	3.08	1.68	6.48	1.41	1.09	1.19	0.55	2.05	0.26	0.23	0.27	0.13	0.42	0.26	0.35	0.0	0.0	0.5	0.45	0.21	0.5	0.33	0.6	0.62	0.15	0.64	0.53	0.7	249.32	442.07	124.86	66.68	243.34	918.25	2061.64	455.22	235.34	867.46	905	0.27
0.18	0.3	0.28	0.31	0.12	0.49	0.69	0.12	0.7	0.63	0.77	0.28	0.25	0.3	0.12	0.45	6.01	6.78	3.33	1.71	7.53	1.51	1.26	1.21	0.54	2.1	0.21	0.19	0.21	0.08	0.33	0.23	0.28	0.0	0.0	0.33	0.42	0.17	0.44	0.33	0.56	0.6	0.12	0.6	0.5	0.69	184.96	336.26	115.45	68.28	202.44	972.24	2150.85	576.77	320.59	1039.2	1764	0.43
0.32	0.17	0.27	0.18	-0.01	0.36	0.54	0.14	0.55	0.45	0.65	0.16	0.25	0.16	-0.01	0.33	7.56	7.96	4.8	2.32	10.09	1.68	1.33	1.37	0.63	2.43	0.11	0.18	0.11	-0.0	0.24	0.17	0.25	0.0	0.0	0.33	0.36	0.17	0.33	0.22	0.44	0.55	0.12	0.56	0.5	0.62	202.86	318.84	126.42	73.19	222.98	2233.4	16076.9	1091.36	622.27	2027.31	4912	1.0


==> data_new/ra/mr/xlnet/IG_auc.tex <==
0.14

==> data_new/ra/mr/xlnet/IG_ppl.tex <==
10.0

==> data_new/ra/mr/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	252.33	449.58	137.09	77.08	259.92	252.33	449.58	137.09	77.08	259.92	2631	0.0
0.03	0.93	0.08	0.96	0.91	0.98	0.94	0.04	0.95	0.93	0.97	0.94	0.06	0.96	0.92	0.98	149.84	324.05	42.0	19.23	124.44	0.41	0.43	0.28	0.12	0.54	0.83	0.09	0.85	0.79	0.9	0.75	0.26	0.67	0.67	1.0	0.87	0.11	0.89	0.78	0.89	0.91	0.07	0.93	0.88	0.94	161.5	185.98	113.43	67.13	192.84	228.0	256.52	155.33	92.71	273.07	1425	0.04
0.06	0.89	0.11	0.92	0.85	0.97	0.89	0.07	0.91	0.87	0.94	0.9	0.08	0.93	0.88	0.96	230.13	534.72	69.17	29.55	197.3	0.46	0.47	0.31	0.13	0.65	0.78	0.11	0.79	0.72	0.85	0.67	0.34	0.67	0.5	1.0	0.82	0.14	0.83	0.75	0.89	0.89	0.08	0.88	0.85	0.94	198.56	291.7	122.97	70.45	214.72	390.27	702.3	226.15	125.49	420.36	1989	0.1
0.11	0.83	0.14	0.86	0.76	0.93	0.82	0.09	0.84	0.77	0.88	0.85	0.1	0.88	0.8	0.93	295.72	499.14	109.45	44.5	325.04	0.64	0.63	0.45	0.18	0.88	0.71	0.12	0.72	0.64	0.79	0.58	0.31	0.67	0.33	0.67	0.77	0.14	0.78	0.67	0.89	0.86	0.09	0.88	0.81	0.93	196.41	312.43	125.03	73.32	218.9	586.46	1561.71	332.61	191.52	607.73	2564	0.2
0.15	0.81	0.15	0.84	0.73	0.93	0.75	0.11	0.77	0.68	0.83	0.83	0.12	0.86	0.78	0.91	402.02	762.1	147.76	64.99	408.3	0.47	0.46	0.33	0.13	0.66	0.69	0.13	0.69	0.62	0.78	0.55	0.39	0.5	0.0	1.0	0.75	0.17	0.75	0.67	0.86	0.85	0.1	0.86	0.79	0.92	249.52	443.37	124.89	66.84	243.86	923.48	2081.4	450.11	235.12	861.52	901	0.27
0.18	0.74	0.17	0.78	0.66	0.86	0.69	0.11	0.7	0.62	0.77	0.78	0.13	0.81	0.71	0.88	424.74	670.15	163.65	70.28	485.48	0.73	0.67	0.54	0.23	1.03	0.62	0.13	0.64	0.54	0.72	0.47	0.32	0.5	0.33	0.67	0.7	0.15	0.67	0.62	0.78	0.82	0.09	0.81	0.75	0.88	184.32	335.25	115.44	68.1	202.08	975.85	2187.16	581.35	325.84	1026.6	1765	0.43
0.32	0.64	0.2	0.67	0.52	0.8	0.55	0.14	0.55	0.45	0.65	0.68	0.18	0.71	0.59	0.81	599.76	798.72	300.49	112.14	784.55	0.86	0.82	0.62	0.26	1.2	0.53	0.16	0.54	0.43	0.64	0.4	0.33	0.33	0.0	0.67	0.63	0.16	0.67	0.56	0.75	0.77	0.11	0.77	0.69	0.85	203.03	319.37	126.32	73.19	223.05	2251.81	16153.95	1088.75	624.1	2041.01	4914	1.0


==> data_new/ra/mr/xlnet/S_auc.tex <==
0.25

==> data_new/ra/mr/xlnet/S_ppl.tex <==
10.1

==> data_new/ra/yelp/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.94	0.05	0.94	0.91	0.98	0.98	0.02	0.98	0.97	0.99	0.95	0.03	0.95	0.93	0.98	0.96	0.59	1.05	0.62	1.36	1.31	1.67	0.76	0.12	1.74	0.86	0.08	0.84	0.81	0.88	0.88	0.07	0.86	0.83	0.92	0.9	0.05	0.89	0.87	0.93	0.93	0.04	0.92	0.91	0.95	140.66	614.42	55.51	39.65	77.59	148.14	613.57	62.63	46.75	86.22	800	0.01
0.03	0.85	0.06	0.85	0.81	0.9	0.95	0.03	0.95	0.93	0.97	0.89	0.04	0.89	0.86	0.91	1.61	0.48	1.64	1.3	1.93	2.13	2.23	1.46	0.59	2.93	0.73	0.05	0.73	0.71	0.76	0.77	0.06	0.77	0.73	0.8	0.82	0.04	0.82	0.8	0.84	0.87	0.02	0.87	0.86	0.88	64.58	49.58	54.75	38.89	71.06	87.98	70.36	73.19	54.59	93.03	619	0.05
0.06	0.76	0.09	0.76	0.71	0.82	0.91	0.04	0.91	0.89	0.94	0.81	0.05	0.81	0.78	0.85	2.0	0.57	2.04	1.61	2.4	2.97	2.85	2.12	0.88	3.99	0.64	0.06	0.64	0.61	0.68	0.68	0.08	0.68	0.64	0.72	0.75	0.04	0.75	0.73	0.78	0.82	0.03	0.82	0.81	0.84	69.49	61.38	55.69	39.59	74.0	117.56	82.22	95.31	71.39	129.21	381	0.09
0.11	0.69	0.09	0.69	0.63	0.75	0.87	0.05	0.87	0.84	0.89	0.75	0.06	0.75	0.71	0.79	2.28	0.58	2.32	1.89	2.68	3.29	3.2	2.27	0.87	4.71	0.57	0.06	0.58	0.54	0.61	0.62	0.08	0.62	0.58	0.65	0.7	0.04	0.7	0.67	0.72	0.79	0.03	0.79	0.77	0.81	125.71	589.85	55.57	39.61	73.03	239.16	1012.0	120.41	92.12	157.8	344	0.12
0.15	0.59	0.1	0.59	0.52	0.65	0.8	0.05	0.79	0.77	0.83	0.66	0.07	0.66	0.62	0.7	2.65	0.6	2.67	2.27	3.05	4.07	3.72	3.18	1.27	5.73	0.49	0.06	0.49	0.45	0.52	0.54	0.08	0.54	0.5	0.59	0.64	0.05	0.64	0.62	0.66	0.75	0.03	0.75	0.73	0.76	73.8	150.37	54.89	39.33	71.22	221.52	358.28	170.92	129.81	221.39	332	0.27
0.18	0.52	0.11	0.51	0.43	0.58	0.73	0.06	0.73	0.69	0.77	0.59	0.08	0.6	0.55	0.64	2.86	0.68	2.9	2.41	3.37	4.35	3.99	3.33	1.44	6.02	0.43	0.06	0.43	0.39	0.47	0.49	0.08	0.48	0.44	0.54	0.6	0.04	0.6	0.57	0.63	0.71	0.03	0.72	0.7	0.73	83.91	231.65	55.37	39.5	71.92	704.3	5623.51	230.42	186.6	305.58	339	1.0
0.32	0.42	0.12	0.41	0.34	0.49	0.6	0.09	0.6	0.53	0.67	0.49	0.09	0.5	0.43	0.56	3.07	0.71	3.16	2.56	3.58	4.63	4.56	3.39	1.38	6.47	0.35	0.07	0.35	0.3	0.4	0.42	0.09	0.41	0.36	0.47	0.54	0.05	0.54	0.51	0.58	0.67	0.04	0.67	0.65	0.7	94.25	412.91	55.16	39.55	71.7	641.91	4659.24	386.81	286.81	534.62	680	0.79


==> data_new/ra/yelp/bert/A_auc.tex <==
0.20

==> data_new/ra/yelp/bert/A_ppl.tex <==
7.4

==> data_new/ra/yelp/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.84	0.23	0.91	0.78	0.97	0.98	0.02	0.98	0.97	0.99	0.81	0.22	0.86	0.77	0.93	8.27	11.75	3.74	0.46	11.73	5.98	7.66	3.66	0.6	7.77	0.7	0.23	0.71	0.62	0.81	0.73	0.22	0.75	0.6	0.88	0.79	0.16	0.8	0.73	0.88	0.85	0.11	0.86	0.8	0.91	164.12	711.92	56.55	40.26	79.54	171.44	710.92	64.16	48.03	85.52	591	0.01
0.03	0.63	0.3	0.71	0.52	0.84	0.95	0.03	0.96	0.93	0.97	0.6	0.27	0.67	0.53	0.76	14.41	15.51	9.18	2.6	20.59	9.77	11.33	6.39	2.58	12.06	0.46	0.22	0.51	0.39	0.6	0.52	0.2	0.55	0.4	0.67	0.64	0.15	0.66	0.58	0.73	0.73	0.11	0.76	0.69	0.8	64.89	52.17	54.76	38.81	69.77	88.68	75.55	71.85	53.77	93.67	427	0.05
0.06	0.47	0.32	0.54	0.31	0.7	0.91	0.04	0.91	0.89	0.94	0.42	0.27	0.49	0.33	0.59	16.29	15.93	11.2	3.76	24.32	10.74	10.64	7.38	2.97	15.09	0.32	0.2	0.36	0.24	0.44	0.41	0.22	0.41	0.25	0.55	0.53	0.14	0.56	0.45	0.62	0.65	0.11	0.67	0.61	0.72	70.59	65.34	55.69	39.6	74.5	118.76	84.96	95.31	71.44	129.12	374	0.09
0.11	0.35	0.31	0.4	0.2	0.56	0.87	0.05	0.87	0.84	0.89	0.31	0.25	0.35	0.2	0.46	21.06	18.26	18.09	6.03	30.12	12.2	12.85	8.55	3.85	15.91	0.23	0.19	0.25	0.14	0.34	0.35	0.21	0.35	0.22	0.5	0.47	0.14	0.49	0.4	0.56	0.61	0.1	0.62	0.57	0.67	124.85	578.39	55.69	39.51	73.93	237.02	992.1	121.12	91.87	159.44	359	0.12
0.15	0.22	0.28	0.26	0.05	0.41	0.8	0.05	0.79	0.77	0.83	0.2	0.22	0.23	0.06	0.35	23.52	18.73	21.33	7.69	34.55	14.43	16.54	9.11	3.59	18.81	0.14	0.16	0.16	0.04	0.25	0.28	0.17	0.27	0.17	0.36	0.42	0.13	0.43	0.33	0.5	0.57	0.09	0.57	0.52	0.63	74.04	147.5	55.01	38.98	71.46	222.97	351.94	171.21	130.76	226.13	347	0.27
0.18	0.17	0.26	0.18	-0.0	0.34	0.73	0.06	0.73	0.69	0.77	0.14	0.19	0.18	0.03	0.27	25.13	18.26	23.37	10.84	35.94	14.87	15.58	10.38	4.42	20.55	0.1	0.14	0.12	0.03	0.19	0.24	0.17	0.24	0.14	0.33	0.39	0.11	0.4	0.33	0.46	0.55	0.08	0.56	0.5	0.6	83.91	231.65	55.37	39.5	71.92	704.3	5623.51	230.42	186.6	305.58	339	1.0
0.32	0.1	0.23	0.11	-0.04	0.24	0.6	0.09	0.6	0.53	0.67	0.07	0.17	0.08	-0.03	0.17	27.57	20.37	24.75	13.28	38.28	16.13	15.55	11.42	4.85	21.68	0.05	0.12	0.06	-0.02	0.12	0.21	0.15	0.2	0.11	0.3	0.36	0.11	0.36	0.3	0.42	0.52	0.07	0.52	0.49	0.56	94.25	412.91	55.16	39.55	71.7	641.91	4659.24	386.81	286.81	534.62	680	0.79


==> data_new/ra/yelp/bert/IG_auc.tex <==
0.10

==> data_new/ra/yelp/bert/IG_ppl.tex <==
7.4

==> data_new/ra/yelp/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.91	0.11	0.95	0.88	0.99	0.98	0.02	0.98	0.97	0.99	0.93	0.06	0.94	0.9	0.98	45.33	75.58	11.23	2.07	57.43	2.24	3.17	1.17	0.22	2.97	0.82	0.11	0.81	0.75	0.88	0.81	0.15	0.82	0.72	0.93	0.87	0.09	0.87	0.82	0.93	0.91	0.06	0.91	0.87	0.95	129.94	559.62	55.48	39.61	77.58	137.49	558.82	62.61	46.52	86.2	793	0.01
0.03	0.81	0.14	0.85	0.74	0.92	0.95	0.03	0.96	0.93	0.97	0.85	0.08	0.87	0.82	0.91	86.46	118.15	34.3	7.5	121.26	3.31	3.86	2.0	0.82	4.6	0.69	0.09	0.7	0.64	0.76	0.66	0.17	0.67	0.56	0.77	0.78	0.08	0.79	0.73	0.83	0.85	0.06	0.85	0.82	0.88	65.1	52.43	54.8	38.8	70.3	88.9	75.98	71.85	53.66	93.85	422	0.05
0.06	0.74	0.17	0.78	0.66	0.86	0.91	0.04	0.91	0.89	0.94	0.79	0.1	0.81	0.75	0.85	107.25	136.61	48.89	8.94	153.77	3.65	4.05	2.29	0.97	5.05	0.62	0.1	0.63	0.58	0.69	0.57	0.2	0.6	0.5	0.68	0.72	0.09	0.73	0.68	0.78	0.81	0.07	0.82	0.78	0.85	69.46	61.91	55.66	39.55	73.87	117.38	83.06	95.1	71.32	128.78	364	0.1
0.11	0.67	0.17	0.69	0.56	0.8	0.87	0.05	0.87	0.84	0.89	0.74	0.11	0.77	0.69	0.82	127.16	153.58	67.5	12.5	200.23	4.26	4.19	2.98	1.29	6.2	0.57	0.1	0.58	0.51	0.63	0.52	0.2	0.53	0.4	0.65	0.68	0.1	0.69	0.62	0.74	0.78	0.07	0.79	0.75	0.83	126.55	587.99	55.66	39.62	73.8	240.84	1008.43	121.06	92.68	159.06	347	0.13
0.15	0.6	0.17	0.61	0.48	0.73	0.8	0.05	0.79	0.77	0.83	0.68	0.12	0.71	0.62	0.76	147.91	159.01	95.17	17.54	231.24	4.82	4.95	3.38	1.24	6.53	0.51	0.1	0.52	0.46	0.57	0.46	0.18	0.45	0.36	0.56	0.64	0.11	0.64	0.58	0.7	0.76	0.07	0.76	0.72	0.8	73.48	141.51	55.69	39.6	71.71	220.18	337.13	171.14	131.48	226.32	379	0.29
0.18	0.53	0.18	0.53	0.42	0.66	0.73	0.07	0.73	0.69	0.77	0.63	0.12	0.64	0.56	0.71	168.91	166.63	112.54	16.68	284.94	4.97	5.19	3.06	1.13	7.24	0.46	0.1	0.46	0.4	0.53	0.42	0.17	0.42	0.32	0.52	0.6	0.1	0.61	0.55	0.67	0.73	0.06	0.73	0.7	0.77	83.57	219.68	55.9	39.61	73.87	652.19	5280.49	232.35	186.41	316.8	385	1.0
0.32	0.45	0.18	0.45	0.31	0.59	0.6	0.09	0.6	0.53	0.67	0.53	0.14	0.54	0.44	0.63	197.8	180.77	157.42	41.52	307.01	5.91	6.51	3.53	1.41	8.2	0.38	0.11	0.39	0.31	0.46	0.35	0.17	0.33	0.25	0.48	0.55	0.11	0.56	0.5	0.62	0.7	0.07	0.7	0.66	0.74	94.25	412.91	55.16	39.55	71.7	641.91	4659.24	386.81	286.81	534.62	680	0.85


==> data_new/ra/yelp/bert/S_auc.tex <==
0.20

==> data_new/ra/yelp/bert/S_ppl.tex <==
6.8

==> data_new/ra/yelp/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.9	0.16	0.96	0.89	1.0	0.98	0.01	0.99	0.98	1.0	0.9	0.15	0.94	0.88	0.99	10.47	14.8	6.43	0.68	13.3	2.2	4.81	0.87	0.03	2.78	0.85	0.17	0.89	0.82	0.97	0.87	0.15	0.9	0.8	1.0	0.9	0.11	0.93	0.88	1.0	0.93	0.09	0.95	0.91	0.98	169.82	1025.97	63.33	46.96	95.97	176.27	1025.39	70.3	52.96	105.15	2139	0.01
0.03	0.79	0.21	0.85	0.73	0.93	0.96	0.02	0.96	0.94	0.97	0.77	0.18	0.82	0.73	0.88	19.09	20.16	13.3	7.25	22.67	3.87	6.5	2.12	0.86	4.86	0.69	0.18	0.74	0.62	0.8	0.74	0.18	0.76	0.67	0.86	0.8	0.12	0.83	0.75	0.88	0.85	0.1	0.88	0.81	0.91	77.16	58.24	59.63	45.84	84.88	98.14	71.42	78.15	60.32	107.65	1964	0.08
0.06	0.68	0.23	0.73	0.58	0.84	0.92	0.03	0.92	0.9	0.94	0.66	0.19	0.7	0.59	0.78	24.74	22.85	18.69	11.12	29.96	4.74	7.3	2.99	1.19	6.15	0.56	0.17	0.59	0.47	0.67	0.64	0.2	0.67	0.52	0.76	0.72	0.12	0.74	0.66	0.8	0.79	0.09	0.81	0.74	0.85	85.26	120.36	60.75	46.14	87.16	131.22	161.17	96.31	75.62	134.57	2034	0.15
0.11	0.59	0.24	0.63	0.46	0.76	0.88	0.04	0.88	0.86	0.9	0.57	0.19	0.6	0.48	0.68	30.64	27.6	22.62	14.45	38.32	5.68	9.45	3.65	1.57	7.2	0.46	0.16	0.49	0.38	0.57	0.56	0.19	0.56	0.44	0.67	0.66	0.12	0.67	0.6	0.73	0.74	0.09	0.76	0.69	0.8	90.04	253.68	60.27	46.04	86.19	165.77	364.95	117.27	91.36	161.57	1999	0.24
0.15	0.47	0.24	0.49	0.33	0.63	0.82	0.04	0.82	0.79	0.85	0.44	0.18	0.47	0.35	0.56	37.56	29.8	29.06	18.81	46.81	6.94	10.83	4.48	1.89	8.6	0.35	0.15	0.36	0.27	0.44	0.46	0.19	0.48	0.35	0.57	0.59	0.12	0.59	0.52	0.66	0.68	0.09	0.7	0.64	0.73	84.51	112.59	59.31	45.69	84.5	208.44	267.27	155.12	122.72	213.43	1930	0.41
0.18	0.37	0.23	0.39	0.23	0.53	0.76	0.05	0.76	0.73	0.79	0.35	0.17	0.37	0.25	0.45	45.08	38.16	34.86	21.92	54.18	7.32	9.34	4.95	2.12	9.69	0.27	0.13	0.28	0.19	0.35	0.4	0.18	0.4	0.3	0.5	0.53	0.11	0.54	0.48	0.6	0.64	0.08	0.65	0.6	0.69	110.84	773.46	60.03	45.93	85.67	405.77	4035.0	205.07	161.7	275.36	1990	0.75
0.32	0.25	0.23	0.25	0.11	0.4	0.65	0.07	0.65	0.59	0.7	0.24	0.17	0.24	0.14	0.34	56.09	43.55	44.3	28.48	69.57	8.26	10.82	5.64	2.48	10.96	0.18	0.13	0.18	0.1	0.25	0.33	0.18	0.33	0.22	0.42	0.47	0.1	0.47	0.41	0.53	0.6	0.08	0.6	0.55	0.64	87.34	199.62	60.05	46.02	86.02	398.09	564.25	305.18	229.59	420.68	3968	1.0


==> data_new/ra/yelp/cnn/IG_auc.tex <==
0.16

==> data_new/ra/yelp/cnn/IG_ppl.tex <==
3.6

==> data_new/ra/yelp/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.94	0.16	0.98	0.95	1.0	0.98	0.01	0.99	0.98	1.0	0.96	0.1	0.98	0.95	1.0	318.79	709.03	140.01	0.0	299.79	1.14	1.57	0.55	0.02	1.62	0.92	0.08	0.94	0.89	0.99	0.9	0.15	1.0	0.83	1.0	0.93	0.09	0.95	0.89	1.0	0.95	0.07	0.97	0.93	1.0	169.79	1026.16	63.28	46.94	96.0	176.25	1025.58	70.23	52.98	105.13	2139	0.01
0.03	0.89	0.17	0.94	0.89	0.97	0.96	0.02	0.96	0.94	0.97	0.91	0.11	0.93	0.89	0.96	623.78	1043.14	309.98	165.75	577.26	2.03	2.18	1.3	0.51	2.8	0.82	0.1	0.84	0.78	0.89	0.78	0.21	0.8	0.67	0.97	0.86	0.11	0.87	0.81	0.92	0.9	0.08	0.91	0.87	0.95	77.16	58.24	59.63	45.84	84.88	98.14	71.42	78.15	60.32	107.65	1964	0.08
0.06	0.84	0.18	0.89	0.83	0.94	0.92	0.03	0.92	0.9	0.94	0.86	0.13	0.88	0.83	0.93	797.16	1105.06	453.55	261.71	796.9	2.6	2.64	1.76	0.7	3.73	0.74	0.11	0.75	0.68	0.81	0.69	0.24	0.72	0.57	0.86	0.79	0.13	0.81	0.74	0.87	0.86	0.09	0.87	0.82	0.91	85.26	120.36	60.75	46.14	87.16	131.22	161.17	96.31	75.62	134.57	2034	0.15
0.11	0.8	0.19	0.85	0.77	0.91	0.88	0.04	0.88	0.86	0.9	0.81	0.15	0.84	0.77	0.89	1028.62	1272.31	603.7	357.82	1064.94	3.12	3.0	2.2	0.95	4.35	0.67	0.11	0.68	0.61	0.74	0.63	0.24	0.67	0.5	0.8	0.75	0.13	0.76	0.68	0.83	0.82	0.09	0.83	0.78	0.88	90.04	253.66	60.27	46.04	86.19	165.64	364.87	117.27	91.36	161.57	1999	0.24
0.15	0.75	0.2	0.8	0.69	0.87	0.82	0.05	0.82	0.79	0.85	0.76	0.16	0.78	0.7	0.85	1303.89	1474.34	828.27	509.81	1373.84	3.77	3.57	2.76	1.15	5.18	0.6	0.12	0.61	0.54	0.67	0.56	0.25	0.57	0.42	0.75	0.71	0.14	0.72	0.64	0.79	0.79	0.09	0.8	0.75	0.84	84.52	112.75	59.26	45.69	84.59	211.18	297.41	155.12	122.69	213.24	1929	0.42
0.18	0.7	0.21	0.75	0.64	0.84	0.76	0.05	0.76	0.73	0.79	0.71	0.19	0.74	0.64	0.81	1674.7	1964.61	1016.55	634.38	1783.66	4.09	3.72	3.01	1.28	5.68	0.55	0.13	0.56	0.48	0.63	0.52	0.26	0.53	0.36	0.68	0.67	0.15	0.68	0.6	0.75	0.77	0.1	0.77	0.72	0.83	110.85	773.27	60.05	45.94	85.73	402.79	3908.54	205.01	162.5	275.15	1991	0.74
0.32	0.64	0.22	0.69	0.56	0.79	0.65	0.07	0.65	0.6	0.7	0.64	0.2	0.68	0.57	0.76	2268.54	2363.24	1414.86	884.5	2572.06	4.54	4.18	3.34	1.38	6.41	0.49	0.14	0.5	0.42	0.57	0.46	0.27	0.48	0.29	0.64	0.64	0.16	0.64	0.56	0.72	0.74	0.1	0.75	0.69	0.8	87.32	199.6	60.06	46.02	86.03	398.2	555.03	303.81	229.06	421.88	3968	1.0


==> data_new/ra/yelp/cnn/S_auc.tex <==
0.24

==> data_new/ra/yelp/cnn/S_ppl.tex <==
3.6

==> data_new/ra/yelp/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.64	0.43	0.8	0.48	0.98	0.98	0.02	0.99	0.98	0.99	0.63	0.35	0.71	0.48	0.91	61.25	379.94	15.9	4.58	37.18	9.73	13.99	4.35	0.53	12.85	0.55	0.34	0.56	0.37	0.79	0.63	0.29	0.64	0.43	0.89	0.7	0.23	0.7	0.57	0.87	0.77	0.17	0.78	0.68	0.89	122.65	452.28	61.88	46.27	93.46	129.17	451.64	69.06	52.37	101.48	2437	0.02
0.03	0.46	0.4	0.55	0.25	0.76	0.96	0.02	0.96	0.94	0.97	0.43	0.29	0.48	0.27	0.63	77.59	433.81	24.88	13.82	49.63	12.12	13.41	7.35	2.76	17.16	0.33	0.23	0.36	0.2	0.49	0.45	0.24	0.45	0.29	0.6	0.56	0.16	0.57	0.45	0.67	0.66	0.12	0.67	0.59	0.74	75.1	53.95	59.12	45.37	83.73	95.1	62.52	76.58	59.84	105.57	2253	0.08
0.06	0.34	0.37	0.39	0.13	0.62	0.92	0.03	0.92	0.9	0.94	0.31	0.27	0.34	0.17	0.5	68.3	187.55	28.41	16.23	55.27	12.25	13.38	7.48	2.97	16.85	0.24	0.2	0.25	0.12	0.37	0.37	0.23	0.36	0.21	0.5	0.49	0.15	0.5	0.4	0.59	0.62	0.11	0.62	0.55	0.68	84.64	114.81	60.34	45.77	86.89	129.16	150.56	95.56	74.52	135.82	2354	0.15
0.11	0.26	0.34	0.28	0.06	0.5	0.88	0.04	0.88	0.86	0.9	0.23	0.24	0.24	0.1	0.39	73.91	232.53	32.26	18.48	58.91	12.73	13.79	7.93	3.0	17.5	0.17	0.18	0.17	0.07	0.29	0.32	0.21	0.3	0.19	0.44	0.45	0.14	0.44	0.36	0.53	0.58	0.1	0.59	0.53	0.65	94.14	320.65	59.87	45.47	85.41	163.43	356.34	116.82	90.45	160.91	2300	0.21
0.15	0.17	0.31	0.17	-0.01	0.36	0.82	0.04	0.82	0.79	0.84	0.15	0.22	0.16	0.03	0.29	79.73	174.84	36.98	22.66	66.93	13.17	14.08	8.03	3.6	17.84	0.11	0.16	0.12	0.03	0.21	0.27	0.19	0.25	0.14	0.37	0.41	0.12	0.4	0.33	0.48	0.55	0.09	0.55	0.5	0.61	79.02	94.19	58.98	45.28	83.73	193.08	181.57	155.0	122.19	209.55	2232	0.41
0.18	0.13	0.28	0.12	-0.02	0.3	0.76	0.05	0.76	0.73	0.79	0.11	0.2	0.11	0.0	0.24	98.62	515.64	38.83	24.3	68.03	13.02	13.93	8.53	3.43	17.54	0.08	0.14	0.08	0.0	0.17	0.24	0.17	0.22	0.12	0.33	0.39	0.11	0.38	0.31	0.45	0.54	0.08	0.54	0.49	0.59	79.53	70.65	59.7	45.59	84.88	260.45	259.66	203.24	160.05	274.34	2291	0.64
0.32	0.09	0.25	0.08	-0.05	0.23	0.65	0.07	0.65	0.6	0.7	0.07	0.17	0.07	-0.03	0.18	144.39	2316.98	43.35	27.76	73.01	12.7	12.84	8.54	3.59	17.69	0.05	0.13	0.05	-0.02	0.12	0.21	0.16	0.2	0.1	0.29	0.37	0.11	0.36	0.3	0.42	0.52	0.08	0.52	0.48	0.57	88.05	240.6	59.7	45.55	85.33	398.78	1014.01	300.76	229.78	414.35	4587	1.0


==> data_new/ra/yelp/lstm/IG_auc.tex <==
0.07

==> data_new/ra/yelp/lstm/IG_ppl.tex <==
3.5

==> data_new/ra/yelp/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.79	0.3	0.89	0.76	0.98	0.98	0.02	0.99	0.98	0.99	0.88	0.18	0.9	0.84	1.0	942.76	8134.2	418.44	0.0	915.42	3.51	5.15	1.68	0.11	4.66	0.78	0.15	0.76	0.68	0.88	0.78	0.22	0.8	0.64	1.0	0.84	0.15	0.85	0.77	1.0	0.89	0.1	0.89	0.84	1.0	122.68	452.72	61.88	46.27	93.46	129.19	452.09	69.06	52.37	101.48	2437	0.02
0.03	0.66	0.29	0.75	0.59	0.85	0.96	0.02	0.96	0.94	0.97	0.76	0.21	0.79	0.72	0.86	1293.58	7900.25	784.84	389.68	1432.55	5.13	6.02	3.28	1.13	6.6	0.61	0.1	0.62	0.55	0.68	0.6	0.24	0.6	0.48	0.75	0.73	0.16	0.73	0.67	0.81	0.81	0.11	0.81	0.77	0.86	75.1	53.96	59.12	45.37	83.73	95.2	62.47	76.58	59.84	105.53	2253	0.08
0.06	0.57	0.27	0.64	0.46	0.76	0.92	0.03	0.92	0.9	0.94	0.68	0.22	0.71	0.61	0.79	1571.13	8330.16	1045.99	530.27	1787.99	5.93	6.39	3.88	1.55	7.89	0.52	0.11	0.53	0.46	0.59	0.51	0.26	0.5	0.36	0.67	0.66	0.17	0.67	0.59	0.74	0.76	0.12	0.77	0.71	0.81	84.68	115.08	60.32	45.76	86.89	131.21	170.25	95.72	74.25	136.45	2352	0.16
0.11	0.51	0.26	0.56	0.39	0.69	0.88	0.04	0.88	0.86	0.9	0.62	0.22	0.65	0.55	0.73	1798.43	8649.55	1219.29	618.52	2058.73	6.72	7.23	4.45	1.73	9.3	0.47	0.11	0.47	0.4	0.53	0.45	0.25	0.44	0.31	0.59	0.62	0.17	0.62	0.55	0.69	0.74	0.12	0.73	0.69	0.78	94.19	321.11	59.82	45.46	85.46	164.28	353.15	116.4	91.33	161.29	2298	0.21
0.15	0.45	0.25	0.49	0.33	0.62	0.82	0.04	0.82	0.79	0.84	0.56	0.23	0.58	0.48	0.68	2037.78	8597.65	1398.13	750.13	2429.36	7.77	8.17	5.18	2.2	10.46	0.41	0.11	0.41	0.35	0.48	0.41	0.25	0.4	0.25	0.5	0.58	0.17	0.58	0.5	0.65	0.71	0.12	0.71	0.66	0.75	79.04	94.25	58.88	45.28	83.74	195.32	212.29	154.97	122.14	206.1	2230	0.42
0.18	0.41	0.24	0.43	0.27	0.58	0.76	0.05	0.76	0.73	0.79	0.52	0.23	0.53	0.42	0.63	2339.29	8241.29	1668.67	848.32	2766.49	8.35	8.78	5.49	2.17	11.57	0.37	0.12	0.38	0.31	0.44	0.37	0.25	0.33	0.2	0.5	0.56	0.17	0.55	0.47	0.62	0.69	0.12	0.69	0.64	0.73	79.65	71.04	59.77	45.62	85.0	260.33	258.02	203.26	160.05	274.87	2294	0.65
0.32	0.36	0.23	0.37	0.21	0.52	0.65	0.07	0.65	0.6	0.7	0.46	0.24	0.47	0.35	0.57	2753.67	8442.07	2010.6	1023.55	3408.83	8.95	9.16	5.97	2.56	12.46	0.33	0.12	0.33	0.26	0.4	0.33	0.25	0.3	0.17	0.44	0.52	0.17	0.51	0.43	0.59	0.66	0.12	0.66	0.61	0.71	88.02	240.91	59.67	45.49	85.3	394.13	822.62	300.1	229.22	412.05	4582	1.0


==> data_new/ra/yelp/lstm/S_auc.tex <==
0.15

==> data_new/ra/yelp/lstm/S_ppl.tex <==
3.5

==> data_new/ra/yelp/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.97	0.08	1.0	0.98	1.0	0.98	0.01	0.99	0.98	1.0	0.98	0.01	0.99	0.98	0.99	0.06	0.08	0.04	0.01	0.08	3.19	5.98	1.08	0.06	3.63	0.93	0.05	0.92	0.9	0.96	0.92	0.08	0.93	0.88	1.0	0.95	0.04	0.95	0.92	1.0	0.96	0.03	0.96	0.95	1.0	170.24	1006.52	62.63	46.72	95.46	176.74	1005.94	69.9	52.78	103.42	2722	0.01
0.03	0.93	0.12	0.97	0.91	0.99	0.96	0.02	0.96	0.95	0.97	0.96	0.02	0.96	0.95	0.97	0.12	0.1	0.09	0.06	0.15	5.74	8.52	2.63	0.84	7.01	0.85	0.05	0.85	0.83	0.88	0.85	0.11	0.86	0.8	0.92	0.9	0.05	0.9	0.87	0.93	0.93	0.03	0.93	0.91	0.95	76.1	55.96	59.2	45.55	84.73	96.91	67.42	77.82	60.06	107.33	2499	0.08
0.06	0.88	0.15	0.93	0.83	0.98	0.92	0.03	0.92	0.9	0.94	0.92	0.04	0.93	0.91	0.95	0.17	0.12	0.14	0.09	0.21	7.34	10.13	3.68	1.16	9.24	0.79	0.06	0.79	0.76	0.83	0.78	0.15	0.8	0.71	0.87	0.85	0.07	0.86	0.82	0.89	0.9	0.04	0.9	0.88	0.92	83.66	109.3	60.44	46.13	87.99	126.88	135.13	96.09	74.63	133.52	2601	0.15
0.11	0.82	0.19	0.89	0.75	0.97	0.88	0.04	0.88	0.86	0.9	0.89	0.05	0.9	0.87	0.92	0.21	0.13	0.18	0.12	0.26	9.26	11.96	5.0	1.77	11.77	0.74	0.06	0.74	0.7	0.78	0.73	0.15	0.74	0.67	0.82	0.82	0.07	0.82	0.78	0.86	0.87	0.05	0.87	0.85	0.9	91.15	294.09	60.19	45.77	86.9	162.1	325.85	116.34	91.14	161.08	2551	0.23
0.15	0.75	0.22	0.81	0.62	0.93	0.82	0.05	0.82	0.79	0.85	0.85	0.06	0.85	0.81	0.88	0.25	0.14	0.22	0.16	0.31	11.36	14.7	6.08	2.28	14.03	0.68	0.07	0.68	0.64	0.72	0.67	0.16	0.67	0.59	0.75	0.77	0.07	0.78	0.73	0.82	0.84	0.05	0.84	0.81	0.87	87.71	253.76	59.09	45.47	84.71	204.49	268.01	154.34	122.68	211.7	2474	0.39
0.18	0.7	0.24	0.74	0.53	0.9	0.76	0.05	0.76	0.73	0.79	0.8	0.07	0.81	0.76	0.85	0.29	0.16	0.26	0.18	0.36	12.55	15.8	7.03	2.58	16.38	0.62	0.07	0.62	0.58	0.67	0.61	0.16	0.61	0.5	0.7	0.74	0.08	0.74	0.7	0.79	0.81	0.05	0.81	0.78	0.85	103.57	685.36	59.91	45.75	86.04	315.39	1833.4	202.85	162.14	276.24	2538	0.6
0.32	0.59	0.27	0.62	0.39	0.82	0.65	0.07	0.65	0.59	0.7	0.73	0.09	0.74	0.68	0.79	0.34	0.16	0.31	0.23	0.41	15.15	17.78	8.92	3.24	20.26	0.55	0.08	0.55	0.5	0.6	0.54	0.17	0.53	0.44	0.64	0.68	0.09	0.68	0.63	0.73	0.78	0.06	0.78	0.74	0.81	87.45	250.01	59.84	45.75	85.99	385.92	620.2	297.5	226.52	412.39	5063	1.0


==> data_new/ra/yelp/lstmatt/A_auc.tex <==
0.24

==> data_new/ra/yelp/lstmatt/A_ppl.tex <==
3.4

==> data_new/ra/yelp/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.95	0.08	0.98	0.94	1.0	0.98	0.01	0.99	0.98	1.0	0.93	0.07	0.94	0.9	0.99	0.75	0.86	0.58	0.19	1.04	2.7	4.27	1.23	0.1	3.5	0.84	0.12	0.83	0.77	0.92	0.87	0.12	0.88	0.8	1.0	0.89	0.08	0.89	0.84	0.96	0.92	0.06	0.92	0.88	0.97	170.26	1007.16	62.55	46.72	95.43	176.77	1006.59	69.87	52.76	103.25	2721	0.01
0.03	0.88	0.12	0.92	0.85	0.96	0.96	0.02	0.96	0.94	0.97	0.83	0.1	0.85	0.79	0.9	1.43	1.09	1.16	0.73	1.79	4.48	5.32	2.71	1.09	5.84	0.69	0.11	0.7	0.64	0.76	0.75	0.16	0.76	0.67	0.85	0.79	0.09	0.8	0.75	0.85	0.84	0.06	0.85	0.81	0.88	76.08	55.93	59.18	45.56	84.67	96.72	66.37	77.53	60.07	106.92	2500	0.08
0.06	0.8	0.16	0.84	0.74	0.91	0.92	0.03	0.92	0.9	0.94	0.74	0.13	0.75	0.67	0.82	1.92	1.37	1.59	1.04	2.4	5.66	6.69	3.35	1.32	7.76	0.59	0.12	0.6	0.52	0.67	0.66	0.18	0.67	0.56	0.76	0.72	0.1	0.73	0.67	0.78	0.79	0.07	0.79	0.76	0.83	83.65	109.1	60.44	46.13	87.99	128.91	158.87	96.09	74.63	133.43	2601	0.16
0.11	0.73	0.19	0.77	0.65	0.86	0.88	0.04	0.88	0.86	0.9	0.65	0.14	0.67	0.57	0.74	2.29	1.51	1.97	1.25	2.86	6.71	7.66	4.21	1.8	8.6	0.51	0.12	0.51	0.43	0.58	0.6	0.19	0.6	0.5	0.71	0.67	0.1	0.67	0.61	0.72	0.75	0.07	0.75	0.71	0.79	91.1	294.08	60.18	45.75	86.81	161.45	323.53	116.56	91.65	161.67	2551	0.23
0.15	0.64	0.2	0.66	0.52	0.78	0.82	0.05	0.82	0.79	0.85	0.54	0.15	0.55	0.46	0.64	2.75	1.77	2.37	1.59	3.39	7.89	8.46	5.05	2.16	10.79	0.41	0.12	0.41	0.34	0.48	0.52	0.18	0.5	0.4	0.61	0.61	0.1	0.6	0.54	0.67	0.7	0.07	0.7	0.66	0.74	87.52	253.3	59.06	45.46	84.57	205.45	283.17	154.46	122.1	207.51	2472	0.4
0.18	0.55	0.22	0.57	0.41	0.71	0.75	0.05	0.75	0.72	0.78	0.46	0.15	0.46	0.37	0.55	3.08	1.82	2.68	1.82	3.81	8.63	9.26	5.77	2.28	11.48	0.34	0.12	0.34	0.27	0.41	0.46	0.19	0.45	0.33	0.56	0.56	0.1	0.56	0.5	0.62	0.67	0.07	0.67	0.63	0.71	103.7	684.75	59.96	45.77	86.12	266.84	310.44	201.91	160.85	275.3	2539	0.46
0.32	0.43	0.23	0.43	0.28	0.59	0.65	0.07	0.65	0.59	0.7	0.34	0.16	0.34	0.25	0.44	3.54	1.95	3.16	2.19	4.38	9.96	10.45	6.6	2.75	13.47	0.25	0.12	0.25	0.17	0.32	0.38	0.18	0.38	0.28	0.5	0.5	0.1	0.49	0.43	0.56	0.62	0.07	0.62	0.58	0.67	87.51	250.22	59.82	45.76	86.02	384.72	617.16	297.73	224.5	411.61	5064	1.0


==> data_new/ra/yelp/lstmatt/IG_auc.tex <==
0.21

==> data_new/ra/yelp/lstmatt/IG_ppl.tex <==
3.4

==> data_new/ra/yelp/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.05	0.99	0.97	1.0	0.98	0.01	0.99	0.98	0.99	0.96	0.06	0.98	0.95	0.99	20.32	33.3	10.76	2.77	24.24	2.72	4.56	1.12	0.09	3.29	0.87	0.1	0.88	0.82	0.95	0.9	0.13	0.93	0.83	1.0	0.92	0.08	0.93	0.88	1.0	0.93	0.06	0.94	0.9	0.98	170.21	1007.28	62.55	46.7	95.39	176.64	1006.69	69.95	52.81	103.81	2721	0.01
0.03	0.94	0.08	0.97	0.93	0.99	0.96	0.02	0.96	0.94	0.97	0.9	0.09	0.93	0.87	0.96	36.56	40.16	23.9	13.58	44.92	4.77	6.56	2.48	0.85	6.0	0.77	0.11	0.79	0.71	0.85	0.8	0.16	0.82	0.71	0.92	0.84	0.1	0.85	0.78	0.91	0.88	0.07	0.89	0.84	0.92	76.08	55.93	59.18	45.56	84.67	96.72	66.37	77.53	60.07	106.92	2500	0.08
0.06	0.9	0.11	0.94	0.87	0.97	0.92	0.03	0.92	0.9	0.94	0.85	0.12	0.88	0.81	0.93	48.39	50.17	33.37	19.57	59.0	5.91	7.56	3.17	1.12	7.85	0.69	0.13	0.71	0.63	0.79	0.73	0.2	0.75	0.6	0.88	0.79	0.12	0.8	0.72	0.87	0.84	0.08	0.85	0.8	0.9	83.65	109.1	60.44	46.13	87.99	128.91	158.87	96.09	74.63	133.43	2601	0.16
0.11	0.87	0.13	0.91	0.82	0.96	0.88	0.04	0.88	0.86	0.9	0.8	0.14	0.83	0.74	0.9	60.33	59.83	41.48	24.78	73.23	7.35	9.15	4.16	1.51	9.55	0.64	0.14	0.65	0.56	0.74	0.68	0.2	0.69	0.55	0.82	0.75	0.13	0.77	0.67	0.83	0.81	0.09	0.82	0.76	0.87	91.12	293.69	60.18	45.76	86.86	161.55	323.28	116.56	91.66	161.72	2552	0.23
0.15	0.82	0.14	0.86	0.76	0.93	0.82	0.05	0.82	0.79	0.85	0.73	0.16	0.77	0.66	0.85	71.91	64.7	52.17	32.62	88.16	9.09	10.89	5.3	1.98	12.07	0.57	0.15	0.59	0.48	0.67	0.61	0.21	0.62	0.48	0.76	0.7	0.13	0.71	0.62	0.79	0.78	0.09	0.78	0.72	0.84	87.64	253.64	59.06	45.46	84.57	204.09	276.02	154.5	122.19	207.27	2472	0.39
0.18	0.78	0.17	0.83	0.7	0.91	0.76	0.05	0.76	0.73	0.79	0.68	0.18	0.72	0.59	0.82	82.36	72.66	61.74	37.11	102.03	9.58	11.3	5.61	2.09	12.98	0.52	0.16	0.54	0.43	0.63	0.57	0.22	0.57	0.41	0.74	0.67	0.14	0.67	0.57	0.76	0.75	0.1	0.76	0.7	0.82	103.5	685.33	59.91	45.75	86.04	294.95	1434.69	202.83	162.12	276.24	2538	0.54
0.32	0.73	0.19	0.76	0.63	0.87	0.65	0.07	0.65	0.59	0.7	0.6	0.21	0.64	0.48	0.76	100.19	82.4	76.92	47.33	126.82	11.06	12.91	6.59	2.36	15.17	0.45	0.17	0.47	0.35	0.58	0.51	0.23	0.5	0.33	0.67	0.61	0.15	0.62	0.51	0.71	0.72	0.1	0.72	0.65	0.79	87.48	250.14	59.84	45.75	86.02	387.22	745.48	297.22	225.62	410.5	5064	1.0


==> data_new/ra/yelp/lstmatt/S_auc.tex <==
0.26

==> data_new/ra/yelp/lstmatt/S_ppl.tex <==
3.4

==> data_new/ra/yelp/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.92	0.06	0.92	0.88	0.97	0.98	0.02	0.98	0.97	0.99	0.97	0.02	0.97	0.96	0.98	1.5	0.95	1.58	0.95	2.12	1.29	2.13	0.69	0.12	1.84	0.87	0.07	0.86	0.83	0.91	0.87	0.07	0.86	0.83	0.91	0.91	0.05	0.91	0.88	0.94	0.94	0.03	0.93	0.92	0.95	112.41	395.84	50.17	36.4	70.88	119.44	394.94	56.29	42.62	78.54	781	0.01
0.03	0.82	0.07	0.83	0.78	0.87	0.95	0.02	0.95	0.94	0.97	0.92	0.03	0.93	0.91	0.94	2.4	0.82	2.38	1.77	3.01	2.16	2.22	1.38	0.59	2.94	0.77	0.05	0.78	0.75	0.8	0.77	0.06	0.77	0.74	0.81	0.84	0.03	0.85	0.83	0.87	0.89	0.02	0.89	0.88	0.9	58.48	39.39	48.9	35.55	65.71	79.19	49.44	67.42	49.33	91.69	540	0.05
0.06	0.73	0.09	0.72	0.68	0.79	0.91	0.04	0.92	0.89	0.93	0.87	0.05	0.88	0.85	0.9	2.86	0.92	2.85	2.14	3.55	2.5	2.61	1.67	0.7	3.17	0.7	0.06	0.71	0.67	0.73	0.69	0.08	0.7	0.65	0.74	0.79	0.05	0.8	0.77	0.82	0.85	0.03	0.86	0.84	0.87	63.36	48.64	50.57	36.17	69.34	110.77	79.86	86.92	65.67	123.45	434	0.11
0.11	0.66	0.1	0.66	0.61	0.72	0.87	0.04	0.87	0.84	0.89	0.82	0.07	0.84	0.8	0.87	3.15	1.03	3.16	2.51	4.0	2.94	2.82	2.07	0.9	4.02	0.64	0.07	0.66	0.61	0.69	0.63	0.09	0.65	0.59	0.69	0.75	0.06	0.76	0.72	0.79	0.82	0.04	0.83	0.81	0.85	109.5	429.32	51.22	35.9	69.91	230.82	913.45	115.44	86.03	156.26	379	0.17
0.15	0.58	0.09	0.57	0.53	0.63	0.8	0.05	0.8	0.77	0.84	0.78	0.06	0.79	0.75	0.82	3.64	1.07	3.62	2.86	4.48	3.48	3.21	2.34	1.04	4.82	0.59	0.06	0.6	0.56	0.63	0.58	0.08	0.6	0.54	0.64	0.72	0.05	0.73	0.69	0.75	0.8	0.03	0.8	0.78	0.82	72.93	164.34	49.31	35.8	66.87	269.53	916.97	165.36	127.81	223.97	547	0.41
0.18	0.51	0.1	0.51	0.46	0.58	0.73	0.06	0.73	0.68	0.77	0.73	0.07	0.74	0.7	0.78	3.82	1.13	3.79	3.05	4.67	3.88	3.62	2.73	1.05	5.93	0.54	0.07	0.55	0.51	0.59	0.54	0.09	0.55	0.49	0.59	0.68	0.06	0.69	0.65	0.72	0.77	0.04	0.78	0.76	0.8	82.86	304.09	50.9	35.85	67.96	298.84	338.66	232.22	185.08	319.48	385	0.39
0.32	0.43	0.1	0.43	0.36	0.49	0.61	0.09	0.62	0.54	0.68	0.66	0.09	0.67	0.61	0.72	4.1	1.15	4.1	3.27	4.98	4.56	4.08	3.37	1.49	6.58	0.48	0.07	0.49	0.44	0.53	0.47	0.09	0.48	0.41	0.54	0.64	0.06	0.65	0.61	0.68	0.74	0.04	0.75	0.72	0.77	75.82	225.37	49.38	35.85	67.14	578.4	1291.47	398.51	288.77	576.43	783	1.0


==> data_new/ra/yelp/roberta/A_auc.tex <==
0.19

==> data_new/ra/yelp/roberta/A_ppl.tex <==
6.6

==> data_new/ra/yelp/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.86	0.22	0.93	0.82	0.99	0.98	0.02	0.98	0.97	0.99	0.84	0.17	0.88	0.76	0.98	6.15	14.86	2.29	0.62	7.88	5.44	7.98	2.42	0.25	7.19	0.74	0.2	0.73	0.6	0.92	0.76	0.2	0.77	0.63	0.94	0.82	0.14	0.82	0.72	0.95	0.87	0.1	0.87	0.8	0.96	145.73	514.27	51.69	36.29	72.77	153.03	513.14	58.21	42.03	82.11	610	0.01
0.03	0.71	0.27	0.76	0.59	0.93	0.95	0.02	0.95	0.94	0.97	0.68	0.21	0.7	0.55	0.85	11.36	19.78	6.33	2.43	14.65	8.43	9.99	5.32	1.96	10.48	0.55	0.2	0.53	0.41	0.69	0.58	0.22	0.57	0.44	0.75	0.69	0.15	0.68	0.59	0.8	0.77	0.1	0.77	0.7	0.85	58.71	40.29	48.92	35.56	65.53	79.53	51.69	68.37	49.43	91.55	665	0.05
0.06	0.59	0.32	0.62	0.4	0.84	0.91	0.03	0.91	0.89	0.93	0.55	0.25	0.53	0.37	0.76	12.82	19.62	8.29	3.57	16.8	10.61	12.24	6.11	2.46	14.6	0.43	0.22	0.4	0.27	0.59	0.49	0.23	0.48	0.33	0.64	0.6	0.16	0.59	0.49	0.71	0.71	0.11	0.7	0.64	0.8	61.24	46.35	49.32	35.85	67.0	106.18	73.47	85.85	65.24	119.67	667	0.11
0.11	0.5	0.36	0.53	0.28	0.78	0.87	0.04	0.87	0.84	0.89	0.46	0.26	0.43	0.29	0.66	14.74	16.67	11.68	4.13	20.06	11.38	13.0	7.15	2.79	15.1	0.35	0.22	0.32	0.21	0.5	0.43	0.24	0.4	0.25	0.6	0.55	0.16	0.53	0.45	0.67	0.67	0.11	0.66	0.6	0.76	109.44	429.03	51.22	35.9	69.91	231.19	911.52	115.44	86.03	157.27	379	0.17
0.15	0.42	0.34	0.39	0.18	0.69	0.8	0.06	0.8	0.77	0.83	0.38	0.26	0.33	0.2	0.56	15.05	14.74	12.6	5.12	20.06	12.88	12.91	8.65	3.7	17.54	0.29	0.21	0.24	0.14	0.42	0.36	0.22	0.33	0.2	0.5	0.51	0.15	0.47	0.41	0.61	0.65	0.11	0.62	0.57	0.71	70.73	153.06	49.28	35.75	65.98	255.42	845.54	165.77	127.85	226.1	642	0.39
0.18	0.36	0.37	0.34	0.11	0.64	0.73	0.06	0.73	0.68	0.77	0.32	0.26	0.28	0.14	0.49	16.68	15.37	14.39	6.79	21.16	12.7	13.44	8.02	3.55	18.35	0.24	0.2	0.2	0.09	0.37	0.31	0.22	0.27	0.16	0.44	0.46	0.15	0.44	0.37	0.56	0.62	0.1	0.6	0.55	0.69	83.37	312.79	49.4	35.8	66.97	295.01	341.23	228.7	184.61	316.82	363	0.38
0.32	0.26	0.33	0.21	0.05	0.47	0.61	0.09	0.61	0.54	0.67	0.23	0.21	0.19	0.09	0.34	18.07	16.27	15.36	9.13	23.19	14.13	13.89	9.79	4.54	19.84	0.17	0.16	0.13	0.06	0.24	0.26	0.18	0.22	0.13	0.35	0.42	0.13	0.4	0.33	0.49	0.59	0.09	0.57	0.53	0.62	76.93	236.49	49.39	35.74	66.87	587.41	1350.46	403.83	290.18	581.46	706	1.0


==> data_new/ra/yelp/roberta/IG_auc.tex <==
0.15

==> data_new/ra/yelp/roberta/IG_ppl.tex <==
6.6

==> data_new/ra/yelp/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.87	0.15	0.92	0.83	0.98	0.98	0.02	0.98	0.97	0.99	0.91	0.08	0.92	0.87	0.96	83.6	135.88	23.84	5.1	106.07	2.92	4.25	1.46	0.26	3.71	0.79	0.13	0.78	0.71	0.86	0.76	0.18	0.76	0.62	0.9	0.85	0.1	0.86	0.79	0.93	0.9	0.07	0.89	0.85	0.94	129.72	454.9	51.29	36.21	71.99	137.12	453.85	58.15	41.92	81.6	601	0.01
0.03	0.75	0.17	0.79	0.67	0.88	0.95	0.02	0.96	0.94	0.97	0.82	0.09	0.84	0.78	0.88	163.39	216.74	65.56	19.45	221.79	4.46	5.39	2.91	1.0	5.96	0.65	0.1	0.66	0.59	0.72	0.6	0.17	0.61	0.5	0.7	0.76	0.09	0.77	0.71	0.82	0.83	0.06	0.83	0.79	0.87	58.81	39.22	49.25	35.85	66.81	79.93	50.54	68.47	49.75	92.27	400	0.05
0.06	0.66	0.18	0.7	0.56	0.79	0.91	0.04	0.92	0.89	0.93	0.75	0.12	0.77	0.69	0.83	202.04	238.53	101.18	25.78	322.26	4.93	5.69	3.02	1.03	7.25	0.58	0.11	0.58	0.51	0.65	0.52	0.2	0.5	0.4	0.64	0.71	0.1	0.71	0.65	0.78	0.79	0.07	0.8	0.76	0.84	65.36	51.79	51.22	36.49	71.37	114.64	85.85	88.05	66.25	129.3	446	0.11
0.11	0.59	0.18	0.61	0.49	0.72	0.87	0.04	0.87	0.84	0.89	0.7	0.13	0.72	0.65	0.79	251.09	317.41	133.88	31.1	379.44	5.58	6.06	3.76	1.39	7.83	0.53	0.11	0.53	0.47	0.6	0.45	0.18	0.44	0.33	0.55	0.67	0.1	0.67	0.62	0.73	0.77	0.07	0.77	0.73	0.81	93.02	363.6	49.32	35.75	66.91	190.86	707.47	112.46	84.86	148.75	665	0.15
0.15	0.54	0.17	0.55	0.43	0.66	0.8	0.05	0.8	0.77	0.84	0.66	0.12	0.67	0.58	0.74	289.0	329.57	167.78	39.25	433.38	5.92	6.56	3.83	1.58	7.6	0.49	0.11	0.49	0.42	0.55	0.4	0.18	0.4	0.29	0.5	0.63	0.1	0.62	0.58	0.68	0.75	0.07	0.75	0.71	0.79	72.93	164.34	49.31	35.8	66.87	269.53	916.97	165.36	127.81	223.97	547	0.38
0.18	0.51	0.17	0.53	0.4	0.64	0.73	0.06	0.73	0.68	0.77	0.62	0.13	0.64	0.54	0.71	332.07	402.84	189.51	44.82	440.73	6.06	6.1	4.29	1.58	8.35	0.45	0.11	0.46	0.38	0.52	0.37	0.18	0.36	0.25	0.5	0.6	0.09	0.61	0.55	0.67	0.74	0.07	0.74	0.7	0.78	82.4	304.74	50.24	35.85	67.58	295.0	333.97	231.93	184.98	317.58	383	0.37
0.32	0.48	0.16	0.47	0.37	0.58	0.61	0.09	0.61	0.54	0.68	0.57	0.12	0.58	0.5	0.65	399.44	394.47	288.12	70.88	608.12	6.26	6.62	4.1	1.62	8.5	0.41	0.1	0.41	0.35	0.47	0.33	0.17	0.33	0.23	0.42	0.57	0.1	0.57	0.51	0.64	0.71	0.07	0.71	0.67	0.75	76.71	233.4	49.4	35.85	67.14	585.82	1335.82	402.44	290.43	580.52	727	0.94


==> data_new/ra/yelp/roberta/S_auc.tex <==
0.19

==> data_new/ra/yelp/roberta/S_ppl.tex <==
7.0

==> data_new/ra/yelp/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.98	0.01	0.99	0.98	0.99	0.98	0.02	0.98	0.97	0.99	0.98	0.02	0.98	0.97	0.99	0.41	0.24	0.44	0.28	0.58	0.4	0.47	0.22	0.04	0.58	0.91	0.05	0.9	0.88	0.93	0.94	0.04	0.93	0.91	0.96	0.94	0.03	0.94	0.92	0.96	0.96	0.02	0.95	0.94	0.97	140.69	529.78	52.19	39.22	76.35	148.88	528.71	60.27	46.04	90.38	838	0.01
0.03	0.96	0.02	0.97	0.96	0.98	0.95	0.03	0.95	0.93	0.97	0.95	0.02	0.95	0.94	0.96	0.69	0.21	0.69	0.55	0.82	0.67	0.64	0.49	0.21	0.91	0.83	0.04	0.83	0.81	0.85	0.87	0.04	0.88	0.86	0.9	0.89	0.03	0.89	0.88	0.91	0.92	0.02	0.92	0.91	0.93	61.81	43.41	48.84	38.36	67.22	84.59	55.09	69.11	54.71	93.37	759	0.06
0.06	0.93	0.04	0.94	0.93	0.95	0.91	0.04	0.91	0.89	0.94	0.91	0.04	0.91	0.89	0.93	0.91	0.23	0.92	0.74	1.07	0.89	0.86	0.63	0.27	1.22	0.76	0.05	0.77	0.74	0.79	0.82	0.05	0.82	0.8	0.85	0.84	0.04	0.85	0.83	0.86	0.88	0.03	0.89	0.87	0.9	66.45	53.06	49.62	38.89	69.84	116.15	94.92	87.81	69.04	121.63	787	0.11
0.11	0.9	0.07	0.91	0.9	0.93	0.87	0.05	0.87	0.84	0.9	0.87	0.05	0.87	0.85	0.89	1.09	0.25	1.11	0.9	1.28	1.04	0.92	0.77	0.37	1.49	0.71	0.05	0.71	0.68	0.74	0.77	0.07	0.77	0.75	0.8	0.8	0.05	0.81	0.79	0.83	0.85	0.03	0.86	0.84	0.87	94.39	338.53	49.45	38.56	69.67	194.17	574.78	113.59	89.37	152.13	780	0.16
0.15	0.87	0.05	0.88	0.85	0.9	0.79	0.07	0.8	0.76	0.84	0.8	0.06	0.81	0.78	0.84	1.31	0.29	1.35	1.1	1.53	1.4	1.21	1.06	0.49	1.99	0.63	0.06	0.63	0.6	0.66	0.71	0.06	0.71	0.69	0.74	0.75	0.04	0.75	0.73	0.77	0.81	0.03	0.82	0.8	0.83	67.22	59.33	51.32	38.21	68.19	202.23	134.88	163.12	128.08	222.15	632	0.3
0.18	0.82	0.07	0.84	0.81	0.86	0.72	0.07	0.73	0.68	0.77	0.74	0.06	0.75	0.72	0.78	1.51	0.3	1.54	1.3	1.73	1.58	1.43	1.17	0.5	2.35	0.56	0.06	0.57	0.54	0.6	0.66	0.06	0.66	0.63	0.69	0.71	0.05	0.71	0.68	0.73	0.78	0.03	0.78	0.77	0.8	64.92	51.9	49.27	37.76	67.38	275.01	212.49	226.71	177.76	294.63	872	0.48
0.32	0.78	0.07	0.79	0.75	0.82	0.63	0.09	0.63	0.58	0.69	0.68	0.07	0.68	0.64	0.72	1.71	0.33	1.73	1.47	1.94	1.82	1.62	1.32	0.63	2.6	0.5	0.06	0.5	0.46	0.54	0.61	0.07	0.61	0.57	0.64	0.66	0.05	0.66	0.63	0.69	0.75	0.03	0.75	0.73	0.77	79.8	257.53	49.64	37.85	67.73	436.18	473.06	324.47	248.7	459.76	1098	0.67


==> data_new/ra/yelp/xlnet/A_auc.tex <==
0.28

==> data_new/ra/yelp/xlnet/A_ppl.tex <==
6.7

==> data_new/ra/yelp/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.77	0.36	0.92	0.72	0.98	0.98	0.02	0.98	0.97	0.99	0.79	0.27	0.88	0.74	0.95	1.14	4.17	0.25	0.1	0.66	2.78	4.98	1.11	0.25	3.0	0.69	0.27	0.74	0.59	0.84	0.72	0.23	0.76	0.6	0.89	0.79	0.18	0.82	0.71	0.89	0.85	0.13	0.87	0.8	0.93	136.9	534.28	49.62	37.68	73.0	144.51	533.21	57.84	44.22	83.23	885	0.01
0.03	0.63	0.38	0.78	0.5	0.89	0.95	0.03	0.95	0.93	0.97	0.66	0.28	0.74	0.59	0.84	2.07	9.33	0.49	0.25	1.17	3.89	6.87	1.72	0.73	4.06	0.53	0.23	0.58	0.45	0.69	0.57	0.21	0.6	0.44	0.72	0.68	0.16	0.71	0.62	0.78	0.77	0.12	0.79	0.73	0.84	61.81	43.41	48.84	38.36	67.22	84.59	55.09	69.11	54.71	93.37	759	0.06
0.06	0.53	0.36	0.61	0.37	0.8	0.91	0.04	0.91	0.89	0.94	0.55	0.26	0.6	0.43	0.73	1.75	3.52	0.7	0.36	1.53	4.0	6.1	2.21	1.02	4.47	0.42	0.21	0.46	0.32	0.56	0.47	0.21	0.48	0.33	0.62	0.6	0.15	0.62	0.53	0.7	0.71	0.11	0.73	0.66	0.78	65.95	52.65	49.5	38.62	68.92	115.14	93.81	87.36	68.99	119.67	778	0.12
0.11	0.41	0.37	0.48	0.21	0.68	0.87	0.05	0.87	0.84	0.9	0.43	0.27	0.49	0.32	0.6	1.96	3.74	0.85	0.46	1.67	4.32	6.86	2.39	1.07	5.32	0.32	0.21	0.36	0.23	0.45	0.4	0.2	0.4	0.28	0.54	0.53	0.15	0.55	0.46	0.63	0.67	0.11	0.69	0.62	0.73	103.48	380.66	50.37	38.67	71.59	212.9	673.96	115.67	92.02	153.0	491	0.18
0.15	0.32	0.34	0.36	0.13	0.55	0.79	0.07	0.8	0.76	0.84	0.33	0.23	0.36	0.22	0.47	2.14	3.63	0.96	0.53	2.05	4.72	5.75	3.04	1.38	5.83	0.24	0.17	0.25	0.16	0.34	0.33	0.18	0.32	0.23	0.43	0.47	0.12	0.48	0.41	0.55	0.62	0.1	0.63	0.58	0.68	68.74	60.87	51.32	38.92	70.45	205.74	141.32	162.87	130.23	219.55	456	0.33
0.18	0.27	0.3	0.27	0.1	0.48	0.72	0.07	0.73	0.68	0.77	0.25	0.21	0.27	0.14	0.38	2.15	4.6	0.99	0.55	1.96	4.86	5.6	3.31	1.54	6.15	0.18	0.15	0.19	0.1	0.27	0.28	0.16	0.28	0.17	0.38	0.43	0.11	0.44	0.37	0.5	0.59	0.08	0.59	0.55	0.64	64.71	51.48	49.27	37.82	67.31	272.71	207.14	226.06	177.17	293.78	871	0.54
0.32	0.18	0.27	0.18	0.03	0.35	0.62	0.09	0.63	0.57	0.68	0.18	0.19	0.18	0.08	0.3	2.25	6.78	1.0	0.6	1.92	5.47	6.38	3.58	1.66	7.17	0.12	0.14	0.13	0.05	0.21	0.24	0.16	0.23	0.14	0.32	0.39	0.1	0.39	0.33	0.45	0.56	0.08	0.57	0.52	0.61	79.33	254.67	50.43	37.92	68.03	453.19	428.07	339.18	259.09	477.71	842	0.78


==> data_new/ra/yelp/xlnet/IG_auc.tex <==
0.12

==> data_new/ra/yelp/xlnet/IG_ppl.tex <==
6.0

==> data_new/ra/yelp/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.9	0.16	0.97	0.88	0.99	0.98	0.02	0.98	0.97	0.99	0.93	0.1	0.96	0.92	0.99	120.74	801.97	11.67	4.69	31.13	3.59	6.7	1.14	0.21	3.79	0.84	0.14	0.87	0.78	0.92	0.82	0.17	0.85	0.72	1.0	0.88	0.12	0.91	0.84	0.96	0.92	0.08	0.94	0.89	0.97	139.78	531.27	52.08	39.19	75.37	148.03	530.21	60.06	45.96	89.67	833	0.01
0.03	0.82	0.2	0.9	0.75	0.97	0.95	0.03	0.95	0.93	0.97	0.87	0.13	0.9	0.83	0.95	195.53	993.62	27.17	13.0	69.58	4.94	7.08	2.41	0.75	6.09	0.73	0.14	0.77	0.68	0.83	0.71	0.19	0.72	0.6	0.84	0.8	0.12	0.82	0.75	0.88	0.87	0.08	0.88	0.84	0.92	61.21	42.64	48.81	38.36	66.89	83.61	52.73	69.66	54.39	92.2	722	0.04
0.06	0.77	0.22	0.85	0.67	0.94	0.91	0.04	0.91	0.89	0.94	0.81	0.14	0.85	0.76	0.91	160.14	701.39	35.08	19.09	84.35	6.33	8.9	3.07	1.1	7.63	0.66	0.14	0.69	0.59	0.76	0.64	0.2	0.67	0.5	0.8	0.76	0.12	0.78	0.69	0.83	0.83	0.08	0.85	0.79	0.89	65.56	52.54	49.46	38.72	67.86	114.66	94.77	87.28	68.75	118.36	740	0.08
0.11	0.71	0.23	0.78	0.61	0.9	0.87	0.05	0.87	0.84	0.9	0.77	0.14	0.8	0.72	0.87	182.04	823.61	45.25	25.26	94.87	6.77	9.18	3.53	1.12	8.62	0.61	0.14	0.63	0.55	0.71	0.58	0.22	0.6	0.44	0.72	0.72	0.13	0.73	0.67	0.8	0.81	0.09	0.82	0.77	0.86	103.73	378.35	50.43	38.76	72.51	209.0	615.92	116.65	92.02	153.33	497	0.1
0.15	0.68	0.23	0.73	0.52	0.86	0.79	0.06	0.8	0.76	0.84	0.73	0.15	0.75	0.68	0.83	220.17	996.41	49.76	29.64	106.33	6.66	8.3	3.5	1.27	8.84	0.56	0.14	0.58	0.5	0.66	0.56	0.2	0.57	0.41	0.69	0.69	0.12	0.7	0.62	0.75	0.78	0.08	0.79	0.74	0.84	65.94	56.24	51.1	38.09	67.92	201.56	139.22	162.67	127.91	221.0	625	0.21
0.18	0.63	0.22	0.67	0.46	0.82	0.73	0.07	0.73	0.69	0.77	0.69	0.14	0.71	0.62	0.79	203.68	941.75	56.42	34.48	116.87	7.19	8.99	3.79	1.35	9.43	0.53	0.12	0.53	0.45	0.61	0.52	0.21	0.5	0.38	0.67	0.65	0.11	0.66	0.59	0.72	0.76	0.07	0.77	0.71	0.81	65.43	52.59	50.22	38.13	67.9	277.02	228.56	228.37	177.41	300.38	618	0.33
0.32	0.58	0.24	0.6	0.4	0.77	0.61	0.09	0.61	0.55	0.67	0.62	0.15	0.64	0.53	0.73	231.25	1074.45	65.97	38.61	130.04	7.62	9.2	4.36	1.57	10.23	0.46	0.13	0.47	0.38	0.55	0.47	0.21	0.47	0.33	0.6	0.62	0.11	0.62	0.55	0.68	0.73	0.07	0.74	0.69	0.78	79.56	246.03	50.4	38.21	68.29	488.08	472.78	365.56	272.9	522.68	1212	0.52


==> data_new/ra/yelp/xlnet/S_auc.tex <==
0.22

==> data_new/ra/yelp/xlnet/S_ppl.tex <==
9.9

==> data_new/tef/agnews/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.87	0.16	0.93	0.76	1.0	0.99	0.03	0.99	0.99	1.0	0.94	0.07	0.95	0.89	1.0	1.48	1.53	1.4	0.0	2.66	2.48	3.81	0.62	0.0	3.68	0.87	0.12	0.85	0.78	1.0	0.86	0.14	0.84	0.75	1.0	0.91	0.08	0.9	0.85	1.0	0.94	0.06	0.93	0.9	1.0	247.5	244.84	195.44	129.75	299.09	265.28	250.8	211.37	140.01	324.18	3792	0.02
0.03	0.7	0.18	0.72	0.61	0.83	0.97	0.04	0.98	0.97	0.99	0.83	0.08	0.84	0.79	0.89	2.91	1.2	2.82	2.12	3.66	4.62	4.47	3.31	1.37	6.44	0.71	0.08	0.71	0.66	0.76	0.68	0.11	0.68	0.61	0.75	0.79	0.06	0.8	0.76	0.84	0.86	0.04	0.87	0.84	0.89	246.09	232.39	195.46	129.73	299.63	303.77	252.65	245.52	163.86	370.52	3822	0.05
0.06	0.6	0.22	0.62	0.46	0.75	0.94	0.05	0.95	0.93	0.97	0.74	0.09	0.75	0.69	0.81	3.42	1.2	3.35	2.59	4.18	5.46	4.99	4.06	1.7	7.75	0.59	0.09	0.6	0.54	0.66	0.56	0.12	0.57	0.49	0.65	0.71	0.07	0.71	0.67	0.76	0.81	0.05	0.81	0.78	0.84	247.31	236.76	196.79	129.98	299.74	373.89	352.76	303.5	201.22	449.45	3926	0.12
0.11	0.52	0.23	0.53	0.37	0.68	0.91	0.06	0.93	0.89	0.95	0.67	0.11	0.68	0.61	0.74	3.71	1.16	3.63	2.92	4.42	6.04	5.26	4.7	2.08	8.68	0.52	0.09	0.52	0.46	0.58	0.49	0.13	0.5	0.41	0.58	0.65	0.07	0.66	0.61	0.7	0.77	0.05	0.77	0.74	0.8	243.55	239.97	192.98	129.03	295.42	446.64	519.44	361.89	243.66	536.92	3668	0.19
0.15	0.42	0.24	0.43	0.26	0.6	0.86	0.07	0.88	0.83	0.91	0.58	0.12	0.59	0.51	0.66	3.98	1.11	3.88	3.21	4.64	6.7	5.55	5.3	2.41	9.54	0.43	0.1	0.44	0.37	0.5	0.41	0.13	0.41	0.33	0.5	0.59	0.07	0.59	0.54	0.64	0.73	0.05	0.73	0.69	0.76	246.92	316.7	194.19	128.27	298.98	575.61	444.55	479.91	331.93	712.83	2019	0.3
0.18	0.36	0.24	0.35	0.19	0.53	0.81	0.08	0.83	0.77	0.87	0.5	0.13	0.51	0.42	0.6	4.11	1.06	3.98	3.38	4.7	7.17	5.71	5.85	2.83	10.26	0.37	0.1	0.37	0.3	0.44	0.36	0.13	0.36	0.27	0.45	0.54	0.08	0.55	0.49	0.6	0.69	0.05	0.69	0.66	0.73	248.4	310.82	194.98	129.47	299.92	748.79	457.99	635.86	435.79	940.18	2109	0.46
0.32	0.22	0.23	0.19	0.03	0.38	0.7	0.11	0.71	0.62	0.78	0.36	0.16	0.36	0.25	0.47	4.33	1.02	4.18	3.61	4.86	8.26	6.2	7.04	3.44	11.78	0.25	0.12	0.25	0.17	0.33	0.27	0.13	0.26	0.16	0.35	0.46	0.08	0.47	0.41	0.52	0.63	0.06	0.63	0.59	0.67	245.91	264.55	194.98	130.09	297.98	1304.59	887.31	1088.55	712.14	1620.98	5745	0.99


==> data_new/tef/agnews/bert/A_auc.tex <==
0.14

==> data_new/tef/agnews/bert/A_ppl.tex <==
4.4

==> data_new/tef/agnews/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.63	0.39	0.66	0.34	1.0	0.99	0.02	0.99	0.99	1.0	0.7	0.31	0.73	0.49	1.0	2.28	7.13	0.23	0.0	0.85	4.93	7.08	1.52	0.0	7.71	0.64	0.34	0.59	0.37	1.0	0.66	0.33	0.67	0.4	1.0	0.76	0.23	0.74	0.58	1.0	0.83	0.17	0.81	0.69	1.0	247.7	244.65	195.64	129.77	300.21	262.19	249.9	206.75	138.35	316.22	3800	0.01
0.03	0.19	0.3	0.22	0.0	0.41	0.97	0.03	0.98	0.96	0.99	0.34	0.26	0.37	0.18	0.53	5.28	12.7	0.85	0.41	3.64	9.11	7.69	7.3	3.26	12.89	0.27	0.2	0.28	0.14	0.41	0.3	0.22	0.33	0.17	0.5	0.51	0.15	0.5	0.41	0.62	0.64	0.11	0.65	0.57	0.72	245.66	231.53	195.5	129.87	298.49	295.19	291.03	236.11	156.49	352.99	3851	0.05
0.06	-0.05	0.28	-0.04	-0.24	0.14	0.94	0.04	0.95	0.93	0.97	0.13	0.25	0.14	-0.03	0.3	6.39	13.8	1.17	0.53	5.65	10.8	8.57	8.81	4.33	15.28	0.1	0.18	0.11	-0.02	0.22	0.19	0.18	0.2	0.0	0.33	0.4	0.14	0.4	0.31	0.5	0.57	0.1	0.57	0.5	0.64	243.4	233.56	194.8	128.92	296.0	345.46	322.02	281.18	183.55	418.45	3911	0.1
0.11	-0.21	0.26	-0.21	-0.38	-0.03	0.91	0.05	0.92	0.89	0.94	-0.03	0.24	-0.02	-0.19	0.14	7.74	19.54	1.36	0.61	7.09	11.2	8.87	9.05	4.34	16.08	-0.01	0.18	-0.01	-0.13	0.11	0.12	0.15	0.0	0.0	0.2	0.33	0.14	0.33	0.24	0.42	0.51	0.1	0.52	0.44	0.58	249.4	301.99	194.86	129.52	298.04	420.08	316.72	342.48	222.53	508.81	2482	0.17
0.15	-0.34	0.22	-0.35	-0.5	-0.2	0.87	0.06	0.88	0.83	0.91	-0.15	0.21	-0.15	-0.3	-0.01	7.81	15.16	1.54	0.7	8.22	12.32	9.47	10.06	4.9	17.61	-0.1	0.15	-0.1	-0.21	0.0	0.07	0.12	0.0	0.0	0.17	0.27	0.12	0.27	0.19	0.36	0.47	0.09	0.47	0.41	0.53	240.64	234.04	191.7	128.3	292.04	516.35	373.57	424.51	286.67	628.85	3743	0.28
0.18	-0.43	0.2	-0.45	-0.56	-0.3	0.82	0.07	0.83	0.78	0.87	-0.26	0.19	-0.26	-0.4	-0.13	8.36	15.99	1.77	0.73	9.96	12.3	9.6	10.38	4.66	17.11	-0.18	0.14	-0.18	-0.28	-0.09	0.05	0.1	0.0	0.0	0.0	0.22	0.11	0.21	0.14	0.29	0.43	0.09	0.43	0.37	0.5	250.71	255.07	199.21	132.65	306.91	663.8	451.02	553.74	374.03	800.91	2201	0.4
0.32	-0.52	0.17	-0.54	-0.64	-0.42	0.75	0.09	0.76	0.69	0.82	-0.36	0.17	-0.37	-0.48	-0.25	8.55	16.39	1.86	0.79	10.71	12.36	9.45	10.4	4.83	17.67	-0.26	0.13	-0.26	-0.34	-0.18	0.03	0.08	0.0	0.0	0.0	0.18	0.1	0.17	0.11	0.25	0.39	0.09	0.39	0.33	0.45	247.09	273.44	195.39	129.68	303.54	986.94	699.78	799.46	536.5	1225.63	5166	0.73


==> data_new/tef/agnews/bert/IG_auc.tex <==
-0.08

==> data_new/tef/agnews/bert/IG_ppl.tex <==
4.1

==> data_new/tef/agnews/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.82	0.2	0.86	0.69	1.0	0.99	0.02	0.99	0.99	1.0	0.9	0.12	0.94	0.85	1.0	9.59	36.87	0.77	0.0	3.14	1.26	1.78	0.41	0.0	1.96	0.82	0.18	0.81	0.69	1.0	0.73	0.28	0.8	0.5	1.0	0.86	0.15	0.88	0.74	1.0	0.91	0.09	0.93	0.84	1.0	247.7	244.92	195.46	129.76	299.63	261.0	247.84	207.52	137.95	316.63	3794	0.01
0.03	0.6	0.19	0.62	0.48	0.73	0.97	0.03	0.98	0.96	0.99	0.77	0.14	0.8	0.7	0.87	23.07	55.61	3.76	1.71	14.64	2.24	1.98	1.67	0.76	3.11	0.62	0.13	0.63	0.54	0.71	0.42	0.23	0.4	0.25	0.6	0.69	0.13	0.7	0.61	0.79	0.82	0.08	0.82	0.77	0.88	245.88	231.31	195.8	129.88	299.33	293.83	256.89	235.94	157.55	359.71	3837	0.05
0.06	0.43	0.2	0.45	0.3	0.58	0.94	0.04	0.95	0.93	0.97	0.66	0.17	0.69	0.57	0.79	35.41	84.46	5.96	2.5	23.44	2.94	2.42	2.33	1.06	4.2	0.51	0.14	0.52	0.42	0.61	0.28	0.21	0.25	0.17	0.4	0.6	0.13	0.61	0.5	0.69	0.76	0.09	0.77	0.71	0.83	245.76	257.9	194.8	129.88	297.25	351.93	430.46	279.02	191.38	417.92	4517	0.12
0.11	0.32	0.2	0.33	0.19	0.46	0.91	0.05	0.92	0.89	0.94	0.58	0.19	0.61	0.47	0.72	45.34	97.07	7.63	2.98	33.17	3.52	2.81	2.8	1.38	5.05	0.43	0.15	0.44	0.34	0.54	0.2	0.18	0.2	0.0	0.33	0.54	0.14	0.54	0.44	0.63	0.73	0.1	0.73	0.67	0.79	244.01	266.91	193.9	129.12	296.1	409.03	301.72	339.5	231.33	491.44	3733	0.18
0.15	0.21	0.19	0.21	0.07	0.34	0.86	0.06	0.88	0.83	0.91	0.46	0.22	0.5	0.33	0.62	54.3	113.93	10.56	4.12	46.29	4.18	3.12	3.61	1.63	5.94	0.34	0.16	0.35	0.24	0.45	0.13	0.16	0.0	0.0	0.2	0.47	0.14	0.47	0.37	0.56	0.68	0.1	0.68	0.62	0.75	244.84	301.61	193.16	126.82	298.98	521.28	367.45	432.51	300.79	630.7	2300	0.3
0.18	0.13	0.18	0.12	0.01	0.25	0.81	0.08	0.83	0.77	0.87	0.36	0.23	0.39	0.21	0.53	67.69	128.87	14.0	5.0	66.59	4.27	3.15	3.66	1.79	6.03	0.26	0.16	0.27	0.15	0.37	0.09	0.14	0.0	0.0	0.2	0.41	0.14	0.42	0.32	0.5	0.64	0.1	0.64	0.57	0.71	247.0	303.31	194.49	130.09	296.78	681.24	464.28	561.4	401.43	831.05	2305	0.47
0.32	0.01	0.18	-0.01	-0.12	0.12	0.71	0.11	0.72	0.64	0.79	0.17	0.26	0.17	-0.02	0.35	98.33	155.94	25.46	7.36	125.57	4.82	3.43	4.28	2.03	6.96	0.12	0.18	0.12	-0.01	0.24	0.06	0.11	0.0	0.0	0.0	0.32	0.14	0.32	0.22	0.42	0.56	0.11	0.56	0.5	0.64	248.25	292.01	195.72	130.09	298.98	1168.76	799.66	948.8	649.35	1445.12	5428	0.99


==> data_new/tef/agnews/bert/S_auc.tex <==
0.08

==> data_new/tef/agnews/bert/S_ppl.tex <==
3.7

==> data_new/tef/agnews/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.92	0.13	1.0	0.88	1.0	0.99	0.01	1.0	0.99	1.0	0.96	0.08	1.0	0.93	1.0	2.07	3.19	0.0	0.0	3.91	0.63	1.38	0.0	0.0	0.6	0.94	0.11	1.0	0.89	1.0	0.91	0.14	1.0	0.8	1.0	0.96	0.07	1.0	0.94	1.0	0.97	0.05	1.0	0.96	1.0	261.32	241.49	204.95	137.92	315.57	268.2	240.91	213.72	144.21	322.01	3714	0.01
0.03	0.71	0.18	0.76	0.63	0.85	0.97	0.02	0.97	0.96	0.98	0.82	0.12	0.83	0.75	0.91	6.01	3.07	5.39	3.71	7.7	1.85	1.95	1.2	0.52	2.53	0.76	0.13	0.78	0.7	0.85	0.65	0.17	0.67	0.6	0.75	0.85	0.1	0.87	0.8	0.92	0.89	0.07	0.91	0.86	0.95	256.06	221.49	203.96	137.78	312.66	295.17	222.69	237.7	163.05	360.15	3720	0.05
0.06	0.51	0.23	0.54	0.37	0.68	0.93	0.04	0.94	0.92	0.96	0.66	0.15	0.67	0.57	0.76	8.11	3.69	7.39	5.33	10.3	2.72	2.51	2.01	0.84	3.82	0.59	0.14	0.6	0.51	0.69	0.46	0.21	0.5	0.33	0.6	0.74	0.11	0.75	0.68	0.82	0.83	0.08	0.83	0.79	0.88	259.59	229.12	205.79	138.7	316.41	346.55	273.38	280.27	193.47	423.76	3954	0.11
0.11	0.36	0.25	0.38	0.2	0.54	0.9	0.05	0.91	0.87	0.93	0.51	0.17	0.53	0.41	0.63	9.64	4.14	8.91	6.5	12.2	3.48	2.91	2.74	1.23	4.94	0.45	0.15	0.46	0.36	0.55	0.36	0.22	0.33	0.25	0.5	0.66	0.12	0.67	0.58	0.74	0.77	0.08	0.78	0.72	0.82	259.22	235.75	203.39	136.49	313.36	401.21	318.13	324.74	223.65	480.91	3621	0.19
0.15	0.19	0.26	0.2	0.01	0.38	0.85	0.06	0.86	0.82	0.89	0.34	0.17	0.35	0.24	0.46	11.38	4.7	10.5	7.71	14.46	4.3	3.26	3.63	1.77	6.08	0.3	0.14	0.3	0.21	0.4	0.28	0.21	0.25	0.17	0.4	0.56	0.11	0.57	0.5	0.64	0.7	0.08	0.71	0.65	0.76	250.13	224.73	199.22	135.45	304.97	473.39	357.47	390.75	273.48	572.82	3395	0.3
0.18	0.08	0.27	0.07	-0.11	0.26	0.8	0.07	0.81	0.76	0.85	0.2	0.18	0.2	0.08	0.32	12.48	5.11	11.56	8.49	15.96	4.75	3.49	4.08	2.06	6.69	0.18	0.14	0.18	0.09	0.27	0.24	0.2	0.25	0.0	0.33	0.48	0.12	0.5	0.4	0.56	0.64	0.08	0.65	0.59	0.7	256.43	229.62	202.61	136.96	311.01	585.01	397.94	488.02	344.46	705.8	3677	0.44
0.32	-0.1	0.28	-0.12	-0.3	0.09	0.69	0.1	0.7	0.62	0.76	-0.03	0.21	-0.04	-0.18	0.11	14.43	5.84	13.31	9.88	18.34	5.11	3.7	4.51	2.2	7.35	-0.01	0.16	-0.01	-0.12	0.09	0.17	0.18	0.2	0.0	0.25	0.36	0.13	0.36	0.27	0.45	0.54	0.09	0.54	0.48	0.6	256.16	218.01	203.73	137.58	312.82	936.04	676.34	771.74	534.28	1136.33	10622	0.9


==> data_new/tef/agnews/cnn/IG_auc.tex <==
0.08

==> data_new/tef/agnews/cnn/IG_ppl.tex <==
2.9

==> data_new/tef/agnews/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.08	1.0	0.94	1.0	0.99	0.02	1.0	0.99	1.0	0.96	0.07	1.0	0.96	1.0	23.73	38.33	0.0	0.0	42.12	0.43	0.76	0.0	0.0	0.68	0.94	0.1	1.0	0.89	1.0	0.89	0.21	1.0	0.83	1.0	0.94	0.11	1.0	0.89	1.0	0.96	0.07	1.0	0.94	1.0	261.46	241.55	205.17	137.99	315.55	268.93	241.02	213.79	143.97	322.39	3714	0.01
0.03	0.84	0.13	0.88	0.79	0.93	0.97	0.02	0.98	0.97	0.99	0.85	0.12	0.89	0.79	0.95	68.85	39.66	59.97	40.67	87.82	1.17	0.91	0.98	0.49	1.61	0.77	0.13	0.79	0.69	0.86	0.61	0.31	0.67	0.4	1.0	0.78	0.14	0.79	0.69	0.88	0.87	0.09	0.88	0.81	0.94	256.07	221.61	203.71	137.76	312.86	297.97	225.58	240.87	166.05	359.45	3716	0.06
0.06	0.72	0.18	0.76	0.63	0.85	0.95	0.03	0.95	0.93	0.97	0.74	0.17	0.77	0.65	0.87	96.29	47.07	87.27	61.15	122.27	1.57	1.19	1.33	0.63	2.25	0.62	0.15	0.64	0.53	0.73	0.45	0.32	0.5	0.2	0.67	0.67	0.15	0.68	0.57	0.78	0.8	0.1	0.81	0.74	0.87	259.73	229.15	205.85	138.89	316.36	354.39	269.9	286.59	197.31	423.42	3955	0.12
0.11	0.61	0.22	0.65	0.5	0.77	0.92	0.05	0.93	0.9	0.95	0.64	0.2	0.67	0.52	0.79	119.61	54.77	110.28	77.7	150.21	1.94	1.42	1.66	0.82	2.79	0.51	0.17	0.53	0.41	0.63	0.34	0.3	0.33	0.0	0.5	0.59	0.17	0.59	0.47	0.71	0.74	0.11	0.75	0.68	0.82	259.2	235.68	203.3	136.16	313.45	412.29	298.82	336.58	230.65	497.29	3627	0.2
0.15	0.49	0.25	0.53	0.34	0.68	0.87	0.06	0.88	0.85	0.91	0.51	0.24	0.54	0.36	0.69	147.54	65.14	138.4	96.78	185.55	2.32	1.7	2.01	0.95	3.35	0.39	0.18	0.4	0.27	0.52	0.26	0.28	0.2	0.0	0.5	0.5	0.18	0.5	0.38	0.62	0.68	0.12	0.69	0.6	0.76	251.57	225.33	200.44	135.89	306.74	488.89	321.33	416.15	290.05	591.34	3400	0.32
0.18	0.37	0.27	0.4	0.2	0.58	0.83	0.07	0.84	0.79	0.88	0.38	0.27	0.42	0.22	0.59	169.99	75.35	158.88	109.33	216.35	2.61	1.88	2.28	1.09	3.84	0.29	0.2	0.3	0.16	0.43	0.19	0.26	0.0	0.0	0.33	0.42	0.19	0.42	0.29	0.55	0.62	0.13	0.63	0.54	0.71	255.84	229.3	202.44	136.8	310.86	603.91	392.58	509.98	363.04	735.93	3674	0.46
0.32	0.08	0.34	0.1	-0.16	0.33	0.71	0.1	0.72	0.64	0.79	0.07	0.34	0.09	-0.17	0.33	226.39	103.6	207.84	143.61	292.94	3.19	2.21	2.88	1.4	4.58	0.06	0.24	0.07	-0.11	0.23	0.12	0.22	0.0	0.0	0.2	0.28	0.19	0.27	0.13	0.41	0.49	0.15	0.5	0.39	0.6	255.78	217.99	203.63	137.21	312.02	907.96	628.36	758.62	521.5	1110.67	10511	0.87


==> data_new/tef/agnews/cnn/S_auc.tex <==
0.15

==> data_new/tef/agnews/cnn/S_ppl.tex <==
2.9

==> data_new/tef/agnews/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.86	0.24	1.0	0.78	1.0	0.99	0.01	1.0	0.99	1.0	0.93	0.15	1.0	0.88	1.0	0.59	1.08	0.0	0.0	1.0	1.1	2.95	0.0	0.0	0.9	0.9	0.18	1.0	0.83	1.0	0.89	0.19	1.0	0.8	1.0	0.93	0.12	1.0	0.88	1.0	0.95	0.09	1.0	0.93	1.0	260.36	238.32	204.89	138.46	315.3	267.74	238.3	213.04	145.7	320.48	3751	0.01
0.03	0.54	0.3	0.59	0.36	0.77	0.97	0.02	0.97	0.96	0.98	0.73	0.2	0.78	0.67	0.85	1.68	1.27	1.41	0.96	2.02	3.16	4.17	1.73	0.74	3.84	0.65	0.2	0.7	0.56	0.79	0.6	0.23	0.67	0.5	0.75	0.77	0.15	0.8	0.7	0.88	0.84	0.11	0.86	0.79	0.91	255.73	218.25	204.45	138.44	313.37	294.37	204.68	239.77	164.06	357.74	3758	0.05
0.06	0.3	0.32	0.32	0.08	0.54	0.93	0.04	0.94	0.92	0.96	0.57	0.22	0.6	0.47	0.71	2.19	1.46	1.86	1.36	2.59	4.25	4.74	2.8	1.24	5.45	0.5	0.2	0.53	0.4	0.64	0.41	0.23	0.4	0.25	0.6	0.68	0.15	0.7	0.6	0.79	0.77	0.11	0.79	0.71	0.85	259.32	226.49	205.86	139.82	316.46	346.28	243.08	281.85	194.3	423.34	3992	0.11
0.11	0.14	0.33	0.14	-0.09	0.37	0.9	0.05	0.91	0.87	0.93	0.42	0.23	0.46	0.3	0.58	2.54	1.61	2.15	1.64	2.96	5.29	5.45	3.62	1.58	7.01	0.37	0.2	0.4	0.26	0.51	0.3	0.22	0.25	0.17	0.5	0.6	0.16	0.62	0.5	0.71	0.72	0.12	0.74	0.65	0.8	258.81	231.32	203.96	137.41	315.36	402.76	283.67	329.22	226.53	490.07	3698	0.19
0.15	-0.02	0.32	-0.03	-0.25	0.19	0.85	0.06	0.86	0.82	0.89	0.27	0.23	0.29	0.14	0.42	2.93	1.83	2.44	1.9	3.35	6.53	6.1	4.83	2.17	8.92	0.25	0.19	0.26	0.14	0.38	0.24	0.22	0.25	0.0	0.4	0.52	0.15	0.53	0.42	0.62	0.66	0.11	0.68	0.59	0.74	250.32	221.7	200.78	136.69	307.22	473.06	317.52	401.55	278.44	570.52	3479	0.3
0.18	-0.11	0.31	-0.14	-0.33	0.08	0.8	0.07	0.81	0.76	0.85	0.14	0.23	0.16	0.01	0.3	3.09	1.81	2.57	2.03	3.57	7.32	6.61	5.52	2.52	9.88	0.14	0.18	0.16	0.03	0.27	0.2	0.21	0.2	0.0	0.33	0.45	0.15	0.46	0.36	0.55	0.62	0.11	0.62	0.55	0.69	255.59	226.09	202.44	137.47	311.05	588.81	390.17	495.65	348.84	714.73	3786	0.44
0.32	-0.24	0.29	-0.27	-0.45	-0.05	0.7	0.1	0.71	0.63	0.77	-0.03	0.23	-0.03	-0.18	0.12	3.34	1.99	2.75	2.2	3.79	8.33	7.13	6.51	3.05	11.56	-0.0	0.18	-0.0	-0.12	0.11	0.16	0.19	0.0	0.0	0.25	0.36	0.14	0.36	0.25	0.45	0.54	0.11	0.55	0.47	0.62	255.23	217.34	203.64	137.89	312.12	927.37	654.28	766.96	525.08	1135.7	10597	0.9


==> data_new/tef/agnews/lstm/IG_auc.tex <==
0.02

==> data_new/tef/agnews/lstm/IG_ppl.tex <==
2.9

==> data_new/tef/agnews/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.88	0.19	1.0	0.79	1.0	0.99	0.01	1.0	0.99	1.0	0.94	0.11	1.0	0.92	1.0	17.93	33.49	0.0	0.0	27.67	1.07	2.21	0.0	0.0	1.23	0.9	0.16	1.0	0.82	1.0	0.85	0.23	1.0	0.67	1.0	0.92	0.13	1.0	0.87	1.0	0.95	0.08	1.0	0.92	1.0	260.36	238.32	204.89	138.46	315.3	268.07	238.62	214.11	145.12	321.35	3751	0.01
0.03	0.61	0.2	0.62	0.47	0.75	0.97	0.02	0.98	0.96	0.99	0.79	0.14	0.81	0.71	0.89	51.8	43.01	40.81	26.13	62.11	2.59	2.57	1.85	0.8	3.52	0.67	0.16	0.68	0.56	0.79	0.5	0.23	0.5	0.33	0.67	0.73	0.14	0.75	0.64	0.83	0.83	0.09	0.84	0.78	0.91	255.74	218.26	204.45	138.44	313.37	297.7	212.12	241.09	163.47	363.59	3758	0.06
0.06	0.43	0.19	0.44	0.29	0.57	0.94	0.03	0.95	0.93	0.97	0.67	0.16	0.69	0.57	0.78	69.37	54.2	54.44	37.01	83.08	3.16	2.94	2.33	1.08	4.39	0.53	0.15	0.54	0.43	0.64	0.35	0.21	0.33	0.2	0.5	0.63	0.14	0.64	0.54	0.73	0.77	0.1	0.78	0.71	0.84	259.69	226.66	205.96	139.35	316.86	356.42	265.17	286.57	196.27	431.0	4003	0.13
0.11	0.32	0.18	0.31	0.18	0.44	0.91	0.05	0.92	0.89	0.94	0.57	0.18	0.59	0.46	0.7	84.9	72.77	65.08	45.95	98.65	3.63	3.22	2.78	1.31	5.03	0.44	0.15	0.45	0.34	0.54	0.26	0.19	0.25	0.17	0.4	0.56	0.13	0.56	0.46	0.65	0.73	0.1	0.73	0.67	0.8	257.81	231.36	203.25	137.0	313.36	410.11	301.29	331.6	230.55	492.5	3672	0.2
0.15	0.2	0.16	0.19	0.09	0.31	0.87	0.06	0.88	0.84	0.91	0.45	0.18	0.46	0.33	0.58	99.39	76.08	77.6	54.79	116.78	4.08	3.53	3.2	1.46	5.66	0.33	0.14	0.34	0.24	0.43	0.17	0.17	0.2	0.0	0.25	0.47	0.13	0.47	0.38	0.57	0.68	0.09	0.68	0.62	0.74	249.56	221.88	200.12	135.82	306.0	488.89	337.91	409.15	285.27	593.3	3446	0.33
0.18	0.11	0.15	0.1	0.01	0.21	0.82	0.07	0.83	0.78	0.87	0.34	0.19	0.34	0.21	0.47	111.79	86.8	87.32	59.96	129.96	4.36	3.7	3.43	1.58	6.18	0.24	0.14	0.24	0.15	0.34	0.12	0.15	0.0	0.0	0.25	0.4	0.13	0.4	0.31	0.5	0.63	0.09	0.63	0.57	0.69	255.95	226.13	203.63	138.35	312.38	614.32	417.27	516.02	361.72	753.07	3726	0.48
0.32	-0.02	0.14	-0.03	-0.12	0.07	0.71	0.1	0.72	0.65	0.78	0.13	0.21	0.13	-0.02	0.28	131.87	99.75	104.09	71.13	153.82	5.14	3.98	4.27	2.0	7.31	0.09	0.15	0.09	-0.01	0.19	0.06	0.11	0.0	0.0	0.0	0.29	0.13	0.29	0.2	0.38	0.54	0.1	0.55	0.48	0.61	255.47	216.87	203.64	137.99	312.8	949.79	658.72	793.59	547.58	1152.64	10742	0.92


==> data_new/tef/agnews/lstm/S_auc.tex <==
0.08

==> data_new/tef/agnews/lstm/S_ppl.tex <==
2.9

==> data_new/tef/agnews/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.86	0.27	1.0	0.81	1.0	0.99	0.01	1.0	0.99	1.0	0.85	0.28	1.0	0.81	1.0	0.02	0.03	0.0	0.0	0.03	1.06	2.04	0.0	0.0	1.41	0.82	0.29	1.0	0.68	1.0	0.79	0.34	1.0	0.67	1.0	0.85	0.25	1.0	0.75	1.0	0.9	0.17	1.0	0.83	1.0	260.74	239.05	204.55	138.34	315.81	268.89	238.87	215.45	146.29	322.15	3757	0.01
0.03	0.54	0.36	0.63	0.36	0.82	0.97	0.02	0.97	0.96	0.98	0.52	0.37	0.61	0.3	0.82	0.05	0.03	0.05	0.03	0.07	2.79	2.5	2.12	0.97	3.86	0.44	0.31	0.49	0.25	0.67	0.35	0.36	0.25	0.0	0.67	0.54	0.27	0.57	0.33	0.75	0.69	0.19	0.71	0.57	0.83	256.7	220.58	203.73	138.35	313.66	299.81	222.3	244.17	164.66	362.32	3767	0.06
0.06	0.29	0.4	0.35	0.02	0.61	0.94	0.04	0.95	0.92	0.96	0.27	0.42	0.32	-0.03	0.61	0.07	0.04	0.07	0.04	0.09	3.87	3.06	3.11	1.53	5.4	0.23	0.33	0.25	-0.0	0.48	0.19	0.3	0.0	0.0	0.33	0.38	0.27	0.38	0.15	0.58	0.58	0.2	0.58	0.43	0.72	259.74	227.69	205.45	139.25	316.53	352.82	261.03	287.12	195.07	431.05	3997	0.12
0.11	0.1	0.42	0.12	-0.21	0.42	0.9	0.05	0.91	0.88	0.94	0.09	0.43	0.08	-0.25	0.41	0.09	0.04	0.08	0.05	0.11	4.8	3.59	4.01	2.06	6.76	0.09	0.33	0.08	-0.16	0.32	0.13	0.25	0.0	0.0	0.2	0.29	0.25	0.25	0.07	0.46	0.5	0.2	0.5	0.35	0.64	257.85	231.68	202.38	137.02	312.47	410.9	328.57	332.2	228.99	493.1	3701	0.2
0.15	-0.12	0.41	-0.14	-0.44	0.19	0.86	0.06	0.87	0.83	0.9	-0.11	0.42	-0.16	-0.44	0.18	0.1	0.04	0.09	0.06	0.13	5.84	4.09	5.08	2.63	8.28	-0.07	0.32	-0.1	-0.3	0.15	0.07	0.19	0.0	0.0	0.0	0.2	0.22	0.13	0.0	0.33	0.42	0.19	0.4	0.28	0.54	249.17	221.65	198.93	135.77	304.8	481.61	326.07	409.87	282.7	580.53	3474	0.32
0.18	-0.26	0.39	-0.31	-0.57	0.0	0.81	0.07	0.82	0.77	0.86	-0.25	0.4	-0.31	-0.55	0.01	0.11	0.05	0.11	0.07	0.14	6.32	4.41	5.55	2.8	9.15	-0.17	0.31	-0.2	-0.39	0.02	0.05	0.15	0.0	0.0	0.0	0.15	0.2	0.07	0.0	0.25	0.36	0.18	0.35	0.23	0.48	255.89	226.36	202.08	137.99	311.75	603.17	391.58	508.58	357.09	729.27	3825	0.46
0.32	-0.47	0.34	-0.55	-0.73	-0.28	0.71	0.09	0.72	0.65	0.78	-0.45	0.35	-0.53	-0.71	-0.27	0.12	0.05	0.12	0.09	0.16	7.04	4.83	6.3	3.13	10.19	-0.33	0.28	-0.38	-0.53	-0.18	0.02	0.1	0.0	0.0	0.0	0.08	0.15	0.0	0.0	0.11	0.28	0.16	0.26	0.17	0.38	256.34	219.24	202.62	137.72	313.48	940.25	657.3	774.78	526.79	1140.79	10669	0.91


==> data_new/tef/agnews/lstmatt/A_auc.tex <==
-0.01

==> data_new/tef/agnews/lstmatt/A_ppl.tex <==
2.9

==> data_new/tef/agnews/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.87	0.24	1.0	0.79	1.0	0.99	0.01	1.0	0.99	1.0	0.91	0.16	1.0	0.86	1.0	0.54	1.3	0.0	0.0	0.65	1.76	4.13	0.0	0.0	1.68	0.88	0.2	1.0	0.77	1.0	0.87	0.2	1.0	0.8	1.0	0.92	0.13	1.0	0.87	1.0	0.94	0.1	1.0	0.9	1.0	260.74	239.05	204.55	138.34	315.81	269.29	238.97	215.69	146.24	323.17	3757	0.01
0.03	0.53	0.3	0.59	0.37	0.75	0.97	0.02	0.97	0.96	0.98	0.7	0.21	0.74	0.62	0.83	1.81	2.12	1.23	0.71	2.07	4.48	5.26	2.85	1.18	5.78	0.6	0.2	0.64	0.51	0.74	0.57	0.21	0.6	0.4	0.75	0.75	0.15	0.77	0.67	0.85	0.81	0.11	0.83	0.75	0.89	256.69	220.0	204.26	138.57	313.36	301.87	221.77	246.91	164.7	366.48	3788	0.06
0.06	0.28	0.32	0.3	0.08	0.51	0.93	0.04	0.94	0.92	0.96	0.51	0.24	0.54	0.39	0.67	2.45	3.32	1.81	1.13	2.74	6.08	6.13	4.25	1.92	8.17	0.43	0.2	0.46	0.32	0.57	0.38	0.23	0.33	0.25	0.5	0.64	0.15	0.67	0.55	0.75	0.73	0.12	0.75	0.67	0.82	259.43	227.44	205.09	138.64	316.67	353.05	255.64	285.18	193.5	432.61	4012	0.12
0.11	0.11	0.32	0.11	-0.11	0.34	0.89	0.05	0.91	0.87	0.93	0.36	0.25	0.4	0.22	0.53	2.85	3.87	2.15	1.44	3.23	7.81	7.54	5.8	2.65	10.62	0.3	0.21	0.33	0.18	0.45	0.29	0.22	0.25	0.17	0.5	0.56	0.16	0.58	0.46	0.67	0.67	0.13	0.69	0.61	0.76	256.63	229.02	201.79	137.29	311.41	407.59	292.96	331.19	224.94	500.64	3823	0.2
0.15	-0.03	0.3	-0.04	-0.24	0.17	0.85	0.06	0.86	0.82	0.9	0.23	0.24	0.25	0.09	0.39	3.16	3.27	2.42	1.66	3.57	9.18	8.73	6.9	3.29	11.84	0.2	0.19	0.21	0.08	0.34	0.24	0.21	0.25	0.0	0.4	0.49	0.15	0.5	0.4	0.6	0.63	0.12	0.64	0.56	0.71	248.79	221.08	197.7	135.77	303.24	471.68	304.49	401.31	273.01	577.21	3620	0.31
0.18	-0.13	0.29	-0.14	-0.33	0.06	0.81	0.07	0.81	0.77	0.86	0.13	0.23	0.15	-0.02	0.29	3.23	3.0	2.6	1.83	3.74	9.35	8.23	7.39	3.68	12.44	0.12	0.18	0.13	0.01	0.25	0.21	0.2	0.2	0.0	0.33	0.44	0.15	0.45	0.35	0.55	0.59	0.11	0.6	0.52	0.67	253.85	224.29	200.75	136.09	310.83	581.72	387.45	490.83	341.44	722.63	3863	0.44
0.32	-0.25	0.27	-0.27	-0.45	-0.08	0.71	0.1	0.72	0.65	0.78	-0.01	0.23	-0.01	-0.17	0.16	3.22	2.41	2.69	1.96	3.79	9.52	8.07	7.67	3.68	13.08	0.02	0.18	0.01	-0.11	0.14	0.15	0.18	0.0	0.0	0.25	0.38	0.14	0.38	0.29	0.47	0.54	0.11	0.55	0.47	0.62	257.55	218.27	204.55	138.35	314.29	900.13	640.33	745.27	513.35	1095.69	10359	0.85


==> data_new/tef/agnews/lstmatt/IG_auc.tex <==
0.02

==> data_new/tef/agnews/lstmatt/IG_ppl.tex <==
2.9

==> data_new/tef/agnews/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.86	0.22	1.0	0.75	1.0	0.99	0.01	1.0	0.99	1.0	0.92	0.14	1.0	0.89	1.0	11.86	28.54	0.0	0.0	11.76	1.77	3.33	0.0	0.0	2.2	0.87	0.2	1.0	0.74	1.0	0.82	0.28	1.0	0.6	1.0	0.9	0.16	1.0	0.8	1.0	0.93	0.11	1.0	0.88	1.0	260.74	239.05	204.55	138.34	315.81	268.93	239.03	215.1	146.27	323.75	3757	0.01
0.03	0.57	0.21	0.59	0.43	0.74	0.97	0.02	0.98	0.97	0.99	0.76	0.18	0.81	0.68	0.9	36.73	47.19	23.89	11.43	44.65	4.31	3.82	3.24	1.38	6.25	0.62	0.18	0.64	0.51	0.76	0.44	0.25	0.5	0.25	0.67	0.69	0.17	0.71	0.6	0.82	0.81	0.11	0.83	0.74	0.89	256.7	220.59	203.73	138.35	313.6	303.42	337.93	244.36	164.62	368.92	3767	0.06
0.06	0.4	0.2	0.4	0.26	0.54	0.94	0.04	0.95	0.93	0.97	0.65	0.21	0.7	0.54	0.81	49.08	53.37	33.71	17.14	61.78	5.45	4.32	4.46	2.1	7.91	0.51	0.18	0.53	0.39	0.64	0.28	0.22	0.25	0.0	0.4	0.6	0.17	0.62	0.5	0.73	0.75	0.12	0.77	0.68	0.84	259.73	227.65	205.25	139.18	316.43	356.64	284.63	288.53	198.93	438.77	4002	0.13
0.11	0.28	0.19	0.28	0.15	0.41	0.91	0.05	0.92	0.89	0.94	0.56	0.23	0.6	0.42	0.74	60.43	69.51	41.27	20.71	76.24	6.42	4.89	5.35	2.6	9.24	0.42	0.19	0.44	0.3	0.56	0.2	0.19	0.2	0.0	0.33	0.53	0.17	0.54	0.42	0.67	0.71	0.12	0.73	0.64	0.8	257.75	231.75	202.75	136.84	313.33	414.18	322.8	335.45	230.13	504.97	3705	0.21
0.15	0.17	0.17	0.17	0.05	0.28	0.87	0.05	0.88	0.84	0.91	0.45	0.25	0.49	0.3	0.64	70.68	75.81	49.61	24.45	90.18	7.4	5.21	6.51	3.17	10.66	0.33	0.18	0.34	0.21	0.47	0.12	0.16	0.0	0.0	0.25	0.46	0.16	0.47	0.33	0.57	0.67	0.12	0.68	0.59	0.76	249.92	221.63	198.87	136.12	307.17	487.39	338.42	403.22	286.31	591.85	3483	0.33
0.18	0.09	0.16	0.09	-0.01	0.19	0.83	0.06	0.84	0.79	0.87	0.36	0.25	0.39	0.2	0.55	82.14	85.82	58.37	28.35	103.95	7.92	5.39	7.1	3.57	11.51	0.26	0.18	0.27	0.14	0.4	0.08	0.13	0.0	0.0	0.17	0.4	0.16	0.4	0.29	0.5	0.63	0.12	0.64	0.55	0.71	255.13	225.79	202.03	136.96	310.65	608.4	403.68	511.0	354.06	746.49	3813	0.48
0.32	-0.03	0.16	-0.04	-0.14	0.06	0.73	0.09	0.74	0.67	0.8	0.18	0.26	0.19	0.0	0.37	99.05	97.57	71.23	35.9	129.44	9.13	5.79	8.56	4.42	13.07	0.13	0.18	0.13	0.0	0.25	0.04	0.1	0.0	0.0	0.0	0.29	0.15	0.29	0.19	0.4	0.56	0.12	0.56	0.48	0.64	256.55	216.46	203.57	138.29	313.47	931.25	641.56	772.92	526.76	1144.66	10725	0.91


==> data_new/tef/agnews/lstmatt/S_auc.tex <==
0.07

==> data_new/tef/agnews/lstmatt/S_ppl.tex <==
2.9

==> data_new/tef/agnews/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.8	0.19	0.81	0.67	1.0	0.99	0.02	0.99	0.99	1.0	0.89	0.1	0.9	0.83	1.0	0.81	0.8	0.66	0.0	1.27	1.35	1.87	0.66	0.0	1.97	0.78	0.17	0.74	0.66	1.0	0.73	0.21	0.69	0.57	1.0	0.84	0.13	0.81	0.74	1.0	0.89	0.08	0.88	0.83	1.0	191.33	148.2	153.74	103.67	232.79	207.0	153.24	168.16	113.87	252.37	3773	0.01
0.03	0.59	0.18	0.6	0.48	0.72	0.97	0.03	0.98	0.97	0.99	0.77	0.11	0.78	0.71	0.85	1.41	0.82	1.24	0.82	1.8	2.39	2.4	1.69	0.75	3.23	0.6	0.11	0.61	0.53	0.67	0.51	0.14	0.51	0.41	0.61	0.7	0.09	0.71	0.65	0.76	0.81	0.06	0.81	0.77	0.85	190.35	141.73	153.95	103.76	232.64	239.67	172.01	196.39	132.29	292.7	3792	0.03
0.06	0.44	0.19	0.44	0.31	0.57	0.94	0.04	0.95	0.93	0.97	0.66	0.14	0.68	0.58	0.76	1.76	0.95	1.58	1.08	2.23	3.06	2.91	2.23	1.0	4.22	0.49	0.12	0.5	0.42	0.58	0.4	0.14	0.4	0.3	0.49	0.62	0.09	0.63	0.56	0.69	0.75	0.06	0.76	0.71	0.8	191.91	147.28	154.35	103.8	234.24	306.34	220.84	248.96	169.83	371.91	3855	0.06
0.11	0.34	0.18	0.32	0.21	0.45	0.91	0.05	0.92	0.9	0.95	0.58	0.16	0.59	0.48	0.69	2.03	1.05	1.85	1.29	2.55	3.6	3.26	2.71	1.26	4.96	0.42	0.13	0.43	0.33	0.51	0.33	0.14	0.31	0.23	0.42	0.57	0.1	0.57	0.5	0.63	0.72	0.07	0.72	0.67	0.77	190.95	142.76	154.52	104.16	233.66	397.31	275.67	324.13	224.37	480.56	3853	0.11
0.15	0.22	0.17	0.2	0.1	0.32	0.86	0.06	0.88	0.84	0.91	0.48	0.18	0.49	0.36	0.61	2.38	1.15	2.19	1.55	2.98	4.49	3.92	3.47	1.63	6.31	0.34	0.14	0.34	0.25	0.44	0.26	0.14	0.24	0.16	0.34	0.51	0.1	0.51	0.44	0.58	0.68	0.07	0.68	0.63	0.73	187.58	141.49	150.66	103.02	228.88	565.29	372.07	472.81	328.31	684.75	3982	0.2
0.18	0.15	0.16	0.12	0.04	0.23	0.81	0.08	0.83	0.78	0.87	0.4	0.2	0.41	0.27	0.55	2.62	1.18	2.42	1.79	3.25	5.07	4.28	4.0	1.9	7.16	0.28	0.15	0.28	0.19	0.38	0.22	0.13	0.19	0.12	0.29	0.47	0.11	0.47	0.39	0.54	0.65	0.08	0.65	0.59	0.7	189.23	145.54	152.76	103.12	229.44	804.54	528.5	675.81	471.06	994.71	4275	0.32
0.32	0.05	0.15	0.04	-0.04	0.13	0.72	0.1	0.73	0.66	0.8	0.27	0.23	0.28	0.12	0.44	2.76	1.19	2.55	1.89	3.43	5.82	4.7	4.78	2.24	8.17	0.19	0.16	0.19	0.08	0.3	0.16	0.12	0.13	0.07	0.22	0.4	0.12	0.4	0.32	0.48	0.6	0.09	0.6	0.54	0.66	190.28	142.22	154.35	103.55	232.19	1567.64	1188.74	1249.19	832.48	1928.63	10335	0.72


==> data_new/tef/agnews/roberta/A_auc.tex <==
0.09

==> data_new/tef/agnews/roberta/A_ppl.tex <==
10.1

==> data_new/tef/agnews/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.28	0.61	0.25	-0.19	1.0	0.99	0.02	0.99	0.98	1.0	0.49	0.46	0.51	0.17	1.0	9.61	27.81	5.8	0.0	12.2	7.19	8.16	4.39	0.0	11.68	0.45	0.44	0.38	0.13	1.0	0.52	0.37	0.4	0.2	1.0	0.63	0.29	0.6	0.41	1.0	0.73	0.22	0.71	0.57	1.0	190.44	147.26	151.99	103.81	231.62	209.16	153.72	170.06	116.46	256.63	3864	0.01
0.03	-0.12	0.45	-0.09	-0.46	0.19	0.97	0.03	0.98	0.96	0.98	0.16	0.37	0.18	-0.07	0.42	16.16	22.6	11.42	6.73	19.6	10.13	8.21	8.2	3.65	14.41	0.13	0.29	0.13	-0.05	0.32	0.25	0.23	0.2	0.0	0.4	0.42	0.19	0.42	0.29	0.56	0.58	0.15	0.58	0.48	0.69	190.8	141.9	154.6	104.03	232.64	251.61	244.62	203.01	140.7	302.42	4040	0.04
0.06	-0.3	0.37	-0.28	-0.61	-0.02	0.94	0.04	0.95	0.93	0.96	-0.02	0.32	0.0	-0.22	0.21	23.7	39.78	15.18	9.38	25.89	10.7	8.51	8.63	4.17	15.37	-0.01	0.25	0.01	-0.16	0.15	0.16	0.18	0.17	0.0	0.25	0.34	0.16	0.33	0.21	0.44	0.51	0.13	0.52	0.43	0.59	186.29	135.77	151.9	101.72	230.1	326.31	359.27	263.71	180.32	390.04	5421	0.09
0.11	-0.38	0.33	-0.38	-0.65	-0.13	0.9	0.05	0.91	0.88	0.94	-0.11	0.3	-0.1	-0.31	0.1	22.87	24.22	16.38	10.43	26.45	11.5	8.85	9.39	4.51	16.66	-0.08	0.22	-0.07	-0.22	0.08	0.12	0.16	0.0	0.0	0.2	0.29	0.15	0.29	0.19	0.39	0.48	0.12	0.48	0.4	0.56	186.66	132.75	152.8	104.65	227.87	441.58	286.41	369.03	256.67	536.84	6434	0.16
0.15	-0.41	0.29	-0.41	-0.63	-0.19	0.86	0.06	0.87	0.83	0.9	-0.14	0.27	-0.14	-0.32	0.04	20.68	23.78	15.8	10.35	24.13	11.53	9.01	9.61	4.1	17.26	-0.1	0.2	-0.09	-0.22	0.03	0.09	0.14	0.0	0.0	0.17	0.28	0.14	0.27	0.18	0.37	0.47	0.11	0.47	0.39	0.55	190.22	144.16	154.8	102.63	233.46	633.12	509.76	528.89	359.46	775.47	4315	0.28
0.18	-0.43	0.27	-0.43	-0.63	-0.23	0.82	0.07	0.83	0.78	0.87	-0.18	0.24	-0.17	-0.34	-0.02	19.29	33.18	14.84	9.97	23.33	11.26	8.84	9.21	4.18	16.37	-0.12	0.18	-0.12	-0.24	-0.01	0.08	0.13	0.0	0.0	0.17	0.26	0.13	0.26	0.17	0.33	0.46	0.11	0.46	0.39	0.53	196.02	162.17	153.22	103.77	233.02	878.93	698.57	727.91	503.93	1056.53	2689	0.41
0.32	-0.45	0.24	-0.46	-0.63	-0.28	0.76	0.1	0.78	0.7	0.83	-0.21	0.22	-0.22	-0.36	-0.07	19.1	20.87	14.94	9.74	23.22	10.47	8.18	8.5	3.8	15.37	-0.15	0.17	-0.15	-0.25	-0.05	0.07	0.12	0.0	0.0	0.17	0.25	0.13	0.24	0.16	0.33	0.44	0.1	0.44	0.38	0.5	204.18	187.55	155.7	103.97	251.04	1431.22	1208.1	1059.19	724.98	1691.47	2192	0.71


==> data_new/tef/agnews/roberta/IG_auc.tex <==
-0.11

==> data_new/tef/agnews/roberta/IG_ppl.tex <==
8.5

==> data_new/tef/agnews/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.63	0.32	0.58	0.35	1.0	0.99	0.02	0.99	0.99	1.0	0.83	0.16	0.85	0.74	1.0	27.85	130.31	3.39	0.0	10.16	1.58	1.97	0.9	0.0	2.43	0.73	0.21	0.69	0.57	1.0	0.64	0.3	0.6	0.4	1.0	0.8	0.17	0.79	0.67	1.0	0.87	0.11	0.86	0.78	1.0	191.28	148.17	153.77	103.66	232.35	208.14	153.53	169.22	115.5	255.19	3773	0.01
0.03	0.35	0.22	0.32	0.19	0.49	0.97	0.03	0.98	0.97	0.99	0.68	0.16	0.71	0.59	0.8	61.57	190.12	9.68	4.62	28.8	2.43	2.14	1.88	0.84	3.39	0.53	0.15	0.54	0.44	0.63	0.37	0.23	0.33	0.2	0.5	0.64	0.13	0.65	0.56	0.74	0.77	0.09	0.78	0.72	0.83	190.31	141.72	153.95	103.69	232.33	245.42	190.71	200.7	136.52	300.05	3792	0.03
0.06	0.21	0.17	0.19	0.08	0.32	0.95	0.04	0.95	0.93	0.97	0.56	0.19	0.59	0.45	0.7	105.64	324.35	14.18	6.65	47.13	2.92	2.5	2.25	1.06	4.08	0.42	0.16	0.44	0.32	0.53	0.24	0.2	0.2	0.0	0.33	0.55	0.14	0.56	0.47	0.67	0.72	0.1	0.72	0.66	0.78	190.25	143.77	153.37	103.8	231.13	314.44	213.88	258.46	178.52	379.55	3938	0.07
0.11	0.12	0.15	0.1	0.01	0.2	0.91	0.05	0.92	0.89	0.94	0.46	0.2	0.48	0.34	0.61	126.22	351.32	19.89	9.38	67.12	3.38	2.71	2.72	1.24	4.78	0.34	0.16	0.34	0.24	0.45	0.16	0.18	0.17	0.0	0.25	0.49	0.14	0.5	0.4	0.59	0.68	0.09	0.68	0.61	0.75	189.76	147.32	154.38	102.27	232.27	427.48	284.58	359.96	242.12	522.29	2999	0.13
0.15	0.04	0.13	0.04	-0.04	0.11	0.86	0.06	0.88	0.83	0.91	0.35	0.21	0.37	0.2	0.5	153.46	427.96	24.24	11.29	81.21	3.64	2.78	3.02	1.49	5.12	0.25	0.15	0.26	0.14	0.36	0.11	0.15	0.0	0.0	0.2	0.42	0.14	0.42	0.33	0.53	0.63	0.09	0.62	0.57	0.7	186.88	145.94	150.19	103.13	225.95	620.89	413.41	520.45	350.28	746.08	3173	0.25
0.18	-0.0	0.12	-0.02	-0.08	0.08	0.82	0.07	0.84	0.79	0.87	0.27	0.22	0.27	0.12	0.43	178.58	448.24	29.14	13.38	84.68	3.86	3.03	3.09	1.48	5.5	0.2	0.16	0.19	0.09	0.31	0.07	0.13	0.0	0.0	0.17	0.39	0.14	0.38	0.29	0.47	0.6	0.1	0.6	0.53	0.67	182.49	141.59	146.12	102.15	222.89	840.08	552.8	699.61	480.8	1042.98	2703	0.39
0.32	-0.06	0.12	-0.07	-0.14	0.02	0.76	0.1	0.78	0.7	0.83	0.16	0.23	0.15	0.0	0.33	229.57	512.44	36.24	15.32	150.88	4.07	3.02	3.42	1.68	5.92	0.12	0.16	0.11	0.0	0.23	0.04	0.1	0.0	0.0	0.0	0.32	0.14	0.32	0.22	0.42	0.56	0.1	0.56	0.5	0.63	198.15	157.47	159.08	106.57	240.67	1441.36	1088.36	1169.23	783.3	1770.69	4149	0.67


==> data_new/tef/agnews/roberta/S_auc.tex <==
0.03

==> data_new/tef/agnews/roberta/S_ppl.tex <==
9.3

==> data_new/tef/agnews/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.89	0.09	0.89	0.84	0.96	0.99	0.02	0.99	0.98	1.0	0.94	0.05	0.94	0.91	0.98	0.67	0.43	0.74	0.44	0.94	1.0	1.2	0.59	0.09	1.47	0.84	0.1	0.82	0.77	0.9	0.81	0.12	0.79	0.73	0.89	0.88	0.08	0.87	0.83	0.93	0.92	0.05	0.92	0.89	0.96	198.9	148.55	160.5	107.88	246.89	220.37	155.94	180.43	122.77	276.0	3756	0.02
0.03	0.8	0.09	0.81	0.75	0.86	0.97	0.03	0.98	0.96	0.98	0.88	0.06	0.88	0.84	0.92	1.01	0.31	0.98	0.81	1.19	1.48	1.37	1.09	0.5	2.06	0.72	0.08	0.73	0.68	0.78	0.68	0.09	0.68	0.63	0.74	0.8	0.06	0.8	0.77	0.84	0.87	0.04	0.87	0.85	0.9	199.74	152.16	160.76	107.9	246.97	253.99	175.84	209.09	140.68	313.65	3759	0.04
0.06	0.69	0.11	0.71	0.63	0.77	0.93	0.05	0.95	0.92	0.96	0.8	0.08	0.81	0.76	0.85	1.24	0.33	1.21	1.01	1.43	1.89	1.66	1.47	0.68	2.65	0.63	0.08	0.64	0.58	0.69	0.58	0.1	0.58	0.52	0.64	0.73	0.06	0.73	0.69	0.77	0.82	0.04	0.83	0.8	0.85	199.7	150.06	160.75	107.75	247.1	317.68	214.47	263.72	180.33	398.55	3830	0.09
0.11	0.61	0.12	0.63	0.54	0.7	0.9	0.06	0.91	0.88	0.94	0.74	0.09	0.75	0.68	0.8	1.41	0.35	1.36	1.16	1.6	2.23	1.93	1.71	0.78	3.12	0.56	0.09	0.57	0.51	0.62	0.51	0.1	0.51	0.44	0.57	0.68	0.06	0.68	0.64	0.72	0.79	0.05	0.79	0.76	0.82	198.07	144.4	160.49	107.85	246.38	401.93	260.87	339.54	232.49	496.06	3791	0.16
0.15	0.51	0.13	0.52	0.43	0.6	0.84	0.08	0.86	0.81	0.89	0.66	0.11	0.67	0.59	0.73	1.6	0.38	1.56	1.34	1.8	2.7	2.27	2.16	0.97	3.78	0.49	0.09	0.49	0.43	0.55	0.43	0.1	0.43	0.36	0.5	0.62	0.07	0.62	0.58	0.67	0.75	0.05	0.75	0.72	0.78	199.21	152.26	159.7	107.78	246.3	559.48	343.92	472.56	333.13	692.34	3766	0.27
0.18	0.43	0.13	0.43	0.34	0.53	0.77	0.09	0.79	0.73	0.84	0.59	0.12	0.59	0.52	0.67	1.74	0.41	1.7	1.46	1.96	3.11	2.57	2.51	1.15	4.38	0.43	0.09	0.43	0.37	0.49	0.37	0.1	0.37	0.3	0.44	0.58	0.07	0.58	0.53	0.62	0.72	0.05	0.72	0.69	0.75	198.72	147.24	160.8	107.89	246.89	780.55	488.3	663.86	465.24	951.72	4103	0.44
0.32	0.31	0.13	0.31	0.22	0.4	0.65	0.13	0.66	0.57	0.74	0.47	0.14	0.48	0.38	0.57	1.9	0.42	1.86	1.62	2.13	3.61	2.92	2.96	1.34	5.13	0.33	0.1	0.33	0.26	0.4	0.29	0.09	0.28	0.22	0.35	0.51	0.08	0.51	0.46	0.56	0.67	0.06	0.67	0.63	0.71	198.27	147.32	160.49	107.9	246.55	1423.72	1050.13	1162.49	792.96	1755.75	10739	0.94


==> data_new/tef/agnews/xlnet/A_auc.tex <==
0.17

==> data_new/tef/agnews/xlnet/A_ppl.tex <==
6.6

==> data_new/tef/agnews/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.55	0.39	0.61	0.35	0.83	0.98	0.02	0.99	0.98	0.99	0.62	0.32	0.67	0.45	0.85	1.95	4.13	0.53	0.18	1.62	1.15	1.37	0.75	0.14	1.66	0.53	0.31	0.51	0.33	0.7	0.53	0.31	0.5	0.33	0.8	0.67	0.22	0.67	0.53	0.82	0.77	0.16	0.77	0.68	0.88	199.21	146.33	163.03	109.13	245.97	220.97	154.36	181.32	122.65	279.2	3967	0.02
0.03	0.28	0.37	0.35	0.08	0.55	0.96	0.04	0.97	0.95	0.98	0.38	0.31	0.44	0.2	0.6	3.43	7.06	1.08	0.49	3.21	1.67	1.43	1.3	0.64	2.31	0.29	0.24	0.32	0.15	0.46	0.31	0.22	0.33	0.17	0.5	0.51	0.17	0.53	0.41	0.63	0.66	0.13	0.68	0.59	0.75	199.02	149.03	159.58	107.49	247.1	254.74	183.41	207.33	141.25	317.21	4161	0.04
0.06	0.05	0.31	0.05	-0.14	0.27	0.93	0.05	0.94	0.91	0.96	0.17	0.27	0.19	-0.02	0.36	5.41	10.94	1.72	0.74	5.37	2.02	1.71	1.62	0.77	2.82	0.12	0.2	0.14	-0.01	0.26	0.19	0.18	0.17	0.0	0.33	0.4	0.15	0.4	0.31	0.5	0.58	0.11	0.59	0.5	0.66	199.54	148.02	158.75	108.13	249.69	324.12	234.58	267.45	179.87	403.91	5169	0.09
0.11	-0.08	0.28	-0.07	-0.27	0.11	0.88	0.06	0.9	0.86	0.93	0.04	0.25	0.05	-0.13	0.22	5.22	11.12	1.79	0.81	5.89	2.05	1.66	1.66	0.77	2.9	0.03	0.18	0.04	-0.09	0.16	0.14	0.16	0.17	0.0	0.2	0.34	0.14	0.33	0.26	0.42	0.53	0.1	0.53	0.46	0.6	196.36	143.72	157.84	105.01	246.55	415.47	286.49	340.69	234.82	512.79	4660	0.17
0.15	-0.21	0.24	-0.22	-0.37	-0.06	0.82	0.08	0.84	0.78	0.88	-0.1	0.22	-0.1	-0.25	0.06	5.79	8.97	1.86	0.89	6.47	2.26	1.75	1.89	0.89	3.22	-0.07	0.16	-0.07	-0.18	0.04	0.08	0.13	0.0	0.0	0.17	0.28	0.12	0.27	0.2	0.37	0.48	0.09	0.48	0.41	0.55	197.06	149.94	158.77	108.01	239.57	578.9	387.71	492.87	333.03	697.91	4238	0.29
0.18	-0.3	0.22	-0.31	-0.45	-0.18	0.77	0.09	0.78	0.72	0.83	-0.2	0.21	-0.21	-0.34	-0.06	6.23	8.81	2.1	0.93	8.1	2.33	1.82	1.86	0.93	3.35	-0.14	0.15	-0.14	-0.24	-0.04	0.06	0.11	0.0	0.0	0.17	0.24	0.11	0.22	0.16	0.32	0.45	0.09	0.44	0.38	0.5	198.49	144.4	164.75	108.55	246.35	784.8	494.59	676.69	467.94	970.54	4163	0.45
0.32	-0.38	0.17	-0.39	-0.5	-0.28	0.69	0.11	0.71	0.63	0.77	-0.28	0.17	-0.29	-0.4	-0.17	6.7	9.17	2.27	1.0	8.95	2.35	1.85	1.93	0.92	3.34	-0.19	0.13	-0.2	-0.28	-0.11	0.04	0.09	0.0	0.0	0.0	0.2	0.1	0.2	0.12	0.26	0.42	0.08	0.41	0.36	0.47	200.08	151.83	160.75	108.17	247.28	1277.18	958.14	1035.17	720.61	1554.91	7032	0.81


==> data_new/tef/agnews/xlnet/IG_auc.tex <==
-0.04

==> data_new/tef/agnews/xlnet/IG_ppl.tex <==
6.6

==> data_new/tef/agnews/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.76	0.25	0.83	0.66	0.95	0.98	0.02	0.99	0.98	0.99	0.87	0.17	0.94	0.84	0.98	210.43	725.71	30.32	8.38	127.16	1.61	2.03	1.0	0.17	2.28	0.77	0.2	0.81	0.69	0.89	0.66	0.28	0.67	0.5	0.83	0.82	0.17	0.84	0.74	0.95	0.89	0.11	0.91	0.84	0.97	197.6	145.82	159.97	107.93	244.91	217.34	151.36	178.72	120.97	273.12	4052	0.02
0.03	0.6	0.27	0.67	0.42	0.81	0.96	0.03	0.97	0.95	0.98	0.77	0.22	0.86	0.7	0.93	329.71	831.39	86.82	29.55	322.4	2.33	2.25	1.61	0.72	3.15	0.63	0.21	0.7	0.53	0.78	0.46	0.26	0.5	0.25	0.67	0.71	0.19	0.75	0.62	0.84	0.82	0.12	0.84	0.77	0.91	200.26	149.88	163.41	107.41	250.93	255.57	184.93	207.89	141.36	318.51	4464	0.04
0.06	0.42	0.26	0.44	0.2	0.64	0.93	0.05	0.94	0.91	0.96	0.65	0.24	0.71	0.5	0.85	533.58	1116.27	167.69	53.73	507.77	3.35	2.99	2.52	1.14	4.65	0.51	0.21	0.54	0.36	0.68	0.29	0.23	0.33	0.17	0.5	0.61	0.18	0.63	0.47	0.75	0.76	0.12	0.78	0.69	0.86	196.67	137.22	162.68	108.62	248.68	328.66	246.27	270.84	183.97	410.05	5910	0.1
0.11	0.39	0.23	0.39	0.22	0.56	0.88	0.06	0.9	0.85	0.93	0.64	0.21	0.69	0.52	0.8	533.16	1049.66	183.78	65.38	566.04	3.44	2.91	2.72	1.18	4.81	0.49	0.18	0.51	0.37	0.62	0.27	0.2	0.25	0.17	0.4	0.59	0.16	0.61	0.5	0.71	0.76	0.11	0.77	0.69	0.83	200.33	149.22	160.93	107.03	246.94	434.21	323.85	358.23	245.56	533.58	5296	0.18
0.15	0.35	0.2	0.35	0.21	0.5	0.82	0.08	0.84	0.78	0.88	0.61	0.19	0.65	0.51	0.75	683.34	1094.11	236.87	71.15	801.18	3.29	2.61	2.69	1.27	4.7	0.46	0.15	0.48	0.37	0.57	0.24	0.19	0.2	0.0	0.33	0.58	0.14	0.58	0.5	0.67	0.74	0.1	0.75	0.69	0.81	193.58	143.58	155.86	105.86	240.66	565.97	408.09	473.52	322.78	708.3	3692	0.29
0.18	0.3	0.19	0.3	0.17	0.43	0.76	0.1	0.78	0.71	0.83	0.56	0.18	0.58	0.44	0.7	927.18	1584.63	304.04	92.77	1133.19	3.43	2.65	2.91	1.4	4.83	0.41	0.15	0.42	0.32	0.52	0.2	0.18	0.17	0.0	0.33	0.54	0.13	0.54	0.47	0.63	0.72	0.09	0.72	0.66	0.78	200.65	155.94	157.45	109.39	244.99	790.17	595.72	664.62	469.1	960.74	3403	0.44
0.32	0.2	0.18	0.19	0.07	0.32	0.65	0.13	0.67	0.57	0.75	0.42	0.21	0.44	0.28	0.58	1208.63	1489.38	571.26	152.94	1783.88	3.75	2.79	3.18	1.49	5.42	0.31	0.16	0.31	0.2	0.42	0.15	0.16	0.17	0.0	0.25	0.47	0.13	0.47	0.38	0.56	0.67	0.1	0.67	0.61	0.73	201.12	156.55	160.93	108.62	247.28	1343.12	976.13	1115.6	741.88	1658.76	6938	0.86


==> data_new/tef/agnews/xlnet/S_auc.tex <==
0.12

==> data_new/tef/agnews/xlnet/S_ppl.tex <==
6.6

==> data_new/tef/fakenews/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.61	0.39	0.87	0.13	0.91	0.98	0.01	0.99	0.98	0.99	0.8	0.25	0.94	0.7	0.97	4.46	6.29	1.31	0.95	4.25	56.19	85.29	4.09	2.06	114.61	0.7	0.26	0.84	0.53	0.89	0.8	0.1	0.83	0.76	0.85	0.81	0.17	0.89	0.7	0.9	0.85	0.14	0.92	0.76	0.95	53.71	29.0	42.47	38.95	53.13	63.22	33.93	49.4	46.78	63.65	18	0.03
0.03	0.43	0.4	0.31	0.08	0.82	0.97	0.02	0.97	0.96	0.98	0.69	0.25	0.74	0.51	0.91	7.08	8.08	1.69	1.04	13.31	87.45	99.48	26.16	3.91	170.94	0.57	0.26	0.61	0.37	0.78	0.76	0.1	0.74	0.7	0.84	0.75	0.18	0.84	0.6	0.89	0.78	0.13	0.78	0.68	0.9	54.81	35.1	41.43	38.6	48.29	76.27	53.93	55.36	53.28	67.36	12	0.07
0.06	0.4	0.37	0.29	0.07	0.76	0.93	0.04	0.94	0.92	0.95	0.68	0.24	0.74	0.51	0.9	7.36	8.22	1.98	1.2	13.97	90.01	98.19	31.99	5.95	171.21	0.55	0.24	0.59	0.38	0.77	0.73	0.11	0.72	0.66	0.82	0.74	0.16	0.83	0.6	0.86	0.77	0.12	0.76	0.68	0.88	54.81	35.1	41.43	38.6	48.29	92.05	55.96	71.09	65.99	90.08	12	0.12
0.11	0.25	0.31	0.09	0.04	0.53	0.88	0.04	0.87	0.84	0.91	0.64	0.18	0.68	0.55	0.73	12.38	8.77	18.87	2.0	20.12	118.71	80.74	153.59	28.09	162.02	0.5	0.17	0.51	0.4	0.61	0.75	0.09	0.77	0.67	0.83	0.72	0.13	0.79	0.63	0.85	0.74	0.09	0.75	0.69	0.77	47.54	28.44	41.43	31.36	41.9	109.54	51.24	93.55	92.75	106.91	20	0.24
0.15	0.4	0.3	0.46	0.04	0.67	0.85	0.06	0.87	0.79	0.89	0.57	0.24	0.59	0.29	0.78	7.57	9.03	2.03	1.44	17.9	101.48	99.49	45.19	30.82	228.72	0.44	0.21	0.43	0.21	0.64	0.68	0.11	0.66	0.56	0.79	0.63	0.14	0.62	0.49	0.77	0.71	0.12	0.69	0.59	0.81	47.53	30.62	41.23	33.01	41.53	142.2	77.29	133.68	95.53	145.13	14	0.36
0.18	0.57	0.25	0.66	0.58	0.71	0.81	0.07	0.81	0.77	0.84	0.71	0.24	0.82	0.66	0.86	2.8	3.18	2.11	0.93	2.34	57.3	82.66	31.28	14.33	37.47	0.56	0.21	0.66	0.5	0.68	0.63	0.08	0.62	0.56	0.68	0.7	0.12	0.73	0.71	0.77	0.78	0.13	0.84	0.71	0.87	62.54	43.88	42.56	39.8	57.87	262.23	190.79	202.05	170.92	218.13	6	0.58
0.32	0.53	0.23	0.62	0.48	0.67	0.7	0.1	0.68	0.64	0.75	0.65	0.23	0.77	0.53	0.8	2.89	3.1	2.19	0.61	2.45	62.59	77.12	38.14	10.92	52.64	0.5	0.19	0.6	0.39	0.63	0.6	0.08	0.56	0.55	0.66	0.66	0.1	0.69	0.65	0.71	0.76	0.11	0.81	0.67	0.84	62.54	41.84	42.56	39.19	62.66	408.26	226.4	346.39	282.13	434.09	12	1.0


==> data_new/tef/fakenews/bert/A_auc.tex <==
0.15

==> data_new/tef/fakenews/bert/A_ppl.tex <==
5.5

==> data_new/tef/fakenews/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.14	0.78	0.19	-0.35	0.68	0.99	0.0	0.99	0.99	0.99	0.44	0.51	0.58	0.3	0.72	0.81	1.05	0.52	0.0	1.33	19.7	25.62	10.94	2.41	28.23	0.4	0.44	0.48	0.26	0.62	0.46	0.17	0.45	0.39	0.52	0.6	0.24	0.63	0.5	0.73	0.73	0.22	0.78	0.67	0.83	64.69	57.11	38.62	36.37	66.94	77.61	72.83	43.75	41.77	79.58	4	0.05
0.03	0.01	0.75	-0.03	-0.43	0.41	0.98	0.0	0.98	0.98	0.98	0.33	0.49	0.37	0.09	0.6	0.93	1.2	0.6	0.01	1.53	37.59	35.12	34.61	12.55	59.65	0.28	0.42	0.29	0.08	0.5	0.4	0.14	0.39	0.3	0.49	0.54	0.25	0.52	0.39	0.67	0.66	0.19	0.66	0.57	0.75	64.69	57.11	38.62	36.37	66.94	81.13	68.68	50.12	47.64	83.62	4	0.07
0.06	-0.19	0.47	-0.32	-0.32	-0.32	0.96	0.02	0.97	0.97	0.97	0.2	0.25	0.18	0.18	0.18	1.13	0.75	1.29	1.29	1.29	29.33	25.99	18.98	18.98	18.98	0.17	0.21	0.14	0.14	0.14	0.29	0.11	0.24	0.24	0.24	0.44	0.12	0.41	0.41	0.41	0.62	0.1	0.61	0.61	0.61	50.52	37.47	39.19	39.19	39.19	80.3	75.0	54.85	54.85	54.85	9	0.16
0.11	0.04	0.86	0.11	-0.37	0.49	0.92	0.03	0.93	0.91	0.94	0.19	0.46	0.29	-0.01	0.44	0.83	1.42	0.01	0.01	1.24	55.02	41.23	60.23	35.83	76.81	0.16	0.37	0.23	-0.0	0.36	0.31	0.05	0.33	0.29	0.33	0.45	0.17	0.51	0.39	0.55	0.62	0.2	0.64	0.52	0.72	73.19	66.77	38.06	34.69	94.12	151.75	130.53	79.09	76.4	190.76	3	0.28
0.15	0.03	0.85	0.08	-0.39	0.46	0.87	0.03	0.88	0.86	0.88	0.15	0.42	0.24	-0.03	0.37	0.86	1.47	0.01	0.01	1.28	56.35	45.02	60.66	35.0	79.86	0.12	0.33	0.19	-0.02	0.3	0.31	0.05	0.33	0.29	0.33	0.43	0.15	0.46	0.36	0.51	0.6	0.19	0.62	0.52	0.7	73.19	66.77	38.06	34.69	94.12	179.05	116.22	118.17	112.05	215.61	3	0.38
0.18	-0.86	0.0	-0.86	-0.86	-0.86	0.79	0.0	0.79	0.79	0.79	-0.31	0.0	-0.31	-0.31	-0.31	2.58	0.0	2.58	2.58	2.58	61.56	0.0	61.56	61.56	61.56	-0.24	0.0	-0.24	-0.24	-0.24	0.25	0.0	0.25	0.25	0.25	0.25	0.0	0.25	0.25	0.25	0.41	0.0	0.41	0.41	0.41	31.33	0.0	31.33	31.33	31.33	150.28	0.0	150.28	150.28	150.28	3	1.0


==> data_new/tef/fakenews/bert/IG_auc.tex <==
-0.01

==> data_new/tef/fakenews/bert/IG_ppl.tex <==
3.8

==> data_new/tef/fakenews/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.49	0.28	0.44	0.24	0.74	0.98	0.01	0.98	0.98	0.99	0.73	0.2	0.81	0.6	0.87	1374.23	3046.18	2.59	0.07	302.45	34.07	41.63	14.2	5.66	39.12	0.58	0.19	0.62	0.43	0.7	0.56	0.19	0.61	0.35	0.69	0.71	0.14	0.74	0.58	0.82	0.79	0.1	0.82	0.72	0.86	53.04	37.82	41.63	32.31	52.19	60.81	39.88	48.31	38.34	63.76	59	0.03
0.03	0.41	0.3	0.38	0.15	0.64	0.97	0.02	0.97	0.96	0.98	0.66	0.24	0.75	0.49	0.84	166.04	288.21	7.32	0.08	280.52	35.94	41.39	13.95	7.63	47.35	0.51	0.21	0.57	0.34	0.66	0.49	0.22	0.59	0.28	0.67	0.65	0.16	0.7	0.54	0.78	0.76	0.11	0.79	0.69	0.84	53.98	37.79	41.9	39.03	52.19	71.14	41.08	59.42	52.49	72.37	39	0.06
0.06	0.38	0.25	0.32	0.25	0.47	0.93	0.03	0.94	0.92	0.95	0.67	0.18	0.73	0.6	0.81	80.32	106.06	18.55	0.18	164.62	28.63	37.11	12.25	10.01	26.23	0.5	0.16	0.55	0.42	0.62	0.49	0.18	0.54	0.33	0.65	0.65	0.11	0.67	0.61	0.72	0.76	0.08	0.76	0.69	0.83	61.2	37.1	48.16	42.71	58.22	105.89	47.05	96.13	74.75	101.8	44	0.14
0.11	0.47	0.24	0.44	0.3	0.66	0.9	0.03	0.91	0.89	0.92	0.72	0.13	0.73	0.67	0.83	122.9	468.87	0.21	0.05	4.98	16.02	16.29	10.97	5.17	21.88	0.54	0.12	0.56	0.48	0.64	0.5	0.16	0.5	0.4	0.62	0.68	0.09	0.66	0.62	0.76	0.78	0.06	0.79	0.76	0.83	60.19	46.95	43.04	38.83	55.21	117.31	51.51	101.04	91.49	126.3	23	0.19
0.15	0.34	0.21	0.28	0.22	0.43	0.85	0.03	0.84	0.83	0.87	0.65	0.14	0.68	0.57	0.74	86.05	390.13	0.21	0.09	1.53	29.69	32.23	23.95	5.91	32.87	0.48	0.12	0.5	0.42	0.55	0.44	0.16	0.41	0.33	0.55	0.64	0.09	0.65	0.56	0.71	0.75	0.06	0.76	0.72	0.79	53.08	38.04	41.68	38.06	53.59	151.9	65.53	147.33	126.84	163.36	38	0.37
0.18	0.34	0.19	0.38	0.2	0.44	0.79	0.05	0.8	0.76	0.82	0.65	0.13	0.69	0.6	0.77	172.23	544.88	0.7	0.09	9.72	18.75	14.58	15.11	9.9	25.93	0.48	0.11	0.51	0.43	0.58	0.43	0.19	0.44	0.26	0.62	0.63	0.1	0.65	0.58	0.71	0.75	0.06	0.76	0.73	0.79	51.54	37.61	41.63	35.78	51.89	206.83	116.75	197.61	152.6	233.26	39	0.59
0.32	0.35	0.19	0.32	0.22	0.43	0.74	0.07	0.74	0.7	0.78	0.6	0.19	0.66	0.56	0.74	407.19	896.34	0.59	0.07	67.8	17.35	19.83	9.2	3.55	27.84	0.44	0.15	0.47	0.41	0.55	0.43	0.16	0.45	0.33	0.57	0.61	0.12	0.62	0.56	0.7	0.73	0.07	0.74	0.72	0.77	64.71	51.54	42.61	36.44	62.66	338.24	211.39	265.24	232.67	346.95	36	0.83


==> data_new/tef/fakenews/bert/S_auc.tex <==
0.12

==> data_new/tef/fakenews/bert/S_ppl.tex <==
5.1

==> data_new/tef/fakenews/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.69	0.26	0.73	0.49	0.93	0.98	0.02	0.98	0.97	0.99	0.84	0.09	0.86	0.79	0.91	3.58	2.48	3.23	2.16	4.47	17.52	17.83	11.47	3.12	27.86	0.79	0.12	0.79	0.7	0.89	0.81	0.09	0.8	0.75	0.86	0.88	0.07	0.88	0.83	0.94	0.9	0.06	0.9	0.86	0.95	79.71	235.83	42.98	34.52	56.45	85.66	235.28	49.1	39.54	63.69	4050	0.02
0.03	0.6	0.27	0.6	0.39	0.86	0.96	0.02	0.96	0.95	0.97	0.75	0.09	0.76	0.69	0.81	4.43	2.91	3.83	2.82	5.21	21.66	20.08	15.87	5.26	32.64	0.69	0.11	0.69	0.61	0.78	0.7	0.09	0.7	0.63	0.76	0.83	0.07	0.83	0.78	0.88	0.86	0.06	0.87	0.83	0.91	55.64	66.71	42.49	34.4	54.81	70.16	72.63	56.36	46.04	70.35	3895	0.06
0.06	0.54	0.28	0.52	0.32	0.82	0.93	0.03	0.93	0.91	0.95	0.64	0.1	0.64	0.57	0.7	5.21	3.68	4.4	3.32	5.85	23.77	21.8	17.57	6.19	36.0	0.58	0.11	0.58	0.51	0.66	0.59	0.12	0.59	0.52	0.65	0.77	0.07	0.77	0.73	0.81	0.82	0.06	0.83	0.79	0.87	61.32	124.92	42.49	34.17	55.1	90.59	164.4	68.94	56.63	85.59	3788	0.12
0.11	0.49	0.28	0.44	0.27	0.75	0.89	0.04	0.9	0.87	0.92	0.53	0.11	0.53	0.46	0.6	5.66	3.92	4.83	3.71	6.32	25.08	22.47	19.1	6.74	37.49	0.48	0.11	0.48	0.41	0.55	0.52	0.12	0.51	0.44	0.59	0.71	0.07	0.71	0.67	0.75	0.78	0.06	0.79	0.75	0.82	61.53	117.5	42.6	34.36	55.02	109.26	177.34	84.09	69.85	102.89	2873	0.19
0.15	0.43	0.27	0.37	0.23	0.66	0.84	0.04	0.84	0.82	0.87	0.39	0.11	0.39	0.32	0.46	6.32	4.21	5.4	4.19	6.96	26.06	22.96	19.7	7.17	39.47	0.35	0.1	0.35	0.29	0.41	0.46	0.12	0.45	0.38	0.51	0.63	0.06	0.62	0.58	0.66	0.72	0.05	0.73	0.69	0.76	56.84	76.98	42.38	34.41	54.52	134.27	155.63	111.25	94.5	133.02	2096	0.33
0.18	0.39	0.27	0.33	0.19	0.59	0.78	0.05	0.79	0.75	0.81	0.3	0.13	0.28	0.21	0.36	6.86	4.57	5.84	4.58	7.51	26.06	23.52	19.57	6.78	40.26	0.26	0.1	0.25	0.19	0.31	0.41	0.13	0.39	0.33	0.46	0.56	0.07	0.55	0.52	0.59	0.67	0.05	0.67	0.64	0.71	59.17	77.42	42.27	34.31	54.78	173.66	156.47	145.58	123.93	171.29	1620	0.47
0.32	0.34	0.27	0.27	0.16	0.5	0.69	0.07	0.69	0.64	0.74	0.19	0.13	0.18	0.11	0.27	7.84	5.54	6.44	5.15	8.7	26.44	23.55	19.76	7.59	40.08	0.16	0.11	0.15	0.09	0.21	0.35	0.13	0.33	0.26	0.41	0.48	0.08	0.48	0.43	0.52	0.61	0.06	0.61	0.57	0.64	59.85	110.11	42.0	33.84	54.74	252.1	212.42	215.9	173.85	277.55	2348	0.78


==> data_new/tef/fakenews/cnn/IG_auc.tex <==
0.15

==> data_new/tef/fakenews/cnn/IG_ppl.tex <==
4.1

==> data_new/tef/fakenews/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.85	0.11	0.87	0.8	0.92	0.98	0.01	0.98	0.98	0.99	0.92	0.05	0.93	0.9	0.96	40.24	38.89	29.86	20.76	45.25	11.25	12.0	7.68	2.75	15.29	0.85	0.09	0.87	0.78	0.91	0.77	0.11	0.76	0.69	0.83	0.88	0.07	0.89	0.84	0.92	0.93	0.05	0.94	0.9	0.96	79.73	235.77	42.96	34.43	56.42	86.47	235.28	49.88	40.2	64.15	4057	0.02
0.03	0.77	0.12	0.79	0.71	0.85	0.96	0.02	0.96	0.95	0.97	0.86	0.06	0.86	0.82	0.9	51.57	46.09	38.33	28.66	55.94	14.24	13.89	10.48	4.1	19.65	0.75	0.09	0.76	0.7	0.81	0.66	0.12	0.67	0.59	0.73	0.81	0.07	0.82	0.77	0.85	0.89	0.05	0.89	0.86	0.92	55.98	69.22	42.49	34.37	54.82	72.41	80.14	57.38	46.98	72.01	3899	0.08
0.06	0.7	0.14	0.72	0.62	0.79	0.93	0.03	0.93	0.91	0.95	0.78	0.08	0.78	0.73	0.83	67.54	67.54	47.41	35.85	70.86	16.38	15.84	11.59	4.61	23.35	0.65	0.09	0.65	0.6	0.7	0.59	0.14	0.58	0.51	0.67	0.73	0.08	0.73	0.69	0.78	0.84	0.05	0.84	0.8	0.87	62.36	132.46	42.35	34.02	55.1	93.6	129.46	70.58	58.17	88.19	4021	0.13
0.11	0.63	0.15	0.64	0.54	0.73	0.89	0.03	0.9	0.88	0.92	0.7	0.1	0.7	0.65	0.76	70.65	56.11	55.41	41.82	80.37	18.51	17.64	13.49	5.32	26.48	0.56	0.09	0.56	0.51	0.61	0.53	0.15	0.51	0.44	0.6	0.67	0.08	0.66	0.62	0.71	0.79	0.06	0.79	0.76	0.82	64.05	126.42	42.88	34.68	55.41	115.53	182.7	87.45	73.11	107.74	3929	0.22
0.15	0.55	0.15	0.55	0.45	0.65	0.84	0.04	0.84	0.82	0.87	0.6	0.1	0.6	0.53	0.66	84.95	63.28	67.9	51.09	98.99	21.35	19.85	15.74	6.11	30.74	0.46	0.09	0.45	0.4	0.5	0.45	0.14	0.45	0.37	0.53	0.58	0.08	0.58	0.54	0.62	0.73	0.05	0.73	0.7	0.76	58.49	123.51	42.51	34.55	54.74	141.54	143.87	116.82	99.16	140.64	3134	0.38
0.18	0.47	0.16	0.47	0.37	0.57	0.79	0.05	0.79	0.76	0.81	0.5	0.12	0.5	0.43	0.57	96.04	65.6	79.34	58.03	115.85	23.16	21.86	16.91	6.73	33.26	0.37	0.09	0.36	0.31	0.42	0.4	0.15	0.39	0.31	0.47	0.52	0.09	0.51	0.47	0.56	0.68	0.05	0.67	0.64	0.7	58.57	72.32	42.55	34.55	54.99	182.02	145.29	153.74	131.58	183.04	2427	0.57
0.32	0.37	0.17	0.36	0.25	0.48	0.68	0.07	0.69	0.63	0.74	0.34	0.15	0.35	0.24	0.44	117.4	79.81	100.02	70.0	141.38	27.85	24.73	21.3	8.75	40.21	0.24	0.11	0.24	0.16	0.31	0.32	0.16	0.31	0.24	0.41	0.44	0.1	0.43	0.38	0.49	0.6	0.07	0.6	0.56	0.64	58.6	99.25	42.18	34.28	54.24	262.57	225.09	223.38	181.62	285.27	3397	0.94


==> data_new/tef/fakenews/cnn/S_auc.tex <==
0.18

==> data_new/tef/fakenews/cnn/S_ppl.tex <==
3.7

==> data_new/tef/fakenews/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.46	0.45	0.66	0.01	0.85	0.99	0.01	0.99	0.98	0.99	0.85	0.08	0.85	0.8	0.89	4.13	3.15	3.61	1.45	6.33	11.63	12.61	7.28	2.15	18.15	0.79	0.1	0.79	0.73	0.86	0.78	0.11	0.78	0.71	0.84	0.88	0.07	0.88	0.84	0.92	0.91	0.05	0.91	0.88	0.95	80.12	236.13	43.02	34.57	56.71	86.19	235.67	49.06	39.34	64.27	4036	0.02
0.03	0.37	0.43	0.52	-0.05	0.76	0.97	0.02	0.97	0.96	0.98	0.76	0.08	0.77	0.72	0.81	4.66	3.16	4.26	1.96	6.75	14.38	14.71	9.73	3.4	21.11	0.7	0.09	0.7	0.65	0.76	0.69	0.11	0.69	0.62	0.75	0.82	0.06	0.83	0.78	0.86	0.87	0.05	0.88	0.85	0.91	56.17	69.85	42.49	34.42	54.91	70.81	75.14	55.81	45.74	71.33	3887	0.07
0.06	0.33	0.42	0.47	-0.07	0.7	0.94	0.03	0.94	0.92	0.96	0.67	0.09	0.67	0.61	0.72	4.84	3.4	4.34	2.18	6.93	16.3	16.51	11.63	4.21	23.51	0.6	0.09	0.61	0.55	0.66	0.6	0.12	0.6	0.53	0.67	0.76	0.07	0.76	0.73	0.81	0.83	0.05	0.84	0.8	0.87	60.97	122.75	42.41	34.16	55.09	90.05	132.57	68.43	56.51	86.52	3979	0.13
0.11	0.29	0.4	0.39	-0.08	0.63	0.9	0.04	0.91	0.88	0.93	0.58	0.09	0.58	0.52	0.64	5.15	3.65	4.64	2.52	7.08	17.67	17.35	12.69	4.81	25.54	0.51	0.09	0.52	0.46	0.57	0.53	0.13	0.53	0.45	0.61	0.71	0.07	0.71	0.67	0.76	0.79	0.05	0.8	0.77	0.83	61.78	115.01	42.84	34.63	55.3	107.22	114.72	84.12	70.27	104.0	3224	0.2
0.15	0.24	0.38	0.31	-0.11	0.57	0.85	0.04	0.85	0.82	0.88	0.47	0.11	0.47	0.4	0.54	5.56	5.07	4.94	2.81	7.39	18.74	18.67	13.11	5.24	27.11	0.41	0.09	0.41	0.35	0.47	0.48	0.12	0.47	0.4	0.55	0.64	0.07	0.63	0.59	0.69	0.75	0.05	0.75	0.71	0.78	58.28	82.45	42.21	34.47	54.77	138.22	144.9	113.0	95.68	136.3	2331	0.38
0.18	0.23	0.37	0.28	-0.11	0.54	0.8	0.05	0.8	0.76	0.83	0.38	0.12	0.38	0.3	0.47	5.86	5.88	5.13	3.02	7.63	18.7	18.43	13.68	5.24	26.83	0.33	0.1	0.32	0.26	0.39	0.45	0.13	0.43	0.37	0.51	0.58	0.08	0.58	0.53	0.64	0.7	0.05	0.7	0.67	0.74	58.95	76.12	42.26	34.38	55.0	176.93	139.34	147.41	125.89	178.01	1804	0.55
0.32	0.19	0.36	0.23	-0.12	0.49	0.71	0.07	0.71	0.66	0.75	0.29	0.14	0.3	0.2	0.4	6.31	6.18	5.5	3.36	7.89	21.24	21.28	15.35	5.94	30.2	0.24	0.11	0.24	0.16	0.32	0.4	0.13	0.39	0.31	0.47	0.52	0.09	0.51	0.46	0.58	0.65	0.06	0.65	0.61	0.69	58.93	103.66	42.0	34.13	54.51	252.65	176.55	214.49	176.65	275.06	2928	0.9


==> data_new/tef/fakenews/lstm/IG_auc.tex <==
0.09

==> data_new/tef/fakenews/lstm/IG_ppl.tex <==
3.6

==> data_new/tef/fakenews/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.47	0.22	0.42	0.3	0.6	0.99	0.01	0.99	0.98	0.99	0.89	0.09	0.91	0.85	0.96	94.96	74.04	79.2	37.46	137.03	36.86	33.59	27.7	8.74	58.16	0.79	0.13	0.79	0.71	0.89	0.65	0.17	0.66	0.55	0.76	0.84	0.1	0.84	0.78	0.91	0.9	0.07	0.91	0.86	0.95	80.11	236.39	43.02	34.56	56.72	86.84	235.92	49.83	40.22	64.45	4039	0.02
0.03	0.36	0.18	0.32	0.22	0.45	0.97	0.02	0.97	0.96	0.98	0.83	0.1	0.85	0.78	0.9	112.03	80.05	96.99	52.3	155.23	41.4	34.85	32.77	12.19	63.09	0.7	0.12	0.71	0.63	0.79	0.53	0.14	0.55	0.45	0.63	0.77	0.1	0.78	0.71	0.84	0.86	0.06	0.87	0.83	0.91	56.05	69.82	42.4	34.35	54.89	73.59	100.69	57.19	46.74	72.25	3899	0.09
0.06	0.3	0.18	0.26	0.17	0.38	0.94	0.03	0.94	0.93	0.96	0.76	0.11	0.77	0.7	0.83	122.55	90.37	106.69	56.58	169.24	41.88	35.92	33.62	11.42	64.19	0.62	0.11	0.62	0.55	0.7	0.43	0.15	0.43	0.34	0.53	0.7	0.09	0.71	0.65	0.76	0.83	0.06	0.83	0.79	0.87	63.64	135.92	42.5	34.18	55.35	96.78	160.39	70.57	57.77	88.64	4003	0.14
0.11	0.24	0.15	0.21	0.13	0.32	0.91	0.04	0.91	0.89	0.93	0.69	0.12	0.7	0.62	0.76	136.4	99.84	118.49	66.7	181.27	42.7	36.18	34.06	12.36	64.67	0.54	0.11	0.54	0.47	0.61	0.35	0.14	0.35	0.27	0.43	0.64	0.09	0.65	0.59	0.7	0.79	0.06	0.79	0.75	0.83	63.2	123.31	42.86	34.7	55.6	117.61	172.64	87.6	72.84	108.97	3906	0.24
0.15	0.18	0.14	0.16	0.09	0.25	0.86	0.04	0.86	0.83	0.88	0.58	0.13	0.58	0.5	0.66	156.25	115.95	136.08	79.6	199.84	42.96	35.76	34.04	13.16	65.3	0.43	0.11	0.43	0.36	0.5	0.27	0.13	0.27	0.19	0.33	0.56	0.09	0.56	0.5	0.61	0.74	0.06	0.74	0.7	0.78	59.07	125.65	42.46	34.57	54.88	144.37	190.27	118.02	99.77	142.76	3064	0.4
0.18	0.14	0.13	0.12	0.05	0.21	0.8	0.05	0.81	0.78	0.83	0.47	0.14	0.48	0.39	0.56	174.59	138.88	150.28	86.63	215.39	42.58	35.48	34.14	13.4	65.54	0.34	0.11	0.34	0.28	0.41	0.21	0.12	0.2	0.14	0.27	0.48	0.08	0.48	0.43	0.54	0.69	0.06	0.69	0.65	0.73	58.27	70.2	42.46	34.56	55.07	188.55	165.73	157.49	133.55	188.99	2414	0.61
0.32	0.09	0.12	0.06	0.01	0.15	0.71	0.07	0.71	0.66	0.76	0.32	0.16	0.33	0.21	0.43	214.15	203.56	174.51	102.31	256.2	45.35	37.78	35.67	14.48	68.69	0.22	0.12	0.22	0.14	0.3	0.16	0.11	0.14	0.08	0.22	0.4	0.09	0.4	0.34	0.46	0.62	0.07	0.62	0.58	0.67	58.77	99.74	42.11	34.29	54.56	267.96	215.99	229.43	187.22	290.03	3429	0.98


==> data_new/tef/fakenews/lstm/S_auc.tex <==
0.07

==> data_new/tef/fakenews/lstm/S_ppl.tex <==
3.6

==> data_new/tef/fakenews/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.51	0.36	0.61	0.08	0.83	0.98	0.01	0.99	0.98	0.99	0.85	0.18	0.94	0.78	0.98	0.39	0.25	0.31	0.2	0.58	86.78	86.89	48.95	12.15	164.4	0.75	0.21	0.82	0.61	0.92	0.76	0.19	0.82	0.59	0.92	0.84	0.14	0.88	0.74	0.95	0.87	0.11	0.91	0.8	0.96	79.64	235.26	42.89	34.42	56.4	85.63	234.77	48.96	39.56	63.67	4076	0.02
0.03	0.41	0.32	0.44	0.05	0.68	0.96	0.02	0.96	0.95	0.98	0.81	0.19	0.89	0.73	0.95	0.45	0.23	0.4	0.27	0.61	96.89	87.57	66.35	18.83	173.1	0.69	0.2	0.75	0.56	0.86	0.7	0.18	0.75	0.55	0.86	0.8	0.13	0.84	0.71	0.91	0.85	0.11	0.88	0.78	0.93	55.98	69.59	42.36	34.35	54.81	70.4	72.73	55.76	45.82	70.66	3922	0.07
0.06	0.36	0.31	0.35	0.04	0.6	0.93	0.03	0.93	0.91	0.95	0.79	0.18	0.86	0.71	0.91	0.46	0.22	0.43	0.3	0.62	99.39	87.95	71.32	20.73	175.13	0.66	0.18	0.71	0.54	0.8	0.66	0.18	0.69	0.51	0.8	0.78	0.12	0.8	0.7	0.88	0.83	0.1	0.86	0.77	0.91	63.32	135.49	42.35	34.06	55.17	91.94	130.35	68.41	56.28	86.05	4041	0.12
0.11	0.32	0.29	0.29	0.03	0.52	0.9	0.04	0.9	0.88	0.92	0.76	0.17	0.82	0.68	0.88	0.49	0.21	0.46	0.33	0.64	104.68	88.39	80.58	24.66	182.39	0.62	0.17	0.67	0.52	0.75	0.6	0.18	0.62	0.47	0.74	0.76	0.11	0.78	0.68	0.84	0.82	0.09	0.84	0.77	0.89	63.38	124.4	42.85	34.65	55.4	112.07	179.15	84.24	70.0	103.84	3956	0.21
0.15	0.28	0.27	0.23	0.02	0.46	0.85	0.04	0.85	0.82	0.87	0.72	0.15	0.77	0.64	0.83	0.5	0.2	0.46	0.35	0.64	109.92	89.26	87.64	29.41	186.99	0.58	0.15	0.61	0.48	0.68	0.53	0.17	0.53	0.41	0.65	0.73	0.1	0.74	0.66	0.8	0.8	0.08	0.82	0.75	0.86	59.47	129.47	42.59	34.6	54.97	138.0	210.95	112.13	93.81	135.61	3396	0.36
0.18	0.26	0.27	0.21	0.01	0.43	0.79	0.05	0.8	0.77	0.82	0.68	0.15	0.72	0.6	0.78	0.49	0.2	0.46	0.35	0.63	112.19	90.84	88.41	30.29	192.51	0.53	0.14	0.56	0.45	0.63	0.46	0.16	0.46	0.35	0.57	0.69	0.09	0.7	0.63	0.76	0.78	0.07	0.79	0.73	0.84	59.56	83.9	42.77	34.56	55.38	178.88	161.02	148.22	125.01	176.58	2558	0.54
0.32	0.24	0.26	0.18	0.01	0.39	0.7	0.07	0.71	0.65	0.75	0.61	0.15	0.63	0.53	0.72	0.49	0.19	0.45	0.35	0.62	111.42	87.32	88.93	32.25	194.56	0.46	0.13	0.47	0.38	0.55	0.39	0.16	0.37	0.29	0.47	0.64	0.09	0.64	0.58	0.7	0.75	0.07	0.75	0.7	0.8	58.42	98.51	42.18	34.29	54.62	257.98	304.22	216.24	174.79	277.87	3591	0.92


==> data_new/tef/fakenews/lstmatt/A_auc.tex <==
0.10

==> data_new/tef/fakenews/lstmatt/A_ppl.tex <==
3.7

==> data_new/tef/fakenews/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.63	0.35	0.75	0.43	0.9	0.98	0.01	0.99	0.98	0.99	0.76	0.18	0.8	0.66	0.89	6.17	16.13	1.73	0.93	3.61	23.11	26.54	15.29	4.96	32.97	0.68	0.18	0.7	0.55	0.81	0.73	0.15	0.74	0.63	0.83	0.8	0.11	0.81	0.73	0.88	0.85	0.09	0.86	0.79	0.92	79.77	235.54	42.93	34.48	56.45	85.7	235.02	48.86	39.33	63.77	4070	0.02
0.03	0.54	0.35	0.63	0.35	0.81	0.96	0.02	0.97	0.95	0.98	0.68	0.16	0.72	0.6	0.79	8.49	35.84	2.14	1.32	4.02	30.03	33.55	20.14	7.49	41.51	0.6	0.16	0.62	0.5	0.71	0.66	0.13	0.67	0.57	0.75	0.75	0.1	0.76	0.69	0.82	0.82	0.08	0.83	0.77	0.88	55.9	69.55	42.33	34.32	54.8	70.32	75.61	55.56	45.24	70.5	3929	0.07
0.06	0.49	0.35	0.57	0.31	0.74	0.93	0.03	0.93	0.91	0.95	0.62	0.16	0.64	0.54	0.72	10.63	78.56	2.33	1.56	4.21	34.87	40.16	24.06	8.69	47.86	0.54	0.15	0.55	0.45	0.63	0.6	0.14	0.61	0.51	0.68	0.71	0.1	0.72	0.65	0.78	0.79	0.08	0.8	0.75	0.84	61.73	130.12	42.43	34.18	55.13	89.15	122.33	67.52	55.48	85.44	4012	0.13
0.11	0.44	0.34	0.52	0.27	0.69	0.9	0.04	0.9	0.88	0.92	0.57	0.15	0.59	0.49	0.67	23.09	542.12	2.53	1.74	4.46	39.09	44.87	27.22	10.3	53.81	0.49	0.14	0.5	0.41	0.57	0.57	0.13	0.57	0.49	0.65	0.68	0.09	0.68	0.62	0.74	0.77	0.08	0.78	0.73	0.82	61.22	113.06	42.8	34.6	55.41	107.43	148.2	82.23	68.43	102.45	3500	0.22
0.15	0.4	0.35	0.47	0.23	0.64	0.85	0.04	0.85	0.82	0.87	0.51	0.15	0.53	0.43	0.61	10.53	36.07	2.71	1.92	4.89	42.82	49.34	30.24	12.37	58.21	0.43	0.13	0.44	0.36	0.52	0.54	0.13	0.55	0.45	0.61	0.64	0.09	0.65	0.59	0.7	0.74	0.07	0.75	0.7	0.79	57.78	81.78	42.08	34.43	54.5	131.72	123.7	109.1	91.67	132.53	2354	0.37
0.18	0.39	0.35	0.46	0.23	0.63	0.79	0.05	0.79	0.76	0.82	0.47	0.15	0.49	0.39	0.57	17.73	290.1	2.77	1.99	5.11	44.81	54.81	30.79	12.02	60.84	0.39	0.13	0.41	0.32	0.47	0.53	0.13	0.53	0.44	0.61	0.61	0.09	0.62	0.56	0.67	0.72	0.07	0.73	0.68	0.77	59.15	75.93	42.34	34.42	54.9	173.41	154.76	143.54	121.35	171.98	1901	0.56
0.32	0.37	0.34	0.43	0.21	0.6	0.7	0.07	0.71	0.66	0.75	0.43	0.14	0.44	0.35	0.53	13.02	137.23	2.87	2.09	5.01	46.36	52.61	32.79	13.35	63.65	0.35	0.12	0.35	0.28	0.42	0.51	0.13	0.51	0.43	0.59	0.59	0.09	0.59	0.54	0.64	0.69	0.07	0.7	0.65	0.73	59.17	105.6	42.03	33.87	54.7	246.53	245.45	208.68	168.47	268.22	2689	0.91


==> data_new/tef/fakenews/lstmatt/IG_auc.tex <==
0.14

==> data_new/tef/fakenews/lstmatt/IG_ppl.tex <==
3.5

==> data_new/tef/fakenews/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.67	0.22	0.7	0.5	0.86	0.98	0.01	0.99	0.98	0.99	0.85	0.12	0.87	0.79	0.94	430.09	8553.12	61.43	30.51	155.42	62.72	62.26	43.57	10.57	100.2	0.7	0.15	0.71	0.61	0.8	0.68	0.16	0.69	0.58	0.78	0.79	0.11	0.79	0.72	0.86	0.85	0.08	0.86	0.8	0.91	79.77	235.54	42.93	34.48	56.45	86.04	235.0	49.37	39.58	63.75	4070	0.02
0.03	0.6	0.21	0.6	0.44	0.77	0.96	0.02	0.96	0.95	0.98	0.79	0.14	0.82	0.72	0.89	1047.7	33671.01	76.53	42.61	210.68	72.83	66.27	56.86	16.8	113.24	0.64	0.14	0.64	0.55	0.73	0.6	0.16	0.61	0.5	0.71	0.74	0.11	0.74	0.67	0.81	0.82	0.08	0.82	0.77	0.88	55.7	69.48	42.25	34.19	54.74	70.73	74.57	55.88	45.62	71.13	3945	0.07
0.06	0.55	0.21	0.55	0.39	0.7	0.93	0.03	0.93	0.92	0.95	0.75	0.15	0.77	0.67	0.86	4112.05	79118.17	86.92	49.89	241.55	77.66	69.3	62.36	18.4	120.53	0.59	0.15	0.6	0.5	0.69	0.56	0.18	0.57	0.44	0.67	0.7	0.11	0.71	0.63	0.78	0.8	0.08	0.8	0.75	0.85	62.5	131.82	42.51	34.29	55.18	92.3	144.12	68.72	56.6	86.3	4022	0.13
0.11	0.51	0.21	0.51	0.36	0.65	0.9	0.04	0.9	0.88	0.92	0.72	0.16	0.74	0.63	0.83	834.3	17650.64	96.57	56.24	284.17	81.93	71.16	67.08	21.68	125.79	0.55	0.14	0.56	0.47	0.65	0.53	0.18	0.53	0.41	0.65	0.68	0.11	0.68	0.61	0.75	0.78	0.08	0.78	0.73	0.83	63.34	135.26	42.81	34.65	55.42	112.39	170.74	85.07	70.39	104.28	3982	0.21
0.15	0.47	0.2	0.47	0.33	0.61	0.85	0.04	0.85	0.82	0.88	0.67	0.17	0.69	0.58	0.79	22480.69	1110963.55	105.74	61.21	348.65	87.07	72.86	73.96	24.26	133.43	0.51	0.14	0.52	0.42	0.61	0.5	0.19	0.5	0.37	0.63	0.64	0.11	0.65	0.57	0.72	0.75	0.08	0.76	0.7	0.81	56.94	75.13	42.28	34.16	54.75	138.24	159.69	114.2	95.84	136.16	2583	0.38
0.18	0.46	0.21	0.45	0.31	0.59	0.8	0.05	0.8	0.77	0.83	0.63	0.18	0.66	0.53	0.76	573.96	3235.15	104.3	62.12	319.31	87.13	74.1	71.61	22.08	136.0	0.48	0.15	0.49	0.38	0.58	0.48	0.19	0.49	0.34	0.61	0.62	0.12	0.62	0.55	0.7	0.74	0.08	0.74	0.69	0.79	58.58	73.41	42.3	34.43	54.95	179.57	164.91	149.04	125.64	178.28	1893	0.55
0.32	0.43	0.21	0.42	0.28	0.57	0.71	0.07	0.72	0.67	0.76	0.57	0.2	0.6	0.47	0.71	479.15	2334.9	100.96	62.04	267.93	89.1	74.96	74.84	23.09	138.88	0.42	0.16	0.44	0.33	0.53	0.45	0.19	0.47	0.31	0.59	0.59	0.13	0.59	0.51	0.68	0.71	0.09	0.71	0.66	0.77	57.57	71.72	42.18	34.29	54.65	259.08	348.54	212.56	171.81	272.11	2837	0.94


==> data_new/tef/fakenews/lstmatt/S_auc.tex <==
0.16

==> data_new/tef/fakenews/lstmatt/S_ppl.tex <==
3.7

==> data_new/tef/fakenews/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.74	0.1	0.72	0.69	0.78	0.98	0.01	0.98	0.98	0.99	0.96	0.02	0.96	0.95	0.97	5.08	1.92	5.28	4.05	6.33	18.51	18.99	12.84	5.93	21.02	0.84	0.04	0.84	0.82	0.86	0.86	0.03	0.85	0.84	0.87	0.9	0.02	0.9	0.89	0.92	0.93	0.01	0.92	0.92	0.94	47.19	30.43	36.62	32.56	42.35	55.51	29.57	45.28	43.16	50.41	12	0.02
0.03	0.68	0.07	0.71	0.67	0.71	0.96	0.01	0.96	0.96	0.96	0.95	0.02	0.96	0.94	0.97	6.2	1.19	6.43	6.3	6.43	15.14	15.64	9.28	9.28	10.0	0.83	0.04	0.84	0.8	0.87	0.85	0.04	0.88	0.83	0.89	0.89	0.03	0.9	0.87	0.92	0.92	0.02	0.93	0.9	0.94	42.23	26.97	37.18	34.45	37.18	56.22	26.07	49.71	49.71	52.73	14	0.04
0.06	0.61	0.09	0.59	0.56	0.63	0.92	0.04	0.92	0.89	0.92	0.91	0.02	0.91	0.9	0.93	6.49	1.74	6.91	6.45	7.37	21.66	21.34	9.51	7.73	30.13	0.75	0.03	0.76	0.74	0.77	0.78	0.03	0.76	0.76	0.8	0.84	0.02	0.84	0.83	0.86	0.88	0.01	0.89	0.87	0.89	47.27	38.94	33.92	30.59	37.19	83.75	49.25	70.38	61.72	73.25	7	0.09
0.11	0.55	0.09	0.57	0.53	0.6	0.88	0.05	0.88	0.85	0.89	0.88	0.03	0.87	0.86	0.91	7.0	1.68	7.09	6.75	7.72	25.89	20.07	16.37	12.97	32.88	0.72	0.04	0.7	0.69	0.75	0.74	0.04	0.74	0.73	0.76	0.81	0.03	0.79	0.79	0.84	0.86	0.02	0.85	0.85	0.88	47.27	38.94	33.92	30.59	37.19	114.8	73.29	91.78	83.04	101.54	7	0.16
0.15	0.49	0.1	0.48	0.41	0.58	0.84	0.06	0.83	0.8	0.85	0.85	0.03	0.84	0.83	0.88	7.62	1.81	8.11	7.35	8.59	31.39	22.45	32.86	12.53	44.8	0.67	0.03	0.66	0.66	0.7	0.7	0.04	0.7	0.68	0.72	0.78	0.03	0.77	0.77	0.8	0.84	0.02	0.84	0.83	0.86	47.27	38.94	33.92	30.59	37.19	169.5	97.99	150.48	124.23	150.87	7	0.29
0.18	0.49	0.11	0.56	0.39	0.58	0.79	0.07	0.8	0.75	0.8	0.83	0.03	0.83	0.83	0.86	7.04	2.44	7.9	3.92	9.02	24.62	20.05	13.18	13.18	31.88	0.65	0.04	0.67	0.64	0.67	0.69	0.04	0.71	0.67	0.71	0.77	0.03	0.77	0.76	0.79	0.83	0.02	0.84	0.82	0.84	66.79	51.36	36.06	30.76	135.12	277.27	126.29	212.47	191.45	444.24	9	0.36
0.32	0.39	0.11	0.38	0.3	0.51	0.7	0.11	0.68	0.65	0.72	0.8	0.05	0.81	0.76	0.83	9.15	1.14	9.28	8.1	9.85	40.09	29.2	39.28	9.24	70.52	0.61	0.05	0.62	0.57	0.64	0.65	0.05	0.66	0.6	0.68	0.74	0.04	0.74	0.71	0.77	0.81	0.02	0.81	0.79	0.82	32.63	4.14	32.34	30.42	36.06	320.2	75.98	290.6	265.29	341.87	12	1.0


==> data_new/tef/fakenews/roberta/A_auc.tex <==
0.17

==> data_new/tef/fakenews/roberta/A_ppl.tex <==
8.8

==> data_new/tef/fakenews/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.03	0.03	0.03	0.02	0.05	0.99	0.0	0.98	0.98	0.99	0.2	0.14	0.24	0.13	0.26	375.08	396.91	181.95	160.29	386.34	144.2	61.69	165.59	107.43	195.62	0.14	0.09	0.16	0.09	0.17	0.2	0.07	0.2	0.16	0.21	0.4	0.06	0.39	0.37	0.44	0.55	0.05	0.56	0.54	0.58	35.01	8.42	33.61	29.65	40.06	41.02	11.34	39.02	33.51	45.36	8	0.02
0.03	0.08	0.09	0.05	0.03	0.1	0.97	0.01	0.98	0.97	0.98	0.31	0.24	0.33	0.1	0.42	312.93	203.78	346.34	197.09	380.0	104.21	69.28	129.61	22.68	158.67	0.22	0.17	0.22	0.06	0.29	0.23	0.12	0.25	0.21	0.28	0.48	0.13	0.47	0.43	0.52	0.61	0.11	0.6	0.52	0.66	40.14	7.14	38.3	36.48	41.63	54.92	11.8	53.4	46.71	59.83	12	0.05
0.06	0.04	0.12	0.01	-0.01	0.03	0.94	0.04	0.95	0.94	0.96	0.36	0.29	0.39	0.29	0.55	498.65	365.52	421.29	340.44	596.93	19.99	10.03	24.11	16.39	26.58	0.26	0.2	0.26	0.2	0.39	0.14	0.13	0.16	0.04	0.16	0.44	0.17	0.41	0.34	0.54	0.64	0.12	0.63	0.62	0.71	63.25	43.43	45.37	35.78	84.5	120.55	90.38	80.72	74.43	148.6	6	0.11
0.11	0.05	0.01	0.05	0.04	0.05	0.9	0.03	0.9	0.89	0.91	0.46	0.05	0.46	0.44	0.48	867.16	1010.47	867.16	509.9	1224.41	47.14	38.95	47.14	33.37	60.91	0.32	0.03	0.32	0.31	0.33	0.2	0.02	0.2	0.19	0.21	0.5	0.01	0.5	0.5	0.51	0.64	0.04	0.64	0.63	0.66	51.92	30.4	51.92	41.17	62.67	152.23	120.8	152.23	109.52	194.94	2	0.24
0.32	0.1	0.05	0.1	0.08	0.12	0.69	0.16	0.69	0.64	0.75	0.54	0.07	0.54	0.52	0.57	22.38	10.39	22.38	18.71	26.06	6.94	9.13	6.94	3.72	10.17	0.4	0.04	0.4	0.39	0.41	0.26	0.13	0.26	0.21	0.31	0.54	0.09	0.54	0.51	0.57	0.72	0.09	0.72	0.69	0.75	145.1	154.66	145.1	90.42	199.78	1079.74	1159.66	1079.74	669.74	1489.74	2	0.8


==> data_new/tef/fakenews/roberta/S_auc.tex <==
0.03

==> data_new/tef/fakenews/roberta/S_ppl.tex <==
8.1

==> data_new/tef/fakenews/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.68	0.13	0.68	0.58	0.76	0.98	0.02	0.98	0.98	0.99	0.89	0.08	0.91	0.85	0.94	3.14	1.1	3.2	2.56	3.78	14.58	13.05	11.13	4.56	21.34	0.77	0.11	0.8	0.71	0.84	0.75	0.1	0.78	0.69	0.82	0.85	0.07	0.87	0.81	0.9	0.9	0.05	0.91	0.87	0.93	71.81	338.88	39.88	32.31	52.3	81.83	339.2	49.26	40.18	64.16	3637	0.02
0.03	0.57	0.13	0.57	0.48	0.66	0.96	0.03	0.96	0.95	0.97	0.84	0.08	0.85	0.78	0.9	3.71	1.12	3.69	3.09	4.36	17.48	15.0	13.43	5.36	25.5	0.69	0.1	0.71	0.62	0.77	0.67	0.09	0.69	0.6	0.73	0.79	0.07	0.81	0.75	0.84	0.86	0.05	0.87	0.83	0.9	54.56	83.35	39.72	32.41	52.15	79.16	98.04	60.43	49.66	77.29	2594	0.07
0.06	0.48	0.13	0.47	0.38	0.56	0.93	0.04	0.93	0.91	0.95	0.78	0.1	0.79	0.71	0.85	4.19	1.29	4.19	3.5	4.93	19.36	16.29	15.57	6.45	28.31	0.62	0.1	0.63	0.55	0.7	0.59	0.09	0.6	0.52	0.66	0.74	0.07	0.75	0.69	0.79	0.83	0.05	0.83	0.79	0.86	58.06	112.39	39.06	31.77	52.61	109.43	161.24	79.9	66.16	103.3	1467	0.14
0.11	0.4	0.13	0.39	0.31	0.47	0.89	0.05	0.9	0.86	0.92	0.72	0.11	0.72	0.64	0.81	4.65	1.43	4.61	3.83	5.5	20.88	17.83	16.16	6.69	30.82	0.56	0.11	0.56	0.48	0.64	0.53	0.1	0.53	0.46	0.6	0.69	0.07	0.7	0.64	0.75	0.8	0.05	0.8	0.76	0.84	64.29	248.76	39.41	31.96	52.31	149.19	241.72	108.97	89.47	137.37	1641	0.21
0.15	0.31	0.11	0.29	0.23	0.37	0.84	0.06	0.83	0.8	0.87	0.65	0.13	0.64	0.55	0.75	5.3	1.59	5.27	4.3	6.25	23.73	19.86	18.92	7.87	35.04	0.49	0.11	0.48	0.41	0.57	0.46	0.09	0.46	0.39	0.53	0.64	0.07	0.64	0.59	0.7	0.76	0.05	0.75	0.72	0.8	53.24	64.21	39.39	31.94	52.63	206.66	191.76	168.89	138.58	209.43	1206	0.46
0.18	0.25	0.11	0.23	0.17	0.3	0.77	0.07	0.77	0.73	0.81	0.59	0.14	0.58	0.48	0.71	5.81	1.8	5.85	4.69	6.9	25.61	21.56	20.17	8.34	37.54	0.44	0.11	0.43	0.35	0.53	0.41	0.09	0.41	0.34	0.48	0.6	0.07	0.6	0.55	0.66	0.73	0.06	0.73	0.69	0.77	58.53	104.47	39.26	31.78	52.99	309.63	278.13	249.1	207.54	312.06	949	0.69
0.32	0.2	0.1	0.18	0.13	0.24	0.7	0.09	0.7	0.65	0.75	0.53	0.15	0.53	0.41	0.67	6.31	1.92	6.36	5.2	7.49	27.34	22.91	21.23	9.34	40.31	0.39	0.12	0.38	0.29	0.49	0.37	0.09	0.37	0.31	0.44	0.57	0.08	0.56	0.51	0.63	0.7	0.06	0.7	0.66	0.75	63.22	257.77	39.81	32.26	52.74	458.84	379.49	375.63	306.34	473.12	1395	1.0


==> data_new/tef/fakenews/xlnet/A_auc.tex <==
0.11

==> data_new/tef/fakenews/xlnet/A_ppl.tex <==
6.3

==> data_new/tef/fakenews/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	-0.37	0.43	-0.44	-0.71	-0.03	0.98	0.02	0.99	0.98	0.99	-0.12	0.41	-0.15	-0.44	0.18	3.86	22.95	0.38	0.17	0.92	7.88	7.5	5.98	2.68	11.34	-0.09	0.33	-0.11	-0.34	0.13	0.21	0.17	0.16	0.1	0.29	0.3	0.19	0.27	0.16	0.41	0.46	0.17	0.45	0.34	0.57	57.7	250.91	37.81	31.37	49.47	64.91	251.22	45.18	36.68	56.65	1442	0.02
0.03	-0.3	0.37	-0.29	-0.61	-0.02	0.97	0.03	0.97	0.96	0.98	-0.05	0.34	-0.06	-0.33	0.22	5.95	18.78	0.54	0.2	2.78	7.92	7.29	5.78	2.34	11.29	-0.04	0.26	-0.04	-0.24	0.16	0.2	0.13	0.18	0.1	0.29	0.32	0.15	0.32	0.2	0.43	0.49	0.14	0.5	0.39	0.59	51.82	57.26	38.86	30.67	52.64	71.5	70.1	55.04	44.25	71.83	856	0.06
0.06	-0.3	0.35	-0.32	-0.59	-0.04	0.93	0.04	0.94	0.91	0.95	-0.03	0.29	-0.0	-0.25	0.16	8.91	23.03	0.67	0.2	6.48	8.47	7.54	7.1	3.05	11.0	-0.02	0.21	0.0	-0.18	0.11	0.19	0.12	0.18	0.1	0.27	0.32	0.13	0.33	0.22	0.4	0.5	0.12	0.51	0.43	0.56	60.65	70.37	44.25	34.25	56.45	105.13	102.13	79.06	63.57	106.14	658	0.11
0.11	-0.42	0.28	-0.46	-0.65	-0.21	0.89	0.06	0.9	0.86	0.92	-0.09	0.26	-0.08	-0.33	0.12	6.78	10.92	0.71	0.18	9.12	8.33	8.01	6.37	2.31	12.07	-0.06	0.2	-0.05	-0.23	0.09	0.16	0.11	0.16	0.09	0.25	0.31	0.13	0.31	0.19	0.42	0.48	0.11	0.5	0.39	0.57	68.79	89.41	44.69	33.2	57.2	159.88	155.65	119.86	88.22	160.94	298	0.2
0.15	-0.55	0.26	-0.62	-0.78	-0.4	0.84	0.06	0.85	0.82	0.87	-0.16	0.25	-0.12	-0.37	0.03	4.34	8.2	0.53	0.14	3.67	9.79	6.5	8.73	5.31	14.61	-0.11	0.18	-0.09	-0.26	0.02	0.15	0.1	0.14	0.06	0.24	0.27	0.11	0.29	0.18	0.35	0.45	0.11	0.46	0.37	0.55	77.21	123.18	39.4	31.73	52.23	219.45	226.54	147.26	115.26	214.6	115	0.27
0.18	-0.52	0.23	-0.52	-0.69	-0.39	0.79	0.1	0.82	0.78	0.83	-0.11	0.23	-0.1	-0.28	0.1	3.54	6.46	0.34	0.13	5.44	7.62	6.4	5.77	2.82	10.06	-0.07	0.17	-0.07	-0.19	0.07	0.13	0.1	0.16	0.02	0.2	0.3	0.1	0.3	0.23	0.4	0.47	0.09	0.48	0.4	0.56	118.03	165.47	46.52	33.79	109.35	449.85	471.26	233.17	191.45	428.99	59	0.42
0.32	-0.53	0.23	-0.48	-0.73	-0.34	0.78	0.07	0.79	0.75	0.82	-0.18	0.22	-0.25	-0.36	0.01	1.38	2.57	0.18	0.09	1.52	8.92	8.2	6.03	3.57	10.96	-0.12	0.17	-0.16	-0.25	0.02	0.12	0.1	0.14	0.0	0.19	0.27	0.1	0.23	0.18	0.35	0.43	0.12	0.45	0.36	0.53	179.91	272.87	35.44	31.62	191.03	735.61	795.74	308.73	190.11	1447.23	22	0.46


==> data_new/tef/fakenews/xlnet/IG_auc.tex <==
-0.14

==> data_new/tef/fakenews/xlnet/IG_ppl.tex <==
6.7

==> data_new/tef/fakenews/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.19	0.22	0.12	0.04	0.26	0.98	0.01	0.98	0.98	0.99	0.42	0.26	0.39	0.23	0.62	80.83	259.23	32.27	16.79	65.41	63.27	55.32	46.26	19.06	92.57	0.31	0.21	0.27	0.16	0.44	0.25	0.19	0.18	0.11	0.33	0.48	0.16	0.44	0.37	0.58	0.66	0.11	0.64	0.58	0.73	61.2	284.66	38.3	31.33	50.19	69.56	285.27	46.15	36.26	60.22	2308	0.02
0.03	0.17	0.2	0.11	0.04	0.24	0.97	0.02	0.97	0.96	0.98	0.41	0.25	0.41	0.23	0.61	116.73	459.5	38.82	17.5	69.96	68.61	59.4	51.24	21.03	103.31	0.3	0.19	0.29	0.16	0.44	0.24	0.17	0.2	0.12	0.33	0.48	0.15	0.45	0.37	0.57	0.65	0.1	0.64	0.58	0.73	47.01	42.36	39.54	31.78	50.0	64.62	56.72	54.93	43.84	69.33	1999	0.06
0.06	0.21	0.2	0.18	0.06	0.3	0.94	0.03	0.95	0.93	0.96	0.45	0.25	0.48	0.25	0.65	274.82	1310.73	33.3	16.8	70.97	50.97	50.94	37.97	11.61	67.99	0.33	0.19	0.34	0.17	0.48	0.25	0.18	0.22	0.12	0.35	0.5	0.14	0.49	0.39	0.61	0.66	0.1	0.67	0.59	0.74	63.75	84.01	41.47	33.88	58.35	109.84	137.0	73.84	63.48	104.66	842	0.12
0.11	0.21	0.17	0.15	0.09	0.33	0.89	0.05	0.9	0.87	0.92	0.49	0.23	0.53	0.33	0.68	111.46	402.71	29.31	16.61	68.84	38.91	41.01	22.48	10.67	51.37	0.36	0.18	0.38	0.23	0.49	0.27	0.17	0.24	0.16	0.37	0.5	0.14	0.5	0.39	0.62	0.68	0.1	0.69	0.63	0.75	129.55	567.85	46.52	34.09	80.63	216.44	389.85	118.96	90.58	193.65	276	0.11
0.15	0.25	0.19	0.23	0.11	0.42	0.81	0.07	0.83	0.77	0.85	0.47	0.25	0.52	0.29	0.65	518.21	1988.44	29.34	10.49	66.33	24.82	47.72	5.29	1.16	25.23	0.34	0.19	0.37	0.21	0.48	0.25	0.21	0.24	0.0	0.43	0.52	0.15	0.53	0.4	0.63	0.66	0.11	0.67	0.6	0.75	144.66	131.32	94.38	55.61	158.95	443.23	331.67	333.59	188.47	564.1	101	0.34
0.18	0.23	0.16	0.2	0.1	0.27	0.78	0.09	0.78	0.72	0.84	0.45	0.16	0.44	0.34	0.59	780.7	1919.58	19.07	8.61	115.97	26.28	31.58	11.22	2.14	48.63	0.32	0.13	0.33	0.23	0.41	0.24	0.2	0.22	0.0	0.4	0.5	0.11	0.51	0.44	0.57	0.66	0.07	0.64	0.62	0.71	145.4	158.56	87.03	37.03	170.0	651.25	670.84	370.13	212.49	797.71	44	0.57
0.32	0.23	0.22	0.25	0.06	0.41	0.68	0.12	0.7	0.6	0.79	0.42	0.24	0.45	0.37	0.58	400.4	1320.53	20.47	3.58	112.7	7.84	12.22	2.81	0.88	7.49	0.31	0.18	0.32	0.26	0.41	0.22	0.23	0.13	0.0	0.4	0.43	0.2	0.5	0.29	0.57	0.65	0.11	0.68	0.61	0.7	633.74	1649.17	135.12	53.61	337.93	1350.76	1491.09	844.71	309.52	1569.2	30	0.19


==> data_new/tef/fakenews/xlnet/S_auc.tex <==
0.07

==> data_new/tef/fakenews/xlnet/S_ppl.tex <==
6.1

==> data_new/tef/imdb/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.33	0.28	0.26	0.08	0.52	0.97	0.02	0.98	0.97	0.98	0.79	0.17	0.85	0.71	0.91	6.78	4.23	6.78	3.51	9.78	19.41	21.73	11.53	3.67	27.79	0.65	0.18	0.7	0.53	0.79	0.63	0.17	0.67	0.51	0.77	0.77	0.13	0.8	0.68	0.87	0.84	0.1	0.86	0.77	0.91	70.88	39.4	62.93	47.15	84.51	80.52	41.79	72.35	54.55	96.17	3548	0.03
0.03	0.19	0.23	0.1	0.01	0.28	0.95	0.02	0.95	0.93	0.96	0.67	0.2	0.73	0.55	0.83	8.09	4.08	8.41	5.37	11.04	23.99	23.92	16.07	5.59	35.01	0.53	0.18	0.56	0.39	0.68	0.51	0.16	0.52	0.38	0.64	0.68	0.13	0.7	0.58	0.79	0.77	0.1	0.79	0.69	0.86	70.54	36.71	62.93	47.13	84.47	92.62	44.87	83.8	63.76	110.44	3543	0.07
0.06	0.1	0.17	0.02	-0.01	0.13	0.91	0.03	0.91	0.89	0.93	0.57	0.2	0.6	0.42	0.73	8.93	3.76	9.27	6.73	11.56	27.37	25.09	20.44	7.89	39.78	0.43	0.17	0.44	0.29	0.57	0.4	0.15	0.39	0.29	0.51	0.61	0.12	0.61	0.51	0.71	0.72	0.1	0.72	0.64	0.8	70.73	39.36	62.84	46.99	84.31	114.82	68.6	104.35	79.85	135.38	3573	0.13
0.11	0.05	0.13	-0.0	-0.01	0.05	0.87	0.04	0.87	0.85	0.89	0.47	0.2	0.49	0.32	0.64	9.32	3.35	9.43	7.35	11.58	29.23	25.16	22.48	9.28	42.52	0.35	0.16	0.34	0.22	0.48	0.32	0.13	0.31	0.22	0.41	0.55	0.11	0.54	0.46	0.64	0.68	0.09	0.67	0.61	0.75	69.57	37.28	61.82	46.63	83.19	142.09	71.42	130.09	100.04	169.36	3980	0.22
0.15	0.01	0.1	-0.01	-0.02	0.0	0.81	0.04	0.81	0.78	0.83	0.39	0.19	0.39	0.25	0.54	9.17	3.0	9.06	7.4	11.05	28.94	24.04	23.26	9.7	41.2	0.28	0.14	0.27	0.17	0.38	0.25	0.11	0.24	0.17	0.32	0.5	0.1	0.49	0.42	0.57	0.64	0.08	0.64	0.58	0.7	70.35	37.17	62.37	46.79	84.3	199.36	84.21	183.04	143.64	237.44	4512	0.38
0.18	-0.01	0.08	-0.02	-0.03	-0.01	0.75	0.05	0.75	0.72	0.79	0.35	0.18	0.35	0.21	0.49	8.66	2.83	8.57	6.96	10.33	27.16	22.96	21.37	9.37	39.16	0.25	0.14	0.24	0.14	0.35	0.21	0.1	0.2	0.13	0.27	0.48	0.1	0.47	0.41	0.55	0.63	0.08	0.62	0.57	0.69	70.49	37.69	62.62	46.86	84.63	262.4	110.75	243.77	192.32	309.98	4074	0.57
0.32	-0.01	0.08	-0.02	-0.04	-0.01	0.69	0.06	0.69	0.65	0.73	0.34	0.17	0.36	0.22	0.47	8.11	2.8	7.99	6.54	9.77	26.22	22.27	20.49	9.28	37.3	0.24	0.13	0.25	0.15	0.34	0.18	0.1	0.17	0.11	0.24	0.47	0.09	0.47	0.4	0.53	0.63	0.07	0.63	0.57	0.69	72.06	38.83	64.65	48.16	85.76	364.01	184.19	332.38	256.42	429.35	5130	0.85


==> data_new/tef/imdb/bert/A_auc.tex <==
0.02

==> data_new/tef/imdb/bert/A_ppl.tex <==
4.8

==> data_new/tef/imdb/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.18	0.38	0.25	-0.04	0.46	0.97	0.02	0.98	0.97	0.99	0.37	0.39	0.48	0.16	0.66	12.3	13.92	8.49	0.32	20.45	21.4	21.82	14.3	6.18	29.28	0.3	0.31	0.37	0.12	0.53	0.41	0.23	0.44	0.24	0.6	0.54	0.2	0.58	0.41	0.7	0.66	0.16	0.69	0.57	0.77	70.83	39.32	62.94	47.17	84.37	80.83	42.74	72.48	54.38	96.45	3564	0.03
0.03	-0.03	0.35	0.02	-0.24	0.22	0.95	0.02	0.95	0.93	0.96	0.21	0.37	0.3	-0.03	0.51	14.46	15.26	11.04	0.45	24.06	24.77	23.92	17.52	7.49	34.15	0.16	0.29	0.22	-0.01	0.4	0.31	0.19	0.32	0.14	0.47	0.46	0.18	0.49	0.33	0.61	0.59	0.15	0.62	0.5	0.71	70.43	36.67	62.86	47.07	84.4	93.11	47.1	83.83	63.72	111.33	3593	0.07
0.06	-0.18	0.31	-0.14	-0.39	0.05	0.91	0.03	0.91	0.89	0.93	0.08	0.35	0.15	-0.17	0.37	15.53	18.66	10.3	0.42	25.59	27.53	25.28	19.71	8.82	38.27	0.07	0.27	0.11	-0.11	0.29	0.24	0.17	0.23	0.08	0.36	0.4	0.17	0.42	0.27	0.54	0.55	0.14	0.57	0.46	0.66	70.77	37.15	63.53	47.06	84.82	114.88	58.8	104.96	78.73	136.41	2726	0.13
0.11	-0.29	0.31	-0.26	-0.5	-0.07	0.87	0.04	0.87	0.85	0.9	-0.04	0.35	0.03	-0.29	0.25	16.05	19.0	10.5	0.41	26.51	28.71	26.04	20.86	9.51	39.7	-0.02	0.27	0.03	-0.2	0.19	0.18	0.15	0.16	0.05	0.28	0.34	0.16	0.36	0.21	0.48	0.51	0.14	0.53	0.41	0.62	70.38	38.37	62.53	46.48	84.29	143.79	75.42	128.61	99.71	169.43	2305	0.22
0.15	-0.4	0.28	-0.38	-0.61	-0.19	0.81	0.04	0.81	0.78	0.84	-0.14	0.32	-0.09	-0.38	0.12	16.13	18.4	10.51	0.51	26.75	31.06	27.55	22.2	10.3	45.95	-0.1	0.24	-0.05	-0.27	0.1	0.13	0.12	0.1	0.0	0.2	0.3	0.15	0.31	0.17	0.42	0.47	0.13	0.49	0.38	0.58	69.85	41.6	62.8	46.8	81.93	197.62	103.98	181.32	143.82	229.46	1763	0.38
0.18	-0.42	0.24	-0.41	-0.59	-0.25	0.76	0.06	0.76	0.73	0.8	-0.15	0.28	-0.11	-0.37	0.06	18.01	17.85	15.39	1.25	28.7	29.61	26.24	21.44	10.36	41.65	-0.11	0.21	-0.07	-0.26	0.06	0.11	0.11	0.09	0.0	0.19	0.29	0.13	0.3	0.18	0.39	0.47	0.11	0.49	0.39	0.55	73.28	43.77	65.32	47.95	86.62	266.49	150.86	243.74	191.69	309.97	1237	0.55
0.32	-0.39	0.19	-0.39	-0.51	-0.27	0.69	0.07	0.7	0.65	0.74	-0.12	0.21	-0.09	-0.24	0.03	24.37	20.56	23.13	8.42	35.69	25.98	23.92	18.64	8.84	35.78	-0.08	0.15	-0.05	-0.17	0.03	0.12	0.1	0.12	0.04	0.18	0.3	0.1	0.31	0.24	0.38	0.49	0.08	0.51	0.44	0.55	71.21	33.93	64.67	47.58	86.07	360.66	181.36	327.7	257.41	428.99	1224	0.85


==> data_new/tef/imdb/bert/IG_auc.tex <==
-0.09

==> data_new/tef/imdb/bert/IG_ppl.tex <==
4.8

==> data_new/tef/imdb/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.31	0.18	0.28	0.18	0.41	0.98	0.02	0.98	0.97	0.99	0.57	0.15	0.58	0.48	0.67	75.54	200.34	1.44	0.69	8.54	10.7	8.84	8.74	3.86	15.28	0.42	0.13	0.42	0.34	0.5	0.3	0.16	0.28	0.19	0.39	0.56	0.11	0.56	0.49	0.63	0.72	0.07	0.72	0.67	0.76	70.08	38.53	62.29	46.66	83.43	80.02	41.47	71.58	54.79	95.49	3830	0.03
0.03	0.18	0.14	0.16	0.08	0.26	0.95	0.02	0.96	0.94	0.97	0.46	0.15	0.47	0.37	0.56	85.98	239.06	1.72	0.88	8.28	12.64	10.05	10.37	4.56	18.43	0.33	0.11	0.33	0.26	0.4	0.2	0.12	0.2	0.12	0.28	0.49	0.09	0.49	0.43	0.55	0.67	0.06	0.67	0.63	0.71	69.87	35.61	62.66	46.92	84.04	91.83	44.63	83.49	63.34	109.71	4513	0.07
0.06	0.09	0.11	0.08	0.02	0.15	0.92	0.03	0.92	0.9	0.94	0.37	0.16	0.38	0.26	0.47	91.52	463.86	1.96	1.03	7.15	14.18	10.56	11.85	6.08	20.02	0.26	0.12	0.26	0.18	0.33	0.14	0.1	0.12	0.07	0.2	0.43	0.09	0.43	0.38	0.5	0.64	0.07	0.64	0.6	0.68	68.88	35.67	62.04	46.51	81.46	111.18	58.76	101.15	77.23	131.45	6400	0.13
0.11	0.03	0.1	0.02	-0.03	0.09	0.87	0.04	0.88	0.85	0.9	0.27	0.17	0.29	0.17	0.39	88.37	270.93	2.08	1.12	7.99	14.3	10.99	11.87	5.62	20.27	0.19	0.12	0.2	0.11	0.27	0.1	0.09	0.08	0.04	0.16	0.38	0.09	0.38	0.33	0.45	0.6	0.07	0.61	0.56	0.65	70.84	40.79	62.34	46.81	85.36	151.22	88.12	135.16	105.02	180.09	6620	0.24
0.15	0.0	0.1	-0.01	-0.07	0.06	0.82	0.04	0.82	0.79	0.85	0.22	0.17	0.23	0.1	0.33	158.36	417.16	2.73	1.39	58.51	14.5	11.2	12.21	5.6	20.87	0.15	0.12	0.15	0.07	0.23	0.08	0.08	0.07	0.0	0.12	0.35	0.09	0.36	0.29	0.41	0.58	0.07	0.59	0.54	0.62	71.46	36.58	63.42	47.9	85.19	203.22	94.09	185.48	146.13	238.98	4107	0.39
0.18	-0.01	0.1	-0.01	-0.07	0.04	0.77	0.05	0.77	0.74	0.8	0.18	0.17	0.19	0.07	0.3	265.62	532.12	4.84	1.62	367.37	14.81	12.02	12.08	5.5	21.27	0.13	0.12	0.13	0.05	0.2	0.07	0.07	0.06	0.0	0.12	0.34	0.09	0.34	0.28	0.39	0.57	0.07	0.57	0.53	0.62	72.33	36.98	64.75	47.81	88.02	259.88	111.8	242.73	190.08	307.91	1897	0.54
0.32	-0.03	0.11	-0.03	-0.09	0.03	0.73	0.06	0.73	0.7	0.76	0.14	0.18	0.14	0.04	0.26	345.74	530.12	104.7	2.19	518.81	14.03	11.81	10.45	5.16	20.62	0.09	0.13	0.1	0.03	0.18	0.07	0.08	0.05	0.0	0.12	0.32	0.09	0.32	0.26	0.38	0.55	0.07	0.55	0.51	0.6	81.84	48.52	71.76	54.49	96.67	356.18	195.66	318.31	254.67	413.81	993	0.7


==> data_new/tef/imdb/bert/S_auc.tex <==
0.02

==> data_new/tef/imdb/bert/S_ppl.tex <==
4.8

==> data_new/tef/imdb/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.53	0.23	0.56	0.4	0.7	0.98	0.02	0.98	0.97	0.99	0.73	0.19	0.78	0.64	0.85	7.28	4.25	6.28	4.28	9.29	8.11	8.14	5.66	2.51	11.09	0.65	0.2	0.7	0.53	0.81	0.68	0.16	0.7	0.57	0.8	0.79	0.13	0.82	0.71	0.89	0.84	0.11	0.86	0.77	0.92	75.15	38.44	68.19	52.45	88.78	82.01	39.52	74.99	58.41	96.34	3353	0.03
0.03	0.29	0.24	0.3	0.14	0.46	0.95	0.02	0.96	0.94	0.97	0.57	0.19	0.61	0.47	0.7	9.4	5.14	8.0	5.61	12.23	10.09	9.15	7.79	3.39	13.88	0.5	0.19	0.53	0.39	0.64	0.53	0.14	0.54	0.44	0.63	0.7	0.12	0.72	0.63	0.8	0.77	0.1	0.79	0.71	0.85	75.17	38.51	68.19	52.42	88.81	91.28	43.64	83.86	66.17	106.25	3351	0.07
0.06	0.1	0.23	0.1	-0.06	0.25	0.92	0.03	0.92	0.9	0.94	0.39	0.19	0.42	0.3	0.52	11.13	6.05	9.49	6.67	14.45	11.16	9.66	8.71	3.86	15.58	0.35	0.17	0.37	0.25	0.47	0.39	0.13	0.39	0.31	0.48	0.61	0.11	0.63	0.55	0.7	0.71	0.1	0.73	0.66	0.78	75.34	39.51	68.24	52.46	88.83	106.6	50.77	98.05	78.65	122.95	3355	0.13
0.11	-0.03	0.22	-0.04	-0.18	0.11	0.88	0.04	0.88	0.86	0.9	0.25	0.17	0.27	0.16	0.37	12.32	6.69	10.51	7.31	15.92	11.82	10.15	9.14	4.28	16.39	0.23	0.15	0.25	0.15	0.33	0.29	0.12	0.29	0.21	0.36	0.54	0.1	0.55	0.48	0.62	0.66	0.09	0.68	0.62	0.73	75.4	40.35	68.19	52.43	88.81	125.07	61.05	115.12	93.6	143.37	3352	0.2
0.15	-0.15	0.21	-0.17	-0.3	-0.03	0.82	0.04	0.82	0.79	0.84	0.07	0.15	0.08	-0.02	0.17	13.54	7.44	11.53	7.93	17.61	12.05	10.22	9.55	4.35	16.87	0.09	0.13	0.09	0.01	0.17	0.2	0.1	0.2	0.12	0.26	0.45	0.09	0.45	0.39	0.51	0.6	0.08	0.61	0.55	0.65	74.64	35.26	68.13	52.35	88.72	159.43	59.72	149.84	123.43	183.5	3366	0.35
0.18	-0.23	0.2	-0.25	-0.37	-0.11	0.75	0.05	0.75	0.72	0.78	-0.06	0.14	-0.06	-0.15	0.03	14.28	7.99	12.04	8.24	18.49	12.25	10.19	9.9	4.63	17.0	-0.02	0.11	-0.02	-0.09	0.05	0.16	0.09	0.15	0.08	0.21	0.37	0.08	0.37	0.32	0.42	0.54	0.07	0.54	0.49	0.59	75.22	39.3	68.04	52.29	88.56	205.21	76.45	192.25	160.92	232.88	3425	0.54
0.32	-0.29	0.2	-0.31	-0.42	-0.17	0.66	0.06	0.67	0.62	0.7	-0.19	0.14	-0.19	-0.28	-0.1	15.27	8.58	12.97	8.69	19.76	12.12	10.22	9.52	4.52	16.71	-0.13	0.11	-0.13	-0.2	-0.06	0.13	0.09	0.12	0.07	0.18	0.3	0.08	0.29	0.25	0.34	0.47	0.06	0.47	0.43	0.51	75.05	37.98	68.22	52.5	88.84	292.54	116.33	271.55	220.48	338.33	6606	0.9


==> data_new/tef/imdb/cnn/IG_auc.tex <==
-0.02

==> data_new/tef/imdb/cnn/IG_ppl.tex <==
3.2

==> data_new/tef/imdb/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.83	0.11	0.85	0.79	0.9	0.98	0.02	0.98	0.97	0.99	0.88	0.09	0.89	0.85	0.93	113.25	69.14	99.58	61.27	151.02	4.08	3.77	3.05	1.37	5.64	0.78	0.1	0.79	0.71	0.86	0.66	0.15	0.67	0.56	0.76	0.82	0.09	0.83	0.78	0.88	0.89	0.06	0.9	0.86	0.94	74.96	38.4	68.03	52.28	88.6	83.28	40.17	76.46	58.92	98.25	3374	0.03
0.03	0.73	0.12	0.75	0.67	0.81	0.95	0.02	0.96	0.94	0.97	0.79	0.11	0.81	0.75	0.86	146.7	82.69	125.93	83.39	195.51	5.34	4.64	4.1	1.93	7.53	0.67	0.1	0.67	0.6	0.74	0.51	0.16	0.52	0.4	0.62	0.74	0.09	0.74	0.68	0.8	0.84	0.06	0.84	0.8	0.88	75.16	38.44	68.17	52.4	88.87	94.02	43.41	86.5	67.72	110.39	3366	0.08
0.06	0.62	0.14	0.64	0.55	0.72	0.92	0.03	0.92	0.9	0.94	0.69	0.12	0.71	0.63	0.77	179.8	97.79	152.87	102.56	245.11	6.49	5.5	5.17	2.29	9.18	0.55	0.1	0.55	0.49	0.62	0.39	0.17	0.4	0.28	0.5	0.64	0.09	0.65	0.59	0.71	0.78	0.06	0.79	0.74	0.82	75.34	39.47	68.22	52.46	88.91	111.3	51.09	102.43	81.96	129.67	3364	0.15
0.11	0.53	0.15	0.54	0.44	0.63	0.88	0.03	0.88	0.86	0.9	0.6	0.13	0.61	0.52	0.69	206.27	111.78	172.46	117.92	278.74	7.41	6.18	5.84	2.78	10.41	0.46	0.1	0.46	0.39	0.53	0.31	0.17	0.31	0.2	0.42	0.57	0.1	0.57	0.51	0.63	0.73	0.06	0.73	0.69	0.77	75.32	40.28	68.08	52.45	88.63	131.24	58.39	121.37	98.5	151.83	3365	0.23
0.15	0.4	0.16	0.41	0.3	0.51	0.82	0.04	0.82	0.79	0.85	0.46	0.15	0.47	0.36	0.56	243.25	131.23	204.49	140.7	327.05	8.52	6.97	6.75	3.26	12.03	0.33	0.11	0.34	0.26	0.41	0.23	0.16	0.21	0.12	0.32	0.47	0.1	0.47	0.41	0.54	0.66	0.07	0.66	0.62	0.7	74.76	35.33	68.24	52.51	88.78	166.01	59.54	155.18	128.79	191.29	3341	0.38
0.18	0.29	0.17	0.29	0.18	0.4	0.75	0.05	0.75	0.72	0.78	0.33	0.16	0.33	0.22	0.44	276.14	148.25	232.17	162.11	371.16	9.24	7.51	7.42	3.37	13.15	0.23	0.12	0.23	0.16	0.31	0.17	0.15	0.16	0.06	0.25	0.4	0.11	0.39	0.33	0.46	0.6	0.07	0.6	0.55	0.65	75.14	38.62	68.15	52.32	88.75	208.02	78.6	195.91	161.88	236.8	3350	0.54
0.32	0.13	0.19	0.12	-0.01	0.25	0.65	0.07	0.65	0.61	0.7	0.12	0.2	0.12	-0.02	0.26	331.89	184.72	276.45	192.57	441.05	10.24	8.22	8.41	3.86	14.42	0.08	0.14	0.08	-0.01	0.18	0.12	0.13	0.08	0.0	0.2	0.31	0.11	0.3	0.23	0.38	0.52	0.08	0.52	0.46	0.57	75.17	38.41	68.3	52.49	88.77	286.11	110.33	266.55	217.9	331.43	6648	0.86


==> data_new/tef/imdb/cnn/S_auc.tex <==
0.13

==> data_new/tef/imdb/cnn/S_ppl.tex <==
3.3

==> data_new/tef/imdb/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.41	0.28	0.43	0.23	0.62	0.98	0.02	0.98	0.97	0.99	0.8	0.09	0.81	0.75	0.87	2.03	0.84	1.92	1.47	2.51	13.27	13.25	9.08	3.72	18.34	0.74	0.1	0.74	0.67	0.8	0.7	0.12	0.71	0.64	0.78	0.84	0.07	0.84	0.8	0.88	0.89	0.05	0.89	0.86	0.92	76.17	44.49	68.61	53.04	89.3	83.66	45.67	75.82	59.42	97.18	3584	0.03
0.03	0.16	0.27	0.17	-0.02	0.35	0.95	0.02	0.95	0.94	0.97	0.66	0.1	0.67	0.6	0.73	2.49	0.85	2.38	1.89	3.0	17.0	15.34	12.72	5.69	23.73	0.59	0.1	0.6	0.53	0.66	0.55	0.12	0.56	0.48	0.64	0.76	0.07	0.76	0.71	0.8	0.83	0.05	0.84	0.8	0.87	75.68	38.9	68.56	53.0	89.3	93.39	45.65	84.94	67.45	108.45	3580	0.07
0.06	0.0	0.26	-0.02	-0.18	0.16	0.91	0.03	0.92	0.89	0.94	0.52	0.11	0.52	0.45	0.59	2.79	0.86	2.68	2.17	3.3	18.78	16.35	14.39	6.42	26.81	0.46	0.09	0.46	0.4	0.52	0.41	0.12	0.4	0.33	0.5	0.68	0.07	0.68	0.64	0.72	0.78	0.05	0.78	0.75	0.81	76.45	45.77	68.62	53.05	89.35	110.88	54.99	101.53	81.26	127.42	3587	0.14
0.11	-0.09	0.25	-0.11	-0.26	0.06	0.87	0.04	0.88	0.85	0.9	0.4	0.11	0.4	0.33	0.47	2.96	0.86	2.85	2.35	3.47	19.69	16.81	15.3	7.02	27.88	0.36	0.09	0.36	0.3	0.41	0.33	0.12	0.33	0.25	0.41	0.61	0.07	0.62	0.57	0.66	0.74	0.05	0.74	0.71	0.77	75.93	40.63	68.6	53.06	89.29	130.78	61.0	120.75	97.26	150.12	3581	0.22
0.15	-0.17	0.24	-0.2	-0.34	-0.02	0.81	0.05	0.81	0.78	0.84	0.25	0.11	0.25	0.18	0.33	3.11	0.87	3.01	2.51	3.61	20.29	17.0	16.01	7.51	28.81	0.23	0.09	0.23	0.18	0.29	0.27	0.11	0.27	0.2	0.35	0.53	0.07	0.54	0.49	0.58	0.68	0.05	0.68	0.65	0.71	75.27	38.66	68.5	52.89	89.08	168.55	68.65	157.27	129.02	193.02	3583	0.38
0.18	-0.22	0.23	-0.24	-0.38	-0.07	0.74	0.05	0.75	0.71	0.78	0.15	0.12	0.15	0.07	0.23	3.19	0.88	3.11	2.58	3.71	20.05	17.13	15.65	6.94	28.4	0.14	0.09	0.14	0.09	0.2	0.24	0.11	0.24	0.16	0.32	0.47	0.07	0.47	0.43	0.51	0.63	0.05	0.64	0.6	0.66	76.48	45.63	68.55	52.99	89.38	217.33	101.26	201.61	168.79	245.18	3624	0.57
0.32	-0.26	0.23	-0.28	-0.42	-0.11	0.66	0.06	0.66	0.61	0.7	0.05	0.13	0.05	-0.04	0.14	3.29	0.89	3.21	2.67	3.81	19.61	16.63	15.26	7.02	27.85	0.06	0.1	0.06	-0.01	0.12	0.21	0.11	0.2	0.14	0.28	0.41	0.07	0.41	0.36	0.46	0.58	0.05	0.58	0.55	0.62	75.67	39.66	68.63	53.07	89.29	299.27	109.61	278.6	226.79	348.36	7109	0.91


==> data_new/tef/imdb/lstm/IG_auc.tex <==
-0.03

==> data_new/tef/imdb/lstm/IG_ppl.tex <==
3.2

==> data_new/tef/imdb/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.64	0.16	0.65	0.55	0.74	0.97	0.02	0.98	0.97	0.99	0.88	0.12	0.9	0.85	0.94	59.35	30.93	53.26	39.25	72.47	8.88	7.8	6.67	2.94	13.02	0.8	0.09	0.81	0.74	0.87	0.66	0.15	0.68	0.6	0.76	0.83	0.1	0.84	0.79	0.89	0.9	0.07	0.91	0.87	0.94	76.18	44.28	68.84	53.11	89.33	84.56	45.4	76.94	60.15	97.88	3633	0.03
0.03	0.48	0.15	0.49	0.39	0.58	0.95	0.03	0.95	0.93	0.97	0.79	0.13	0.81	0.75	0.87	75.43	32.98	68.54	52.8	89.92	11.06	9.49	8.47	3.89	15.75	0.68	0.1	0.68	0.62	0.75	0.52	0.14	0.52	0.44	0.6	0.75	0.1	0.76	0.71	0.81	0.85	0.07	0.85	0.81	0.89	75.4	38.74	68.32	52.92	88.95	94.52	44.91	86.12	68.44	108.86	3627	0.08
0.06	0.36	0.13	0.35	0.27	0.44	0.91	0.03	0.91	0.89	0.93	0.69	0.12	0.7	0.63	0.77	89.76	36.09	82.45	64.55	107.18	13.0	10.88	10.35	4.64	18.36	0.56	0.1	0.56	0.49	0.63	0.38	0.12	0.38	0.3	0.46	0.67	0.08	0.67	0.62	0.72	0.8	0.06	0.8	0.76	0.84	76.47	45.74	68.63	53.05	89.44	113.62	68.43	103.53	82.29	130.09	3591	0.15
0.11	0.28	0.13	0.27	0.19	0.36	0.87	0.04	0.87	0.85	0.9	0.59	0.13	0.6	0.52	0.68	99.12	38.52	92.12	71.43	118.02	14.27	11.68	11.19	5.47	20.45	0.46	0.1	0.46	0.39	0.53	0.28	0.12	0.28	0.2	0.36	0.59	0.09	0.59	0.54	0.64	0.75	0.06	0.75	0.71	0.79	75.89	40.57	68.62	52.95	89.32	133.23	57.87	123.31	99.42	152.6	3592	0.23
0.15	0.19	0.12	0.18	0.1	0.26	0.81	0.05	0.81	0.78	0.84	0.45	0.13	0.46	0.37	0.54	110.36	41.26	103.15	80.86	132.36	15.1	12.09	12.2	5.9	21.72	0.33	0.1	0.33	0.27	0.4	0.19	0.11	0.18	0.12	0.25	0.49	0.08	0.49	0.44	0.54	0.69	0.06	0.69	0.65	0.72	75.49	38.85	68.57	53.01	89.28	171.49	74.93	160.4	131.49	196.25	3562	0.39
0.18	0.12	0.12	0.11	0.04	0.19	0.74	0.05	0.74	0.71	0.78	0.33	0.14	0.33	0.24	0.42	119.11	43.45	112.36	87.29	143.62	15.45	12.41	12.29	5.94	21.92	0.23	0.1	0.23	0.17	0.3	0.14	0.1	0.12	0.07	0.2	0.41	0.08	0.41	0.36	0.47	0.63	0.06	0.63	0.59	0.67	76.15	44.56	68.58	52.95	89.3	218.6	119.05	204.14	169.84	247.03	3572	0.58
0.32	0.04	0.12	0.02	-0.05	0.11	0.65	0.07	0.65	0.6	0.69	0.13	0.17	0.13	0.02	0.24	133.9	48.27	126.72	98.0	161.82	15.98	12.52	13.05	6.2	22.9	0.09	0.11	0.09	0.01	0.17	0.09	0.09	0.08	0.04	0.14	0.32	0.09	0.32	0.26	0.38	0.55	0.07	0.55	0.51	0.59	75.88	40.43	68.62	53.08	89.31	303.73	120.48	282.97	230.37	351.35	7071	0.93


==> data_new/tef/imdb/lstm/S_auc.tex <==
0.07

==> data_new/tef/imdb/lstm/S_ppl.tex <==
3.2

==> data_new/tef/imdb/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.58	0.18	0.59	0.46	0.71	0.97	0.02	0.98	0.97	0.99	0.9	0.07	0.92	0.87	0.95	0.15	0.07	0.14	0.11	0.19	18.33	17.64	13.22	5.59	25.35	0.81	0.09	0.82	0.76	0.87	0.61	0.14	0.61	0.52	0.71	0.83	0.08	0.84	0.78	0.88	0.91	0.05	0.91	0.88	0.95	75.12	36.29	68.37	52.83	89.04	83.63	38.03	76.84	59.94	98.06	3563	0.03
0.03	0.37	0.18	0.35	0.24	0.49	0.95	0.03	0.95	0.93	0.96	0.8	0.11	0.82	0.74	0.88	0.2	0.07	0.19	0.15	0.24	24.74	22.21	18.48	8.25	34.55	0.68	0.11	0.68	0.61	0.75	0.42	0.15	0.43	0.32	0.52	0.73	0.09	0.73	0.67	0.79	0.85	0.06	0.85	0.81	0.89	75.14	36.36	68.36	52.81	89.07	94.53	41.59	86.85	68.61	111.08	3561	0.08
0.06	0.21	0.16	0.19	0.09	0.3	0.91	0.04	0.91	0.88	0.93	0.67	0.14	0.68	0.58	0.77	0.24	0.08	0.23	0.19	0.28	30.07	25.57	23.76	10.9	41.95	0.54	0.12	0.55	0.46	0.63	0.27	0.14	0.27	0.17	0.36	0.62	0.1	0.62	0.55	0.68	0.78	0.08	0.79	0.73	0.83	75.4	37.84	68.39	52.86	89.08	112.31	48.29	103.89	83.23	129.77	3566	0.15
0.11	0.12	0.14	0.09	0.02	0.19	0.86	0.04	0.87	0.84	0.89	0.55	0.17	0.56	0.44	0.67	0.26	0.08	0.25	0.21	0.3	32.29	26.2	25.87	12.19	45.84	0.43	0.13	0.43	0.34	0.52	0.18	0.12	0.16	0.08	0.25	0.53	0.11	0.53	0.46	0.6	0.73	0.08	0.73	0.68	0.78	75.17	36.54	68.36	52.81	89.05	132.57	52.76	123.36	100.15	152.62	3561	0.23
0.15	0.03	0.12	0.0	-0.05	0.08	0.8	0.05	0.8	0.77	0.83	0.39	0.19	0.39	0.26	0.52	0.26	0.07	0.26	0.22	0.3	33.0	25.73	27.02	12.93	47.68	0.29	0.14	0.29	0.2	0.39	0.1	0.1	0.08	0.0	0.16	0.43	0.11	0.42	0.35	0.5	0.66	0.09	0.66	0.6	0.71	74.77	34.52	68.26	52.76	88.98	170.64	59.55	160.71	132.16	195.89	3564	0.39
0.18	-0.03	0.11	-0.05	-0.09	0.01	0.74	0.05	0.74	0.7	0.77	0.25	0.2	0.25	0.12	0.4	0.25	0.06	0.25	0.21	0.29	31.86	24.72	26.34	12.62	45.62	0.19	0.14	0.18	0.09	0.29	0.06	0.08	0.04	0.0	0.09	0.35	0.11	0.34	0.28	0.41	0.6	0.09	0.6	0.54	0.66	75.16	36.42	68.35	52.77	89.08	216.86	72.49	204.83	171.1	246.65	3571	0.58
0.32	-0.11	0.11	-0.12	-0.18	-0.06	0.64	0.07	0.64	0.59	0.68	0.03	0.23	0.02	-0.14	0.19	0.23	0.06	0.23	0.2	0.26	31.73	23.9	26.88	12.67	45.85	0.03	0.16	0.02	-0.08	0.13	0.03	0.06	0.0	0.0	0.05	0.25	0.11	0.24	0.17	0.32	0.51	0.09	0.51	0.45	0.57	75.05	36.17	68.37	52.86	89.04	308.11	110.29	288.83	235.37	357.77	7102	0.95


==> data_new/tef/imdb/lstmatt/A_auc.tex <==
0.03

==> data_new/tef/imdb/lstmatt/A_ppl.tex <==
3.3

==> data_new/tef/imdb/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.34	0.29	0.36	0.16	0.55	0.97	0.02	0.98	0.97	0.99	0.65	0.18	0.68	0.57	0.77	9.19	64.3	3.56	2.02	5.58	16.25	17.43	10.74	4.18	22.37	0.55	0.16	0.57	0.47	0.66	0.56	0.17	0.56	0.45	0.68	0.72	0.11	0.72	0.66	0.79	0.8	0.08	0.81	0.76	0.85	75.12	36.29	68.37	52.83	89.04	83.15	37.98	75.96	59.37	97.65	3563	0.03
0.03	0.1	0.28	0.11	-0.08	0.3	0.95	0.03	0.95	0.93	0.97	0.49	0.18	0.52	0.4	0.62	18.08	124.91	4.68	3.01	6.98	19.61	19.53	13.9	5.68	27.06	0.41	0.15	0.42	0.33	0.51	0.42	0.16	0.42	0.32	0.52	0.63	0.11	0.64	0.57	0.7	0.74	0.08	0.75	0.7	0.8	75.14	36.36	68.36	52.81	89.07	93.58	42.41	85.7	67.62	109.54	3561	0.08
0.06	-0.07	0.26	-0.07	-0.24	0.11	0.91	0.03	0.91	0.89	0.93	0.34	0.18	0.36	0.24	0.46	56.15	592.53	5.44	3.75	8.24	21.91	21.24	16.07	6.62	30.25	0.28	0.14	0.3	0.2	0.38	0.31	0.14	0.31	0.2	0.4	0.55	0.11	0.56	0.49	0.62	0.68	0.08	0.69	0.64	0.74	75.25	37.84	68.34	52.69	89.04	110.52	50.55	101.41	81.13	127.85	3583	0.14
0.11	-0.17	0.24	-0.17	-0.33	-0.02	0.87	0.04	0.87	0.84	0.9	0.21	0.19	0.23	0.11	0.34	250.98	3220.35	6.01	4.19	9.8	24.11	23.93	17.18	7.12	33.29	0.18	0.15	0.2	0.1	0.28	0.24	0.13	0.24	0.15	0.32	0.48	0.11	0.49	0.42	0.55	0.64	0.08	0.65	0.59	0.69	74.9	36.38	68.24	52.46	88.81	130.58	54.74	121.25	97.5	150.44	3785	0.23
0.15	-0.26	0.23	-0.27	-0.42	-0.12	0.8	0.05	0.81	0.77	0.84	0.09	0.17	0.1	-0.01	0.21	199.59	2310.23	6.25	4.45	9.97	24.44	23.53	17.49	7.51	34.52	0.09	0.13	0.09	0.01	0.18	0.19	0.11	0.18	0.12	0.26	0.42	0.1	0.43	0.36	0.49	0.59	0.07	0.6	0.55	0.64	74.17	33.88	67.86	52.57	88.24	167.03	59.95	156.67	129.43	191.7	3753	0.38
0.18	-0.31	0.22	-0.32	-0.46	-0.16	0.75	0.05	0.75	0.71	0.78	0.02	0.16	0.02	-0.08	0.12	91.43	707.75	6.19	4.49	9.25	24.1	22.26	17.44	7.72	34.33	0.03	0.12	0.04	-0.04	0.11	0.17	0.11	0.16	0.08	0.24	0.38	0.09	0.38	0.33	0.44	0.56	0.07	0.57	0.52	0.61	75.22	36.15	68.35	52.84	89.61	213.97	73.96	200.82	169.0	243.94	3656	0.57
0.32	-0.36	0.2	-0.37	-0.5	-0.22	0.67	0.06	0.67	0.63	0.71	-0.05	0.15	-0.05	-0.15	0.05	78.7	2226.73	5.89	4.39	8.05	23.29	21.49	16.88	7.79	32.52	-0.02	0.11	-0.03	-0.1	0.05	0.15	0.1	0.14	0.08	0.21	0.35	0.09	0.34	0.29	0.4	0.53	0.06	0.53	0.49	0.57	75.59	36.77	68.68	53.23	89.45	293.63	111.92	272.8	222.42	338.59	6587	0.89


==> data_new/tef/imdb/lstmatt/IG_auc.tex <==
-0.06

==> data_new/tef/imdb/lstmatt/IG_ppl.tex <==
3.3

==> data_new/tef/imdb/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.71	0.14	0.72	0.62	0.81	0.97	0.02	0.98	0.96	0.99	0.84	0.12	0.87	0.78	0.92	99.99	71.96	82.74	45.65	134.9	16.82	14.83	12.72	5.38	24.4	0.69	0.13	0.7	0.62	0.78	0.6	0.15	0.6	0.5	0.69	0.76	0.1	0.77	0.7	0.83	0.85	0.07	0.85	0.8	0.9	75.12	36.29	68.37	52.83	89.04	83.91	37.92	77.12	60.6	98.34	3563	0.04
0.03	0.55	0.15	0.55	0.45	0.66	0.94	0.03	0.95	0.93	0.96	0.72	0.16	0.75	0.63	0.84	137.24	88.88	119.76	68.13	183.6	22.64	18.56	17.75	8.2	32.81	0.56	0.14	0.57	0.47	0.67	0.46	0.15	0.47	0.36	0.56	0.66	0.11	0.67	0.59	0.74	0.78	0.08	0.79	0.73	0.84	75.1	36.34	68.32	52.81	89.04	94.88	41.46	87.43	69.27	110.63	3561	0.08
0.06	0.41	0.15	0.41	0.31	0.51	0.91	0.04	0.91	0.89	0.93	0.57	0.2	0.6	0.45	0.73	174.0	104.25	158.86	92.68	227.44	28.22	21.74	23.41	10.96	40.84	0.44	0.16	0.44	0.33	0.55	0.37	0.15	0.36	0.27	0.47	0.57	0.12	0.58	0.5	0.65	0.71	0.09	0.72	0.65	0.78	75.36	37.83	68.36	52.83	89.09	112.98	48.48	103.72	84.11	131.43	3566	0.15
0.11	0.32	0.15	0.31	0.22	0.42	0.87	0.04	0.87	0.84	0.89	0.46	0.22	0.48	0.32	0.62	203.96	116.08	189.04	115.0	265.42	32.19	24.15	27.43	12.69	47.32	0.34	0.16	0.35	0.23	0.46	0.31	0.14	0.31	0.2	0.4	0.51	0.12	0.51	0.43	0.59	0.66	0.1	0.67	0.6	0.73	75.13	36.52	68.32	52.81	89.03	133.63	52.91	123.73	100.94	155.35	3561	0.24
0.15	0.23	0.15	0.22	0.13	0.32	0.8	0.05	0.8	0.77	0.83	0.33	0.24	0.34	0.18	0.5	235.63	125.83	220.78	144.14	300.84	35.41	26.16	30.54	14.17	52.13	0.24	0.17	0.24	0.13	0.36	0.25	0.14	0.24	0.14	0.33	0.44	0.12	0.45	0.36	0.53	0.61	0.1	0.61	0.54	0.67	74.69	34.43	68.24	52.7	89.02	172.52	61.42	161.64	133.91	198.66	3570	0.4
0.18	0.17	0.15	0.16	0.07	0.26	0.74	0.05	0.74	0.71	0.77	0.23	0.24	0.23	0.06	0.39	254.77	133.52	234.99	163.59	320.47	36.1	26.36	31.26	14.68	52.66	0.17	0.17	0.17	0.05	0.28	0.21	0.14	0.2	0.1	0.29	0.39	0.12	0.39	0.31	0.49	0.57	0.1	0.57	0.5	0.63	75.26	37.36	68.31	52.69	89.03	219.31	73.62	206.08	173.46	250.76	3597	0.59
0.32	0.11	0.16	0.09	-0.0	0.2	0.66	0.06	0.66	0.62	0.7	0.09	0.25	0.08	-0.09	0.26	264.52	132.25	245.41	179.22	325.75	35.6	25.93	30.57	14.47	52.35	0.07	0.17	0.06	-0.05	0.18	0.16	0.13	0.14	0.06	0.24	0.34	0.13	0.33	0.25	0.42	0.51	0.1	0.51	0.44	0.58	75.0	35.7	68.38	52.91	89.03	299.74	108.89	279.94	229.13	346.85	7070	0.92


==> data_new/tef/imdb/lstmatt/S_auc.tex <==
0.09

==> data_new/tef/imdb/lstmatt/S_ppl.tex <==
3.3

==> data_new/tef/imdb/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.8	0.14	0.82	0.7	0.91	0.97	0.02	0.98	0.97	0.99	0.94	0.02	0.94	0.92	0.95	4.09	1.84	3.75	2.84	4.98	10.11	12.71	5.93	2.42	12.14	0.8	0.04	0.8	0.77	0.83	0.79	0.06	0.79	0.76	0.83	0.87	0.03	0.87	0.85	0.89	0.91	0.02	0.91	0.89	0.92	60.61	30.11	55.11	42.63	71.35	69.74	32.8	63.48	49.48	82.72	3748	0.02
0.03	0.72	0.15	0.71	0.63	0.85	0.95	0.03	0.95	0.94	0.97	0.89	0.03	0.9	0.87	0.91	4.86	1.79	4.66	3.6	5.83	12.26	13.19	8.04	3.44	16.29	0.73	0.04	0.73	0.7	0.76	0.72	0.06	0.72	0.68	0.76	0.82	0.03	0.82	0.8	0.84	0.87	0.02	0.87	0.86	0.89	60.61	30.12	55.14	42.61	71.35	82.23	38.91	75.74	58.45	97.67	3745	0.05
0.06	0.64	0.16	0.63	0.54	0.77	0.91	0.03	0.92	0.89	0.94	0.84	0.04	0.85	0.82	0.87	5.59	1.81	5.5	4.33	6.64	14.67	14.11	10.57	4.52	20.42	0.67	0.05	0.67	0.64	0.7	0.65	0.07	0.66	0.61	0.7	0.78	0.04	0.78	0.75	0.8	0.84	0.03	0.84	0.82	0.86	60.7	30.65	55.14	42.57	71.35	104.02	47.44	95.87	74.39	122.46	3759	0.1
0.11	0.56	0.17	0.56	0.45	0.68	0.87	0.04	0.88	0.85	0.9	0.8	0.05	0.81	0.77	0.84	6.19	1.88	6.17	4.87	7.35	16.79	15.12	12.57	5.42	23.75	0.62	0.05	0.62	0.58	0.65	0.6	0.07	0.61	0.56	0.65	0.74	0.04	0.74	0.72	0.77	0.81	0.03	0.82	0.8	0.83	60.46	29.57	55.04	42.56	71.3	132.6	58.4	122.56	95.81	156.38	3769	0.17
0.15	0.46	0.17	0.45	0.34	0.57	0.81	0.05	0.81	0.78	0.84	0.74	0.06	0.75	0.71	0.79	6.99	2.03	7.07	5.56	8.35	20.03	16.98	15.89	6.91	29.0	0.56	0.06	0.56	0.52	0.6	0.54	0.08	0.55	0.5	0.59	0.7	0.04	0.7	0.67	0.73	0.78	0.03	0.79	0.77	0.81	60.39	29.93	54.95	42.4	71.21	192.53	80.61	177.77	140.55	226.83	3811	0.31
0.18	0.37	0.16	0.35	0.25	0.48	0.75	0.06	0.75	0.71	0.78	0.7	0.07	0.71	0.65	0.75	7.65	2.15	7.72	6.14	9.06	23.24	19.25	18.81	8.26	33.3	0.51	0.06	0.52	0.47	0.56	0.5	0.08	0.5	0.45	0.55	0.67	0.05	0.67	0.64	0.7	0.76	0.03	0.76	0.74	0.78	60.1	30.58	54.68	41.99	71.12	271.51	115.57	250.7	200.86	316.65	5152	0.5
0.32	0.29	0.15	0.26	0.18	0.38	0.68	0.07	0.68	0.63	0.72	0.65	0.08	0.66	0.6	0.71	8.25	2.28	8.31	6.66	9.78	26.01	21.15	21.03	9.61	37.13	0.47	0.07	0.48	0.43	0.52	0.46	0.08	0.46	0.41	0.51	0.64	0.05	0.64	0.61	0.67	0.74	0.04	0.74	0.72	0.77	60.99	31.2	55.5	42.96	71.8	410.57	211.91	369.36	285.22	484.18	7427	0.82


==> data_new/tef/imdb/roberta/A_auc.tex <==
0.15

==> data_new/tef/imdb/roberta/A_ppl.tex <==
7.0

==> data_new/tef/imdb/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.34	0.41	0.4	0.09	0.66	0.98	0.02	0.98	0.97	0.99	0.58	0.38	0.76	0.3	0.9	15.62	45.19	3.58	1.49	16.51	23.46	25.96	13.47	5.95	31.71	0.49	0.34	0.61	0.21	0.8	0.53	0.28	0.6	0.27	0.78	0.66	0.23	0.74	0.46	0.87	0.76	0.17	0.82	0.62	0.91	60.63	30.11	55.17	42.6	71.35	70.14	32.64	64.14	49.69	82.95	3779	0.02
0.03	0.16	0.4	0.16	-0.05	0.49	0.95	0.02	0.96	0.94	0.97	0.44	0.4	0.49	0.13	0.81	23.96	60.84	6.44	2.06	26.65	28.08	28.74	17.96	7.8	39.03	0.36	0.34	0.37	0.09	0.69	0.41	0.26	0.4	0.17	0.67	0.58	0.23	0.58	0.38	0.8	0.7	0.17	0.71	0.56	0.86	60.33	29.48	54.91	42.84	71.1	82.65	38.44	75.52	59.79	96.98	3689	0.05
0.06	0.03	0.38	0.01	-0.16	0.32	0.92	0.03	0.92	0.9	0.94	0.3	0.4	0.25	0.02	0.69	33.83	81.03	13.28	2.95	36.94	33.28	31.17	23.73	9.62	46.59	0.24	0.33	0.18	0.01	0.57	0.31	0.23	0.24	0.12	0.53	0.5	0.22	0.44	0.32	0.72	0.64	0.17	0.61	0.52	0.81	60.37	30.82	54.4	42.02	71.7	104.91	51.65	96.06	75.63	122.89	2819	0.11
0.11	-0.06	0.35	-0.05	-0.23	0.18	0.87	0.04	0.88	0.85	0.9	0.19	0.36	0.1	-0.05	0.56	35.11	48.11	20.13	3.87	44.01	34.88	30.44	26.31	11.27	49.83	0.16	0.29	0.07	-0.03	0.44	0.25	0.2	0.19	0.08	0.4	0.44	0.2	0.38	0.29	0.63	0.6	0.16	0.55	0.49	0.75	60.07	29.78	54.4	41.61	71.53	137.81	65.54	124.98	98.21	164.8	2189	0.19
0.15	-0.15	0.31	-0.15	-0.31	0.02	0.81	0.05	0.81	0.78	0.85	0.09	0.31	0.0	-0.12	0.36	31.89	39.04	21.33	5.33	40.24	35.91	30.21	27.18	12.17	50.98	0.08	0.24	0.0	-0.08	0.27	0.19	0.17	0.12	0.05	0.31	0.38	0.17	0.33	0.26	0.53	0.56	0.13	0.52	0.48	0.66	62.11	43.49	55.89	42.66	71.93	201.33	119.82	183.68	142.41	232.47	1557	0.33
0.18	-0.21	0.27	-0.23	-0.38	-0.05	0.76	0.05	0.76	0.73	0.8	0.01	0.27	-0.08	-0.17	0.14	29.35	37.61	21.52	7.68	36.0	38.12	30.89	29.05	14.03	55.06	0.02	0.21	-0.05	-0.12	0.11	0.14	0.14	0.09	0.04	0.2	0.34	0.15	0.3	0.24	0.42	0.53	0.11	0.5	0.46	0.59	61.45	36.61	55.39	42.91	71.73	273.79	142.47	252.97	195.54	318.68	1160	0.51
0.32	-0.24	0.24	-0.26	-0.39	-0.11	0.69	0.08	0.69	0.64	0.74	-0.05	0.24	-0.12	-0.21	0.06	26.33	24.59	22.16	8.75	35.81	39.43	30.08	32.35	16.77	56.8	-0.03	0.18	-0.08	-0.14	0.04	0.11	0.12	0.08	0.04	0.16	0.31	0.13	0.27	0.22	0.37	0.51	0.1	0.48	0.44	0.55	60.18	27.3	55.83	42.88	72.22	412.06	196.18	368.25	281.24	499.95	1379	0.86


==> data_new/tef/imdb/roberta/IG_auc.tex <==
-0.03

==> data_new/tef/imdb/roberta/IG_ppl.tex <==
6.8

==> data_new/tef/imdb/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.32	0.2	0.3	0.16	0.45	0.98	0.02	0.98	0.97	0.99	0.68	0.22	0.75	0.58	0.84	161.71	1143.21	10.48	4.51	37.2	16.98	16.73	11.61	4.88	23.62	0.53	0.19	0.57	0.42	0.67	0.45	0.2	0.44	0.3	0.6	0.66	0.15	0.68	0.57	0.77	0.77	0.11	0.79	0.71	0.85	60.54	30.02	54.88	42.72	71.21	69.98	32.71	63.97	49.85	82.42	3775	0.02
0.03	0.21	0.16	0.18	0.08	0.31	0.95	0.02	0.96	0.94	0.97	0.56	0.24	0.61	0.41	0.75	284.79	2067.15	18.55	7.17	81.27	20.91	18.58	15.5	6.53	30.19	0.42	0.19	0.44	0.29	0.57	0.32	0.18	0.32	0.19	0.44	0.57	0.15	0.59	0.47	0.69	0.71	0.11	0.73	0.64	0.8	60.28	29.63	55.15	42.47	71.13	81.83	36.78	74.93	58.41	96.7	3991	0.05
0.06	0.13	0.13	0.1	0.04	0.2	0.92	0.03	0.92	0.9	0.94	0.43	0.24	0.46	0.26	0.62	531.7	3685.1	34.51	11.67	134.43	26.01	21.39	20.63	8.65	38.28	0.31	0.19	0.32	0.18	0.45	0.23	0.16	0.2	0.12	0.32	0.5	0.14	0.5	0.39	0.59	0.66	0.11	0.66	0.58	0.74	60.02	29.46	54.53	42.65	70.56	102.49	44.93	94.4	73.79	121.41	4593	0.1
0.11	0.09	0.11	0.07	0.01	0.14	0.88	0.04	0.89	0.86	0.91	0.38	0.23	0.39	0.22	0.55	345.35	2208.72	34.85	14.58	112.49	24.68	19.84	20.48	8.49	36.16	0.27	0.17	0.27	0.15	0.39	0.19	0.14	0.16	0.08	0.27	0.47	0.13	0.46	0.37	0.55	0.64	0.1	0.64	0.57	0.71	59.23	29.56	53.59	41.72	69.85	130.93	58.18	120.99	94.19	153.84	4734	0.17
0.15	0.05	0.1	0.03	-0.02	0.1	0.83	0.04	0.83	0.8	0.86	0.3	0.23	0.3	0.13	0.46	294.97	1531.87	34.94	15.61	90.96	22.62	18.24	18.07	8.17	32.91	0.21	0.16	0.21	0.09	0.32	0.15	0.12	0.12	0.06	0.2	0.42	0.12	0.41	0.33	0.5	0.61	0.09	0.61	0.54	0.67	59.75	27.76	54.84	42.16	70.48	182.74	75.95	169.26	130.64	216.34	4352	0.29
0.18	0.02	0.1	0.01	-0.04	0.08	0.78	0.05	0.78	0.75	0.81	0.25	0.23	0.26	0.09	0.42	264.75	1189.87	36.64	14.93	107.48	23.71	18.1	20.33	9.46	33.71	0.18	0.16	0.18	0.06	0.29	0.13	0.12	0.11	0.04	0.2	0.4	0.12	0.39	0.31	0.48	0.59	0.09	0.59	0.53	0.66	60.27	29.89	55.13	42.87	72.07	245.39	108.81	225.37	175.52	292.22	2791	0.44
0.32	0.0	0.11	-0.01	-0.06	0.06	0.74	0.06	0.74	0.7	0.78	0.21	0.24	0.2	0.03	0.38	324.52	1100.26	37.59	14.8	144.56	22.95	18.14	18.75	9.09	33.41	0.15	0.17	0.14	0.03	0.26	0.1	0.11	0.08	0.0	0.16	0.37	0.13	0.36	0.28	0.46	0.58	0.1	0.58	0.51	0.65	68.09	40.25	61.36	45.75	77.96	362.46	184.54	325.29	243.29	430.91	1710	0.62


==> data_new/tef/imdb/roberta/S_auc.tex <==
0.03

==> data_new/tef/imdb/roberta/S_ppl.tex <==
7.0

==> data_new/tef/imdb/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.88	0.05	0.89	0.86	0.92	0.97	0.02	0.98	0.97	0.99	0.93	0.03	0.94	0.91	0.95	1.56	0.47	1.59	1.29	1.85	3.06	3.09	2.12	0.88	4.21	0.81	0.06	0.81	0.77	0.84	0.81	0.06	0.81	0.77	0.85	0.87	0.04	0.87	0.85	0.9	0.91	0.03	0.91	0.9	0.93	61.29	30.49	55.71	43.07	72.4	72.02	33.82	65.86	50.98	84.77	3750	0.03
0.03	0.81	0.07	0.81	0.77	0.85	0.95	0.03	0.95	0.93	0.96	0.88	0.05	0.88	0.85	0.91	2.01	0.52	2.04	1.7	2.34	4.12	3.9	3.01	1.29	5.77	0.72	0.06	0.73	0.69	0.76	0.73	0.07	0.73	0.69	0.77	0.81	0.04	0.81	0.79	0.84	0.87	0.03	0.87	0.85	0.89	61.31	30.52	55.72	43.02	72.47	85.7	39.97	78.43	61.11	100.92	3757	0.07
0.06	0.72	0.08	0.73	0.68	0.78	0.9	0.04	0.91	0.88	0.93	0.81	0.06	0.82	0.78	0.85	2.42	0.57	2.46	2.09	2.78	5.21	4.68	3.84	1.67	7.54	0.64	0.06	0.64	0.6	0.68	0.64	0.07	0.65	0.6	0.69	0.75	0.05	0.75	0.72	0.78	0.83	0.03	0.83	0.81	0.85	61.6	32.61	55.75	43.14	72.5	109.65	54.35	100.61	78.83	129.67	3777	0.13
0.11	0.64	0.09	0.65	0.59	0.7	0.86	0.05	0.86	0.83	0.89	0.75	0.07	0.76	0.71	0.8	2.76	0.63	2.78	2.37	3.16	6.21	5.46	4.65	2.1	8.8	0.57	0.07	0.58	0.53	0.62	0.57	0.07	0.57	0.53	0.62	0.7	0.05	0.7	0.67	0.74	0.79	0.04	0.8	0.77	0.82	61.07	28.32	55.83	43.05	72.33	139.39	57.14	129.44	101.84	165.32	3757	0.22
0.15	0.53	0.1	0.54	0.47	0.6	0.79	0.06	0.79	0.75	0.83	0.66	0.08	0.67	0.61	0.72	3.17	0.71	3.18	2.73	3.59	7.51	6.43	5.86	2.52	10.65	0.49	0.07	0.49	0.44	0.54	0.49	0.07	0.49	0.44	0.53	0.64	0.05	0.64	0.6	0.67	0.75	0.04	0.75	0.72	0.78	61.23	30.39	55.72	43.06	72.36	203.64	83.21	188.68	151.26	239.15	3769	0.39
0.18	0.44	0.11	0.44	0.37	0.51	0.72	0.06	0.72	0.68	0.76	0.58	0.09	0.58	0.52	0.65	3.54	0.82	3.5	3.03	3.97	8.81	7.53	6.74	2.99	12.73	0.42	0.08	0.42	0.36	0.47	0.42	0.07	0.42	0.37	0.47	0.59	0.05	0.59	0.55	0.62	0.71	0.04	0.71	0.69	0.74	60.73	30.21	55.29	42.79	71.73	287.84	114.42	268.65	216.63	336.01	3772	0.63
0.32	0.35	0.1	0.35	0.28	0.43	0.64	0.07	0.64	0.59	0.68	0.5	0.1	0.51	0.44	0.58	3.88	0.9	3.83	3.31	4.36	9.67	8.32	7.45	3.29	13.87	0.36	0.08	0.36	0.3	0.41	0.36	0.07	0.36	0.31	0.41	0.54	0.05	0.54	0.5	0.58	0.68	0.04	0.68	0.65	0.71	61.37	30.71	55.87	43.33	72.72	426.88	192.7	388.91	302.77	505.53	5373	1.0


==> data_new/tef/imdb/xlnet/A_auc.tex <==
0.18

==> data_new/tef/imdb/xlnet/A_ppl.tex <==
6.0

==> data_new/tef/imdb/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.15	0.41	0.16	-0.07	0.42	0.97	0.02	0.98	0.96	0.99	0.36	0.34	0.4	0.14	0.6	15.22	65.68	2.45	0.95	8.24	4.92	8.04	2.67	1.14	5.66	0.28	0.27	0.3	0.1	0.46	0.35	0.21	0.33	0.18	0.48	0.51	0.18	0.53	0.38	0.63	0.65	0.14	0.66	0.56	0.75	60.77	29.28	55.74	43.24	72.6	70.48	32.68	64.76	50.12	83.77	3552	0.03
0.03	-0.04	0.35	-0.04	-0.22	0.14	0.95	0.03	0.95	0.93	0.97	0.18	0.29	0.19	0.02	0.36	24.95	178.46	3.95	1.46	12.63	5.45	7.81	3.17	1.33	6.58	0.14	0.22	0.14	0.01	0.27	0.23	0.16	0.2	0.12	0.32	0.42	0.14	0.42	0.32	0.51	0.58	0.11	0.59	0.52	0.66	60.49	30.08	55.11	42.65	71.24	81.49	38.01	74.43	58.17	95.88	2999	0.06
0.06	-0.13	0.29	-0.13	-0.31	0.03	0.9	0.04	0.91	0.88	0.93	0.08	0.25	0.1	-0.06	0.24	12.85	74.39	2.97	1.29	8.74	4.59	5.26	3.21	1.42	5.88	0.07	0.19	0.07	-0.04	0.17	0.19	0.13	0.16	0.1	0.25	0.37	0.12	0.38	0.3	0.45	0.55	0.1	0.55	0.49	0.61	61.61	32.35	55.88	43.14	72.53	105.25	53.53	96.64	74.32	124.13	3883	0.12
0.11	-0.23	0.26	-0.25	-0.41	-0.08	0.86	0.05	0.86	0.83	0.89	-0.02	0.24	-0.01	-0.17	0.13	6.01	10.83	2.56	1.23	6.62	4.72	5.29	3.43	1.55	6.13	-0.01	0.17	-0.0	-0.12	0.09	0.14	0.11	0.12	0.06	0.2	0.32	0.11	0.33	0.25	0.4	0.51	0.09	0.52	0.45	0.57	60.55	27.76	55.13	42.46	72.56	134.45	56.11	124.12	97.45	160.1	2742	0.21
0.15	-0.37	0.22	-0.38	-0.52	-0.24	0.79	0.06	0.79	0.76	0.83	-0.17	0.21	-0.16	-0.32	-0.04	5.37	8.01	2.24	1.18	6.04	4.7	4.52	3.62	1.68	6.26	-0.12	0.15	-0.11	-0.22	-0.02	0.09	0.09	0.08	0.0	0.12	0.26	0.1	0.26	0.19	0.33	0.46	0.08	0.46	0.4	0.52	59.02	31.94	53.57	41.18	69.18	192.35	82.14	180.65	140.57	225.02	1488	0.38
0.18	-0.41	0.19	-0.42	-0.53	-0.3	0.74	0.06	0.74	0.71	0.78	-0.21	0.17	-0.2	-0.33	-0.11	5.01	6.19	2.42	1.31	6.44	4.81	5.03	3.5	1.73	6.43	-0.15	0.12	-0.14	-0.22	-0.07	0.07	0.07	0.06	0.0	0.12	0.24	0.08	0.24	0.18	0.29	0.44	0.07	0.45	0.4	0.49	61.31	32.6	55.94	42.99	74.01	262.24	102.27	247.22	191.94	313.85	1388	0.55
0.32	-0.4	0.17	-0.41	-0.5	-0.29	0.7	0.06	0.7	0.66	0.74	-0.2	0.14	-0.21	-0.29	-0.12	5.99	6.95	3.18	1.5	8.09	4.49	4.85	3.16	1.45	5.89	-0.14	0.1	-0.14	-0.2	-0.08	0.07	0.07	0.06	0.0	0.12	0.24	0.07	0.24	0.2	0.29	0.45	0.06	0.45	0.41	0.48	66.75	42.49	58.97	46.62	77.58	359.38	164.2	325.31	258.29	427.82	1227	0.74


==> data_new/tef/imdb/xlnet/IG_auc.tex <==
-0.09

==> data_new/tef/imdb/xlnet/IG_ppl.tex <==
5.9

==> data_new/tef/imdb/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.56	0.28	0.63	0.38	0.76	0.97	0.02	0.98	0.96	0.99	0.76	0.26	0.88	0.7	0.93	1685.37	6154.64	170.42	62.91	848.78	13.74	15.13	8.56	3.4	18.37	0.63	0.24	0.71	0.53	0.79	0.54	0.25	0.6	0.4	0.72	0.72	0.19	0.79	0.63	0.85	0.82	0.13	0.86	0.77	0.9	60.76	29.36	55.57	42.88	72.13	70.46	33.13	64.54	50.46	83.8	4317	0.03
0.03	0.41	0.26	0.44	0.19	0.61	0.95	0.03	0.95	0.93	0.97	0.66	0.28	0.78	0.45	0.87	1926.53	6333.86	377.89	113.21	1489.39	18.58	17.95	12.86	5.0	25.75	0.51	0.24	0.6	0.31	0.7	0.41	0.22	0.44	0.2	0.59	0.63	0.19	0.7	0.47	0.78	0.76	0.13	0.8	0.66	0.86	61.52	29.2	56.27	43.29	73.04	82.99	38.01	76.07	58.9	98.16	4846	0.06
0.06	0.34	0.21	0.35	0.18	0.49	0.91	0.04	0.91	0.88	0.93	0.63	0.24	0.71	0.47	0.82	2228.76	7031.61	487.38	154.92	1778.44	19.08	17.0	14.28	6.01	27.49	0.48	0.2	0.53	0.33	0.63	0.35	0.19	0.36	0.2	0.48	0.61	0.15	0.64	0.5	0.72	0.75	0.11	0.77	0.67	0.83	61.46	31.87	55.43	42.91	72.74	104.17	52.03	94.95	74.32	122.61	4569	0.12
0.11	0.32	0.18	0.32	0.19	0.44	0.86	0.05	0.86	0.83	0.89	0.63	0.19	0.68	0.54	0.78	1359.09	3149.03	385.84	160.84	1168.81	18.4	15.29	14.64	6.5	26.46	0.47	0.16	0.5	0.38	0.59	0.33	0.16	0.32	0.2	0.44	0.6	0.13	0.62	0.53	0.69	0.74	0.09	0.76	0.69	0.81	61.16	28.05	56.14	42.94	72.78	136.01	56.65	125.42	98.03	160.94	3431	0.21
0.15	0.26	0.16	0.25	0.15	0.36	0.79	0.05	0.79	0.76	0.83	0.56	0.19	0.6	0.46	0.7	1018.7	2696.42	388.34	175.93	1030.06	18.92	15.69	15.31	6.78	27.38	0.41	0.15	0.43	0.33	0.51	0.27	0.15	0.26	0.16	0.36	0.55	0.12	0.57	0.49	0.63	0.71	0.08	0.72	0.66	0.77	58.78	30.6	53.38	41.21	69.12	192.67	81.41	178.7	141.48	229.54	2696	0.39
0.18	0.22	0.14	0.21	0.12	0.31	0.74	0.06	0.74	0.7	0.77	0.51	0.18	0.53	0.41	0.64	961.18	1466.34	431.91	192.09	1099.28	19.43	15.8	15.83	6.76	28.32	0.37	0.14	0.38	0.28	0.47	0.24	0.14	0.24	0.14	0.32	0.53	0.11	0.53	0.46	0.6	0.69	0.08	0.7	0.64	0.74	59.72	30.61	53.93	42.61	70.51	265.4	111.14	243.29	195.46	312.05	2335	0.58
0.32	0.19	0.14	0.18	0.09	0.28	0.69	0.07	0.69	0.64	0.73	0.46	0.19	0.47	0.34	0.6	1100.18	1534.47	509.17	239.33	1335.38	20.07	16.24	16.41	7.11	28.62	0.33	0.14	0.33	0.23	0.43	0.22	0.13	0.21	0.12	0.32	0.5	0.11	0.5	0.43	0.58	0.67	0.08	0.67	0.62	0.73	64.81	35.68	58.61	45.45	74.77	367.7	168.3	336.2	262.15	431.34	2462	0.79


==> data_new/tef/imdb/xlnet/S_auc.tex <==
0.09

==> data_new/tef/imdb/xlnet/S_ppl.tex <==
5.9

==> data_new/tef/mr/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	293.48	483.78	166.34	86.91	307.77	293.48	483.78	166.34	86.91	307.77	2834	0.0
0.03	0.89	0.1	0.89	0.83	0.97	0.95	0.04	0.96	0.94	0.97	0.81	0.14	0.85	0.75	0.91	1.21	0.76	1.18	0.68	1.6	1.95	2.23	1.17	0.37	2.9	0.68	0.15	0.71	0.59	0.79	0.79	0.13	0.78	0.69	0.9	0.78	0.1	0.8	0.72	0.85	0.83	0.09	0.85	0.78	0.89	179.83	170.38	129.91	74.55	218.0	245.15	205.09	188.16	107.88	310.47	1270	0.06
0.06	0.86	0.12	0.88	0.79	0.97	0.91	0.06	0.92	0.88	0.95	0.73	0.18	0.78	0.63	0.87	1.25	0.8	1.18	0.69	1.67	1.92	2.16	1.21	0.39	2.69	0.59	0.18	0.62	0.47	0.72	0.76	0.15	0.76	0.67	0.89	0.73	0.12	0.74	0.65	0.81	0.78	0.1	0.8	0.71	0.86	214.89	255.76	142.75	81.13	248.15	365.54	420.41	242.39	142.07	443.53	1907	0.12
0.11	0.8	0.15	0.81	0.72	0.92	0.84	0.08	0.85	0.8	0.9	0.63	0.2	0.67	0.49	0.78	1.59	0.9	1.53	1.05	2.04	2.43	2.55	1.62	0.57	3.29	0.48	0.18	0.5	0.35	0.62	0.68	0.18	0.68	0.58	0.81	0.67	0.13	0.67	0.58	0.75	0.73	0.1	0.74	0.65	0.8	237.61	364.33	145.75	85.23	253.25	546.39	734.8	362.78	203.69	617.7	2373	0.23
0.15	0.8	0.14	0.8	0.71	0.91	0.76	0.1	0.77	0.7	0.83	0.59	0.21	0.61	0.44	0.76	1.39	0.64	1.41	1.02	1.78	1.99	1.8	1.59	0.54	2.85	0.45	0.19	0.45	0.31	0.58	0.66	0.2	0.67	0.56	0.8	0.66	0.13	0.65	0.56	0.75	0.7	0.11	0.71	0.62	0.79	252.24	365.34	149.64	75.69	278.44	898.71	3027.4	451.5	255.66	849.19	1245	0.44
0.18	0.74	0.16	0.76	0.65	0.85	0.72	0.1	0.73	0.67	0.79	0.53	0.21	0.54	0.36	0.7	1.78	0.79	1.7	1.3	2.18	2.73	2.48	1.99	0.89	3.88	0.39	0.18	0.39	0.24	0.53	0.64	0.18	0.65	0.52	0.75	0.61	0.12	0.6	0.52	0.7	0.68	0.1	0.68	0.6	0.76	224.82	287.16	141.19	78.29	260.21	908.77	1747.67	565.01	320.74	1016.53	1790	0.53
0.32	0.67	0.18	0.69	0.56	0.8	0.61	0.13	0.62	0.53	0.7	0.44	0.22	0.44	0.28	0.61	1.97	0.81	1.89	1.49	2.36	3.07	2.65	2.37	1.07	4.4	0.32	0.17	0.31	0.19	0.45	0.58	0.19	0.59	0.45	0.69	0.57	0.13	0.56	0.48	0.65	0.64	0.1	0.63	0.57	0.71	239.26	359.87	148.1	84.41	266.31	1589.23	2274.3	1008.19	571.93	1804.5	4322	0.98


==> data_new/tef/mr/bert/A_auc.tex <==
0.25

==> data_new/tef/mr/bert/A_ppl.tex <==
5.8

==> data_new/tef/mr/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	293.45	483.79	166.32	86.87	307.68	293.45	483.79	166.32	86.87	307.68	2834	0.0
0.03	0.35	0.44	0.47	0.07	0.69	0.95	0.03	0.96	0.94	0.97	0.44	0.41	0.58	0.27	0.73	6.93	7.83	4.99	0.78	10.31	4.58	4.03	3.44	1.54	6.49	0.37	0.33	0.46	0.2	0.6	0.38	0.3	0.33	0.0	0.67	0.57	0.23	0.62	0.44	0.75	0.69	0.18	0.75	0.62	0.81	178.97	169.26	129.66	73.47	218.04	235.95	217.19	173.14	102.92	285.41	1297	0.06
0.06	0.13	0.48	0.22	-0.2	0.51	0.91	0.06	0.92	0.89	0.95	0.25	0.45	0.37	-0.05	0.59	7.66	8.51	5.37	0.75	11.62	4.78	4.25	3.49	1.54	7.04	0.21	0.35	0.29	-0.03	0.47	0.25	0.32	0.0	0.0	0.5	0.46	0.25	0.5	0.29	0.67	0.61	0.19	0.67	0.5	0.75	214.74	251.47	143.41	82.75	250.39	365.5	476.12	230.62	139.01	430.56	2021	0.12
0.11	-0.07	0.45	-0.04	-0.44	0.27	0.85	0.08	0.86	0.8	0.9	0.07	0.44	0.15	-0.28	0.41	8.35	9.28	5.74	1.0	12.54	5.46	4.78	3.91	1.92	7.88	0.06	0.34	0.12	-0.2	0.33	0.18	0.27	0.0	0.0	0.33	0.37	0.23	0.33	0.2	0.56	0.55	0.19	0.58	0.42	0.69	238.74	362.28	143.84	82.27	253.47	531.71	642.96	333.49	193.97	610.13	2581	0.21
0.15	-0.17	0.47	-0.17	-0.57	0.2	0.78	0.1	0.8	0.73	0.86	-0.04	0.43	0.03	-0.39	0.29	9.08	10.88	6.09	0.94	13.71	4.91	4.14	3.92	1.64	7.28	-0.02	0.34	0.03	-0.29	0.23	0.13	0.27	0.0	0.0	0.0	0.32	0.24	0.33	0.11	0.5	0.51	0.19	0.54	0.36	0.67	254.33	366.45	142.98	76.19	278.29	927.32	3258.73	457.02	251.67	827.05	1265	0.46
0.18	-0.2	0.39	-0.2	-0.5	0.07	0.73	0.11	0.74	0.66	0.81	-0.05	0.36	-0.02	-0.32	0.22	10.18	10.17	8.03	1.9	14.99	5.69	4.74	4.46	2.14	8.0	-0.03	0.28	-0.01	-0.22	0.18	0.12	0.23	0.0	0.0	0.0	0.32	0.2	0.33	0.17	0.44	0.5	0.16	0.5	0.4	0.62	210.27	252.86	138.16	75.41	243.49	782.55	881.9	525.26	324.79	930.38	1701	0.47
0.32	-0.3	0.35	-0.32	-0.55	-0.07	0.62	0.13	0.63	0.53	0.71	-0.15	0.32	-0.14	-0.39	0.08	11.2	10.34	9.53	2.43	16.39	5.47	4.65	4.14	1.97	7.69	-0.11	0.24	-0.1	-0.28	0.07	0.08	0.2	0.0	0.0	0.0	0.26	0.18	0.25	0.12	0.38	0.47	0.14	0.5	0.38	0.56	245.11	374.25	151.76	87.11	269.83	1512.1	3692.13	931.19	536.32	1664.75	4046	0.9


==> data_new/tef/mr/bert/IG_auc.tex <==
-0.01

==> data_new/tef/mr/bert/IG_ppl.tex <==
5.8

==> data_new/tef/mr/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	293.47	484.01	166.15	86.87	307.42	293.47	484.01	166.15	86.87	307.42	2834	0.0
0.03	0.58	0.26	0.63	0.43	0.78	0.95	0.03	0.96	0.94	0.98	0.71	0.23	0.77	0.63	0.87	51.18	83.84	12.93	1.68	69.06	1.47	1.28	1.15	0.54	2.01	0.57	0.2	0.61	0.47	0.72	0.39	0.29	0.5	0.0	0.67	0.67	0.18	0.67	0.56	0.78	0.79	0.12	0.81	0.73	0.88	177.88	169.59	128.02	73.09	215.87	233.46	202.54	173.22	101.05	294.26	1291	0.05
0.06	0.49	0.26	0.52	0.31	0.68	0.91	0.06	0.92	0.89	0.95	0.64	0.24	0.7	0.53	0.82	57.22	94.32	15.7	2.09	79.63	1.41	1.25	1.08	0.5	1.97	0.5	0.2	0.53	0.39	0.65	0.27	0.32	0.0	0.0	0.5	0.6	0.19	0.62	0.5	0.75	0.75	0.13	0.77	0.69	0.86	210.98	253.04	137.39	77.98	243.78	340.9	349.65	234.05	134.07	415.84	1966	0.11
0.11	0.34	0.27	0.35	0.15	0.55	0.85	0.08	0.86	0.81	0.9	0.51	0.27	0.57	0.36	0.72	68.2	100.2	20.38	3.13	100.67	1.82	1.56	1.39	0.6	2.67	0.39	0.21	0.42	0.25	0.55	0.2	0.28	0.0	0.0	0.33	0.51	0.19	0.56	0.4	0.67	0.7	0.13	0.69	0.62	0.8	238.8	361.9	146.46	82.73	259.9	549.58	816.04	359.32	198.69	591.59	2550	0.23
0.15	0.26	0.27	0.23	0.07	0.44	0.78	0.1	0.79	0.73	0.84	0.46	0.29	0.49	0.28	0.68	76.47	117.9	21.79	2.56	113.66	1.67	1.36	1.33	0.59	2.37	0.35	0.23	0.36	0.2	0.51	0.12	0.25	0.0	0.0	0.0	0.47	0.22	0.5	0.33	0.62	0.68	0.14	0.67	0.58	0.78	243.73	349.45	141.6	70.53	279.04	736.33	976.27	453.25	257.32	843.25	1311	0.35
0.18	0.21	0.24	0.2	0.04	0.38	0.72	0.11	0.74	0.66	0.8	0.4	0.26	0.43	0.24	0.59	92.88	126.33	43.8	5.07	139.4	2.05	1.62	1.62	0.72	3.07	0.29	0.2	0.31	0.16	0.43	0.12	0.22	0.0	0.0	0.33	0.43	0.19	0.44	0.33	0.56	0.65	0.13	0.64	0.56	0.75	216.7	261.09	139.88	82.78	243.0	827.12	962.99	565.56	326.45	982.08	1774	0.49
0.32	0.09	0.23	0.08	-0.07	0.25	0.61	0.14	0.61	0.52	0.71	0.25	0.3	0.26	0.04	0.48	112.7	142.31	69.94	7.58	165.9	2.28	1.7	1.9	0.91	3.34	0.18	0.22	0.19	0.03	0.34	0.07	0.18	0.0	0.0	0.0	0.35	0.19	0.33	0.22	0.5	0.59	0.14	0.6	0.5	0.69	246.14	358.3	153.91	88.57	270.63	1543.31	1958.04	995.88	561.88	1775.65	4015	0.91


==> data_new/tef/mr/bert/S_auc.tex <==
0.10

==> data_new/tef/mr/bert/S_ppl.tex <==
5.8

==> data_new/tef/mr/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.95	0.21	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	649.18	1497.52	263.12	139.2	534.81	649.18	1497.52	263.12	139.2	534.81	2760	0.0
0.03	0.38	0.36	0.4	0.0	0.72	0.96	0.03	0.97	0.94	0.98	0.61	0.4	0.76	0.36	0.95	0.89	1.03	0.47	0.03	1.53	1.99	1.87	1.44	0.58	2.89	0.67	0.2	0.72	0.56	0.81	0.51	0.38	0.5	0.0	1.0	0.69	0.29	0.78	0.44	0.89	0.79	0.2	0.86	0.64	0.94	216.81	173.75	161.52	101.86	268.11	248.66	196.7	190.04	122.86	321.57	1468	0.06
0.06	0.4	0.33	0.45	0.0	0.68	0.92	0.05	0.93	0.9	0.96	0.56	0.33	0.63	0.37	0.8	1.41	1.17	1.36	0.18	2.13	1.93	1.82	1.38	0.56	2.75	0.56	0.21	0.6	0.44	0.71	0.37	0.38	0.33	0.0	0.67	0.64	0.25	0.67	0.5	0.8	0.76	0.18	0.8	0.67	0.88	310.01	337.29	213.36	122.89	380.22	386.7	409.91	274.31	157.05	469.93	1885	0.11
0.11	0.3	0.33	0.31	0.01	0.55	0.85	0.07	0.87	0.82	0.9	0.44	0.28	0.46	0.27	0.62	1.92	1.29	1.81	0.91	2.77	2.24	2.01	1.7	0.72	3.14	0.41	0.22	0.43	0.27	0.55	0.3	0.34	0.33	0.0	0.5	0.57	0.21	0.57	0.44	0.67	0.71	0.15	0.75	0.62	0.81	423.51	966.26	210.67	122.79	394.55	614.65	1158.08	337.79	198.99	571.34	1776	0.2
0.15	0.18	0.34	0.16	-0.04	0.43	0.78	0.1	0.79	0.74	0.84	0.3	0.29	0.32	0.13	0.5	2.13	1.42	2.0	1.01	3.17	2.28	2.05	1.73	0.7	3.28	0.27	0.23	0.29	0.13	0.42	0.22	0.33	0.0	0.0	0.5	0.49	0.23	0.5	0.33	0.67	0.67	0.14	0.67	0.58	0.73	540.71	1257.88	242.38	130.79	502.61	1240.74	5525.68	432.77	254.45	819.42	908	0.56
0.18	0.09	0.34	0.07	-0.13	0.33	0.73	0.09	0.74	0.67	0.8	0.22	0.27	0.21	0.07	0.39	2.47	1.49	2.37	1.38	3.56	2.64	2.25	2.07	0.92	3.74	0.2	0.21	0.2	0.08	0.33	0.19	0.29	0.0	0.0	0.33	0.46	0.19	0.44	0.33	0.57	0.63	0.13	0.62	0.56	0.71	380.97	729.21	205.79	118.98	395.86	852.9	1630.71	457.46	284.39	822.41	1317	0.54
0.32	-0.09	0.32	-0.1	-0.31	0.12	0.61	0.11	0.61	0.54	0.69	0.01	0.26	0.02	-0.15	0.18	2.84	1.74	2.99	1.36	4.15	2.84	2.33	2.21	1.06	4.12	0.02	0.21	0.03	-0.11	0.16	0.13	0.24	0.0	0.0	0.33	0.35	0.18	0.33	0.22	0.5	0.54	0.13	0.56	0.46	0.62	410.92	951.57	213.36	125.49	389.9	1200.79	2372.05	694.6	430.4	1173.69	3586	0.83


==> data_new/tef/mr/cnn/IG_auc.tex <==
0.07

==> data_new/tef/mr/cnn/IG_ppl.tex <==
2.3

==> data_new/tef/mr/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.69	0.46	1.0	0.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	649.48	1497.72	263.16	139.31	535.83	649.48	1497.72	263.16	139.31	535.83	2760	0.0
0.03	0.15	0.32	0.0	0.0	0.0	0.96	0.03	0.97	0.95	0.98	0.71	0.47	1.0	0.55	1.0	15.73	23.01	0.0	0.0	27.48	0.71	0.51	0.61	0.29	1.03	0.7	0.16	0.71	0.61	0.81	0.69	0.43	1.0	0.33	1.0	0.79	0.3	1.0	0.62	1.0	0.85	0.21	1.0	0.73	1.0	223.76	181.56	176.0	105.93	272.33	256.1	193.72	210.52	126.79	322.56	2915	0.06
0.06	0.23	0.36	0.0	0.0	0.59	0.93	0.05	0.94	0.9	0.96	0.64	0.48	0.85	0.46	1.0	20.44	22.47	15.3	0.0	34.73	0.66	0.57	0.5	0.21	0.93	0.6	0.19	0.62	0.48	0.74	0.58	0.46	1.0	0.0	1.0	0.7	0.33	0.8	0.5	1.0	0.79	0.25	0.86	0.64	1.0	322.57	330.59	227.71	125.78	405.15	410.44	431.5	291.62	169.48	518.65	2795	0.12
0.11	0.4	0.35	0.45	0.0	0.72	0.86	0.07	0.87	0.82	0.91	0.52	0.44	0.61	0.32	0.86	27.34	18.99	24.96	14.42	39.42	0.84	0.71	0.63	0.29	1.23	0.46	0.23	0.46	0.32	0.63	0.41	0.42	0.33	0.0	1.0	0.6	0.29	0.67	0.43	0.8	0.73	0.19	0.75	0.6	0.88	573.4	1288.07	254.17	137.6	515.26	809.58	1766.28	405.93	216.78	771.25	1485	0.18
0.15	0.39	0.35	0.39	0.0	0.71	0.78	0.09	0.8	0.73	0.85	0.42	0.4	0.47	0.19	0.74	31.78	17.33	29.34	21.14	41.94	0.77	0.66	0.61	0.23	1.11	0.36	0.26	0.37	0.18	0.55	0.32	0.41	0.0	0.0	0.5	0.5	0.29	0.5	0.33	0.67	0.65	0.19	0.67	0.54	0.75	711.21	1631.63	249.15	137.02	602.31	1171.2	2377.6	509.21	269.45	1075.37	690	0.28
0.18	0.36	0.32	0.39	0.14	0.59	0.73	0.1	0.73	0.67	0.8	0.34	0.33	0.37	0.13	0.57	35.86	14.44	33.23	25.09	44.8	1.02	0.79	0.82	0.42	1.46	0.27	0.24	0.27	0.11	0.43	0.26	0.36	0.0	0.0	0.5	0.45	0.24	0.44	0.33	0.62	0.61	0.15	0.6	0.5	0.7	365.47	555.16	196.96	110.1	377.0	857.73	1701.76	466.32	287.42	775.78	886	0.59
0.32	0.15	0.36	0.16	-0.1	0.41	0.61	0.11	0.61	0.53	0.69	0.13	0.35	0.14	-0.12	0.38	41.78	14.3	40.55	30.91	51.26	1.32	0.94	1.15	0.56	1.9	0.1	0.25	0.1	-0.07	0.27	0.16	0.3	0.0	0.0	0.33	0.33	0.22	0.33	0.14	0.5	0.52	0.16	0.5	0.4	0.62	428.94	1083.29	207.95	120.96	386.17	1177.01	2271.57	709.53	443.89	1226.67	2184	0.76


==> data_new/tef/mr/cnn/S_auc.tex <==
0.10

==> data_new/tef/mr/cnn/S_ppl.tex <==
2.3

==> data_new/tef/mr/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.78	0.42	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	614.12	1405.37	266.95	141.02	535.82	614.12	1405.37	266.95	141.02	535.82	2853	0.0
0.03	0.19	0.39	0.0	0.0	0.51	0.96	0.03	0.97	0.94	0.98	0.55	0.48	0.72	0.13	1.0	1.37	4.33	0.03	0.0	1.31	4.24	4.4	2.87	1.23	5.68	0.43	0.34	0.5	0.25	0.7	0.55	0.41	0.5	0.0	1.0	0.69	0.29	0.75	0.44	1.0	0.77	0.21	0.81	0.6	1.0	219.25	195.22	164.59	107.11	263.93	253.37	206.54	197.17	127.26	318.69	1508	0.08
0.06	0.09	0.4	0.0	0.0	0.24	0.92	0.05	0.94	0.9	0.96	0.49	0.51	0.59	0.12	1.0	1.5	4.46	0.03	0.0	1.52	4.48	4.56	3.0	1.32	5.99	0.3	0.4	0.39	0.06	0.59	0.51	0.45	0.5	0.0	1.0	0.65	0.34	0.71	0.38	1.0	0.74	0.25	0.75	0.56	1.0	330.83	374.0	232.54	126.25	409.4	419.94	472.82	295.51	168.45	512.31	2518	0.14
0.11	-0.04	0.48	0.0	-0.38	0.25	0.86	0.07	0.87	0.82	0.91	0.24	0.52	0.31	-0.13	0.61	2.64	6.3	0.36	0.03	2.88	4.96	4.88	3.49	1.4	6.89	0.14	0.41	0.2	-0.15	0.43	0.33	0.39	0.33	0.0	0.67	0.51	0.31	0.5	0.22	0.67	0.63	0.24	0.62	0.47	0.8	476.81	1018.71	230.2	130.58	445.08	669.36	1316.31	354.24	210.12	673.86	1999	0.21
0.15	-0.13	0.48	-0.12	-0.48	0.17	0.79	0.09	0.8	0.74	0.85	0.09	0.51	0.15	-0.32	0.46	2.81	5.75	0.55	0.04	3.22	4.7	4.61	3.18	1.54	6.43	0.05	0.4	0.1	-0.3	0.36	0.2	0.34	0.0	0.0	0.5	0.41	0.31	0.43	0.12	0.67	0.56	0.24	0.57	0.36	0.71	529.5	1276.76	235.34	114.17	449.57	844.89	1805.78	429.72	259.34	769.37	1028	0.31
0.18	-0.18	0.48	-0.23	-0.57	0.15	0.74	0.1	0.76	0.69	0.82	0.01	0.4	0.07	-0.27	0.31	3.05	5.73	1.86	0.06	3.56	5.53	4.97	4.2	1.73	7.81	0.04	0.33	0.08	-0.2	0.27	0.21	0.31	0.0	0.0	0.37	0.39	0.25	0.4	0.22	0.57	0.54	0.19	0.56	0.4	0.69	355.83	698.98	195.11	111.53	376.53	785.07	1318.67	453.56	281.7	751.61	1348	0.62
0.32	-0.23	0.42	-0.28	-0.55	0.07	0.64	0.11	0.64	0.57	0.72	-0.04	0.35	-0.02	-0.26	0.19	4.13	7.0	2.56	0.12	4.4	4.97	4.61	3.64	1.63	6.95	-0.01	0.28	0.01	-0.19	0.18	0.17	0.28	0.0	0.0	0.33	0.37	0.21	0.38	0.22	0.5	0.52	0.16	0.53	0.43	0.64	381.6	920.77	207.08	121.62	380.22	1118.22	2585.96	659.68	410.71	1151.69	2977	1.0


==> data_new/tef/mr/lstm/IG_auc.tex <==
-0.01

==> data_new/tef/mr/lstm/IG_ppl.tex <==
1.9

==> data_new/tef/mr/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.78	0.42	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	614.05	1405.25	266.95	141.02	535.82	614.05	1405.25	266.95	141.02	535.82	2853	0.0
0.03	0.28	0.35	0.0	0.0	0.64	0.96	0.03	0.97	0.94	0.98	0.62	0.41	0.79	0.42	0.97	13.3	23.72	2.28	0.83	18.07	1.99	1.59	1.61	0.72	2.85	0.65	0.16	0.68	0.55	0.76	0.44	0.41	0.5	0.0	1.0	0.62	0.33	0.71	0.29	1.0	0.72	0.26	0.8	0.5	1.0	216.75	189.92	164.21	105.24	263.7	255.49	225.71	199.98	126.59	320.65	1840	0.09
0.06	0.24	0.32	0.0	0.0	0.55	0.92	0.05	0.94	0.9	0.96	0.56	0.46	0.73	0.23	1.0	19.93	52.77	2.13	0.0	21.35	2.05	1.79	1.63	0.71	2.8	0.6	0.17	0.62	0.49	0.71	0.46	0.45	0.5	0.0	1.0	0.63	0.32	0.67	0.38	1.0	0.74	0.25	0.8	0.56	1.0	333.11	422.66	228.06	126.34	409.28	425.99	629.74	292.22	171.03	507.52	2922	0.14
0.11	0.33	0.29	0.34	0.0	0.54	0.86	0.07	0.87	0.82	0.91	0.58	0.38	0.67	0.46	0.82	37.07	75.7	11.12	1.84	51.11	2.5	2.12	1.91	0.79	3.68	0.5	0.18	0.51	0.38	0.63	0.38	0.4	0.33	0.0	0.67	0.62	0.24	0.67	0.44	0.78	0.76	0.18	0.78	0.67	0.88	527.94	1231.82	235.52	131.55	467.24	798.79	2237.83	377.03	224.62	691.21	1879	0.27
0.15	0.31	0.27	0.31	0.03	0.51	0.78	0.09	0.8	0.73	0.85	0.53	0.33	0.59	0.41	0.75	70.65	224.01	34.76	3.11	70.57	2.72	2.27	2.2	0.83	4.08	0.43	0.2	0.44	0.32	0.57	0.24	0.36	0.0	0.0	0.5	0.52	0.24	0.5	0.38	0.67	0.72	0.18	0.73	0.64	0.83	598.7	1405.77	247.99	126.27	528.26	1160.62	5152.59	442.51	247.34	869.04	814	0.49
0.18	0.27	0.24	0.26	0.09	0.41	0.73	0.1	0.74	0.67	0.8	0.48	0.25	0.51	0.33	0.66	61.59	92.45	43.14	4.37	74.48	3.19	2.45	2.68	1.15	4.77	0.37	0.19	0.38	0.24	0.5	0.13	0.26	0.0	0.0	0.33	0.46	0.2	0.5	0.33	0.62	0.68	0.15	0.69	0.6	0.79	358.54	507.44	200.23	112.44	391.55	783.02	1242.56	458.23	289.58	813.57	1180	0.61
0.32	0.14	0.22	0.12	-0.01	0.27	0.63	0.11	0.63	0.55	0.7	0.34	0.25	0.36	0.18	0.53	71.39	102.7	55.86	12.56	84.14	3.54	2.61	3.06	1.34	5.19	0.25	0.19	0.25	0.13	0.38	0.07	0.18	0.0	0.0	0.0	0.36	0.18	0.33	0.25	0.5	0.63	0.13	0.64	0.56	0.73	359.46	777.45	209.65	120.36	378.79	1003.49	1490.33	663.53	414.25	1100.36	2738	0.93


==> data_new/tef/mr/lstm/S_auc.tex <==
0.09

==> data_new/tef/mr/lstm/S_ppl.tex <==
1.9

==> data_new/tef/mr/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	628.89	1516.76	261.89	138.75	528.98	628.89	1516.76	261.89	138.75	528.98	2990	0.0
0.03	0.74	0.17	0.77	0.65	0.87	0.95	0.03	0.96	0.94	0.97	0.84	0.14	0.86	0.78	0.94	0.12	0.06	0.1	0.07	0.14	1.64	1.36	1.3	0.67	2.13	0.73	0.15	0.75	0.66	0.83	0.49	0.29	0.5	0.33	0.67	0.76	0.15	0.78	0.67	0.88	0.86	0.1	0.88	0.81	0.93	222.08	189.38	164.38	100.56	271.06	265.57	219.56	206.83	128.94	327.92	1031	0.08
0.06	0.65	0.22	0.69	0.52	0.83	0.91	0.05	0.93	0.89	0.95	0.76	0.19	0.8	0.67	0.91	0.15	0.07	0.13	0.09	0.18	1.71	1.63	1.2	0.54	2.31	0.66	0.19	0.68	0.55	0.79	0.39	0.38	0.33	0.0	0.67	0.69	0.18	0.71	0.57	0.8	0.82	0.12	0.83	0.75	0.9	299.47	321.98	202.21	118.99	368.65	400.11	420.47	277.37	164.77	469.46	1779	0.14
0.11	0.48	0.29	0.51	0.28	0.7	0.85	0.07	0.86	0.81	0.91	0.61	0.26	0.66	0.45	0.82	0.18	0.08	0.16	0.12	0.22	2.36	2.26	1.64	0.66	3.32	0.51	0.24	0.52	0.35	0.69	0.3	0.36	0.0	0.0	0.5	0.57	0.2	0.56	0.44	0.67	0.75	0.14	0.75	0.67	0.83	408.57	921.86	207.19	118.87	390.93	591.82	889.02	351.19	212.33	621.14	1983	0.19
0.15	0.46	0.28	0.47	0.27	0.66	0.78	0.09	0.8	0.73	0.85	0.59	0.25	0.63	0.44	0.77	0.2	0.09	0.17	0.13	0.24	1.97	1.67	1.56	0.6	2.92	0.49	0.22	0.49	0.35	0.64	0.25	0.37	0.0	0.0	0.5	0.52	0.23	0.5	0.38	0.67	0.73	0.15	0.73	0.64	0.83	492.7	1082.59	235.73	125.7	462.74	968.31	2688.79	461.87	247.91	799.29	1079	0.41
0.18	0.32	0.31	0.32	0.09	0.56	0.73	0.1	0.74	0.68	0.81	0.43	0.31	0.46	0.22	0.68	0.2	0.08	0.19	0.14	0.25	2.79	2.4	2.17	0.92	3.96	0.35	0.25	0.35	0.16	0.54	0.2	0.32	0.0	0.0	0.33	0.46	0.22	0.44	0.33	0.62	0.65	0.15	0.64	0.56	0.77	392.95	1047.71	199.93	109.65	378.25	768.1	1057.36	449.61	287.88	820.11	1571	0.41
0.32	0.14	0.33	0.12	-0.11	0.38	0.62	0.11	0.62	0.54	0.7	0.25	0.37	0.26	-0.01	0.53	0.23	0.08	0.21	0.17	0.28	3.35	2.6	2.89	1.25	4.76	0.2	0.28	0.2	0.0	0.4	0.12	0.27	0.0	0.0	0.0	0.36	0.22	0.33	0.2	0.5	0.58	0.17	0.57	0.45	0.69	382.64	835.18	209.2	122.47	387.35	1148.86	2024.73	699.98	428.98	1212.37	4463	0.85


==> data_new/tef/mr/lstmatt/A_auc.tex <==
0.14

==> data_new/tef/mr/lstmatt/A_ppl.tex <==
2.3

==> data_new/tef/mr/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	628.89	1516.76	261.89	138.75	528.98	628.89	1516.76	261.89	138.75	528.98	2990	0.0
0.03	0.59	0.29	0.65	0.41	0.82	0.95	0.03	0.96	0.94	0.98	0.75	0.19	0.77	0.66	0.89	2.6	3.53	1.31	0.73	2.94	3.67	3.89	2.48	0.81	5.2	0.65	0.19	0.69	0.55	0.79	0.52	0.29	0.5	0.33	0.67	0.75	0.17	0.78	0.67	0.88	0.83	0.11	0.85	0.77	0.92	222.08	189.38	164.38	100.56	271.06	263.69	225.78	195.61	119.51	313.82	1031	0.08
0.06	0.47	0.34	0.51	0.22	0.74	0.92	0.05	0.93	0.9	0.95	0.64	0.23	0.65	0.51	0.8	2.56	3.04	1.55	0.98	2.93	3.8	3.71	2.66	1.09	5.34	0.56	0.21	0.58	0.44	0.71	0.36	0.36	0.33	0.0	0.5	0.68	0.19	0.67	0.57	0.8	0.79	0.12	0.8	0.71	0.88	301.92	325.76	202.79	119.03	371.86	390.23	386.3	273.17	161.1	465.27	1783	0.12
0.11	0.28	0.36	0.28	0.02	0.57	0.86	0.07	0.87	0.82	0.91	0.48	0.24	0.48	0.33	0.64	3.27	4.32	1.87	1.23	3.41	4.31	4.13	3.05	1.29	6.0	0.43	0.21	0.43	0.3	0.56	0.28	0.32	0.33	0.0	0.5	0.59	0.19	0.6	0.5	0.67	0.74	0.12	0.75	0.67	0.81	403.49	910.83	205.16	119.07	387.14	572.99	940.22	330.99	191.88	580.21	1995	0.18
0.15	0.16	0.38	0.15	-0.13	0.46	0.78	0.1	0.8	0.73	0.85	0.35	0.29	0.36	0.15	0.55	3.06	3.08	2.25	1.47	3.52	4.39	4.05	3.25	1.43	6.2	0.31	0.25	0.32	0.15	0.47	0.2	0.32	0.0	0.0	0.5	0.5	0.23	0.5	0.33	0.67	0.68	0.14	0.67	0.6	0.78	507.2	1109.07	240.11	124.57	470.0	848.79	1982.11	435.82	253.22	834.08	1066	0.29
0.18	0.06	0.35	0.04	-0.2	0.32	0.73	0.09	0.75	0.68	0.81	0.25	0.25	0.25	0.08	0.42	3.54	3.94	2.28	1.52	3.95	4.81	4.37	3.58	1.58	6.76	0.23	0.21	0.22	0.1	0.36	0.21	0.31	0.0	0.0	0.33	0.47	0.19	0.5	0.33	0.67	0.64	0.13	0.64	0.57	0.73	395.98	1058.43	200.5	112.01	378.52	716.99	948.07	463.83	270.56	775.96	1546	0.35
0.32	-0.1	0.34	-0.13	-0.35	0.12	0.62	0.12	0.63	0.54	0.7	0.07	0.28	0.07	-0.11	0.26	3.84	4.25	2.53	1.74	4.16	5.15	4.58	3.88	1.85	7.03	0.08	0.22	0.07	-0.06	0.22	0.14	0.25	0.0	0.0	0.33	0.37	0.19	0.33	0.25	0.5	0.57	0.13	0.57	0.5	0.67	384.31	868.38	209.21	121.91	388.67	1091.58	1923.0	676.59	414.96	1161.52	4476	0.78


==> data_new/tef/mr/lstmatt/IG_auc.tex <==
0.07

==> data_new/tef/mr/lstmatt/IG_ppl.tex <==
2.3

==> data_new/tef/mr/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	629.15	1517.39	262.02	138.73	528.98	629.15	1517.39	262.02	138.73	528.98	2990	0.0
0.03	0.74	0.18	0.77	0.65	0.86	0.95	0.03	0.96	0.94	0.97	0.81	0.16	0.86	0.75	0.92	35.55	31.25	26.11	17.37	42.34	1.73	1.49	1.29	0.62	2.51	0.68	0.16	0.72	0.6	0.8	0.49	0.29	0.5	0.33	0.67	0.75	0.16	0.78	0.67	0.88	0.83	0.11	0.86	0.77	0.92	222.08	189.38	164.38	100.56	271.06	270.16	218.56	203.69	129.72	343.29	1031	0.09
0.06	0.64	0.21	0.69	0.52	0.8	0.91	0.05	0.92	0.89	0.95	0.74	0.19	0.8	0.66	0.88	43.27	38.32	31.95	20.63	50.66	1.79	1.6	1.34	0.59	2.47	0.61	0.18	0.65	0.51	0.75	0.36	0.36	0.33	0.0	0.5	0.68	0.18	0.71	0.57	0.8	0.8	0.12	0.81	0.73	0.88	299.57	322.24	202.21	119.03	368.88	407.28	428.17	291.19	169.9	479.25	1779	0.15
0.11	0.52	0.23	0.54	0.36	0.68	0.85	0.07	0.86	0.82	0.9	0.63	0.23	0.67	0.5	0.8	53.77	45.96	39.55	27.01	63.55	2.36	2.0	1.85	0.79	3.46	0.5	0.2	0.51	0.37	0.64	0.27	0.32	0.33	0.0	0.5	0.58	0.19	0.6	0.44	0.67	0.74	0.13	0.75	0.67	0.82	404.92	911.76	207.64	119.33	391.05	670.57	1675.81	361.57	213.59	615.68	1984	0.28
0.15	0.44	0.25	0.47	0.27	0.61	0.79	0.09	0.8	0.75	0.85	0.57	0.25	0.62	0.43	0.75	59.13	50.89	42.87	29.38	68.5	2.16	1.76	1.74	0.77	3.0	0.44	0.2	0.47	0.32	0.59	0.19	0.32	0.0	0.0	0.5	0.52	0.22	0.5	0.38	0.67	0.71	0.14	0.71	0.64	0.82	491.88	1089.42	242.05	126.33	468.27	895.72	1978.84	453.49	260.96	833.93	1044	0.35
0.18	0.34	0.24	0.34	0.17	0.51	0.73	0.1	0.75	0.67	0.81	0.46	0.26	0.49	0.3	0.66	65.58	52.1	50.62	34.53	83.09	3.02	2.32	2.52	1.09	4.55	0.35	0.2	0.35	0.21	0.49	0.15	0.26	0.0	0.0	0.33	0.47	0.2	0.5	0.33	0.62	0.67	0.14	0.67	0.58	0.77	394.74	1036.03	202.62	114.04	382.97	723.39	1058.25	469.44	284.3	791.98	1630	0.35
0.32	0.18	0.25	0.18	0.01	0.35	0.62	0.11	0.63	0.54	0.7	0.31	0.29	0.34	0.13	0.52	75.59	56.42	56.47	40.88	92.73	3.55	2.52	3.18	1.46	5.17	0.23	0.21	0.23	0.09	0.38	0.09	0.21	0.0	0.0	0.0	0.37	0.19	0.38	0.25	0.5	0.61	0.14	0.62	0.5	0.7	383.05	832.88	207.38	120.9	385.8	1087.28	1773.44	657.74	414.52	1134.2	4438	0.78


==> data_new/tef/mr/lstmatt/S_auc.tex <==
0.14

==> data_new/tef/mr/lstmatt/S_ppl.tex <==
2.3

==> data_new/tef/mr/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	245.52	360.13	144.99	83.62	271.53	245.52	360.13	144.99	83.62	271.53	2834	0.0
0.03	0.85	0.09	0.87	0.81	0.92	0.95	0.03	0.96	0.94	0.97	0.88	0.06	0.89	0.85	0.93	1.36	0.41	1.34	1.11	1.6	1.26	1.16	0.9	0.38	1.77	0.73	0.07	0.73	0.69	0.78	0.75	0.1	0.76	0.7	0.82	0.81	0.06	0.82	0.78	0.85	0.87	0.04	0.87	0.84	0.9	146.57	129.39	107.1	69.25	175.31	196.05	166.5	143.39	94.29	236.74	1373	0.04
0.06	0.77	0.13	0.78	0.7	0.86	0.9	0.06	0.92	0.88	0.94	0.81	0.09	0.82	0.77	0.87	1.5	0.51	1.49	1.14	1.85	1.28	1.24	0.89	0.38	1.8	0.64	0.09	0.65	0.59	0.7	0.66	0.14	0.68	0.58	0.75	0.75	0.08	0.75	0.71	0.8	0.83	0.05	0.83	0.8	0.86	179.86	204.5	124.75	76.39	210.92	324.08	468.62	215.66	127.85	377.9	2020	0.09
0.11	0.64	0.16	0.67	0.56	0.76	0.83	0.09	0.85	0.79	0.89	0.73	0.13	0.75	0.68	0.81	1.87	0.57	1.91	1.49	2.27	1.65	1.52	1.23	0.47	2.39	0.56	0.11	0.57	0.5	0.63	0.55	0.15	0.57	0.48	0.65	0.68	0.09	0.69	0.64	0.74	0.78	0.06	0.79	0.75	0.82	194.57	273.97	125.39	74.18	214.95	510.26	968.24	300.24	179.3	550.52	2505	0.19
0.15	0.52	0.21	0.54	0.38	0.68	0.74	0.11	0.76	0.69	0.82	0.64	0.17	0.67	0.56	0.75	1.82	0.56	1.81	1.42	2.21	1.32	1.24	0.93	0.4	1.89	0.47	0.14	0.49	0.4	0.57	0.45	0.18	0.46	0.34	0.57	0.62	0.11	0.63	0.56	0.69	0.74	0.07	0.75	0.7	0.79	223.38	307.12	136.98	78.71	245.19	759.93	989.54	438.84	250.11	865.93	1102	0.28
0.18	0.46	0.19	0.47	0.33	0.6	0.7	0.11	0.71	0.63	0.78	0.61	0.15	0.63	0.54	0.71	2.26	0.59	2.31	1.86	2.66	1.87	1.6	1.45	0.6	2.68	0.44	0.12	0.46	0.38	0.53	0.42	0.15	0.43	0.33	0.52	0.6	0.09	0.61	0.55	0.66	0.73	0.06	0.74	0.7	0.77	181.34	245.08	116.66	71.32	211.73	849.31	974.66	521.86	297.03	1030.92	1839	0.42
0.32	0.28	0.2	0.27	0.14	0.42	0.56	0.14	0.57	0.47	0.66	0.49	0.18	0.51	0.39	0.61	2.54	0.63	2.61	2.12	2.98	2.12	1.71	1.74	0.79	3.05	0.35	0.14	0.36	0.27	0.44	0.3	0.15	0.31	0.2	0.4	0.53	0.1	0.54	0.47	0.6	0.68	0.07	0.69	0.64	0.73	196.93	268.02	130.76	77.86	218.62	1835.22	2955.78	1093.52	598.82	2012.55	4799	0.96


==> data_new/tef/mr/roberta/A_auc.tex <==
0.18

==> data_new/tef/mr/roberta/A_ppl.tex <==
8.7

==> data_new/tef/mr/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	245.52	360.13	144.99	83.62	271.53	245.52	360.13	144.99	83.62	271.53	2834	0.0
0.03	0.2	0.37	0.24	-0.01	0.46	0.95	0.03	0.96	0.94	0.97	0.34	0.3	0.37	0.17	0.55	10.39	14.4	5.15	1.96	12.27	6.82	5.49	5.37	2.27	10.25	0.27	0.24	0.27	0.12	0.43	0.26	0.28	0.33	0.0	0.5	0.49	0.19	0.5	0.38	0.62	0.64	0.13	0.64	0.56	0.75	143.17	126.39	105.56	67.1	170.84	192.79	172.32	142.02	86.39	234.3	1513	0.04
0.06	0.03	0.36	0.04	-0.2	0.26	0.9	0.06	0.92	0.88	0.94	0.2	0.31	0.22	-0.01	0.42	11.92	22.53	6.5	2.91	13.46	6.93	5.48	5.52	2.37	10.59	0.16	0.24	0.16	0.0	0.32	0.17	0.28	0.0	0.0	0.33	0.42	0.2	0.43	0.29	0.56	0.59	0.14	0.6	0.5	0.69	174.49	195.05	121.36	75.18	206.8	301.57	303.28	209.78	126.77	358.67	2349	0.08
0.11	-0.15	0.32	-0.16	-0.34	0.04	0.84	0.08	0.85	0.79	0.89	0.03	0.29	0.04	-0.16	0.22	13.78	21.93	7.73	3.41	15.91	7.65	6.01	6.06	2.64	11.79	0.03	0.22	0.03	-0.11	0.17	0.11	0.23	0.0	0.0	0.0	0.33	0.18	0.33	0.22	0.44	0.53	0.13	0.54	0.44	0.62	191.41	265.95	121.57	72.91	215.15	510.09	936.31	307.28	177.55	523.86	3164	0.19
0.15	-0.23	0.32	-0.26	-0.44	-0.05	0.76	0.1	0.78	0.71	0.83	-0.07	0.29	-0.09	-0.28	0.12	12.54	21.76	7.17	3.68	14.8	6.9	5.95	5.16	2.34	10.02	-0.05	0.22	-0.06	-0.2	0.09	0.07	0.21	0.0	0.0	0.0	0.28	0.19	0.25	0.14	0.38	0.48	0.15	0.5	0.38	0.57	209.07	302.22	128.54	74.18	216.8	759.23	1014.54	441.76	242.33	853.15	1653	0.3
0.18	-0.3	0.25	-0.31	-0.47	-0.15	0.72	0.11	0.73	0.66	0.8	-0.15	0.25	-0.15	-0.32	0.01	10.96	12.15	7.36	3.53	14.23	7.54	5.88	6.29	2.74	11.4	-0.1	0.19	-0.1	-0.22	0.02	0.04	0.13	0.0	0.0	0.0	0.25	0.17	0.25	0.12	0.33	0.46	0.13	0.45	0.38	0.55	185.82	241.97	127.06	73.02	223.44	904.46	1249.37	559.55	335.82	964.2	1898	0.45
0.32	-0.37	0.25	-0.39	-0.54	-0.23	0.63	0.12	0.63	0.54	0.71	-0.22	0.25	-0.24	-0.39	-0.07	11.17	13.35	7.79	4.13	13.79	7.42	6.04	5.88	2.62	10.95	-0.16	0.19	-0.17	-0.28	-0.04	0.03	0.14	0.0	0.0	0.0	0.22	0.16	0.22	0.11	0.33	0.44	0.13	0.44	0.36	0.5	211.43	287.99	136.5	83.28	234.0	1709.22	2383.57	1038.41	593.74	1840.5	3073	0.82


==> data_new/tef/mr/roberta/IG_auc.tex <==
-0.04

==> data_new/tef/mr/roberta/IG_ppl.tex <==
8.7

==> data_new/tef/mr/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	245.59	360.1	144.84	83.77	271.43	245.59	360.1	144.84	83.77	271.43	2834	0.0
0.03	0.3	0.33	0.25	0.04	0.53	0.95	0.04	0.96	0.93	0.98	0.51	0.32	0.59	0.3	0.76	89.43	168.01	36.96	9.04	93.72	1.87	1.71	1.39	0.5	2.81	0.41	0.26	0.43	0.22	0.6	0.25	0.3	0.0	0.0	0.5	0.54	0.22	0.56	0.38	0.67	0.71	0.15	0.73	0.62	0.81	146.6	129.42	106.96	69.35	175.32	197.25	169.82	147.92	92.53	242.6	1373	0.04
0.06	0.22	0.3	0.16	-0.02	0.42	0.91	0.06	0.92	0.88	0.95	0.41	0.32	0.45	0.18	0.66	115.88	190.93	48.7	14.85	132.79	1.75	1.65	1.25	0.46	2.51	0.31	0.26	0.33	0.13	0.51	0.14	0.26	0.0	0.0	0.33	0.46	0.22	0.44	0.33	0.62	0.66	0.15	0.67	0.56	0.78	178.39	203.51	122.4	75.58	210.83	316.75	331.87	211.79	131.88	377.51	2053	0.09
0.11	0.12	0.27	0.06	-0.08	0.27	0.84	0.08	0.85	0.8	0.89	0.29	0.33	0.29	0.05	0.54	172.35	262.99	80.17	29.72	210.9	2.15	1.87	1.67	0.63	3.19	0.22	0.25	0.21	0.03	0.4	0.09	0.21	0.0	0.0	0.0	0.39	0.22	0.33	0.22	0.56	0.61	0.15	0.62	0.5	0.73	197.15	326.97	122.72	72.86	212.86	519.15	885.13	320.99	188.74	555.66	2770	0.19
0.15	0.07	0.26	0.01	-0.12	0.21	0.76	0.11	0.78	0.7	0.84	0.2	0.33	0.17	-0.05	0.46	179.49	268.76	81.24	37.34	208.64	1.75	1.57	1.29	0.56	2.48	0.15	0.25	0.12	-0.04	0.33	0.05	0.18	0.0	0.0	0.0	0.33	0.23	0.33	0.17	0.5	0.58	0.16	0.57	0.46	0.67	209.71	288.01	130.4	70.16	223.38	800.83	1163.26	431.15	251.82	854.67	1439	0.32
0.18	-0.02	0.2	-0.05	-0.16	0.08	0.73	0.1	0.74	0.67	0.8	0.1	0.29	0.08	-0.1	0.28	185.12	282.88	94.41	45.94	213.61	2.31	1.87	1.84	0.81	3.39	0.08	0.21	0.06	-0.07	0.2	0.04	0.13	0.0	0.0	0.0	0.28	0.18	0.25	0.14	0.38	0.54	0.13	0.54	0.44	0.62	173.11	175.64	115.5	72.77	210.35	869.3	1152.79	567.12	320.31	1001.29	2049	0.46
0.32	-0.09	0.18	-0.12	-0.21	0.01	0.62	0.13	0.64	0.55	0.72	-0.01	0.28	-0.03	-0.22	0.17	187.4	294.5	93.89	45.59	200.21	2.47	1.86	2.07	0.98	3.63	-0.01	0.2	-0.02	-0.15	0.12	0.02	0.1	0.0	0.0	0.0	0.22	0.17	0.22	0.11	0.33	0.5	0.13	0.5	0.42	0.57	204.18	259.71	136.71	82.22	227.84	1774.8	3158.87	1032.01	586.28	1916.24	3969	0.89


==> data_new/tef/mr/roberta/S_auc.tex <==
0.04

==> data_new/tef/mr/roberta/S_ppl.tex <==
8.7

==> data_new/tef/mr/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	252.38	449.96	137.18	77.08	260.21	252.38	449.96	137.18	77.08	260.21	2631	0.0
0.03	0.82	0.11	0.84	0.77	0.89	0.94	0.04	0.95	0.93	0.97	0.87	0.09	0.89	0.83	0.93	0.76	0.27	0.75	0.58	0.91	0.88	0.81	0.64	0.27	1.24	0.71	0.11	0.72	0.65	0.78	0.69	0.12	0.71	0.62	0.78	0.8	0.08	0.81	0.76	0.85	0.86	0.06	0.86	0.83	0.9	161.48	185.97	113.5	67.11	192.46	229.04	256.28	156.78	93.7	268.64	1425	0.04
0.06	0.74	0.14	0.77	0.67	0.85	0.89	0.07	0.9	0.85	0.93	0.8	0.12	0.82	0.74	0.88	0.84	0.32	0.83	0.62	1.03	0.99	0.94	0.71	0.31	1.39	0.63	0.12	0.63	0.56	0.71	0.6	0.14	0.61	0.51	0.7	0.73	0.09	0.74	0.68	0.8	0.82	0.07	0.82	0.78	0.86	198.2	290.32	122.99	69.73	214.94	390.1	701.05	215.78	126.2	407.94	2018	0.1
0.11	0.64	0.16	0.66	0.55	0.75	0.8	0.1	0.82	0.75	0.87	0.71	0.14	0.73	0.63	0.81	1.07	0.35	1.06	0.86	1.27	1.33	1.18	1.01	0.42	1.94	0.54	0.13	0.55	0.46	0.62	0.51	0.14	0.52	0.42	0.61	0.67	0.09	0.68	0.62	0.73	0.77	0.07	0.78	0.73	0.82	194.3	308.55	122.36	70.62	212.43	512.66	696.33	324.8	187.45	588.45	2724	0.16
0.15	0.55	0.17	0.57	0.46	0.67	0.72	0.12	0.74	0.65	0.81	0.61	0.16	0.62	0.51	0.73	1.06	0.36	1.04	0.82	1.27	1.31	1.19	0.97	0.43	1.99	0.45	0.14	0.44	0.36	0.54	0.43	0.15	0.44	0.32	0.53	0.61	0.1	0.61	0.54	0.67	0.72	0.08	0.72	0.68	0.78	222.09	379.77	124.45	65.71	225.38	791.28	1015.69	458.04	223.82	958.81	1290	0.26
0.18	0.49	0.17	0.52	0.38	0.61	0.67	0.12	0.68	0.6	0.75	0.57	0.17	0.6	0.48	0.69	1.27	0.37	1.24	1.04	1.47	1.57	1.38	1.13	0.52	2.25	0.42	0.13	0.43	0.34	0.51	0.4	0.15	0.41	0.3	0.5	0.59	0.1	0.6	0.53	0.66	0.71	0.08	0.72	0.67	0.76	189.87	344.48	115.15	70.17	209.03	1071.4	2669.91	612.08	351.8	1058.07	2088	0.46
0.32	0.39	0.18	0.41	0.28	0.53	0.57	0.13	0.58	0.48	0.67	0.46	0.2	0.49	0.35	0.61	1.4	0.39	1.37	1.14	1.63	1.89	1.57	1.43	0.7	2.75	0.33	0.15	0.34	0.25	0.43	0.33	0.14	0.34	0.24	0.44	0.53	0.11	0.54	0.46	0.61	0.67	0.08	0.67	0.62	0.72	208.28	328.58	129.15	75.82	225.96	1937.86	3592.73	1046.33	603.69	1917.09	4037	0.83


==> data_new/tef/mr/xlnet/A_auc.tex <==
0.19

==> data_new/tef/mr/xlnet/A_ppl.tex <==
10.0

==> data_new/tef/mr/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	252.38	449.96	137.18	77.08	260.21	252.38	449.96	137.18	77.08	260.21	2631	0.0
0.03	0.38	0.32	0.43	0.19	0.6	0.94	0.04	0.95	0.93	0.97	0.42	0.3	0.48	0.27	0.62	4.5	5.5	2.34	1.17	5.49	1.32	1.24	0.95	0.45	1.86	0.32	0.24	0.35	0.2	0.48	0.31	0.27	0.33	0.0	0.5	0.52	0.19	0.56	0.43	0.67	0.67	0.14	0.69	0.57	0.75	160.6	185.36	112.76	66.54	191.59	216.09	232.63	153.0	89.35	263.62	1438	0.03
0.06	0.22	0.35	0.25	-0.01	0.47	0.88	0.07	0.9	0.85	0.93	0.26	0.32	0.3	0.06	0.48	6.02	8.53	3.1	1.56	7.4	1.53	1.27	1.24	0.57	2.2	0.19	0.24	0.22	0.05	0.35	0.21	0.3	0.0	0.0	0.33	0.43	0.2	0.44	0.33	0.56	0.6	0.14	0.62	0.5	0.69	194.73	287.21	122.32	68.8	206.95	373.78	664.6	213.24	120.9	389.87	2073	0.09
0.11	-0.03	0.33	-0.04	-0.26	0.19	0.81	0.09	0.82	0.76	0.87	0.04	0.3	0.05	-0.18	0.24	7.37	8.18	4.23	2.06	9.66	1.65	1.36	1.32	0.62	2.38	0.03	0.22	0.03	-0.13	0.18	0.13	0.23	0.0	0.0	0.33	0.32	0.18	0.33	0.22	0.44	0.53	0.13	0.5	0.44	0.62	191.07	296.67	122.46	70.67	210.04	593.18	2049.62	311.99	175.76	574.13	3111	0.21
0.15	-0.17	0.32	-0.2	-0.39	0.02	0.74	0.11	0.76	0.68	0.82	-0.11	0.3	-0.12	-0.32	0.07	7.81	9.26	4.5	2.28	10.43	1.97	1.65	1.65	0.69	2.76	-0.07	0.22	-0.09	-0.22	0.07	0.08	0.22	0.0	0.0	0.0	0.26	0.18	0.25	0.12	0.33	0.46	0.14	0.45	0.38	0.56	224.91	416.74	118.72	69.46	217.76	872.23	2033.17	447.57	259.64	820.11	1590	0.29
0.18	-0.23	0.27	-0.26	-0.41	-0.07	0.69	0.11	0.7	0.62	0.77	-0.17	0.25	-0.19	-0.34	-0.02	8.2	8.69	4.95	2.53	10.94	1.93	1.52	1.59	0.79	2.71	-0.12	0.18	-0.13	-0.24	-0.0	0.06	0.17	0.0	0.0	0.0	0.24	0.16	0.22	0.11	0.33	0.45	0.12	0.44	0.38	0.5	182.67	326.65	114.94	67.2	207.51	972.59	2012.58	595.81	331.88	1034.06	2158	0.43
0.32	-0.32	0.23	-0.35	-0.48	-0.18	0.6	0.13	0.61	0.52	0.69	-0.26	0.22	-0.27	-0.42	-0.11	9.26	9.18	6.09	2.91	12.59	1.98	1.54	1.65	0.77	2.85	-0.18	0.17	-0.19	-0.3	-0.08	0.04	0.14	0.0	0.0	0.0	0.19	0.14	0.2	0.11	0.29	0.42	0.12	0.44	0.33	0.5	218.68	327.92	135.3	80.85	241.47	1745.69	2867.31	976.01	549.53	1905.41	3217	0.7


==> data_new/tef/mr/xlnet/IG_auc.tex <==
-0.01

==> data_new/tef/mr/xlnet/IG_ppl.tex <==
10.0

==> data_new/tef/mr/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	252.38	449.96	137.18	77.08	260.21	252.38	449.96	137.18	77.08	260.21	2631	0.0
0.03	0.77	0.15	0.8	0.69	0.87	0.94	0.04	0.95	0.93	0.97	0.85	0.12	0.88	0.79	0.93	323.5	600.59	113.8	47.99	315.07	0.94	0.76	0.76	0.34	1.35	0.71	0.13	0.73	0.64	0.8	0.52	0.29	0.5	0.33	0.67	0.77	0.14	0.78	0.67	0.89	0.86	0.08	0.88	0.81	0.93	160.99	185.73	113.04	66.22	191.8	227.1	250.46	162.1	93.52	280.7	1431	0.04
0.06	0.71	0.19	0.74	0.6	0.85	0.89	0.07	0.9	0.86	0.93	0.81	0.14	0.84	0.74	0.91	418.18	727.13	153.83	62.64	432.34	0.91	0.86	0.64	0.27	1.3	0.66	0.15	0.68	0.58	0.77	0.41	0.35	0.33	0.0	0.67	0.72	0.16	0.75	0.62	0.8	0.84	0.1	0.85	0.77	0.9	195.85	287.57	121.98	69.49	210.04	380.43	640.49	226.34	131.54	406.12	2063	0.09
0.11	0.57	0.22	0.59	0.42	0.73	0.81	0.09	0.83	0.76	0.88	0.71	0.18	0.74	0.61	0.84	576.13	833.65	251.74	91.14	710.14	1.29	1.1	1.0	0.4	1.99	0.56	0.16	0.57	0.45	0.67	0.3	0.3	0.33	0.0	0.5	0.63	0.17	0.67	0.56	0.78	0.79	0.11	0.81	0.73	0.88	188.53	294.43	121.35	70.91	206.65	499.87	749.09	327.51	186.98	593.05	3031	0.16
0.15	0.53	0.23	0.56	0.38	0.69	0.73	0.11	0.75	0.66	0.82	0.67	0.19	0.7	0.56	0.81	701.11	1046.96	252.77	105.4	891.4	1.17	1.07	0.83	0.34	1.68	0.52	0.18	0.53	0.41	0.64	0.26	0.33	0.0	0.0	0.5	0.61	0.18	0.62	0.5	0.71	0.77	0.11	0.78	0.69	0.86	221.41	406.74	118.33	64.1	219.32	826.04	1126.1	489.21	265.1	920.31	1585	0.27
0.18	0.43	0.22	0.43	0.27	0.59	0.68	0.12	0.7	0.61	0.77	0.59	0.2	0.61	0.47	0.74	814.86	1101.88	417.74	150.34	1076.01	1.44	1.2	1.16	0.48	2.1	0.45	0.17	0.44	0.34	0.56	0.19	0.27	0.0	0.0	0.33	0.55	0.17	0.56	0.44	0.67	0.73	0.11	0.75	0.69	0.81	179.17	308.32	112.66	67.52	206.65	1011.99	1835.03	615.95	327.43	1127.89	2005	0.46
0.32	0.34	0.23	0.33	0.17	0.49	0.57	0.14	0.59	0.48	0.68	0.49	0.23	0.51	0.33	0.67	967.26	1101.16	605.26	204.44	1369.99	1.57	1.28	1.27	0.55	2.29	0.36	0.19	0.36	0.23	0.5	0.14	0.24	0.0	0.0	0.33	0.48	0.17	0.44	0.33	0.6	0.69	0.12	0.69	0.62	0.77	221.36	343.99	138.16	81.24	241.91	1772.95	3055.21	1089.94	597.37	1974.35	3469	0.69


==> data_new/tef/mr/xlnet/S_auc.tex <==
0.17

==> data_new/tef/mr/xlnet/S_ppl.tex <==
10.1

==> data_new/tef/yelp/bert/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.79	0.13	0.77	0.69	0.86	0.98	0.02	0.98	0.97	0.99	0.92	0.05	0.91	0.88	0.95	1.88	1.07	2.09	1.48	2.65	2.97	4.05	1.59	0.27	4.08	0.8	0.11	0.77	0.74	0.83	0.81	0.11	0.77	0.73	0.84	0.87	0.07	0.85	0.82	0.88	0.91	0.05	0.9	0.88	0.92	165.73	708.54	56.41	40.1	76.35	172.8	707.55	63.05	46.87	86.02	489	0.01
0.03	0.61	0.11	0.6	0.53	0.68	0.94	0.03	0.94	0.92	0.96	0.82	0.06	0.82	0.79	0.85	2.78	0.82	2.77	2.18	3.4	4.33	4.62	2.8	1.15	6.38	0.65	0.06	0.65	0.62	0.68	0.65	0.06	0.66	0.61	0.69	0.76	0.04	0.76	0.73	0.79	0.83	0.03	0.83	0.82	0.85	65.77	51.1	55.16	38.91	71.57	88.25	65.38	74.39	54.0	94.82	354	0.05
0.06	0.47	0.11	0.46	0.4	0.54	0.9	0.04	0.9	0.88	0.92	0.72	0.07	0.72	0.68	0.77	3.22	0.98	3.23	2.53	3.89	5.0	4.98	3.92	1.55	6.58	0.55	0.06	0.55	0.52	0.59	0.54	0.08	0.55	0.5	0.59	0.68	0.05	0.69	0.66	0.71	0.78	0.03	0.79	0.76	0.8	69.46	61.91	55.66	39.55	73.87	123.74	104.86	96.87	73.69	127.92	364	0.11
0.11	0.38	0.11	0.35	0.31	0.43	0.84	0.05	0.85	0.82	0.88	0.63	0.09	0.64	0.59	0.69	3.59	1.1	3.56	2.78	4.32	6.08	6.39	4.07	1.6	8.76	0.47	0.07	0.48	0.43	0.52	0.47	0.07	0.47	0.43	0.52	0.63	0.05	0.63	0.6	0.66	0.74	0.04	0.75	0.72	0.77	125.1	587.32	55.48	39.62	72.41	210.05	540.13	121.68	94.04	159.03	347	0.09
0.15	0.26	0.09	0.25	0.2	0.3	0.78	0.06	0.78	0.75	0.81	0.54	0.09	0.55	0.49	0.6	4.12	1.27	4.07	3.19	4.94	7.71	7.98	5.08	2.36	10.7	0.39	0.07	0.39	0.35	0.43	0.39	0.07	0.39	0.34	0.44	0.57	0.05	0.57	0.54	0.6	0.7	0.04	0.7	0.68	0.72	73.64	149.29	54.95	39.12	71.27	231.86	358.92	172.33	134.37	235.5	337	0.29
0.18	0.2	0.08	0.18	0.15	0.23	0.71	0.06	0.71	0.68	0.75	0.46	0.08	0.47	0.41	0.51	4.39	1.44	4.21	3.21	5.4	8.31	8.34	5.87	2.41	11.65	0.33	0.06	0.33	0.29	0.36	0.33	0.07	0.33	0.28	0.37	0.52	0.04	0.53	0.49	0.55	0.67	0.03	0.67	0.65	0.69	82.86	221.42	55.66	38.31	71.85	345.79	662.74	244.3	189.27	348.64	376	0.43
0.32	0.14	0.06	0.13	0.09	0.16	0.64	0.07	0.65	0.6	0.69	0.39	0.1	0.4	0.33	0.45	4.68	1.54	4.49	3.52	5.59	9.66	9.63	6.91	2.89	13.05	0.27	0.07	0.28	0.23	0.32	0.28	0.07	0.27	0.23	0.32	0.48	0.05	0.49	0.46	0.52	0.64	0.04	0.65	0.62	0.67	96.17	422.06	55.38	39.62	71.91	549.23	2188.74	359.87	285.35	503.49	651	0.64


==> data_new/tef/yelp/bert/A_auc.tex <==
0.10

==> data_new/tef/yelp/bert/A_ppl.tex <==
7.4

==> data_new/tef/yelp/bert/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.22	0.55	0.24	-0.22	0.59	0.98	0.02	0.98	0.97	0.99	0.34	0.52	0.45	-0.15	0.72	19.19	20.5	12.04	1.84	31.24	14.78	18.66	8.04	1.21	20.76	0.31	0.46	0.35	-0.1	0.56	0.43	0.35	0.36	0.13	0.6	0.55	0.3	0.56	0.29	0.73	0.66	0.23	0.68	0.46	0.81	159.99	675.23	56.62	40.52	80.52	166.89	674.3	63.21	47.61	86.99	816	0.01
0.03	-0.19	0.36	-0.18	-0.48	0.09	0.94	0.03	0.95	0.93	0.96	-0.01	0.39	0.08	-0.38	0.32	25.59	21.65	22.21	7.81	37.38	18.95	19.56	13.05	4.82	26.17	-0.0	0.29	0.06	-0.27	0.24	0.18	0.17	0.17	0.0	0.3	0.35	0.18	0.37	0.18	0.5	0.51	0.15	0.54	0.37	0.64	65.04	49.65	54.75	39.37	71.18	86.54	59.65	72.4	54.84	96.84	729	0.04
0.06	-0.38	0.32	-0.4	-0.63	-0.14	0.9	0.04	0.91	0.88	0.93	-0.18	0.35	-0.16	-0.48	0.12	26.53	20.61	21.82	9.26	40.57	19.34	20.91	13.44	5.2	25.47	-0.13	0.27	-0.11	-0.35	0.1	0.11	0.13	0.07	0.0	0.2	0.27	0.16	0.25	0.13	0.4	0.45	0.14	0.46	0.34	0.57	68.19	59.2	55.66	39.69	71.22	111.33	76.1	93.3	70.83	121.91	403	0.09
0.11	-0.53	0.28	-0.57	-0.77	-0.31	0.86	0.05	0.87	0.84	0.89	-0.33	0.32	-0.41	-0.61	-0.04	25.07	21.33	20.0	7.4	35.25	21.25	22.55	12.97	6.12	29.46	-0.24	0.24	-0.29	-0.46	-0.02	0.07	0.13	0.0	0.0	0.1	0.21	0.14	0.17	0.1	0.33	0.4	0.13	0.38	0.29	0.51	110.26	498.14	55.88	40.53	73.82	199.5	684.47	123.1	90.34	167.01	485	0.11
0.15	-0.58	0.2	-0.62	-0.73	-0.43	0.8	0.05	0.81	0.78	0.84	-0.36	0.24	-0.39	-0.58	-0.15	27.67	22.6	24.6	8.27	41.47	21.97	22.16	16.4	5.7	30.52	-0.26	0.18	-0.28	-0.43	-0.11	0.05	0.07	0.0	0.0	0.08	0.19	0.12	0.16	0.09	0.28	0.39	0.1	0.37	0.31	0.47	77.06	148.08	55.89	39.6	79.84	215.99	219.6	165.26	127.71	218.16	529	0.24
0.18	-0.57	0.16	-0.57	-0.7	-0.43	0.75	0.05	0.75	0.71	0.78	-0.33	0.2	-0.33	-0.48	-0.2	30.71	22.83	27.06	12.13	46.31	21.56	19.68	14.9	7.21	30.97	-0.24	0.15	-0.23	-0.34	-0.14	0.04	0.06	0.0	0.0	0.08	0.2	0.09	0.2	0.13	0.28	0.4	0.08	0.41	0.34	0.47	83.87	258.62	51.44	35.33	67.27	385.52	1542.56	208.62	161.11	271.49	404	0.49
0.32	-0.53	0.14	-0.52	-0.62	-0.44	0.69	0.07	0.7	0.65	0.74	-0.31	0.15	-0.3	-0.39	-0.21	37.11	27.09	31.65	16.82	49.31	22.87	22.76	13.43	5.8	33.04	-0.22	0.11	-0.21	-0.28	-0.14	0.05	0.08	0.0	0.0	0.08	0.2	0.09	0.2	0.16	0.26	0.42	0.07	0.42	0.38	0.46	122.36	637.93	56.22	41.71	71.67	394.24	477.05	293.0	234.39	394.53	252	0.3


==> data_new/tef/yelp/bert/IG_auc.tex <==
-0.14

==> data_new/tef/yelp/bert/IG_ppl.tex <==
7.4

==> data_new/tef/yelp/bert/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.6	0.26	0.56	0.41	0.8	0.98	0.02	0.98	0.97	0.99	0.81	0.14	0.82	0.73	0.91	127.94	224.54	45.32	7.79	181.46	6.78	8.35	3.7	0.53	10.16	0.68	0.19	0.65	0.55	0.76	0.6	0.24	0.56	0.43	0.75	0.76	0.15	0.74	0.65	0.84	0.85	0.09	0.83	0.79	0.9	156.25	689.23	56.17	40.18	76.36	164.7	688.24	63.12	47.22	86.44	746	0.01
0.03	0.38	0.2	0.37	0.24	0.5	0.95	0.02	0.95	0.93	0.96	0.68	0.14	0.7	0.6	0.78	202.7	287.14	92.8	29.82	309.71	9.82	9.97	6.21	2.49	14.85	0.52	0.12	0.53	0.44	0.6	0.38	0.18	0.38	0.27	0.5	0.63	0.11	0.64	0.56	0.71	0.76	0.07	0.77	0.72	0.81	64.27	49.45	54.4	38.54	71.06	87.98	59.58	73.18	56.14	96.12	625	0.05
0.06	0.27	0.18	0.24	0.14	0.37	0.9	0.04	0.91	0.89	0.93	0.6	0.15	0.6	0.5	0.7	284.15	597.97	100.1	27.58	344.41	10.73	10.57	7.97	2.61	15.66	0.44	0.12	0.44	0.36	0.52	0.26	0.18	0.25	0.14	0.38	0.57	0.11	0.57	0.5	0.64	0.73	0.07	0.73	0.68	0.77	72.56	70.77	55.88	40.18	73.98	126.13	108.14	96.25	73.43	140.25	358	0.11
0.11	0.16	0.15	0.14	0.06	0.26	0.86	0.05	0.87	0.84	0.89	0.48	0.2	0.48	0.37	0.61	295.51	545.9	98.08	30.23	330.7	11.85	11.69	9.29	2.85	17.11	0.35	0.15	0.35	0.26	0.44	0.19	0.16	0.17	0.07	0.32	0.49	0.12	0.5	0.42	0.57	0.68	0.09	0.69	0.62	0.74	103.01	492.59	54.84	35.93	71.92	209.06	716.92	127.28	89.52	159.95	495	0.15
0.15	0.11	0.13	0.07	0.02	0.16	0.81	0.05	0.81	0.78	0.84	0.4	0.18	0.4	0.28	0.52	281.41	468.35	128.52	38.59	378.16	13.21	11.94	10.13	3.2	19.99	0.28	0.14	0.28	0.2	0.37	0.15	0.13	0.14	0.04	0.21	0.45	0.12	0.44	0.38	0.51	0.64	0.09	0.64	0.6	0.7	71.07	130.17	54.86	39.43	70.78	233.88	321.29	177.06	134.42	243.57	455	0.34
0.18	0.06	0.12	0.05	-0.01	0.12	0.75	0.06	0.75	0.71	0.79	0.31	0.2	0.33	0.19	0.45	363.24	459.25	186.14	67.38	446.93	13.8	12.17	10.25	4.13	21.59	0.22	0.14	0.22	0.13	0.32	0.11	0.11	0.09	0.0	0.17	0.39	0.11	0.4	0.33	0.47	0.61	0.08	0.62	0.56	0.67	79.65	202.63	55.7	41.26	71.06	425.54	2003.85	249.91	190.65	322.07	452	0.64
0.32	0.02	0.13	0.02	-0.06	0.09	0.7	0.07	0.7	0.66	0.74	0.23	0.22	0.24	0.07	0.38	374.11	466.03	225.31	81.06	483.46	12.77	11.37	10.27	3.92	18.82	0.16	0.15	0.17	0.04	0.27	0.1	0.11	0.08	0.0	0.15	0.36	0.12	0.36	0.29	0.45	0.58	0.09	0.6	0.52	0.64	121.11	538.94	56.43	40.1	76.18	566.58	2620.43	328.37	258.29	459.57	397	0.54


==> data_new/tef/yelp/bert/S_auc.tex <==
0.05

==> data_new/tef/yelp/bert/S_ppl.tex <==
6.8

==> data_new/tef/yelp/cnn/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.49	0.38	0.48	0.21	0.87	0.98	0.02	0.98	0.97	1.0	0.68	0.28	0.75	0.48	0.99	33.24	38.75	24.43	2.98	45.96	6.56	11.49	3.4	0.15	8.97	0.63	0.3	0.68	0.37	0.9	0.68	0.25	0.68	0.48	1.0	0.78	0.19	0.82	0.62	0.97	0.83	0.15	0.87	0.7	0.98	168.81	1017.9	63.91	47.11	96.45	174.41	1017.44	70.02	52.24	104.94	2174	0.01
0.03	0.12	0.31	0.09	-0.1	0.32	0.95	0.03	0.96	0.94	0.97	0.41	0.25	0.42	0.23	0.6	53.12	44.16	41.79	24.29	67.1	9.61	12.9	6.25	2.64	12.81	0.36	0.23	0.35	0.19	0.55	0.43	0.19	0.43	0.29	0.56	0.61	0.16	0.61	0.5	0.75	0.71	0.13	0.7	0.61	0.82	77.07	58.0	59.67	46.0	84.71	95.61	68.45	75.48	58.66	104.39	1983	0.07
0.06	-0.09	0.28	-0.12	-0.28	0.07	0.91	0.04	0.92	0.89	0.94	0.22	0.22	0.22	0.06	0.38	63.09	50.94	48.22	29.78	81.04	10.52	13.37	7.15	3.06	13.74	0.2	0.2	0.2	0.06	0.35	0.3	0.17	0.29	0.2	0.4	0.52	0.14	0.51	0.42	0.62	0.64	0.11	0.63	0.55	0.72	85.07	120.61	59.92	45.79	86.05	127.64	192.31	91.43	70.87	126.7	2085	0.14
0.11	-0.21	0.26	-0.25	-0.38	-0.06	0.87	0.04	0.88	0.85	0.9	0.09	0.2	0.08	-0.05	0.22	69.26	54.65	54.39	32.43	88.63	10.88	13.22	7.67	3.38	14.33	0.09	0.17	0.09	-0.03	0.21	0.22	0.15	0.2	0.12	0.31	0.45	0.12	0.44	0.36	0.54	0.59	0.1	0.59	0.51	0.67	88.98	245.51	60.73	46.18	86.02	159.04	367.04	110.54	86.71	152.57	2134	0.22
0.15	-0.34	0.23	-0.37	-0.5	-0.21	0.81	0.05	0.81	0.78	0.84	-0.07	0.18	-0.07	-0.19	0.04	76.37	57.57	61.62	37.72	96.63	11.22	13.2	8.08	3.69	14.57	-0.03	0.15	-0.03	-0.13	0.06	0.15	0.14	0.14	0.04	0.22	0.37	0.11	0.37	0.3	0.43	0.53	0.09	0.53	0.47	0.59	84.43	110.37	59.66	45.47	85.03	196.41	203.83	147.35	116.37	206.77	2136	0.37
0.18	-0.4	0.22	-0.43	-0.55	-0.28	0.75	0.05	0.75	0.72	0.78	-0.17	0.18	-0.18	-0.28	-0.07	78.93	59.77	62.83	38.77	100.08	10.82	12.47	8.16	3.64	14.33	-0.11	0.14	-0.12	-0.2	-0.03	0.12	0.13	0.11	0.0	0.18	0.31	0.1	0.31	0.25	0.38	0.49	0.08	0.49	0.44	0.54	108.92	740.89	60.21	45.72	86.09	270.89	430.89	195.82	155.26	269.49	2172	0.42
0.32	-0.45	0.2	-0.48	-0.58	-0.35	0.68	0.06	0.68	0.64	0.72	-0.27	0.16	-0.28	-0.38	-0.18	85.39	61.59	70.63	42.96	107.92	10.62	11.25	7.93	3.61	14.57	-0.19	0.12	-0.2	-0.27	-0.13	0.09	0.11	0.08	0.0	0.14	0.26	0.09	0.26	0.2	0.31	0.44	0.08	0.44	0.4	0.48	88.12	215.27	59.54	46.05	85.86	369.52	667.44	267.88	205.7	371.62	3340	0.9


==> data_new/tef/yelp/cnn/IG_auc.tex <==
-0.08

==> data_new/tef/yelp/cnn/IG_ppl.tex <==
3.6

==> data_new/tef/yelp/cnn/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.68	0.38	0.84	0.62	0.95	0.98	0.02	0.99	0.98	1.0	0.84	0.3	0.94	0.87	1.0	887.0	1334.75	468.98	0.0	1076.22	3.32	3.99	2.09	0.07	5.0	0.85	0.13	0.87	0.75	0.98	0.7	0.3	0.73	0.53	1.0	0.84	0.21	0.89	0.79	1.0	0.9	0.15	0.95	0.87	1.0	149.61	922.71	60.85	47.46	89.1	154.7	922.34	66.38	52.1	96.16	2650	0.01
0.03	0.67	0.24	0.72	0.59	0.82	0.95	0.03	0.96	0.94	0.97	0.77	0.23	0.83	0.75	0.9	1553.32	1634.49	974.0	554.39	1898.36	5.34	5.08	3.72	1.61	7.75	0.7	0.12	0.7	0.62	0.78	0.46	0.27	0.47	0.29	0.62	0.72	0.18	0.75	0.67	0.82	0.83	0.13	0.85	0.8	0.91	79.63	65.06	59.95	45.71	86.1	97.39	70.61	77.45	58.65	106.13	2023	0.06
0.06	0.57	0.23	0.6	0.46	0.73	0.92	0.03	0.92	0.9	0.94	0.68	0.24	0.73	0.62	0.82	1940.06	1923.05	1274.04	749.15	2361.8	6.42	5.97	4.64	1.94	9.34	0.57	0.14	0.58	0.49	0.67	0.34	0.26	0.33	0.14	0.5	0.63	0.15	0.64	0.55	0.73	0.78	0.11	0.8	0.73	0.85	85.88	120.92	61.62	45.79	86.9	125.78	126.66	94.07	72.64	131.81	2021	0.13
0.11	0.47	0.24	0.49	0.35	0.64	0.87	0.04	0.88	0.85	0.9	0.58	0.24	0.62	0.49	0.73	2317.85	2224.57	1519.58	909.95	2837.16	7.33	6.74	5.29	2.33	10.47	0.46	0.16	0.47	0.38	0.57	0.27	0.24	0.24	0.0	0.4	0.54	0.16	0.55	0.45	0.64	0.72	0.11	0.73	0.67	0.8	90.92	255.48	60.39	46.07	87.57	161.08	270.77	113.99	88.74	162.82	1971	0.22
0.15	0.36	0.23	0.36	0.23	0.52	0.81	0.05	0.81	0.79	0.84	0.46	0.22	0.49	0.34	0.6	2865.83	2588.04	1941.57	1177.62	3561.08	8.42	7.5	6.3	2.7	11.84	0.34	0.16	0.35	0.25	0.44	0.2	0.22	0.16	0.0	0.32	0.45	0.16	0.45	0.36	0.54	0.66	0.1	0.66	0.6	0.72	87.02	117.65	59.93	45.86	86.0	203.27	235.1	148.81	118.25	205.37	1858	0.38
0.18	0.25	0.25	0.25	0.1	0.41	0.75	0.06	0.75	0.72	0.78	0.31	0.25	0.33	0.17	0.48	3345.48	2958.77	2303.28	1393.29	4136.4	8.72	7.78	6.41	2.83	12.45	0.23	0.18	0.23	0.12	0.34	0.17	0.21	0.1	0.0	0.27	0.38	0.16	0.37	0.28	0.47	0.59	0.11	0.59	0.52	0.66	111.84	786.52	60.88	45.79	86.16	261.98	294.86	197.11	156.36	269.7	1925	0.38
0.32	0.1	0.26	0.1	-0.06	0.26	0.66	0.07	0.66	0.61	0.7	0.11	0.26	0.12	-0.05	0.29	4117.98	3580.53	2891.45	1789.52	5053.27	9.22	8.04	7.18	3.2	12.79	0.09	0.18	0.09	-0.03	0.2	0.12	0.18	0.0	0.0	0.2	0.3	0.15	0.29	0.2	0.38	0.52	0.12	0.52	0.45	0.59	87.0	208.11	59.73	45.57	86.04	350.06	279.85	273.21	212.13	383.77	3576	0.85


==> data_new/tef/yelp/cnn/S_auc.tex <==
0.12

==> data_new/tef/yelp/cnn/S_ppl.tex <==
3.6

==> data_new/tef/yelp/lstm/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.0	0.64	-0.09	-0.49	0.47	0.98	0.02	0.98	0.97	0.99	0.2	0.55	0.17	-0.2	0.58	1297.39	16661.68	51.05	15.37	210.15	16.81	19.15	10.44	1.41	24.93	0.21	0.49	0.14	-0.13	0.47	0.37	0.36	0.25	0.08	0.57	0.49	0.31	0.44	0.25	0.67	0.62	0.24	0.59	0.45	0.76	120.06	443.88	61.65	46.1	91.21	126.54	443.26	69.32	51.85	100.25	2540	0.02
0.03	-0.38	0.39	-0.35	-0.69	-0.11	0.95	0.02	0.96	0.94	0.97	-0.14	0.38	-0.1	-0.42	0.14	5967.64	144241.62	93.73	37.56	388.25	21.48	20.7	14.84	5.14	31.53	-0.1	0.31	-0.06	-0.29	0.12	0.14	0.16	0.08	0.0	0.22	0.3	0.18	0.3	0.16	0.43	0.47	0.16	0.48	0.36	0.59	73.21	54.24	57.47	43.62	81.44	93.84	70.01	74.74	57.78	104.62	2573	0.08
0.06	-0.55	0.32	-0.54	-0.82	-0.31	0.92	0.03	0.92	0.9	0.94	-0.33	0.32	-0.31	-0.57	-0.09	4601.17	93227.09	153.52	54.41	660.95	26.28	22.24	20.34	8.27	39.67	-0.25	0.26	-0.22	-0.43	-0.06	0.07	0.11	0.0	0.0	0.12	0.21	0.15	0.2	0.11	0.3	0.39	0.14	0.4	0.3	0.49	74.3	93.39	54.49	43.3	78.04	112.83	116.42	87.69	67.99	118.15	4581	0.15
0.11	-0.52	0.24	-0.51	-0.68	-0.36	0.87	0.04	0.88	0.85	0.9	-0.3	0.23	-0.27	-0.44	-0.14	4331.93	74299.27	80.7	44.46	242.07	20.17	18.85	14.21	5.34	29.59	-0.22	0.19	-0.19	-0.32	-0.1	0.07	0.1	0.0	0.0	0.11	0.22	0.11	0.22	0.14	0.3	0.41	0.1	0.42	0.35	0.48	81.27	232.89	58.07	43.88	81.74	150.08	404.12	112.75	88.71	153.14	4802	0.24
0.15	-0.53	0.17	-0.53	-0.64	-0.42	0.81	0.05	0.82	0.79	0.85	-0.27	0.17	-0.26	-0.37	-0.17	712.07	10254.35	49.3	34.33	83.61	11.86	11.56	8.28	3.57	16.02	-0.19	0.13	-0.18	-0.26	-0.11	0.06	0.09	0.0	0.0	0.11	0.24	0.1	0.24	0.17	0.3	0.43	0.08	0.43	0.38	0.48	86.31	91.44	66.46	49.91	94.74	217.55	182.81	172.02	131.43	244.11	2332	0.43
0.18	-0.55	0.17	-0.56	-0.68	-0.45	0.77	0.06	0.77	0.74	0.81	-0.31	0.17	-0.3	-0.39	-0.19	123.57	597.56	43.02	29.1	64.68	7.96	7.94	5.48	2.36	11.37	-0.22	0.13	-0.21	-0.29	-0.13	0.05	0.1	0.0	0.0	0.08	0.22	0.11	0.23	0.14	0.29	0.42	0.09	0.42	0.37	0.47	103.6	83.33	80.41	54.58	115.12	299.93	206.83	241.86	173.93	340.31	1019	0.54
0.32	-0.59	0.16	-0.6	-0.7	-0.5	0.72	0.07	0.73	0.68	0.77	-0.36	0.16	-0.36	-0.48	-0.24	76.4	238.38	40.64	25.71	60.02	6.33	6.16	4.18	2.06	8.43	-0.26	0.14	-0.26	-0.34	-0.17	0.03	0.08	0.0	0.0	0.0	0.19	0.12	0.19	0.11	0.26	0.4	0.09	0.41	0.35	0.46	194.09	623.99	102.61	62.5	157.66	545.21	834.19	338.0	230.5	567.02	593	0.51


==> data_new/tef/yelp/lstm/IG_auc.tex <==
-0.16

==> data_new/tef/yelp/lstm/IG_ppl.tex <==
3.5

==> data_new/tef/yelp/lstm/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.28	0.35	0.0	0.0	0.54	0.99	0.02	0.99	0.98	1.0	0.67	0.41	0.84	0.46	1.0	1498.25	9724.44	453.08	0.0	1400.56	8.96	11.93	5.03	0.26	12.59	0.69	0.2	0.65	0.54	0.84	0.58	0.39	0.56	0.24	1.0	0.72	0.3	0.76	0.49	1.0	0.81	0.21	0.86	0.67	1.0	94.25	328.2	58.55	44.84	83.15	98.83	328.0	63.11	48.07	89.63	4696	0.01
0.03	0.32	0.2	0.32	0.18	0.44	0.95	0.03	0.96	0.94	0.97	0.61	0.24	0.64	0.52	0.75	9849.36	178210.83	1897.42	915.01	3355.5	12.89	13.88	8.46	3.33	17.17	0.48	0.14	0.48	0.39	0.57	0.32	0.24	0.3	0.17	0.43	0.59	0.18	0.6	0.5	0.68	0.74	0.14	0.75	0.68	0.81	84.45	67.69	62.9	46.74	92.8	106.42	79.28	81.29	61.39	116.56	2166	0.07
0.06	0.22	0.17	0.21	0.11	0.32	0.91	0.04	0.92	0.89	0.94	0.47	0.2	0.5	0.36	0.61	92823.17	1323196.23	2647.53	1494.76	4601.17	14.79	15.42	9.85	3.59	20.62	0.35	0.15	0.36	0.26	0.44	0.18	0.16	0.17	0.04	0.28	0.49	0.14	0.5	0.41	0.58	0.67	0.11	0.68	0.62	0.74	87.85	120.79	61.85	46.65	90.66	135.42	183.42	98.85	74.95	140.44	2095	0.16
0.11	0.12	0.17	0.11	0.01	0.21	0.87	0.05	0.87	0.84	0.9	0.33	0.24	0.35	0.19	0.49	619712.5	10560748.45	3359.31	1965.31	6159.7	16.97	18.03	10.55	4.39	22.82	0.24	0.17	0.24	0.14	0.34	0.12	0.14	0.09	0.0	0.2	0.41	0.14	0.41	0.33	0.49	0.62	0.11	0.62	0.56	0.68	103.61	384.44	61.43	45.92	89.47	171.12	276.64	121.49	92.84	169.92	2297	0.19
0.15	0.01	0.15	-0.01	-0.08	0.09	0.81	0.05	0.81	0.78	0.84	0.15	0.22	0.15	0.01	0.29	38366.66	411931.99	4526.23	2545.24	7622.08	18.45	17.31	12.95	5.69	25.71	0.11	0.15	0.1	0.01	0.2	0.07	0.1	0.0	0.0	0.11	0.32	0.12	0.32	0.25	0.39	0.55	0.09	0.55	0.49	0.61	80.74	117.81	58.08	45.42	82.55	251.62	1550.43	158.0	124.25	210.24	2843	0.61
0.18	-0.04	0.14	-0.06	-0.13	0.02	0.76	0.05	0.76	0.73	0.79	0.04	0.21	0.02	-0.09	0.17	39908.43	826234.15	4643.98	2640.5	7334.49	18.39	16.92	13.12	5.58	27.21	0.03	0.14	0.02	-0.06	0.12	0.05	0.09	0.0	0.0	0.08	0.27	0.11	0.26	0.2	0.33	0.51	0.08	0.5	0.45	0.56	74.45	63.99	57.73	43.99	81.81	239.33	193.64	194.95	152.32	260.58	2584	0.64
0.32	-0.08	0.16	-0.1	-0.18	-0.0	0.72	0.06	0.73	0.68	0.76	-0.02	0.22	-0.04	-0.17	0.1	10313.58	87829.37	3937.59	2368.34	6483.04	14.17	14.25	9.55	4.47	19.39	-0.01	0.15	-0.03	-0.11	0.07	0.04	0.09	0.0	0.0	0.04	0.24	0.12	0.23	0.17	0.31	0.48	0.09	0.48	0.42	0.53	100.3	281.38	64.88	47.87	94.94	384.36	755.55	254.43	190.05	367.95	1759	0.81


==> data_new/tef/yelp/lstm/S_auc.tex <==
0.02

==> data_new/tef/yelp/lstm/S_ppl.tex <==
3.5

==> data_new/tef/yelp/lstmatt/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.6	0.31	0.59	0.35	0.94	0.98	0.02	0.98	0.97	0.99	0.97	0.03	0.98	0.96	0.99	0.33	0.26	0.31	0.15	0.48	16.16	23.53	7.52	0.6	20.94	0.89	0.08	0.89	0.85	0.94	0.84	0.13	0.84	0.76	1.0	0.92	0.06	0.93	0.88	0.98	0.95	0.04	0.95	0.92	0.98	170.25	1006.86	62.63	46.72	95.46	176.99	1006.28	70.04	53.27	104.48	2722	0.01
0.03	0.36	0.25	0.32	0.16	0.52	0.94	0.03	0.95	0.93	0.96	0.93	0.05	0.94	0.91	0.96	0.5	0.22	0.46	0.35	0.63	22.44	27.07	12.72	4.45	30.46	0.8	0.07	0.81	0.76	0.85	0.7	0.15	0.71	0.61	0.79	0.86	0.06	0.86	0.82	0.9	0.91	0.04	0.91	0.88	0.94	76.1	55.95	59.2	45.55	84.73	97.55	67.37	77.77	60.26	109.27	2499	0.08
0.06	0.25	0.22	0.2	0.08	0.37	0.9	0.04	0.91	0.88	0.93	0.88	0.06	0.89	0.85	0.92	0.58	0.21	0.56	0.42	0.73	24.76	29.17	13.42	5.09	34.58	0.73	0.08	0.74	0.69	0.78	0.57	0.19	0.6	0.5	0.68	0.8	0.08	0.81	0.76	0.85	0.88	0.05	0.88	0.85	0.91	83.63	109.0	60.49	46.19	87.91	133.11	202.05	96.5	74.7	135.41	2606	0.17
0.11	0.18	0.19	0.12	0.03	0.26	0.86	0.05	0.86	0.83	0.89	0.84	0.08	0.85	0.8	0.89	0.63	0.21	0.61	0.48	0.78	27.51	30.8	16.29	5.95	38.08	0.67	0.08	0.68	0.62	0.73	0.49	0.19	0.5	0.4	0.61	0.76	0.09	0.77	0.72	0.81	0.85	0.06	0.85	0.82	0.88	91.68	293.62	60.25	45.84	87.32	166.94	402.13	116.13	90.57	162.09	2560	0.24
0.15	0.12	0.17	0.07	0.01	0.17	0.79	0.05	0.8	0.77	0.83	0.78	0.09	0.79	0.74	0.84	0.67	0.2	0.65	0.53	0.81	29.5	31.04	18.99	7.39	40.72	0.6	0.09	0.6	0.55	0.66	0.4	0.19	0.4	0.29	0.52	0.71	0.09	0.71	0.67	0.76	0.81	0.06	0.82	0.78	0.85	87.46	251.37	59.17	45.54	84.65	202.74	259.54	153.93	121.97	208.76	2519	0.39
0.18	0.08	0.14	0.03	-0.01	0.11	0.74	0.05	0.74	0.7	0.77	0.72	0.1	0.73	0.66	0.79	0.68	0.18	0.66	0.55	0.81	29.36	30.62	18.43	7.47	40.94	0.54	0.09	0.54	0.48	0.6	0.32	0.19	0.33	0.2	0.44	0.66	0.1	0.67	0.61	0.72	0.78	0.06	0.79	0.75	0.82	102.46	673.94	59.39	45.89	85.58	295.87	1121.27	200.92	160.14	272.09	2623	0.55
0.32	0.04	0.12	0.0	-0.02	0.07	0.66	0.07	0.66	0.62	0.7	0.63	0.13	0.64	0.55	0.71	0.67	0.18	0.65	0.54	0.79	28.92	29.36	18.79	8.11	39.91	0.45	0.11	0.46	0.39	0.52	0.25	0.18	0.24	0.11	0.38	0.6	0.11	0.61	0.54	0.67	0.74	0.07	0.75	0.7	0.78	87.59	253.55	59.76	45.69	86.03	369.6	450.16	278.79	216.23	389.13	4919	0.94


==> data_new/tef/yelp/lstmatt/A_auc.tex <==
0.05

==> data_new/tef/yelp/lstmatt/A_ppl.tex <==
3.4

==> data_new/tef/yelp/lstmatt/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.54	0.36	0.55	0.29	0.86	0.98	0.02	0.98	0.97	0.99	0.7	0.24	0.7	0.55	0.89	2.79	2.56	2.42	1.02	4.01	8.4	12.15	4.09	0.37	11.21	0.61	0.26	0.56	0.44	0.76	0.62	0.25	0.57	0.44	0.82	0.74	0.17	0.72	0.62	0.87	0.82	0.12	0.8	0.73	0.9	170.24	1006.52	62.63	46.72	95.46	176.83	1005.93	69.67	52.5	105.72	2722	0.01
0.03	0.22	0.32	0.23	0.02	0.45	0.95	0.03	0.95	0.93	0.97	0.46	0.2	0.47	0.34	0.59	4.29	2.61	3.73	2.51	5.44	11.37	13.49	6.91	2.81	15.03	0.36	0.17	0.37	0.26	0.47	0.39	0.18	0.38	0.28	0.5	0.58	0.12	0.59	0.5	0.67	0.71	0.09	0.71	0.65	0.76	76.1	55.95	59.2	45.55	84.73	97.38	71.91	77.33	60.11	109.5	2499	0.08
0.06	0.04	0.31	0.03	-0.16	0.24	0.91	0.04	0.91	0.88	0.93	0.3	0.2	0.3	0.18	0.42	5.02	2.95	4.47	2.92	6.4	12.58	14.52	7.54	3.05	16.88	0.24	0.15	0.23	0.14	0.33	0.29	0.18	0.28	0.17	0.38	0.5	0.12	0.5	0.43	0.57	0.65	0.09	0.65	0.6	0.7	83.66	109.3	60.44	46.13	87.99	130.04	157.71	95.3	73.67	136.11	2601	0.16
0.11	-0.09	0.29	-0.09	-0.28	0.08	0.86	0.05	0.87	0.84	0.89	0.18	0.19	0.17	0.05	0.3	5.53	3.14	4.91	3.3	6.98	13.7	15.59	8.34	3.44	18.06	0.14	0.15	0.14	0.05	0.23	0.22	0.16	0.2	0.12	0.32	0.44	0.12	0.44	0.38	0.51	0.6	0.08	0.6	0.55	0.65	91.01	293.8	60.21	45.76	86.72	179.08	986.02	114.25	88.92	162.11	2562	0.28
0.15	-0.22	0.27	-0.23	-0.39	-0.07	0.8	0.05	0.8	0.77	0.83	0.04	0.19	0.04	-0.08	0.15	6.1	3.49	5.37	3.67	7.6	14.84	16.3	9.27	3.77	20.09	0.04	0.15	0.04	-0.05	0.12	0.17	0.14	0.16	0.07	0.24	0.38	0.11	0.38	0.31	0.44	0.55	0.08	0.55	0.5	0.6	91.45	297.96	59.19	45.46	84.77	341.36	3924.0	150.78	119.09	211.63	2558	0.8
0.18	-0.3	0.25	-0.31	-0.46	-0.15	0.74	0.05	0.74	0.71	0.78	-0.05	0.18	-0.05	-0.16	0.06	6.32	3.63	5.54	3.79	7.95	15.4	17.04	9.87	3.94	20.93	-0.03	0.13	-0.03	-0.11	0.05	0.13	0.13	0.12	0.0	0.2	0.33	0.1	0.33	0.27	0.39	0.52	0.08	0.52	0.47	0.56	100.35	659.99	59.21	45.19	85.44	252.98	226.63	196.57	156.81	272.62	2733	0.45
0.32	-0.35	0.22	-0.37	-0.5	-0.22	0.68	0.06	0.68	0.64	0.72	-0.13	0.17	-0.13	-0.23	-0.02	6.35	3.45	5.61	3.93	8.02	15.6	16.62	9.96	4.2	21.2	-0.08	0.12	-0.09	-0.16	-0.01	0.11	0.12	0.09	0.0	0.17	0.29	0.1	0.29	0.24	0.35	0.48	0.07	0.48	0.44	0.53	86.75	228.28	60.09	46.27	86.52	379.24	1795.09	263.05	203.92	371.71	4773	0.99


==> data_new/tef/yelp/lstmatt/IG_auc.tex <==
-0.04

==> data_new/tef/yelp/lstmatt/IG_ppl.tex <==
3.4

==> data_new/tef/yelp/lstmatt/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.74	0.23	0.77	0.6	0.95	0.98	0.02	0.98	0.97	0.99	0.78	0.22	0.83	0.66	0.96	75.86	82.66	56.27	21.45	104.82	13.67	18.36	6.73	0.56	19.04	0.66	0.24	0.65	0.5	0.85	0.6	0.28	0.56	0.38	0.88	0.74	0.19	0.73	0.6	0.91	0.83	0.13	0.83	0.74	0.94	170.24	1006.52	62.63	46.72	95.46	177.12	1005.89	70.49	53.17	105.73	2722	0.01
0.03	0.55	0.23	0.57	0.39	0.73	0.94	0.03	0.95	0.93	0.97	0.6	0.25	0.64	0.44	0.8	115.54	93.57	88.74	55.87	147.91	19.74	22.24	11.62	3.96	27.05	0.46	0.21	0.47	0.32	0.62	0.4	0.22	0.36	0.24	0.5	0.58	0.17	0.58	0.47	0.7	0.72	0.12	0.73	0.64	0.81	76.1	55.95	59.2	45.55	84.73	97.49	66.01	78.18	60.5	108.17	2499	0.08
0.06	0.42	0.24	0.42	0.25	0.59	0.9	0.04	0.91	0.88	0.93	0.47	0.29	0.5	0.28	0.7	137.36	106.6	109.05	68.96	170.38	22.21	24.28	13.5	4.28	31.9	0.36	0.22	0.36	0.21	0.52	0.31	0.22	0.27	0.15	0.43	0.5	0.17	0.5	0.38	0.62	0.67	0.13	0.67	0.57	0.76	83.66	109.3	60.44	46.13	87.99	128.92	150.62	96.73	74.37	136.41	2601	0.16
0.11	0.32	0.23	0.3	0.14	0.48	0.86	0.05	0.87	0.84	0.89	0.36	0.31	0.37	0.14	0.59	160.37	138.42	125.3	82.39	193.83	24.3	25.38	15.15	5.26	35.62	0.27	0.23	0.26	0.12	0.44	0.26	0.21	0.2	0.11	0.33	0.44	0.18	0.43	0.32	0.56	0.62	0.13	0.62	0.53	0.71	91.9	293.79	60.31	45.85	86.9	165.04	394.68	116.0	90.2	163.53	2573	0.23
0.15	0.2	0.23	0.18	0.03	0.34	0.8	0.05	0.8	0.77	0.83	0.21	0.33	0.2	-0.04	0.45	191.43	181.63	144.07	92.83	224.7	26.06	25.47	17.38	6.94	38.62	0.16	0.23	0.15	-0.01	0.32	0.19	0.19	0.14	0.06	0.28	0.37	0.18	0.35	0.25	0.49	0.56	0.14	0.55	0.46	0.65	86.82	247.2	59.16	45.44	84.7	210.12	362.61	152.71	121.59	209.6	2598	0.41
0.18	0.12	0.23	0.09	-0.05	0.26	0.75	0.05	0.75	0.71	0.78	0.09	0.33	0.06	-0.17	0.33	205.1	180.92	154.0	100.75	245.21	26.1	25.23	17.91	6.85	38.58	0.08	0.23	0.06	-0.1	0.23	0.15	0.18	0.1	0.0	0.24	0.32	0.17	0.3	0.2	0.43	0.51	0.14	0.5	0.41	0.6	100.84	648.05	59.89	45.53	85.48	259.96	245.3	200.98	158.16	270.17	2838	0.46
0.32	0.04	0.22	0.01	-0.12	0.17	0.68	0.06	0.69	0.65	0.72	-0.04	0.33	-0.08	-0.29	0.17	212.88	175.86	161.88	108.75	258.1	26.44	25.13	18.21	7.53	38.21	-0.01	0.23	-0.04	-0.18	0.13	0.12	0.16	0.07	0.0	0.18	0.27	0.16	0.25	0.15	0.37	0.46	0.14	0.45	0.37	0.55	88.21	261.07	59.54	46.06	86.48	354.23	760.24	255.1	197.91	361.85	4617	0.88


==> data_new/tef/yelp/lstmatt/S_auc.tex <==
0.08

==> data_new/tef/yelp/lstmatt/S_ppl.tex <==
3.4

==> data_new/tef/yelp/roberta/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.8	0.12	0.78	0.72	0.85	0.98	0.02	0.98	0.97	0.99	0.94	0.04	0.94	0.92	0.96	2.45	1.43	2.62	1.86	3.54	3.01	3.82	1.95	0.36	4.16	0.82	0.09	0.8	0.77	0.84	0.8	0.11	0.78	0.74	0.83	0.88	0.07	0.86	0.84	0.89	0.92	0.04	0.9	0.89	0.92	122.61	429.83	49.4	36.22	70.88	128.81	428.98	55.51	41.97	78.39	725	0.01
0.03	0.64	0.09	0.63	0.59	0.69	0.95	0.03	0.95	0.93	0.97	0.88	0.04	0.89	0.86	0.9	3.49	1.04	3.48	2.69	4.36	4.01	3.85	2.94	1.26	5.27	0.71	0.05	0.71	0.68	0.74	0.67	0.08	0.69	0.63	0.73	0.79	0.04	0.8	0.77	0.82	0.86	0.03	0.86	0.85	0.87	58.24	38.46	46.97	35.7	66.31	76.33	45.55	64.74	47.54	89.11	472	0.05
0.06	0.52	0.09	0.52	0.45	0.57	0.91	0.04	0.91	0.88	0.93	0.81	0.07	0.83	0.79	0.85	3.94	1.21	4.04	3.01	4.89	4.69	4.42	3.47	1.26	6.88	0.63	0.07	0.65	0.6	0.67	0.59	0.09	0.61	0.54	0.66	0.74	0.06	0.75	0.71	0.78	0.82	0.04	0.83	0.81	0.84	63.47	49.34	50.9	35.91	68.94	108.6	77.51	84.23	62.78	122.91	577	0.11
0.11	0.43	0.09	0.43	0.37	0.48	0.86	0.05	0.87	0.83	0.89	0.77	0.08	0.79	0.75	0.82	4.39	1.3	4.49	3.39	5.41	5.44	5.39	3.93	1.45	7.75	0.59	0.08	0.6	0.56	0.63	0.54	0.1	0.56	0.47	0.62	0.71	0.07	0.72	0.68	0.75	0.8	0.04	0.81	0.79	0.82	84.57	316.16	49.28	35.56	65.68	151.61	242.39	106.83	79.88	148.35	708	0.12
0.15	0.32	0.09	0.32	0.26	0.38	0.8	0.05	0.8	0.76	0.83	0.72	0.09	0.74	0.68	0.78	4.82	1.49	4.9	3.73	6.02	6.72	6.07	4.97	2.26	9.13	0.53	0.08	0.54	0.5	0.58	0.47	0.11	0.49	0.4	0.55	0.67	0.06	0.68	0.63	0.71	0.77	0.04	0.78	0.75	0.8	74.88	161.18	50.24	35.85	68.72	240.57	395.53	165.34	128.24	230.09	433	0.33
0.18	0.25	0.08	0.24	0.2	0.3	0.73	0.06	0.73	0.69	0.77	0.67	0.11	0.7	0.62	0.74	5.18	1.59	5.29	3.9	6.4	7.81	6.99	6.16	2.58	11.44	0.49	0.09	0.51	0.45	0.54	0.42	0.12	0.45	0.34	0.51	0.63	0.08	0.65	0.6	0.68	0.75	0.04	0.76	0.73	0.78	75.39	267.31	49.08	35.75	67.11	289.89	212.06	238.1	185.9	309.4	500	0.43
0.32	0.2	0.08	0.2	0.15	0.25	0.68	0.07	0.68	0.64	0.73	0.63	0.12	0.67	0.6	0.71	5.58	1.66	5.72	4.37	6.79	8.54	7.32	6.96	2.84	12.04	0.46	0.1	0.48	0.42	0.52	0.39	0.12	0.41	0.32	0.48	0.62	0.08	0.63	0.58	0.67	0.74	0.05	0.75	0.72	0.77	81.06	261.38	49.4	36.22	65.53	505.12	1191.29	333.27	249.68	465.37	577	0.79


==> data_new/tef/yelp/roberta/A_auc.tex <==
0.12

==> data_new/tef/yelp/roberta/A_ppl.tex <==
6.6

==> data_new/tef/yelp/roberta/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.24	0.52	0.15	-0.07	0.67	0.98	0.02	0.98	0.97	0.99	0.45	0.37	0.4	0.16	0.75	93.1	385.38	17.27	5.15	36.48	21.13	28.54	12.2	2.24	27.65	0.4	0.36	0.31	0.12	0.62	0.44	0.32	0.34	0.2	0.67	0.59	0.25	0.53	0.4	0.74	0.71	0.18	0.68	0.57	0.83	131.72	477.56	51.22	35.86	69.2	138.73	476.55	57.79	41.34	79.41	514	0.01
0.03	-0.12	0.42	-0.12	-0.4	0.12	0.95	0.03	0.95	0.93	0.97	0.2	0.29	0.19	0.02	0.38	199.64	1151.45	26.33	15.92	50.05	28.6	30.68	16.78	6.86	37.07	0.16	0.23	0.14	0.01	0.29	0.24	0.18	0.2	0.11	0.33	0.43	0.16	0.42	0.31	0.51	0.6	0.12	0.59	0.51	0.67	56.97	37.37	46.62	36.43	64.59	77.44	47.68	66.09	49.37	89.26	556	0.05
0.06	-0.22	0.4	-0.21	-0.47	0.01	0.91	0.04	0.91	0.89	0.93	0.08	0.28	0.07	-0.11	0.22	83.39	153.78	32.65	18.72	57.88	23.6	24.95	14.96	7.14	30.67	0.07	0.21	0.05	-0.07	0.16	0.17	0.17	0.12	0.04	0.25	0.38	0.15	0.36	0.28	0.44	0.55	0.11	0.55	0.48	0.62	62.79	47.62	51.15	36.21	70.49	107.56	80.02	86.41	62.11	119.91	429	0.11
0.11	-0.38	0.36	-0.45	-0.65	-0.17	0.86	0.05	0.86	0.83	0.89	-0.04	0.28	-0.05	-0.25	0.14	45.43	59.76	32.31	20.27	47.22	21.36	19.78	14.79	6.24	30.96	-0.02	0.21	-0.03	-0.17	0.11	0.14	0.17	0.08	0.0	0.2	0.32	0.15	0.31	0.21	0.41	0.51	0.11	0.51	0.43	0.57	99.49	375.21	47.05	34.92	67.94	194.7	534.59	115.8	86.7	159.43	497	0.14
0.15	-0.44	0.3	-0.5	-0.62	-0.27	0.81	0.05	0.81	0.78	0.84	-0.14	0.24	-0.17	-0.31	0.0	44.23	60.94	29.35	21.9	41.28	19.96	19.8	12.73	6.11	28.0	-0.09	0.18	-0.12	-0.21	0.01	0.08	0.12	0.04	0.0	0.12	0.28	0.12	0.26	0.19	0.35	0.47	0.1	0.47	0.41	0.53	73.97	160.42	51.37	35.54	67.09	221.56	250.84	165.37	124.59	230.22	581	0.3
0.18	-0.43	0.3	-0.47	-0.63	-0.25	0.76	0.06	0.76	0.72	0.79	-0.11	0.22	-0.15	-0.27	-0.01	34.98	30.96	29.81	20.57	40.47	19.85	22.97	12.39	4.72	25.39	-0.07	0.16	-0.1	-0.18	0.0	0.1	0.13	0.08	0.0	0.15	0.29	0.12	0.27	0.21	0.34	0.49	0.09	0.48	0.43	0.54	97.32	409.32	49.32	35.19	63.62	335.38	578.99	227.55	172.7	299.87	314	0.37
0.32	-0.41	0.3	-0.46	-0.64	-0.15	0.71	0.07	0.71	0.67	0.76	-0.07	0.24	-0.11	-0.24	0.07	38.54	41.42	28.18	19.4	44.77	19.82	21.67	12.07	6.25	25.78	-0.04	0.18	-0.06	-0.16	0.05	0.09	0.12	0.04	0.0	0.12	0.3	0.12	0.29	0.23	0.37	0.5	0.1	0.48	0.44	0.54	72.01	53.78	56.83	41.38	84.45	506.86	571.79	344.32	248.71	530.59	166	0.91


==> data_new/tef/yelp/roberta/IG_auc.tex <==
-0.10

==> data_new/tef/yelp/roberta/IG_ppl.tex <==
6.6

==> data_new/tef/yelp/roberta/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.41	0.35	0.32	0.12	0.65	0.98	0.02	0.98	0.97	0.99	0.66	0.29	0.73	0.5	0.87	1648.47	7880.26	141.23	29.51	655.6	12.77	15.83	6.8	1.29	17.73	0.54	0.28	0.55	0.35	0.7	0.49	0.31	0.47	0.23	0.67	0.67	0.22	0.68	0.51	0.81	0.77	0.14	0.78	0.67	0.87	97.7	344.99	49.27	36.48	66.2	104.11	344.32	55.87	41.73	74.71	1108	0.01
0.03	0.2	0.21	0.17	0.04	0.33	0.96	0.02	0.96	0.94	0.97	0.46	0.28	0.51	0.27	0.69	2678.39	6375.56	438.44	110.1	1772.82	16.6	16.4	10.66	3.89	24.83	0.34	0.22	0.36	0.18	0.52	0.27	0.19	0.25	0.12	0.4	0.52	0.17	0.54	0.39	0.65	0.67	0.11	0.68	0.59	0.76	56.26	36.17	47.05	35.13	64.61	74.68	43.42	64.86	47.38	85.63	483	0.05
0.06	0.15	0.16	0.12	0.04	0.25	0.92	0.03	0.92	0.9	0.94	0.42	0.23	0.45	0.27	0.6	1957.53	5498.11	335.5	125.56	1039.47	12.92	13.92	7.94	2.68	18.81	0.31	0.18	0.31	0.18	0.45	0.22	0.18	0.2	0.08	0.33	0.49	0.15	0.48	0.38	0.6	0.66	0.1	0.67	0.59	0.73	62.88	45.51	51.17	36.19	73.74	107.91	77.36	87.45	64.21	120.44	511	0.1
0.11	0.1	0.14	0.07	0.0	0.17	0.88	0.05	0.88	0.85	0.91	0.36	0.22	0.37	0.21	0.52	1395.43	8636.63	269.16	115.97	768.52	14.91	13.94	10.67	4.34	20.44	0.26	0.16	0.26	0.14	0.37	0.17	0.15	0.14	0.04	0.25	0.45	0.13	0.45	0.36	0.54	0.63	0.09	0.64	0.56	0.7	81.05	286.47	45.95	35.56	68.56	172.43	413.45	109.47	86.93	167.57	649	0.16
0.15	0.06	0.14	0.04	-0.02	0.1	0.82	0.05	0.83	0.8	0.86	0.29	0.21	0.29	0.16	0.44	871.41	1397.16	350.68	159.39	796.94	15.1	14.38	10.25	3.38	22.56	0.21	0.16	0.2	0.11	0.3	0.13	0.16	0.1	0.0	0.18	0.42	0.13	0.41	0.34	0.5	0.61	0.09	0.61	0.55	0.67	69.15	144.07	48.55	33.9	64.9	220.12	237.09	162.9	123.69	226.02	549	0.31
0.18	0.04	0.13	0.0	-0.04	0.09	0.78	0.06	0.79	0.74	0.82	0.25	0.22	0.25	0.11	0.42	1107.4	1991.81	497.78	220.49	1180.09	13.29	16.6	6.76	3.14	16.3	0.18	0.16	0.17	0.07	0.29	0.09	0.11	0.04	0.0	0.15	0.38	0.12	0.38	0.31	0.46	0.6	0.1	0.6	0.53	0.65	104.35	392.28	53.95	40.65	77.16	349.93	482.92	251.82	176.16	389.74	229	0.33
0.32	0.03	0.15	-0.01	-0.05	0.08	0.73	0.07	0.74	0.7	0.78	0.24	0.23	0.25	0.1	0.39	1079.08	1752.92	559.77	207.59	903.73	8.55	10.12	4.1	1.68	12.81	0.17	0.16	0.17	0.07	0.26	0.05	0.08	0.0	0.0	0.11	0.37	0.15	0.36	0.27	0.47	0.58	0.12	0.58	0.53	0.65	221.88	656.47	60.37	44.25	87.98	1783.49	5793.51	374.57	270.81	728.54	86	1.0


==> data_new/tef/yelp/roberta/S_auc.tex <==
0.03

==> data_new/tef/yelp/roberta/S_ppl.tex <==
7.0

==> data_new/tef/yelp/xlnet/A.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.96	0.03	0.96	0.94	0.98	0.98	0.02	0.98	0.97	0.99	0.96	0.02	0.96	0.95	0.98	0.69	0.4	0.73	0.4	1.01	0.6	0.75	0.35	0.08	0.84	0.88	0.06	0.86	0.84	0.9	0.91	0.05	0.9	0.87	0.94	0.92	0.04	0.92	0.9	0.94	0.94	0.03	0.94	0.93	0.96	109.47	403.5	51.32	38.48	72.51	118.16	402.79	60.67	44.94	84.76	979	0.01
0.03	0.92	0.04	0.91	0.89	0.94	0.95	0.03	0.96	0.93	0.97	0.91	0.04	0.91	0.89	0.93	1.07	0.36	1.09	0.77	1.37	0.9	0.84	0.64	0.28	1.24	0.77	0.06	0.77	0.75	0.81	0.83	0.06	0.82	0.79	0.86	0.86	0.04	0.85	0.83	0.88	0.89	0.03	0.89	0.88	0.91	61.18	47.1	49.68	37.02	67.22	86.22	64.84	72.15	51.97	95.03	321	0.06
0.06	0.87	0.05	0.87	0.84	0.9	0.91	0.04	0.91	0.89	0.94	0.85	0.05	0.85	0.83	0.88	1.32	0.37	1.31	1.01	1.64	1.25	1.12	0.93	0.33	1.95	0.69	0.06	0.69	0.66	0.73	0.76	0.06	0.76	0.73	0.8	0.8	0.04	0.8	0.77	0.83	0.85	0.03	0.85	0.83	0.87	68.08	61.34	52.53	37.11	72.51	125.34	113.75	93.61	70.6	127.82	329	0.13
0.11	0.81	0.1	0.82	0.79	0.86	0.87	0.05	0.87	0.83	0.9	0.8	0.07	0.8	0.77	0.83	1.53	0.39	1.56	1.2	1.85	1.45	1.48	1.01	0.37	2.02	0.62	0.07	0.63	0.6	0.66	0.69	0.1	0.7	0.66	0.74	0.75	0.06	0.75	0.72	0.78	0.82	0.04	0.82	0.8	0.84	156.4	609.3	52.45	37.87	72.7	292.47	914.03	123.77	92.89	168.63	325	0.13
0.15	0.76	0.06	0.77	0.73	0.8	0.78	0.07	0.79	0.74	0.83	0.72	0.07	0.72	0.69	0.76	1.79	0.42	1.81	1.42	2.12	1.9	1.72	1.44	0.55	2.7	0.54	0.06	0.54	0.52	0.58	0.64	0.06	0.63	0.6	0.68	0.69	0.05	0.69	0.67	0.72	0.77	0.03	0.77	0.76	0.79	65.81	59.5	51.32	36.63	67.92	232.41	178.34	187.04	142.16	241.11	317	0.38
0.18	0.69	0.1	0.71	0.66	0.74	0.71	0.07	0.71	0.66	0.76	0.65	0.08	0.65	0.62	0.7	2.01	0.43	2.02	1.72	2.36	2.26	2.05	1.71	0.76	2.92	0.48	0.07	0.48	0.45	0.52	0.58	0.08	0.57	0.53	0.62	0.65	0.06	0.65	0.62	0.68	0.74	0.04	0.74	0.72	0.76	71.01	66.24	52.73	37.68	72.9	336.67	246.09	273.72	208.44	371.18	312	0.56
0.32	0.64	0.08	0.65	0.61	0.69	0.62	0.08	0.62	0.57	0.67	0.58	0.08	0.59	0.54	0.63	2.24	0.44	2.29	1.88	2.61	2.52	2.17	1.94	0.86	3.61	0.42	0.06	0.42	0.38	0.46	0.52	0.07	0.52	0.49	0.57	0.61	0.05	0.6	0.58	0.63	0.71	0.03	0.71	0.69	0.73	63.95	52.61	50.23	37.85	67.38	491.2	488.93	384.52	298.4	526.63	838	1.0


==> data_new/tef/yelp/xlnet/A_auc.tex <==
0.24

==> data_new/tef/yelp/xlnet/A_ppl.tex <==
6.7

==> data_new/tef/yelp/xlnet/IG.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.13	0.66	0.09	-0.43	0.85	0.98	0.02	0.98	0.97	0.99	0.37	0.49	0.39	-0.03	0.84	6.44	14.08	1.45	0.36	5.01	7.47	11.77	2.8	0.64	9.1	0.33	0.43	0.29	-0.02	0.69	0.43	0.33	0.36	0.14	0.7	0.55	0.28	0.52	0.32	0.78	0.68	0.21	0.67	0.51	0.85	101.6	378.39	48.45	37.87	68.06	109.89	377.7	55.43	42.83	79.8	1165	0.01
0.03	-0.16	0.54	-0.23	-0.58	0.12	0.95	0.02	0.96	0.94	0.97	0.12	0.43	0.09	-0.12	0.42	9.54	19.84	3.21	1.37	7.89	8.73	12.11	5.04	1.48	11.19	0.1	0.34	0.08	-0.08	0.3	0.25	0.21	0.2	0.09	0.36	0.4	0.2	0.38	0.26	0.54	0.57	0.17	0.57	0.46	0.67	56.25	37.73	45.06	36.18	63.32	77.17	48.47	63.64	49.31	88.35	962	0.06
0.06	-0.27	0.43	-0.3	-0.58	-0.02	0.92	0.03	0.92	0.9	0.94	-0.0	0.35	0.01	-0.2	0.23	8.33	14.71	3.98	1.73	9.4	10.0	12.76	6.0	2.3	11.65	0.0	0.27	0.01	-0.14	0.17	0.18	0.16	0.14	0.05	0.27	0.34	0.16	0.33	0.24	0.43	0.51	0.14	0.52	0.44	0.6	60.41	43.98	49.27	38.25	64.15	105.17	74.81	86.68	64.96	114.96	1193	0.12
0.11	-0.28	0.36	-0.25	-0.52	-0.05	0.86	0.05	0.87	0.83	0.9	-0.07	0.3	-0.06	-0.25	0.15	7.78	11.99	3.66	1.75	8.58	8.4	11.9	3.88	1.74	10.31	-0.05	0.22	-0.04	-0.17	0.11	0.14	0.14	0.12	0.0	0.2	0.29	0.14	0.29	0.2	0.39	0.49	0.12	0.5	0.42	0.57	93.31	327.61	53.23	38.25	74.03	216.08	619.16	133.32	88.3	189.57	500	0.22
0.15	-0.24	0.33	-0.25	-0.47	-0.06	0.79	0.07	0.79	0.75	0.83	-0.07	0.25	-0.07	-0.23	0.08	4.65	5.46	2.4	1.31	5.8	5.66	6.28	3.4	1.75	7.15	-0.05	0.19	-0.05	-0.15	0.06	0.11	0.14	0.06	0.0	0.17	0.3	0.13	0.3	0.22	0.38	0.48	0.11	0.49	0.42	0.55	89.68	77.86	61.44	42.98	96.3	295.36	226.55	218.6	166.38	325.14	346	0.38
0.18	-0.31	0.25	-0.33	-0.46	-0.15	0.74	0.07	0.74	0.69	0.78	-0.14	0.21	-0.16	-0.29	-0.02	3.06	2.65	2.37	1.2	3.41	3.36	3.77	2.17	1.53	3.78	-0.1	0.15	-0.11	-0.19	-0.01	0.08	0.11	0.0	0.0	0.16	0.26	0.13	0.29	0.16	0.34	0.48	0.1	0.48	0.43	0.54	135.63	477.48	66.49	50.4	114.37	538.66	1700.76	282.65	203.39	493.78	105	0.49
0.32	-0.19	0.31	-0.23	-0.39	0.03	0.68	0.13	0.68	0.61	0.77	-0.08	0.24	-0.08	-0.24	0.08	3.99	8.77	2.43	1.21	3.63	3.75	3.42	2.75	1.8	4.78	-0.06	0.18	-0.06	-0.17	0.05	0.11	0.16	0.0	0.0	0.17	0.3	0.14	0.31	0.21	0.4	0.48	0.11	0.5	0.43	0.56	260.24	782.41	76.55	58.05	114.49	1822.96	4242.69	447.36	345.86	768.69	83	1.0


==> data_new/tef/yelp/xlnet/IG_auc.tex <==
-0.07

==> data_new/tef/yelp/xlnet/IG_ppl.tex <==
6.0

==> data_new/tef/yelp/xlnet/S.tex <==
x	expl_sim_mean	expl_sim_std	expl_sim_median	expl_sim_lower_quartile	expl_sim_upper_quartile	sem_sim_mean	sem_sim_std	sem_sim_median	sem_sim_lower_quartile	sem_sim_upper_quartile	spearman_mean	spearman_std	spearman_median	spearman_lower_quartile	spearman_upper_quartile	l2_mean	l2_std	l2_median	l2_lower_quartile	l2_upper_quartile	lom_mean	lom_std	lom_median	lom_lower_quartile	lom_upper_quartile	kendall_mean	kendall_std	kendall_median	kendall_lower_quartile	kendall_upper_quartile	top10_mean	top10_std	top10_median	top10_lower_quartile	top10_upper_quartile	top30_mean	top30_std	top30_median	top30_lower_quartile	top30_upper_quartile	top50_mean	top50_std	top50_median	top50_lower_quartile	top50_upper_quartile	orig_ppl_mean	orig_ppl_std	orig_ppl_median	orig_ppl_lower_quartile	orig_ppl_upper_quartile	adv_ppl_mean	adv_ppl_std	adv_ppl_median	adv_ppl_lower_quartile	adv_ppl_upper_quartile	count	rel_ppl_increase
0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	0.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	1.0	0.0	1.0	1.0	1.0	100.0	0.0	100.0	100.0	100.0	100.0	0.0	100.0	100.0	100.0	4000	0.0
0.01	0.59	0.35	0.62	0.25	0.98	0.98	0.02	0.98	0.97	0.99	0.74	0.26	0.81	0.58	0.97	467.19	1170.52	60.37	14.44	305.81	11.62	15.23	4.53	0.71	18.22	0.63	0.28	0.63	0.42	0.88	0.6	0.29	0.56	0.35	0.86	0.72	0.21	0.72	0.55	0.91	0.81	0.15	0.82	0.7	0.94	136.15	517.23	51.44	39.39	74.65	144.25	516.24	59.05	46.26	86.9	880	0.01
0.03	0.42	0.32	0.33	0.17	0.7	0.95	0.03	0.96	0.94	0.97	0.59	0.27	0.62	0.38	0.83	820.72	1593.5	222.78	64.39	808.7	15.1	17.09	8.37	2.33	23.23	0.46	0.24	0.45	0.26	0.67	0.43	0.24	0.38	0.24	0.6	0.6	0.18	0.59	0.44	0.75	0.73	0.13	0.72	0.62	0.84	61.04	40.85	50.4	38.35	67.11	84.12	57.18	68.97	53.73	92.61	960	0.04
0.06	0.32	0.27	0.24	0.11	0.48	0.91	0.04	0.92	0.89	0.94	0.51	0.24	0.52	0.34	0.7	1007.24	1779.7	332.84	114.7	1154.08	18.16	18.01	11.94	3.53	28.22	0.38	0.2	0.37	0.23	0.52	0.34	0.21	0.31	0.2	0.46	0.54	0.15	0.52	0.43	0.64	0.69	0.11	0.68	0.6	0.77	62.09	47.77	48.07	37.12	65.35	107.2	82.13	84.78	65.54	113.68	1133	0.07
0.11	0.32	0.25	0.27	0.13	0.47	0.87	0.05	0.87	0.84	0.9	0.52	0.21	0.54	0.38	0.67	1064.67	4153.87	306.6	108.14	854.01	13.96	15.47	8.09	2.98	21.8	0.38	0.17	0.38	0.26	0.49	0.34	0.2	0.33	0.2	0.47	0.54	0.14	0.54	0.45	0.62	0.69	0.1	0.69	0.63	0.75	95.11	351.72	49.28	38.25	67.92	227.25	838.74	120.06	92.41	170.86	576	0.14
0.15	0.31	0.27	0.29	0.06	0.54	0.8	0.06	0.8	0.76	0.84	0.51	0.21	0.52	0.37	0.68	444.53	796.74	169.27	98.68	396.23	11.62	12.77	6.5	2.41	16.34	0.38	0.17	0.38	0.26	0.51	0.31	0.23	0.29	0.12	0.45	0.55	0.13	0.54	0.45	0.63	0.7	0.09	0.69	0.63	0.75	72.94	59.91	53.85	39.49	84.47	244.13	174.66	188.34	141.43	264.05	343	0.24
0.18	0.28	0.25	0.21	0.06	0.48	0.74	0.07	0.74	0.7	0.77	0.48	0.22	0.51	0.31	0.65	303.81	491.85	149.62	95.54	266.18	11.92	13.8	6.53	2.39	16.07	0.35	0.18	0.36	0.21	0.48	0.28	0.24	0.25	0.08	0.4	0.52	0.16	0.5	0.39	0.61	0.68	0.1	0.68	0.63	0.75	107.38	380.48	55.14	39.4	87.44	445.66	1351.77	269.67	200.62	374.57	168	0.32
0.32	0.24	0.28	0.25	-0.02	0.46	0.69	0.12	0.71	0.64	0.76	0.39	0.31	0.44	0.21	0.64	289.58	310.95	175.84	128.65	346.49	12.15	18.92	4.86	2.06	10.97	0.29	0.23	0.3	0.15	0.49	0.23	0.23	0.17	0.0	0.4	0.48	0.21	0.5	0.39	0.65	0.64	0.14	0.65	0.59	0.73	110.24	122.55	72.7	43.58	109.3	1200.69	4103.61	429.74	316.56	670.66	54	1.0


==> data_new/tef/yelp/xlnet/S_auc.tex <==
0.10

==> data_new/tef/yelp/xlnet/S_ppl.tex <==
9.9

==> figures/n_syn_combined.tex <==
\addtolength{\tabcolsep}{-8pt}  % Default is 6pt 

\setlength{\plotwidth}{0.55\textwidth}
\setlength{\plotheight}{0.3\textwidth}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \textbf{Fake News with LSTM - Integrated Gradients} & \textbf{Fake News}                                \\
        \input{figures/n_syns/figure_lstm_fakenews_IG}      & \input{figures/n_syns_semantic/figure_fakenews}
    \end{tabular}
    \caption{Influence of factors in TEF estimated PCC of attributions. We compare the PCC of TEF (\textcolor{orange}{$\huge{\bullet}$}), RA (\textcolor{blue}{$\huge{\bullet}$}), TEF with random word order (\textcolor{red}{$\huge{\bullet}$}) and TEF with random final candidate choice (\textcolor{green}{$\huge{\bullet}$}).  We find that curves with random final choice consistently behave similar to the RA curve, while the curves with random word order come close to TEF curves.}
    \label{fig:nsyn}
\end{figure}

\addtolength{\tabcolsep}{8pt}  % Default is 6pt 

==> figures/n_syns/figure_bert_agnews_A.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        legend pos=south west
    ]
    % Add lines of means
    \addplot[name path=fi, orange, mark=triangle, line width=2pt, opacity=\lineopacity] table[x={x}, y={fi}] {figures/n_syns/data/bert_agnews_A.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=ss, blue, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns/data/bert_agnews_A.dat};
    % \addlegendentry{pcc ()}
    \addplot[name path=et, mark=o, red, line width=2pt, opacity=\lineopacity] table[x={x}, y={et}] {figures/n_syns/data/bert_agnews_A.dat};
    % \addlegendentry{KCC ()}
    
    % Add fill lines
    \addplot[name path=lfi, orange!50, opacity=\stdopacity] table[x={x}, y={lfi}] {figures/n_syns/data/bert_agnews_A.dat};
    \addplot[name path=ufi, orange!50, opacity=\stdopacity] table[x={x}, y={ufi}] {figures/n_syns/data/bert_agnews_A.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lfi and ufi];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns/data/bert_agnews_A.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns/data/bert_agnews_A.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=let, red!50, opacity=\stdopacity] table[x={x}, y={let}] {figures/n_syns/data/bert_agnews_A.dat};
    \addplot[name path=uet, red!50, opacity=\stdopacity] table[x={x}, y={uet}] {figures/n_syns/data/bert_agnews_A.dat};
    \addplot[red!50,fill opacity=\stdopacity] fill between[of=let and uet];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns/figure_cnn_yelp_S.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
      xmin=1, xmax=40,
      ymin=0.0, ymax=1,
      ymajorgrids=true,
      ytick={0, 0.5 ,1},
      yticklabels={0, , 1},
      xtick={10, 20, 30, 40},
      xticklabels={10, 20, 30, $N$},
      grid style=dashed,
      legend pos=south west
    ]
    % Add lines of means
    \addplot[name path=fi, orange, line width=2pt, opacity=\lineopacity] table[x={x}, y={fi}] {figures/n_syns/data/cnn_yelp_S.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=ss, blue, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns/data/cnn_yelp_S.dat};
    % \addlegendentry{pcc ()}
    \addplot[name path=et, red, line width=2pt, opacity=\lineopacity] table[x={x}, y={et}] {figures/n_syns/data/cnn_yelp_S.dat};
    % \addlegendentry{KCC ()}
    
    % Add fill lines
    \addplot[name path=lfi, orange!50, opacity=\stdopacity] table[x={x}, y={lfi}] {figures/n_syns/data/cnn_yelp_S.dat};
    \addplot[name path=ufi, orange!50, opacity=\stdopacity] table[x={x}, y={ufi}] {figures/n_syns/data/cnn_yelp_S.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lfi and ufi];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns/data/cnn_yelp_S.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns/data/cnn_yelp_S.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=let, red!50, opacity=\stdopacity] table[x={x}, y={let}] {figures/n_syns/data/cnn_yelp_S.dat};
    \addplot[name path=uet, red!50, opacity=\stdopacity] table[x={x}, y={uet}] {figures/n_syns/data/cnn_yelp_S.dat};
    \addplot[red!50,fill opacity=\stdopacity] fill between[of=let and uet];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns/figure_lstm_fakenews_IG.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        xmajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        % legend pos=south west,
        legend columns=1
    ]
    % Add lines of means
    \addplot[name path=fi, orange, mark=triangle, line width=2pt, opacity=\lineopacity] table[x={x}, y={fi}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addlegendentry{PCC}
    \addplot[name path=ss, blue, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addlegendentry{Sem. s.}
    \addplot[name path=et, red, mark=o, line width=2pt, opacity=\lineopacity] table[x={x}, y={et}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addlegendentry{Run time}
    
    % Add fill lines
    \addplot[name path=lfi, orange!50, opacity=\stdopacity] table[x={x}, y={lfi}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addplot[name path=ufi, orange!50, opacity=\stdopacity] table[x={x}, y={ufi}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lfi and ufi];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=let, red!50, opacity=\stdopacity] table[x={x}, y={let}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addplot[name path=uet, red!50, opacity=\stdopacity] table[x={x}, y={uet}] {figures/n_syns/data/lstm_fakenews_IG.dat};
    \addplot[red!50,fill opacity=\stdopacity] fill between[of=let and uet];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns/figure_lstmatt_imdb_A.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        % legend pos=south west
    ]
    % Add lines of means
    \addplot[name path=fi, orange, mark=triangle, line width=2pt, opacity=\lineopacity] table[x={x}, y={fi}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    % \addlegendentry{PCC}
    \addplot[name path=ss, blue, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    % \addlegendentry{Sem. s.}
    \addplot[name path=et, red, mark=o, line width=2pt, opacity=\lineopacity] table[x={x}, y={et}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    % \addlegendentry{Run time}
    
    % Add fill lines
    \addplot[name path=lfi, orange!50, opacity=\stdopacity] table[x={x}, y={lfi}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    \addplot[name path=ufi, orange!50, opacity=\stdopacity] table[x={x}, y={ufi}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lfi and ufi];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=let, red!50, opacity=\stdopacity] table[x={x}, y={let}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    \addplot[name path=uet, red!50, opacity=\stdopacity] table[x={x}, y={uet}] {figures/n_syns/data/lstmatt_imdb_A.dat};
    \addplot[red!50,fill opacity=\stdopacity] fill between[of=let and uet];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns/table_of_figures.tex <==
% \renewcommand{\arraystretch}{0.6}  % Default is 1
\addtolength{\tabcolsep}{-8pt}  % Default is 6pt 

\setlength{\plotwidth}{0.98\textwidth}
\setlength{\plotheight}{0.6\textwidth}

\begin{figure}[H]
    \centering
    \begin{tabular}{c}
        % \textbf{IMDB LSTMAtt - A}                       \\
        % \input{figures/n_syns/figure_lstmatt_imdb_A}    \\
        \textbf{Fake News with LSTM - Integrated Gradients}                    \\
        \input{figures/n_syns/figure_lstm_fakenews_IG}  \\
    \end{tabular}
    \caption{Pearson correlation (\textcolor{orange}{$\huge{\bullet}$}), semantic similarity (\textcolor{blue}{$\huge{\bullet}$}) and (scaled) batch run time (\textcolor{red}{$\huge{\bullet}$}) as function of number of candidate synonyms in Step 2. of TEF. The attack run time scales linearly with the size of the candidate pool, while PCC starts saturation at $N \approx 15$. The resulting semantic similarity between perturbed and original input stays approximately constant.}
    \label{fig:nsyns}
\end{figure}

\addtolength{\tabcolsep}{8pt}  % Default is 6pt 

==> figures/n_syns_semantic/figure_agnews.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        legend pos=south west
    ]
    
    \addplot[name path=pr, orange, line width=2pt, opacity=\lineopacity] table[x={x}, y={pr}] {figures/n_syns_semantic/data/agnews.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=ss, blue, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns_semantic/data/agnews.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=syns, red, line width=2pt, opacity=\lineopacity] table[x={x}, y={syns}] {figures/n_syns_semantic/data/agnews.dat};
    % \addlegendentry{PCC ()}
    
    % Add fill lines
    \addplot[name path=lpr, orange!50, opacity=\stdopacity] table[x={x}, y={lpr}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[name path=upr, orange!50, opacity=\stdopacity] table[x={x}, y={upr}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lpr and upr];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=lsyns, orange!50, opacity=\stdopacity] table[x={x}, y={lsyns}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[name path=usyns, orange!50, opacity=\stdopacity] table[x={x}, y={usyns}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lsyns and usyns];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns_semantic/figure_fakenews.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        xmajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        % legend pos=south west,
        legend columns=1
    ]
    
    \addplot[name path=pr, orange, mark=triangle, line width=2pt, opacity=\lineopacity] table[x={x}, y={pr}] {figures/n_syns_semantic/data/fakenews.dat};
    \addlegendentry{Pert. ration}
    \addplot[name path=ss, blue, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns_semantic/data/fakenews.dat};
    \addlegendentry{Sem. s.}
    \addplot[name path=syns, red, mark=o, line width=2pt, opacity=\lineopacity] table[x={x}, y={syns}] {figures/n_syns_semantic/data/fakenews.dat};
    \addlegendentry{Syn. dist.}
    
    % Add fill lines
    \addplot[name path=lpr, orange!50, opacity=\stdopacity] table[x={x}, y={lpr}] {figures/n_syns_semantic/data/fakenews.dat};
    \addplot[name path=upr, orange!50, opacity=\stdopacity] table[x={x}, y={upr}] {figures/n_syns_semantic/data/fakenews.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lpr and upr];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns_semantic/data/fakenews.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns_semantic/data/fakenews.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=lsyns, orange!50, opacity=\stdopacity] table[x={x}, y={lsyns}] {figures/n_syns_semantic/data/fakenews.dat};
    \addplot[name path=usyns, orange!50, opacity=\stdopacity] table[x={x}, y={usyns}] {figures/n_syns_semantic/data/fakenews.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lsyns and usyns];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns_semantic/figure_imdb.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        legend pos=south west
    ]
    
    \addplot[name path=pr, orange, line width=2pt, opacity=\lineopacity] table[x={x}, y={pr}] {figures/n_syns_semantic/data/imdb.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=ss, blue,, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns_semantic/data/imdb.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=syns, red, line width=2pt, opacity=\lineopacity] table[x={x}, y={syns}] {figures/n_syns_semantic/data/imdb.dat};
    % \addlegendentry{PCC ()}
    
    % Add fill lines
    \addplot[name path=lpr, orange!50, opacity=\stdopacity] table[x={x}, y={lpr}] {figures/n_syns_semantic/data/imdb.dat};
    \addplot[name path=upr, orange!50, opacity=\stdopacity] table[x={x}, y={upr}] {figures/n_syns_semantic/data/imdb.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lpr and upr];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns_semantic/data/imdb.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns_semantic/data/imdb.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=lsyns, orange!50, opacity=\stdopacity] table[x={x}, y={lsyns}] {figures/n_syns_semantic/data/imdb.dat};
    \addplot[name path=usyns, orange!50, opacity=\stdopacity] table[x={x}, y={usyns}] {figures/n_syns_semantic/data/imdb.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lsyns and usyns];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns_semantic/figure_yelp.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\plotwidth,
        height=\plotheight,
        xmin=1, xmax=40,
        ymin=0.0, ymax=1,
        ymajorgrids=true,
        ytick={0, 0.5 ,1},
        yticklabels={0, , 1},
        xtick={10, 20, 30, 40},
        xticklabels={10, 20, 30, $N$},
        grid style=dashed,
        legend pos=south west
    ]
    
    \addplot[name path=pr, orange, line width=2pt, opacity=\lineopacity] table[x={x}, y={pr}] {figures/n_syns_semantic/data/agnews.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=ss, blue,, line width=2pt, opacity=\lineopacity] table[x={x}, y={ss}] {figures/n_syns_semantic/data/agnews.dat};
    % \addlegendentry{PCC ()}
    \addplot[name path=syns, red, line width=2pt, opacity=\lineopacity] table[x={x}, y={syns}] {figures/n_syns_semantic/data/agnews.dat};
    % \addlegendentry{PCC ()}
    
    % Add fill lines
    \addplot[name path=lpr, orange!50, opacity=\stdopacity] table[x={x}, y={lpr}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[name path=upr, orange!50, opacity=\stdopacity] table[x={x}, y={upr}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lpr and upr];
    
    \addplot[name path=lss, blue!50, opacity=\stdopacity] table[x={x}, y={lss}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[name path=uss, blue!50, opacity=\stdopacity] table[x={x}, y={uss}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[blue!50,fill opacity=\stdopacity] fill between[of=lss and uss];


    \addplot[name path=lsyns, orange!50, opacity=\stdopacity] table[x={x}, y={lsyns}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[name path=usyns, orange!50, opacity=\stdopacity] table[x={x}, y={usyns}] {figures/n_syns_semantic/data/agnews.dat};
    \addplot[orange!50,fill opacity=\stdopacity] fill between[of=lsyns and usyns];

    \end{axis}
\end{tikzpicture}

==> figures/n_syns_semantic/table_of_figures.tex <==
% \renewcommand{\arraystretch}{0.6}  % Default is 1
\addtolength{\tabcolsep}{-8pt}  % Default is 6pt 

\setlength{\plotwidth}{0.98\textwidth}
\setlength{\plotheight}{0.6\textwidth}

\begin{figure}[H]
    \centering
    \begin{tabular}{c}
        \textbf{Fake News}    \\
        \input{figures/n_syns_semantic/figure_fakenews}   \\
    \end{tabular}
    \caption{Perturbation ratio (\textcolor{orange}{$\huge{\bullet}$}), semantic similarity (\textcolor{blue}{$\huge{\bullet}$}) and average cosine distance of replaced token and replacement in the \textit{counter-fitted} synonym embedding space (\textcolor{red}{$\huge{\bullet}$}) as function of the rank of replacement in synonym embedding space. If we replace the tokens in the sentence with synonyms that are further from the original token in the synonym embedding space, the semantic similarity of the resulting sentence stays approximately constant. (Should we not plot Blue as function of red here? - would be easier)}
    \label{fig:nsynsemantic}
\end{figure}


\addtolength{\tabcolsep}{8pt}  % Default is 6pt 

==> tables/nsyn_examples.tex <==
\begin{table}[H]
% \vspace{\baselineskip}
\caption{Tokens of AG New's dataset and their closest synonyms. Some tokens appear to have many synonyms that are sensible in most cases, some might have different meanings, but capture the same overall concept. Many have no relevant low-ranked synonyms. This qualitative assessment is indicated in the quality column.}\label{tbl:nsynexamples}
% \vspace{\baselineskip}
\centering
\begin{tabular}{c|c|c}
% \\ \hline \\
\textbf{Token}      & \textbf{Closest syn.} & \textbf{20-th syn.}           \\\hline%\hline
broken              & ruptured              & \textcolor{green}{fragmented} \\
say                 & said                  & \textcolor{green}{express}    \\
else                & otherwise             & \textcolor{green}{instead}    \\
flawed              & imperfect             & \textcolor{green}{wrongful}   \\
britain             & britannia             & \textcolor{green}{scotsmen}   \\
\hline
police              & constabulary          & \textcolor{orange}{firemen}   \\
web                 & internet              & \textcolor{orange}{twitter}   \\
thrown              & hurdled               & \textcolor{orange}{hurling}   \\
aimed               & targeted              & \textcolor{orange}{signified} \\
giants              & titans                & \textcolor{orange}{panthers}  \\
\hline
lobbyist            & lobbyists             & \textcolor{red}{abramoff}     \\
senate              & senators              & \textcolor{red}{panetta}      \\
building            &  build                & \textcolor{red}{chee}         \\
calendar            & calendars             & \textcolor{red}{bouts}        \\

% \hline
\end{tabular}
\end{table}
\vspace{\baselineskip}
